Sharp global convergence guarantees for iterative nonconvex optimization: A Gaussian process perspective

We consider a general class of regression models with normally distributed covariates, and the associated nonconvex problem of fitting these models from data. We develop a general recipe for analyzing the convergence of iterative algorithms for this task from a random initialization. In particular, provided each iteration can be written as the solution to a convex optimization problem satisfying some natural conditions, we leverage Gaussian comparison theorems to derive a deterministic sequence that provides sharp upper and lower bounds on the error of the algorithm with sample-splitting. Crucially, this deterministic sequence accurately captures both the convergence rate of the algorithm and the eventual error floor in the finite-sample regime, and is distinct from the commonly used "population" sequence that results from taking the infinite-sample limit. We apply our general framework to derive several concrete consequences for parameter estimation in popular statistical models including phase retrieval and mixtures of regressions. Provided the sample size scales near-linearly in the dimension, we show sharp global convergence rates for both higher-order algorithms based on alternating updates and first-order algorithms based on subgradient descent. These corollaries, in turn, yield multiple consequences, including: (a) Proof that higher-order algorithms can converge significantly faster than their first-order counterparts (and sometimes super-linearly), even if the two share the same population update and (b) Intricacies in super-linear convergence behavior for higher-order algorithms, which can be nonstandard (e.g., with exponent 3/2) and sensitive to the noise level in the problem. We complement these results with extensive numerical experiments, which show excellent agreement with our theoretical predictions.

==> command-template.tex <==
%!TEX root = main-paper-template.tex

% The command above makes the PDF compilable from this file if you're using SublimeText

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Some basic packages

\usepackage{comment}
\usepackage{epsf}
\usepackage{graphicx}
%\usepackage{subfigure}
\usepackage{subcaption}
\usepackage{bbm}
\usepackage{color}
\usepackage{nicefrac}
\usepackage{mathtools}
\usepackage{amsfonts}
\usepackage{amsthm}
\usepackage{amsmath, bm}
\usepackage{amssymb}
\usepackage{textcomp}
\usepackage[dvipsnames]{xcolor}
\usepackage{enumitem}
\usepackage{upgreek}
\usepackage[ruled, vlined, lined, commentsnumbered]{algorithm2e}

%\usepackage{enumerate}


\RequirePackage[pagebackref,colorlinks,citecolor={blue!60!black},urlcolor={blue!70!black},linkcolor={red!60!black},breaklinks,hypertexnames=false]{hyperref} %Adds links to references (without boxes)
\renewcommand*{\backref}[1]{}
\renewcommand*{\backrefalt}[4]{({\small%
		\ifcase #1 Not cited.%
		\or Cited on page~#2.%
		\else Cited on pages #2.%
		\fi%
	})}


% Alternative minipage environment, renders better in terms of spacing

\newenvironment{fminipage}%
  {\begin{Sbox}\begin{minipage}}%
  {\end{minipage}\end{Sbox}\fbox{\TheSbox}}
  
\newenvironment{algbox}[0]{\vskip 0.2in
\noindent 
\begin{fminipage}{6.3in}
}{
\end{fminipage}
\vskip 0.2in
}

% Tikz packages
\usepackage{tikz}
\tikzset{
	data/.style={circle, draw, text centered, minimum height=3em ,minimum width = .5em, inner sep = 2pt},
	empty/.style={circle, text centered, minimum height=3em ,minimum width = .5em, inner sep = 2pt},
}
%\usepackage{subcaption}
\usepackage{pgfplots}
\pgfplotsset{compat=1.5}
\usepgfplotslibrary{fillbetween}
\usetikzlibrary{patterns}
\usetikzlibrary{spy}
\usetikzlibrary{backgrounds}
\usetikzlibrary{decorations}
\usepackage{float}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% MACROS BELOW

%%%%%%%

% {Theorem, Proposition, Lemma, Corollary} numbered sequentially
% throughout the paper, not by section number and not combined


\newtheorem{theorem}{Theorem}
\newtheorem{example}{Example}
\newtheorem{assumption}{Assumption}
\newtheorem{proposition}{Proposition}
\newtheorem{fact}{Fact}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{definition}{Definition}
\newtheorem{remark}{Remark}
\newtheorem{conjecture}{Conjecture}
\newtheorem{claim}{Claim}

%%%%%%%%%%%
%References (natbib): Use \citet and \citep to take full advantage

\usepackage{natbib}
\setcitestyle{round}

%%%%%%%%%%%




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Widebar command
\newlength{\widebarargwidth}
\newlength{\widebarargheight}
\newlength{\widebarargdepth}
\DeclareRobustCommand{\widebar}[1]{%
 \settowidth{\widebarargwidth}{\ensuremath{#1}}%
 \settoheight{\widebarargheight}{\ensuremath{#1}}%
 \settodepth{\widebarargdepth}{\ensuremath{#1}}%
 \addtolength{\widebarargwidth}{-0.3\widebarargheight}%
 \addtolength{\widebarargwidth}{-0.3\widebarargdepth}%
 \makebox[0pt][l]{\hspace{0.3\widebarargheight}%
   \hspace{0.3\widebarargdepth}%
   \addtolength{\widebarargheight}{0.3ex}%
   \rule[\widebarargheight]{0.95\widebarargwidth}{0.1ex}}%
 {#1}}



%%% New version of \caption puts things in smaller type, single-spaced 
%%% and indents them to set them off more from the text.
\makeatletter
\long\def\@makecaption#1#2{
       \vskip 0.8ex
       \setbox\@tempboxa\hbox{\small {\bf #1:} #2}
       \parindent 1.5em 
       \dimen0=\hsize
       \advance\dimen0 by -3em
       \ifdim \wd\@tempboxa >\dimen0
               \hbox to \hsize{
                       \parindent 0em
                       \hfil 
                       \parbox{\dimen0}{\def\baselinestretch{0.96}\small
                               {\bf #1.} #2
                               %%\unhbox\@tempboxa
                               } 
                       \hfil}
       \else \hbox to \hsize{\hfil \box\@tempboxa \hfil}
       \fi
       }
\makeatother



%% COMMENTING commands: insert more for more than two collaborators

\long\def\comment#1{}

\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\apcomment}[1]{{\bf{{\blue{{AP --- #1}}}}}}

\newcommand{\purple}[1]{\textcolor{violet!80}{#1}}
\newcommand{\kaccomment}[1]{{\bf{{\purple{{KAC --- #1}}}}}}
\newcommand{\kac}[1]{{\purple{#1}}}

\newcommand{\magenta}[1]{\textcolor{magenta}{#1}}
\newcommand{\ct}[1]{\textcolor{blue}{\textcolor{magenta}{#1}}}
\newcommand{\ctcomment}[1]{\textcolor{blue}{{\bf{{\magenta{{CT --- #1}}}}}}}
\newcommand{\emf}[1]{\textcolor{blue}{?~#1~?}}
\newcommand{\err}[1]{\textcolor{red}{?~#1~?}}
\newcommand{\clr}[1]{\textcolor{darkred}{#1}}
\newcommand{\todo}[1]{\textcolor{magenta}{#1}}
\newcommand{\red}[1]{\textcolor{red}{#1}}


% Some vector/matrix norms. Convention is that we use triple lines for matrix 
% norms and double lines for vector norms.
\newcommand{\matnorm}[3]{|\!|\!| #1 | \! | \!|_{{#2}, {#3}}}
\newcommand{\matsnorm}[2]{|\!|\!| #1 | \! | \!|_{{#2}}}
\newcommand{\vecnorm}[2]{\| #1\|_{#2}}

% Some useful and common operators
% Independence symbol
\newcommand\indpt{\protect\mathpalette{\protect\independenT}{\perp}} 
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}
\newcommand{\defn}{\coloneqq} %This is a properly aligned definition symbol
\DeclareMathOperator*{\minimize}{minimize}
\DeclareMathOperator{\modd}{mod}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\Var}{var}
\DeclareMathOperator{\cov}{cov}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator{\floor}{floor}
\DeclareMathOperator{\vol}{vol}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\card}{card}
\DeclareMathOperator{\range}{range}
\DeclareMathOperator{\dist}{\rho}
\DeclareMathOperator{\sign}{\mathsf{sgn}}

\newcommand{\parcomp}{\alpha}
\newcommand{\perpcomp}{\beta}
\newcommand{\anglecurr}{\phi}

\newcommand{\perpone}{\mu}
\newcommand{\perptwo}{\nu}

% Specific norms
\newcommand{\nucnorm}[1]{\ensuremath{\matsnorm{#1}{\footnotesize{\mbox{nuc}}}}}
\newcommand{\fronorm}[1]{\ensuremath{\matsnorm{#1}{\tiny{\mbox{F}}}}}
\newcommand{\opnorm}[1]{\ensuremath{\matsnorm{#1}{\tiny{\mbox{op}}}}}
\newcommand{\eucnorm}[1]{\left\|#1 \right\|}
\newcommand{\linfnorm}[1]{\left\|#1 \right\|_\infty}

% Bracket notation to make life easier when writing long expressions
\newcommand{\paren}[1]{\left\{ #1 \right\} }
% Inner product
\newcommand{\inprod}[2]{\ensuremath{\langle #1 , \, #2 \rangle}}

% The macros below are useful if you see these quantities changing over the course of writing
\newcommand{\numdim}{\ensuremath{d}}
\newcommand{\numobs}{\ensuremath{n}}

% Distances between distributions
\newcommand{\kull}[2]{\ensuremath{D_{\mathsf{KL}}(#1\; \| \; #2)}}
\newcommand{\KL}{\ensuremath{D_{\mathsf{KL}}}}
\newcommand{\TV}{\ensuremath{d_{\mathsf{TV}}}}
\newcommand{\Hel}{\ensuremath{d_{\mathsf{hel}}}}

% Probability
\newcommand{\EE}{\ensuremath{{\mathbb{E}}}}
\newcommand{\Prob}{\ensuremath{{\Partition}}}
\newcommand{\ind}[1]{\ensuremath{{\mathbb{I}\left\{ #1 \right\}}}}

%Numbering (use with \overset to label steps)
\newcommand{\1}{\ensuremath{{\sf (i)}}}
\newcommand{\2}{\ensuremath{{\sf (ii)}}}
\newcommand{\3}{\ensuremath{{\sf (iii)}}}
\newcommand{\4}{\ensuremath{{\sf (iv)}}}
\newcommand{\5}{\ensuremath{{\sf (v)}}}
\newcommand{\6}{\ensuremath{{\sf (vi)}}}

%Eigenvector / eigenvalue related notation
\newcommand{\eig}[1]{\ensuremath{\lambda_{#1}}}
\newcommand{\eigmax}{\ensuremath{\eig{\max}}}
\newcommand{\eigmin}{\ensuremath{\eig{\min}}}


% Distributions
\newcommand{\NORMAL}{\ensuremath{\mathcal{N}}}
\newcommand{\BER}{\ensuremath{\mbox{\sf Ber}}}
\newcommand{\BIN}{\ensuremath{\mbox{\sf Bin}}}
\newcommand{\Hyp}{\ensuremath{\mbox{\sf Hyp}}}

% Bold
\newcommand{\bd}[1]{\boldsymbol{#1}}

% Script letters
\newcommand{\Aspace}{\ensuremath{\mathcal{A}}}
\newcommand{\Xspace}{\ensuremath{\mathcal{X}}}
\newcommand{\Yspace}{\ensuremath{\mathcal{Y}}}
\newcommand{\Zspace}{\ensuremath{\mathcal{Z}}}
\newcommand{\Fspace}{\ensuremath{\mathcal{F}}}

% Population and sample loss functions
\newcommand{\loss}{\ensuremath{\mathcal{L}}}
\newcommand{\lossn}[1]{\ensuremath{\mathcal{L}^n \left( #1 \right)}}

% True parameter
\newcommand{\thetathree}{\theta^{(3)}}
\newcommand{\thetathreestar}{\theta^{(3)}_\star}
\newcommand{\thetastar}{\ensuremath{\bt^*}}
\newcommand{\btstar}{\ensuremath{\bt^{*}}}
% Estimates
\newcommand{\thetahat}{\ensuremath{\widehat{\bt}}}
\newcommand{\thetabar}{\ensuremath{\overline{\bt}}}
\newcommand{\thetatil}{\ensuremath{\widetilde{\bt}}}
% Iterates
\newcommand{\thetacur}{\ensuremath{\bt_t}}
\newcommand{\thetanext}{\ensuremath{\bt_{t +1}}}
\newcommand{\thetanexthat}{\ensuremath{\hat{\bt}_{t +1}}}
\newcommand{\thetainit}{\ensuremath{\bt_0}}
\newcommand{\thetaplus}{\ensuremath{\bt_+}}
\newcommand{\thetaplushat}{\ensuremath{\widehat{\bt}_+}}

% statistics iterates
% alpha, beta, xi
\newcommand{\xitheta}{\ensuremath{\xi(\theta)}}
\newcommand{\alphatheta}{\ensuremath{\alpha(\theta)}}
\newcommand{\betatheta}{\ensuremath{\beta(\theta)}}
\newcommand{\sigmatheta}{\ensuremath{\sigma(\theta)}}

\newcommand{\xicur}{\ensuremath{\xi_t}}
\newcommand{\alphacur}{\ensuremath{\alpha_t}}
\newcommand{\betacur}{\ensuremath{\beta_t}}
\newcommand{\sigmacur}{\ensuremath{\sigma_t}}

\newcommand{\xit}{\xi_t}
\newcommand{\sigmat}{\sigma_t}

\newcommand{\xinext}{\ensuremath{\xi_{+}}}
\newcommand{\alphanext}{\ensuremath{\alpha_{+}}}
\newcommand{\betanext}{\ensuremath{\beta_{+}}}
\newcommand{\sigmanext}{\ensuremath{\sigma_{+}}}

\newcommand{\xiplus}{\ensuremath{\xi_{+}}}
\newcommand{\alphaplus}{\ensuremath{\alpha_{+}}}
\newcommand{\betaplus}{\ensuremath{\beta_{+}}}
\newcommand{\sigmaplus}{\ensuremath{\sigma_{+}}}

\newcommand{\parcompplus}{\ensuremath{\alpha^{+}}}
\newcommand{\perponeplus}{\ensuremath{\mu^{+}}}
\newcommand{\perptwoplus}{\ensuremath{\nu^{+}}}
\newcommand{\perpcompplus}{\ensuremath{\beta^{+}}}

\newcommand{\xinextstar}{\ensuremath{\xi_{+,\star}}}
\newcommand{\alphanextstar}{\ensuremath{\alpha_{+,\star}}}
\newcommand{\betanextstar}{\ensuremath{\beta_{+,\star}}}
\newcommand{\sigmanextstar}{\ensuremath{\sigma_{+,\star}}}

%From alt file
\newcommand{\parcomptheta}{\ensuremath{\parcomp(\theta)}}
\newcommand{\anglecurrtheta}{\ensuremath{\anglecurr(\theta)}}
\newcommand{\perpcomptheta}{\ensuremath{\perpcomp(\theta)}}

\newcommand{\parcompcur}{\ensuremath{\parcomp_t}}
\newcommand{\anglecurrcur}{\ensuremath{\anglecurr_t}}
\newcommand{\perpcompcur}{\ensuremath{\perpcomp_t}}

\newcommand{\parcompnext}{\ensuremath{\parcomp_{t+1}}}
\newcommand{\anglecurrnext}{\ensuremath{\anglecurr_{t+1}}}
\newcommand{\perpcompnext}{\ensuremath{\perpcomp_{t+1}}}

\newcommand{\parcompnextstar}{\ensuremath{\parcomp_{t+1,\star}}}
\newcommand{\anglecurrnextstar}{\ensuremath{\anglecurr_{t+1,\star}}}
\newcommand{\perpcompnextstar}{\ensuremath{\perpcomp_{t+1,\star}}}
%back to orig

%Sets
\newcommand{\Dcthree}{\Pc_3(\Dc)}
\newcommand{\Dcthreeu}{\Pc_3(\Bc(C_1))}
\newcommand{\Dcthreec}{\Pc_3(\Bc(C_1))\cap\Sc_\eps^c}

% Order notation
\newcommand{\order}{\ensuremath{\mathcal{O}}}
\newcommand{\ordertil}{\ensuremath{\widetilde{\order}}}
\newcommand{\Omegatil}{\ensuremath{\widetilde{\Omega}}}

% Parallel and orthogonal components per iteration
\newcommand{\parcur}{\xi^t}
\newcommand{\perpcur}{\sigma^t}
\newcommand{\parnext}{\xi^{t+1}}
\newcommand{\perpnext}{\sigma^{t+1}}
\newcommand{\empparcur}{\xi_n^t}
\newcommand{\empperpcur}{\sigma_n^t}
\newcommand{\empparnext}{\xi_n^{t+1}}
\newcommand{\empperpnext}{\sigma_n^{t+1}}


\newcommand{\hscal}{h_{\rm scal}}

% Projection
%\newcommand{\proj}{\mathsf{P}}
\newcommand{\proj}{\bP}

% weight function
\newcommand{\wfun}{\omega}


%%%%%%%%%%%%%%%%
%%% Christos %%%%%%%%
%%%%%%%%%%%%%%%%
\newcommand{\W}{\mathbf{W}}
\newcommand{\M}{\mathbf{M}}
\newcommand{\Z}{\mathbf{Z}}
\newcommand{\Ub}{\mathbf{U}}
\newcommand{\G}{\mathbf{G}}
\newcommand{\Hb}{{H}}
%\newcommand{\G}{{G}}
\newcommand{\Sb}{\mathbf{S}}
\newcommand{\X}{\mathbf{X}}
\newcommand{\XXb}{\overline{\mathbf{X}}}
\newcommand{\Lb}{{L}}
\newcommand{\Y}{\mathbf{Y}}
\newcommand{\Vb}{\mathbf{V}}
\newcommand{\A}{\mathbf{A}}
\newcommand{\Db}{\mathbf{D}}
%Bold lower
\newcommand{\ellb}{\boldsymbol{\ell}}
\newcommand{\phib}{\boldsymbol{\phi}}
\newcommand{\x}{\mathbf{x}}
\newcommand{\ub}{\mathbf{u}}
\newcommand{\w}{\mathbf{w}}
\newcommand{\tb}{\mathbf{t}}
\newcommand{\g}{\mathbf{g}}
\newcommand{\vb}{\mathbf{v}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\e}{\mathbf{e}}
\newcommand{\eb}{\mathbf{e}}
\newcommand{\y}{\mathbf{y}}
\newcommand{\s}{\mathbf{s}}
\newcommand{\zb}{\mathbf{z}}
\newcommand{\zo}{\overline{\mathbf{z}}}
\newcommand{\bseta}{{\boldsymbol{\eta}}}
\newcommand{\Iden}{\mathbf{I}}
\newcommand{\cb}{\mathbf{c}}  
\newcommand{\ab}{\mathbf{a}}
\newcommand{\oneb}{\mathbf{1}}
\newcommand{\h}{\mathbf{h}}
\newcommand{\f}{\mathbf{f}}
\newcommand{\betab}{\boldsymbol{\beta}}
%\newcommand{\tb}{\mathbf{t}}


%Calligraphic
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Mc}{\mathcal{M}}
\newcommand{\Ps}{\mathcal{P}}
\newcommand{\Rs}{\mathcal{R}}
\newcommand{\Tc}{{\mathcal{T}}}
\newcommand{\Sc}{{\mathcal{S}}}
\newcommand{\Bc}{{\mathcal{B}}}
\newcommand{\Yc}{\mathcal{Y}}
\newcommand{\Dc}{\mathcal{D}}
\newcommand{\Xc}{\mathcal{X}}
\newcommand{\Zc}{\mathcal{Z}}
%\newcommand{\Ic}{\mathcal{I}}
\newcommand{\Uc}{\mathcal{U}}
\newcommand{\Kc}{\mathcal{K}}
\newcommand{\Nc}{\mathcal{N}}
\newcommand{\Rc}{\mathcal{R}}
\newcommand{\Nn}{\mathcal{N}}
\newcommand{\Lc}{\mathcal{L}}
\newcommand{\Cc}{\mathcal{C}}
\newcommand{\Gc}{{\mathcal{G}}}
\newcommand{\Ac}{\mathcal{A}}
\newcommand{\Pc}{\mathcal{P}}
\newcommand{\Ec}{\mathcal{E}}
\newcommand{\Hc}{\mathcal{H}}
\newcommand{\Qc}{\mathcal{Q}}
\newcommand{\Oc}{\mathcal{O}}
\newcommand{\Jc}{\mathcal{J}}
\newcommand{\Ic}{\mathcal{I}}

\newcommand{\vp}{\vspace{4pt}}

\newcommand{\R}{\mathbb{R}}
%\newcommand{\E}{\mathbb{E}}
\newcommand{\Pro}{\mathbb{P}}
\newcommand{\nn}{\notag}

\newcommand{\rP}{\stackrel{{P}}{\longrightarrow}}

\DeclarePairedDelimiterX{\inp}[2]{\langle}{\rangle}{#1, #2}


\newcommand{\beps}{\boldsymbol{\epsilon}}
\newcommand{\bt}{\boldsymbol{\theta}}
\newcommand{\bbe}{\boldsymbol{\beta}}
\newcommand{\bG}{\boldsymbol{G}}
\newcommand{\bD}{\boldsymbol{D}}
\newcommand{\bw}{\boldsymbol{w}}
\newcommand{\bX}{\boldsymbol{X}}
\newcommand{\by}{\boldsymbol{y}}

\newcommand{\bq}{\boldsymbol{q}}
%\newcommand{\bxi}{\boldsymbol{\xi}}
%\newcommand{\bx}{\boldsymbol{x}}
\newcommand{\bM}{\boldsymbol{M}}
\newcommand{\bL}{\boldsymbol{L}}
\newcommand{\bZ}{\boldsymbol{Z}}
\newcommand{\bz}{\boldsymbol{z}}
\newcommand{\bW}{\boldsymbol{W}}
\newcommand{\bGam}{\boldsymbol{\Gamma}}
\newcommand{\bI}{\boldsymbol{I}}
\newcommand{\bSig}{\boldsymbol{\Sigma}}
\newcommand{\be}{\boldsymbol{e}}
%\newcommand{\bg}{\boldsymbol{g}}
\newcommand{\bg}{\boldsymbol{\gamma}_n}
\newcommand{\bv}{\boldsymbol{v}}
\newcommand{\bu}{\boldsymbol{u}}
\newcommand{\bU}{\boldsymbol{U}}
\newcommand{\bP}{\boldsymbol{P}}
%\newcommand{\bh}{\boldsymbol{h}}
\newcommand{\bh}{\boldsymbol{\gamma}_d}
\newcommand{\bx}{\boldsymbol{x}}
\newcommand{\bA}{\boldsymbol{A}}
\newcommand{\bB}{\boldsymbol{B}}
\newcommand{\ba}{\boldsymbol{a}}
\newcommand{\br}{\boldsymbol{r}}
\newcommand{\bs}{\boldsymbol{s}}
\newcommand{\bgam}{\boldsymbol{\gamma}}
\newcommand{\bOmega}{\boldsymbol{\Omega}}
\newcommand{\bomega}{\boldsymbol{\omega}}
\newcommand{\btsharp}{\boldsymbol{\theta}^{\sharp}}
\newcommand{\Fc}{\mathcal{F}}
\newcommand{\bxi}{\boldsymbol{\xi}}
\newcommand{\bzeta}{\boldsymbol{\zeta}}
\newcommand{\bzetabar}{\overline{\boldsymbol{\zeta}}}


\DeclareMathOperator{\E}{\mathbb{E}}

\providecommand{\norm}[1]{\lVert#1\rVert}
\providecommand{\abs}[1]{\lvert#1\rvert}

 \newcommand{\om}{\omega}
% \newcommand{\betabh}{\hat{\boldsymbol\beta}}
\newcommand{\gammab}{\boldsymbol\gamma}
\newcommand{\omegab}{\boldsymbol\omega}
\newcommand{\epsb}{\boldsymbol\eps}
\newcommand{\ksi}{\xi}
\newcommand{\la}{\lambda}
\newcommand{\eps}{\epsilon}
\newcommand{\wt}{\widetilde}

\newcommand{\GPR}{\mathbb{G}_{\mathsf{PR}}}
\newcommand{\GMR}{\mathbb{G}_{\mathsf{MR}}}

% Following from notes:

\newcommand{\xipop}{\xi^{{\sf pop}}}
\newcommand{\sigmapop}{\sigma^{{\sf pop}}}
\newcommand{\xigordon}{\xi^{{\sf gor}}}
\newcommand{\xigordonplus}{\xi^{{\sf gor, +}}}
\newcommand{\xigordonminus}{\xi^{{\sf gor, -}}}
\newcommand{\sigmagordon}{\sigma^{{\sf gor}}}
\newcommand{\sigmagordonplus}{\sigma^{{\sf gor, +}}}
\newcommand{\sigmagordonminus}{\sigma^{{\sf gor, -}}}
\newcommand{\Sopgordon}{\mathcal{S}_{{\sf gor}}}
\newcommand{\real}{\mathbb{R}}

\newcommand{\xihat}{\widehat{\xi}}
\newcommand{\sigmahat}{\widehat{\sigma}}
\newcommand{\xihatn}{\widehat{\xi}^{(n)}}
\newcommand{\sigmahatn}{\widehat{\sigma}^{(n)}}

\newcommand{\xibar}{\overline{\xi}}
\newcommand{\sigmabar}{\overline{\sigma}}
\newcommand{\alphabar}{\overline{\alpha}}

\newcommand{\Deltasigma}{\Delta^{\perp}}
\newcommand{\Deltaxi}{\Delta^{\|}}
\newcommand{\Tr}{{\sf Tr}}
\newcommand{\ubar}[1]{\text{\b{$#1$}}}


\newcommand{\Fhat}{\widehat{F}}
\newcommand{\Ghat}{\widehat{G}}
\newcommand{\DeltaSE}{\mathsf{d}}
\newcommand{\DeltaSELtwo}{\mathsf{d}_{\ell_2}}
\newcommand{\DeltaSEangle}{\mathsf{d}_{\angle}}
\newcommand{\cperp}{c^{\perp}}
\newcommand{\cpar}{c^{\|}}


%From alt file

\newcommand{\parcomppop}{\parcomp^{{\sf pop}}}
\newcommand{\perpcomppop}{\perpcomp^{{\sf pop}}}
\newcommand{\parcompgordon}{\parcomp^{{\sf gor}}}
\newcommand{\parcompgordonplus}{\parcomp^{{\sf gor, +}}}
\newcommand{\parcompgordonminus}{\parcomp^{{\sf gor, -}}}
\newcommand{\perpcompgordon}{\perpcomp^{{\sf gor}}}
\newcommand{\perpcompgordonplus}{\perpcomp^{{\sf gor, +}}}
\newcommand{\perpcompgordonminus}{\perpcomp^{{\sf gor, -}}}
\newcommand{\Sop}{\mathcal{S}}

\newcommand{\pop}{\mathsf{pop}}
\newcommand{\gor}{\mathsf{gor}}

\newcommand{\parcomphat}{\widehat{\parcomp}}
\newcommand{\perpcomphat}{\widehat{\perpcomp}}
\newcommand{\parcomphatn}{\widehat{\parcomp}^{(n)}}
\newcommand{\perpcomphatn}{\widehat{\perpcomp}^{(n)}}

\newcommand{\parcompbar}{\overline{\parcomp}}
\newcommand{\perpcompbar}{\overline{\perpcomp}}
\newcommand{\anglecurrbar}{\overline{\anglecurr}}
\newcommand{\nubar}{\overline{\nu}}



\newcommand{\B}{\mathbf{B}}
\newcommand{\noisestd}{\sigma}

\newcommand{\Sopbar}{\overline{\Sop}}
\newcommand{\Sophat}{\widehat{\Sop}}
\newcommand{\Fbar}{\overline{F}}
\newcommand{\Gbar}{\overline{G}}

\newcommand{\Goodset}{\mathbb{G}}
\newcommand{\ttilde}{t'}

\newcommand{\var}{\mathsf{var}}
\newcommand{\con}{\mathsf{con}}

\newcommand{\Ztil}{\ensuremath{\widetilde{Z}}}
\newcommand{\sbar}{\ensuremath{\widebar{\sigma}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> sections/deterministic-convergence/deterministic-convergence.tex <==
%!TEX root = ../../convergence-gordon.tex

\section{Proof of Theorem~\ref{thm:AM-PR}: Alternating minimization for phase retrieval}

Recall that the good region for phase retrieval is given by $\GPR$, the set of $\nu = (\xi, \sigma)$ satisfying $\xi \lor \sigma \leq 1.05$, $\xi/\sigma \geq 5$,  and $\xi^2 + \sigma^2 \geq 0.9$. Also recall our assumption that $\delta \geq C$ and $s^2 / \delta \leq c$ for universal constants $(c, C)$. This will be used in multiple steps of the proof.
 
For convenience, we first restate the Gordon state evolution for this case.
\begin{align} \label{eq:Gordon-AM-PR-restated}
\begin{split}
\xigordon &= 1 - \frac{1}{\pi}(2\alpha - \sin(2\alpha))  \quad \text{ and } \\
\sigmagordon &= \sqrt{\frac{4}{\pi^2}\sin^4(\alpha) + \frac{1}{\delta - 1}\left(1 - (1 - \frac{1}{\pi}(2\alpha - \sin(2\alpha)))^2 - \frac{4}{\pi^2}\sin^4(\alpha) + s^2\right)}.
\end{split}
\end{align}
The rest of the proof proceeds in several steps. Steps 1, 2, and 3 are used to prove parts (a), (b), and (c) of the theorem, respectively.

\subsection{Step 1: Convergence of the Gordon state evolution in the good region}

As a first step, we prove part (a) of Theorem~\ref{thm:AM-PR}, providing upper and lower bounds on the error of the Gordon state evolution~\eqref{eq:Gordon-AM-PR-restated}. 
%It is useful to set up some notation. Denote the map $(\xi, \sigma) \mapsto \xigordon$ by $F$ and the map $(\xi, \sigma) \mapsto \sigmagordon$ by $G$. 
The following lemmas establish the claimed superlinear convergence of the Gordon state evolution operator.
\begin{lemma} \label{AM-PR-good-region}
Suppose $\delta \geq C$ and $s^2 / \delta \leq c$. If $\nu \in \GPR$, then $\mathcal{S}_{gor}(\nu) \in \GPR$.
\end{lemma}

\begin{lemma} \label{AM-PR-convergence}
Suppose $\delta \geq C$ and $s^2 / \delta \leq c$. Then for each $\nu = (\xi, \sigma) \in \GPR$, we have
\begin{align*}
[\DeltaSE(\mathcal{S}_{gor}(\nu))]^2 &\leq C_{\delta} \cdot [\DeltaSE(\nu)]^{3} + \frac{s^2}{\delta - 1}, \text{ and } \\
[\DeltaSE(\mathcal{S}^2_{gor}(\nu))]^2 &\geq c_{\delta} \cdot [\DeltaSE(\mathcal{S}_{gor}(\nu))]^{3} + \frac{s^2}{\delta - 1}.
\end{align*}
Here $0 \leq c_{\delta} \leq C_{\delta} \leq 1$ are constants that depend solely on $\delta$.
\end{lemma}

\subsubsection{Proof of Theorem~\ref{thm:AM-PR}(a)}
Taken together, Lemmas~\ref{AM-PR-good-region} and~\ref{AM-PR-convergence} clearly establish part (a) of the theorem. In particular, Lemma~\ref{AM-PR-good-region} guarantees that the Gordon state evolution remains in the good region if it starts in the good region. Lemma~\ref{AM-PR-convergence}, on the other hand, establishes the claimed superlinear convergence with exponent $3/2$, where the lower bound requires the burn-in period $t_0 = 1$. The two conditions of Definition~\ref{def:superlinear} are thus satisfied, and this proves Theorem~\ref{thm:AM-PR}(a). \qed
%\apcomment{Add more detail.} \qed
\medskip

We now prove each lemma in turn. It is useful to set up some notation. Denote the map $(\xi, \sigma) \mapsto \xigordon$ by $F$ and the map $(\xi, \sigma) \mapsto \sigmagordon$ by $G$.

\subsubsection{Proof of Lemma~\ref{AM-PR-good-region}}

We must show that if the pair $(\xi, \sigma)$ satisfies $\xi \lor \sigma \leq 1.05$, $\xi^2 + \sigma^2 \geq 0.9$, and $\xi/\sigma \geq 5$, then the Gordon state evolution~\eqref{eq:Gordon-AM-PR-restated} satisfies $F(\xi, \sigma) \lor G(\xi, \sigma) \leq 1.05$, $[F(\xi, \sigma)]^2 + [G(\xi, \sigma)]^2 \geq 0.9$, and $F(\xi, \sigma)/G(\xi, \sigma) \geq 5$. We show each of these bounds separately.

\paragraph{Bounding $F(\xi, \sigma)$:} This step is immediate, since for all $\alpha \in [0, \pi/2]$, we have $F(\xi, \sigma) \in [0, 1]$.

\paragraph{Bounding $G(\xi, \sigma)$:} Note that for all $\alpha \in [0, \pi/2]$, we have $F(\xi, \sigma) \in [0, 1]$. Consequently,
\begin{align} \label{eq:rec-Gbound}
[G(\xi, \sigma)]^2 = \frac{\delta - 1}{\delta - 2} \cdot \frac{4}{\pi^2} \sin^4 \alpha + \frac{1}{\delta - 1} \left( 1 - [F(\xi, \sigma)]^2 + s^2 \right) \leq \frac{4}{\pi^2} + \frac{1 + s^2}{\delta - 1} \leq 1,
\end{align}
where the final step holds for large enough $\delta$ and small enough $s^2 / \delta$.

\paragraph{Bounding $[F(\xi, \sigma)]^2 + [G(\xi, \sigma)]^2$:} Note that $[F(\xi, \sigma)]^2 + [G(\xi, \sigma)]^2 \geq [F(\xi, \sigma)]^2$, so that it suffices to lower bound $F(\xi, \sigma)$. Since $\sin x \geq x - x^3/6$, we have $2\alpha - \sin(2 \alpha) \leq \frac{4}{3} \alpha^3$. Moreover, when $(\sigma/\xi)^3 \leq \frac{3 \pi}{4}$, we also have $1 - \frac{4}{3\pi} \alpha^3 \geq 1 - \frac{4}{3\pi} \tan^3 \alpha \geq 0$. Consequently, for all such $\alpha$, we have
\begin{align} \label{eq:rec-sqbound}
[F(\xi, \sigma)]^2 = \left( 1 - \frac{1}{\pi} (2\alpha - \sin(2 \alpha)) \right)^2 \geq  \left( 1 - \frac{4}{3\pi} (\sigma/\xi)^3 \right)^2,
\end{align}
and the RHS is clearly lower bounded by $0.9$ provided $\sigma/\xi \leq 1/5$.

\paragraph{Bounding $\frac{F(\xi/\sigma)}{G(\xi, \sigma)}$:} Consider the ratio $\frac{[G(\xi, \sigma)]^2}{[F(\xi, \sigma)]^2}$ instead, for convenience; our goal is to prove that this is less than $1/5^2$. We have
\begin{align*}
(\delta - 1) \cdot \frac{[G(\xi, \sigma)]^2}{[F(\xi, \sigma)]^2} = \frac{4 (\delta - 2) \sin^4 \alpha + \pi^2 - (\pi - 2\alpha + \sin(2\alpha))^2 + s^2}{(\pi - 2\alpha + \sin(2\alpha))^2}
\end{align*}
Since $\alpha \leq 0.2$ in the good region, we have the easily verified bounds
\begin{align*}
(\pi - 2\alpha + \sin(2\alpha))^2 &\geq (1 + \pi/2)^2, \qquad \text{ and } \\
4(\delta - 2) \sin^4 \alpha + \pi^2 - (\pi - 2\alpha + \sin(2\alpha))^2 &\leq 4(\delta - 2) \alpha^4 + 2(2\alpha - \sin(2\alpha)) \\
& \leq 4(\delta - 2) \alpha^4 + \frac{8}{3} \alpha^3.
\end{align*} 
Putting together the pieces yields
\begin{align}
\frac{[G(\xi, \sigma)]^2}{[F(\xi, \sigma)]^2} &\leq \frac{\delta - 2}{\delta - 1} \cdot \alpha^4 + \frac{2}{3(\delta - 1)} \alpha^3 + \frac{s^2}{4(\delta - 1)} \notag \\
&\leq \frac{\delta - 2}{125(\delta - 1)} \alpha^2 + \frac{2}{15(\delta - 1)} \alpha^2 + \frac{s^2}{4(\delta - 1)} \leq 6^{-2},  \label{eq:rec-ratiobound}
\end{align}
where the final step holds for large enough $\delta$ and small enough $s^2 / \delta$.
\qed


%
%We claim that if $\theta \in \mathbb{G}$, then
%\begin{align*}
%\| T(\theta) - \theta^* \|^2 = [F(\xi, \sigma)]^2 + (1 - G(\xi, \sigma))^2 \leq \frac{1}{4} \{ \sigma^2 + (1 - \xi)^2 \}^3 = \frac{1}{2} \| \theta - \theta^* \|^3,
%\end{align*}
%thereby establishing that the Gordon update enjoys $(1/2, 3/2)$-superlinear convergence.
%
\subsubsection{Proof of Lemma~\ref{AM-PR-convergence}}

Let us establish the upper and lower bounds separately. 

\paragraph{Proof of upper bound:} Note that it suffices to establish the bound with $C_{\delta} = 1$. First, recall that any $(\xi, \sigma) \in \GPR$ satisfies $\xi \geq 0.93$ and $\xi^3 \geq 0.7$. We also have $\alpha \leq \sigma/ \xi \leq 1/5$. Thus,
\begin{align}
[G(\xi, \sigma)]^2 &= \frac{\delta - 2}{\delta - 1} \cdot \frac{4}{\pi^2} \cdot \sin^4 \alpha + \frac{1}{\delta - 1} \cdot (1 - [F(\xi, \sigma)]^2 ) + \frac{s^2}{\delta - 1} \notag \\
&\leq \frac{4}{\pi^2} \alpha^4 + \frac{1}{\delta - 1} (1 - F(\xi, \sigma)) (1 + F(\xi, \sigma)) + \frac{s^2}{\delta - 1} \notag \\
&\leq \frac{4}{\pi^2} \alpha^4 + \frac{2}{(\delta - 1)\pi} (2 \alpha - \sin(2\alpha)) + \frac{s^2}{\delta - 1} \notag \\
&\leq \frac{\alpha^3}{4} + \frac{s^2}{\delta - 1} \leq \frac{3\sigma^3}{7} + \frac{s^2}{\delta - 1}, \label{eq:sigma-ineq}
\end{align}
where the last line follows since $\delta \geq 8$, $\alpha \leq 1/5$, and $\xi^3 \geq 0.7$. We also have
\begin{align}
(1 - F(\xi, \sigma))^2 &= \frac{1}{\pi^2} (2 \alpha - \sin(2\alpha))^2 \leq \frac{16}{9 \pi^2} \alpha^6 \leq \frac{16}{9\pi^2} \cdot \frac{\alpha^3}{125} \leq  \sigma^3 / 350, \label{eq:xi-ineq}
\end{align}
where the penultimate inequality follows since $\alpha \geq 1/5$, and the last inequality is a consequence of the condition $\xi^3 \geq 0.7$. 

Putting together the pieces, we have
\begin{align*}
[\DeltaSE(\mathcal{S}_{gor}(\nu))]^2 &= [G(\xi, \sigma)]^2 + (1 - F(\xi, \sigma))^2 \\
&\leq \sigma^3 + \frac{s^2}{\delta - 1} \\
&\leq \left\{ \sigma^2 + (1 - \xi)^2 \right\}^{3/2} + \frac{s^2}{\delta - 1},
\end{align*}
and the desired upper bound follows from the elementary inequality $\sqrt{a + b} \leq \sqrt{a} + \sqrt{b}$.


\paragraph{Proof of lower bound:} Given that we are interested in a burn-in period of $t_0 = 1$, let us now compute two steps of the Gordon update, letting $F_{+} = F^2(\xi, \sigma)$ and $G_+ = G^2(\xi, \sigma)$. Analogously, we let $F = F(\xi, \sigma)$ and $G = G(\xi, \sigma)$, and use $\alpha_+ = \tan^{-1} (G/F)$ to denote the angle after one step of the Gordon update. Recall that $\tan \alpha = \sigma/\xi$. We have
\begin{align*}
G_{+}^2 &\geq \frac{\delta - 2}{\delta - 1} \cdot \frac{4}{\pi^2} \cdot \sin^4 \alpha_+ + \frac{1}{\delta - 1} \cdot (1 - F_+^2 ) + \frac{s^2}{\delta - 1} \\
&\geq \frac{1}{(\delta - 1)\pi} (2 \alpha_+ - \sin(2\alpha_+)) + \frac{s^2}{\delta - 1} \\
&\geq \frac{1}{8(\delta - 1)\pi} \left( \frac{G}{F} \right)^3 + \frac{s^2}{\delta - 1} \\
&\geq \frac{1}{8(\delta - 1)\pi} G^3 + \frac{s^2}{\delta - 1}.
\end{align*}
Here, the penultimate inequality uses the fact that $x - \sin x \geq \frac{\tan^3 x}{8}$ for all $x \leq \pi/6$, and the last inequality makes use of $F \leq 1$, guaranteed by one step of the Gordon update. Turning now to the $F_+$ component, we have
\begin{align*}
\pi^2 (1 - F_+)^2  = (2 \alpha_+ - \sin(2\alpha_+))^2 \geq \frac{G^6}{64}.
\end{align*}
Putting together the pieces yields
\begin{align*}
G_{+}^2 + (1 - F_+)^2 &\geq c_{\delta} \cdot G^3 + \frac{s^2}{\delta - 1} + \frac{G^6}{64\pi^2}  \\
&\geq c_{\delta} \cdot G^3 + \frac{s^2}{\delta - 1} + \frac{1}{64\pi^2} \left( \frac{1}{\delta - 1} \cdot (1 - F^2 ) \right)^3 + \frac{1}{64\pi^2} \left( \frac{s^2}{\delta - 1} \right)^3 \\
&\geq c_{\delta} \cdot G^3 + \frac{1}{16\pi^2 (\delta - 1)^3} \cdot (1 - F)^3 +  \frac{s^2}{\delta - 1} \\
&\geq c'_{\delta} \cdot \left\{ G^2 + (1 - F)^2 \right\}^{3/2} + \frac{s^2}{\delta - 1}
\end{align*}
where the last step follows because $(A + B)^{\kappa} \leq 2^{\kappa} (A^\kappa + B^{\kappa})$ for any positive scalars $(A, B)$ and $\kappa \geq 1$.
%
% (a) we have that for all $\alpha \leq 1/2$,
% \[
% \pi^2 (1 - F)^2 = (2 \alpha - \sin(2\alpha))^2 \geq \alpha^6,
% \] 
% and (b) $s^2 / (\delta - 1) \leq c$ for a small universal constant $c$.
%
% Putting this together with the fact that $\delta \geq 5$ and $1 - F \leq 1/10$, we have
% \[
% \sqrt{G_{+}^2 + (1 - F_+)^2} \leq \sqrt{G^3 + (1 - F)^3 + C \cdot \frac{s^2}{\delta - 1}} \leq \{ G^{2} + (1 - F)^2\}^{3/2} + \frac{s}{\sqrt{\delta }},
% \]
% where the last inequality follows since $\| x \|_p$ is decreasing in $p$ for $p \geq 0$. \apcomment{Need to put in lower bound.}
\qed

\subsection{Step 2: Empirical error is sharply tracked by Gordon state evolution}

We now prove part (b) of Theorem~\ref{thm:AM-PR}, showing that the size of the Gordon state evolution recursion closely tracks the error of the empirical update in the good region. Our result is actually stronger: we show that the empirical $\xi$ and $\sigma$ updates are individually tracked by the Gordon state evolution~\eqref{eq:Gordon-AM-PR-restated}. To state the result, let us make use of some additional notation. Recall that $F$ and $G$ denote the Gordon maps~\eqref{eq:Gordon-AM-PR-restated}. Let $\Fhat$ and $\Ghat$ denote the (random) empirical maps, i.e., $\Fhat(\xi(\theta), \sigma(\theta)) = \xi(\mathcal{T}_n(\theta))$ and $\Ghat(\xi, \sigma) = \sigma(\mathcal{T}_n(\theta))$. 

Recall the following concentration bound relating the iterate maps to their Gordon counterparts, \apcomment{This needs to appear as lemma in one of the previous sections.} where we use the convenient shorthand
\begin{align*}
\Deltaxi_n(\epsilon) := \left( \frac{C\log^{3} (C/ \epsilon)}{n} \right)^{1/2} \qquad \text{ and } \qquad \Deltasigma_n(\epsilon) := \left( \frac{C \log(C n/ \epsilon )}{n} \right)^{1/4}.
\end{align*}
We have
\begin{align*}
\Pr \left\{ |\Fhat (\xi, \sigma) - F (\xi, \sigma) | \geq \Deltaxi_n(\epsilon) \right\} \leq \epsilon \quad \text{ and } \quad
\Pr \left\{ |\Ghat (\xi, \sigma) - G (\xi, \sigma) | \geq \Deltasigma_n(\epsilon) \right\} \leq \epsilon.
\end{align*}
In the following key lemma, we use the shorthand $\Delta_{n, \epsilon, T} := \Deltaxi_n(\epsilon/T) \lor \Deltasigma_n(\epsilon/T)$.

\begin{lemma} \label{lem:elbow-right}
Suppose the initial point $(\xi, \sigma)$ is in the good region $\GPR$, and that $\delta \geq 42$. There are universal positive constants $(c_1,c_2)$ such that if $n$ is large enough to ensure that $\Delta_{n, \epsilon, T} \leq c_1$, then for each $T \geq 1$, we have
\begin{align*}
\sup_{1 \leq t \leq T} \; | \Fhat^t(\xi, \sigma) - F^t(\xi, \sigma)| \lor | \Ghat^t(\xi, \sigma) - G^t(\xi, \sigma)| \leq c_2 \cdot \Delta_{n, \epsilon, T}
\end{align*}
with probability exceeding $1 - 2 \epsilon$.
\end{lemma}

We prove the lemma momentarily, but let us use it to establish part (b) of the theorem. 

\subsubsection{Proof of Theorem~\ref{thm:AM-PR}(b)} \label{sec:thm1bproof}
Note that $\| \mathcal{T}_n^t(\theta) - \thetastar \|^2 = [1 - \Fhat^t(\xi, \sigma)]^2 + [\Ghat^t(\xi, \sigma)]^2$, and $[\DeltaSE(\mathcal{S}^t_{gor}(\nu))]^2 = [1 - F^t(\xi, \sigma)]^2 + [G^t(\xi, \sigma)]^2$. Consequently, for each $1 \leq t \leq T$, we have
\begin{align*}
\Big| \| \mathcal{T}_n^t (\theta) - \thetastar \| - \DeltaSE(\mathcal{S}^t_{gor}(\nu) \Big| \leq  \sqrt{2} \left\{ |\Fhat^t(\xi, \sigma) - F^t(\xi, \sigma) | \lor |\Ghat^t(\xi, \sigma) - G^t(\xi, \sigma)| \right\} \lesssim \Delta_{n, \epsilon, T},
\end{align*}
where the second inequality holds on the event guaranteed by Lemma~\ref{lem:elbow-right}. Putting together the pieces completes the proof of Theorem~\ref{thm:AM-PR}(b). \qed

\subsubsection{Proof of Lemma~\ref{lem:elbow-right}}
%\apcomment{Copy-pasted. Clean for consistency.}
Denote  by $\{\xibar_t, \sigmabar_t\}_{t \geq 0}$ the population Gordon sequence initialized at $(\xi, \sigma)$; in other words, let $\xibar_t = F^t(\xi, \sigma)$ and $\sigmabar_t = G^t (\xi, \sigma)$. Let $\{\xi_t, \sigma_t\}_{t \geq 0}$
denote the empirical sequence, with $\xi_t = \Fhat^t(\xi, \sigma)$ and $\sigma_t = \Ghat(\xi, \sigma)$. Let $c_1 = 1/200$ for concreteness.
%
%\apcomment{Need to show square condition on empirics by showing that Gordon maintains monotonicity?}
%Now if $(\xibar_t, \sigmabar_t) \in \GPR$, then Lemma~\ref{AM-PR-good-region} yields that .
The following claim is the crux of the argument.

\begin{subequations} \label{eq:key-claim}
Suppose the pairs $(\xi_t, \sigma_t)$ and $(\xibar_t, \sigmabar_t)$ satisfy the inequalities
\begin{align} \label{eq:key-claim-condn}
\xibar_t^2 + \sigmabar_t^2 &\geq 0.9, \quad \quad \xibar_t/\sigmabar_t \geq 5, \quad \text{ and } \quad |\xi_t - \xibar_t| \lor |\sigma_t - \sigmabar_t| \leq 1/200.
\end{align}
Then, we have the relations
\begin{align} \label{eq:key-claim-det}
\xibar_{t+1}^2 + \sigmabar_{t+1}^2 \geq 0.9 \qquad \qquad \text{ and } \qquad \qquad \xibar_{t+1}/\sigmabar_{t+1} \geq 5, 
\end{align}
and furthermore, with probability greater than $1 - \frac{2\epsilon}{T}$, we have
\begin{align} \label{eq:key-claim-prob}
|\xi_{t+1} - \xibar_{t+1}| \lor |\sigma_{t+1} - \sigmabar_{t+1}| \leq \Delta_{n, \epsilon, T} + (1 - \tau) \cdot \left( |\xibar_t - \xi_t| \lor |\sigmabar_t - \sigma_t| \right) \leq 1/200.
\end{align}
\end{subequations}

We take this claim as given for the moment, and establish the lemma. The conditions of the claim ensure that we may apply it recursively for $t = 0, \ldots, k - 1$ to obtain
\begin{align*}
| \Fhat^{k-1}(\xi_0, \sigma_0) - F^{k-1}(\xi_0, \sigma_0)| \lor | \Ghat^{k-1}(\xi_0, \sigma_0) - G^{k-1}(\xi_0, \sigma_0)| &=  | \xibar_k - \xi_k | \lor |\sigmabar_k - \sigma_k| \\
&\leq \sum_{i = 0}^{k - 1} (1 - \tau)^i \cdot \Delta_{n, \epsilon, T} \leq \frac{\Delta_{n, \epsilon, T} }{\tau},
\end{align*}
as desired. In stating this, we have used the fact that $\xibar_0 = \xi_0 = \xi$ and $\sigmabar_0 = \sigma_0 = \sigma$.

It remains to prove claim~\eqref{eq:key-claim}. The deterministic sub-claim~\eqref{eq:key-claim-det} follows directly from Lemma~\ref{AM-PR-good-region}, so we provide a proof of the probabilistic assertion~\eqref{eq:key-claim-prob}. By triangle inequality, we have
\begin{align*}
|\xibar_{t+1} - \xi_{t + 1}| &\leq | F(\xibar_t, \sigmabar_t) - F(\xi_t, \sigma_t)| + | F(\xi_t, \sigma_t) - \Fhat(\xi_t, \sigma_t)| \\
&\leq (1 - \tau) \cdot \left( |\xibar_t - \xi_t| \lor |\sigmabar_t - \sigma_t| \right) + | F(\xi_t, \sigma_t) - \Fhat(\xi_t, \sigma_t)|,
\end{align*}
where the second inequality follows from Lemma~\ref{lem:Gordon-pert} in the appendix, and we used the condition~\eqref{eq:key-claim-condn} in applying it.
%
Let $\mathcal{E}_t := \left\{ |\Fhat (\xibar_t, \sigmabar_t) - F (\xibar_t, \sigmabar_t) | \geq \Deltaxi_n(\epsilon/T) \right\}$, which by Lemma~\ref{} \apcomment{Need to label with overall concentration inequality.}, occurs with probability exceeding $1 - \frac{\epsilon}{T}$. On this event, we have
\begin{align*}
|\xibar_{t+1} - \xi_{t + 1}| \leq \Deltaxi_n(\epsilon/T) + (1 - \tau) \cdot \left( |\xibar_t - \xi_t| \lor |\sigmabar_t - \sigma_t| \right) \leq 1/200,
\end{align*}
where the last inequality since $\Delta_{n, \epsilon, T} < \tau/200$.
%
Proceeding identically for the perpendicular term and on the event $\mathcal{E}'_t := \left\{ |\Ghat (\xibar_t, \sigmabar_t) - G (\xibar_t, \sigmabar_t) | \geq \Deltasigma_n(\epsilon/T) \right\}$, we have
\begin{align*}
|\sigmabar_{t+1} - \sigma_{t + 1}| \leq \Deltasigma_n(\epsilon/T) + (1 - \tau) \cdot \left( |\xibar_t - \xi_t| \lor |\sigmabar_t - \sigma_t| \right) \leq 1/200,
\end{align*}
where once again we have used that $\Delta_{n, \epsilon, T} < \tau/200$. 
\qed

%\newpage

\subsection{Step 3: Convergence of empirics from random initialization to good region}

It remains to show that $T^{t_0}_n(\theta_0) \in \GPR$ after $t_0 = \mathcal{O}(\log d)$ iterations.
In order to do so, we employ the following two lemmas on the Gordon maps outside the good region.
% and we do so by splitting the analysis into two parts that focus directly on the empirics. First, in Lemma~\ref{lem:xi-jumps}, we show that $\xi_t$ increases exponentially from its initial value $d^{-1/2}$ up until $\xi/\sigma \geq 1/2$. Then, in Lemma~\ref{lem:ratio-jumps}, we show that provided the initial ratio $\xi_0/\sigma_0$ is larger than $1/2$, the ratio $\xi_t/ \sigma_t$ at time $t$ gets exponentially larger until it is greater than $5$.

\begin{lemma} \label{lem:xi-jumps}
Suppose the pair $(\xi, \sigma)$ satisfies $\frac{\xi}{\sigma} \leq 1/2$. Also suppose that $\delta \geq C$ and $s^2 / \delta \leq c$.
%There are universal positive constants $(c, C)$ such that if $n \geq C \cdot \log^{3}( 1/ \epsilon) \cdot \xi^{-2}$, then  on an event occuring with probability at least $1 - \epsilon$, we have
Then
\begin{align*}
F(\xi, \sigma) \geq 1.06 \cdot \frac{\xi}{\sigma} \quad \text{ and } \quad G(\xi, \sigma) \leq 0.95.
\end{align*}
%\begin{align*}
%\Fhat(\xi, \sigma) \geq (1 + c) \xi \quad \text{ and } \quad \Ghat(\xi, \sigma) \leq 1.
%\end{align*}
%with probability greater than $1 - \epsilon$.
\end{lemma}

%The previous lemma ensures that provided we initialize at random, we will have $\xi_t/\sigma_t \geq 1/2$ after $t = \mathcal{O}(\log d)$ iterations. It remains to boost this result to obtain an iterate in the ``good'' region covered by the previous section. Using the next lemma, we show that this happens after a constant number of further iterations.

\begin{lemma} \label{lem:ratio-jumps}
Suppose $\delta \geq C$ and $s^2 \leq c$. 
%There is a constant $C_{\epsilon}$ depending only on $\epsilon$ and a universal positive constant $c$ such that if $n \geq C_\epsilon$, 
Then for all $(\xi, \sigma)$ pairs satisfying $1/2 \leq \xi/\sigma \leq 5$, we have 
\begin{align*}
\frac{8}{7} \cdot \frac{\xi}{\sigma} \leq \frac{F(\xi, \sigma)}{G(\xi, \sigma)} \leq 50.
\end{align*}
%\begin{align*}
%\frac{\Fhat(\xi, \sigma)}{\Ghat(\xi, \sigma)} \geq (1 + c) \cdot \frac{\xi}{\sigma}
%\end{align*}
%with probability greater than $1 - \epsilon$.
\end{lemma}
We prove both lemmas at the end of this section.
First, we make use of these lemmas to prove Theorem~\ref{thm:AM-PR}(c).

\subsubsection{Proof of Theorem~\ref{thm:AM-PR}(c)} \label{sec:thm1cproof}

Recall that $\xi_0 / \sigma_0 \geq \frac{1}{100{\sqrt{d}}}$ by assumption, and let $(\xi_t, \sigma_t)$ denote the empirical state evolution. 
Set 
\[
t_0 = \log_{1.05} (50 \sqrt{d}) + \log_{64/63} (10) + 2,
\] %for a sufficiently large but universal constant $C$.
and define the scalar $\underline{t} := \log (50 \sqrt{d}) + 1$. For each $t \geq 0$, define the event
%\[
%\mathcal{E}_t = \{ \Fhat(\xi_t, \sigma_t) \geq (1 + c) \xi_t \quad \text{ and } \quad \Ghat(\xi_t, \sigma_t) \leq 1 \}. 
%\]
%
%The first step of the proof is to control $(\xi_1, \sigma_1)$. Let 
\[
\mathcal{E}_t =\left\{ |\Fhat(\xi_t, \sigma_t) - F(\xi_t, \sigma_t)| \leq \frac{\cpar}{\sqrt{d}} \text{ and } |\Ghat(\xi_t, \sigma_t) - G(\xi_t, \sigma_t)| \leq \cperp \right\}, 
\]
for small enough universal constants $\cpar$ and $\cperp$.

By Lemma XXX \apcomment{full general lemma}, for each $t$, we have $\Pr\{ \mathcal{E}_t\} \geq 1 - \frac{\epsilon}{\underline{t}}$ provided $n \geq C d \log^3 \left( \frac{1 + \log d}{\epsilon} \right)$ for a large enough universal constant $C$. By a union bound, the event $\mathcal{E} := \cap_{t = 0}^{\underline{t}} \mathcal{E}_t$ occurs with probability greater than $1 - \epsilon$. Also define the (random) time steps
\begin{align*}
\underline{T} = \inf \left\{ t \mid \frac{\xi_t}{\sigma_t} \geq 1/2 \right\} \qquad \text{ and } \qquad  
T_0 = \inf \left\{ t \mid \frac{\xi_t}{\sigma_t} \geq 5 \right\}.
\end{align*}
The following claim is the crux of the argument.
\begin{claim} \label{clm:t-bound}
On event $\mathcal{E}$, we have $\underline{T} \overset{(a)}{\leq} \underline{t}$ and $T_0 \overset{(b)}{\leq} t_0 - 1$.
\end{claim}
Taking the claim as given for the moment, let us prove the theorem. Working on the event $\mathcal{E}$, we have $\frac{\xi_{T_0}}{\sigma_{T_0}} \geq 5$ and $T_0 \leq t_0 - 1$. Our goal is to show that $(\xi_{T_0 + 1}, \sigma_{T_0 + 1}) \in \GPR$. Owing to claim~\ref{clm:t-bound}(b), we have $T_0 + 1 \leq t_0$, and so
\begin{align} \label{eq:pert-bound}
|\xi_{T_0 + 1} - F(\xi_{T_0}, \sigma_{T_0})| \leq \frac{\cpar}{\sqrt{d}} \qquad \qquad \text{ and } \qquad \qquad |\sigma_{T_0 + 1} - G(\xi_{T_0}, \sigma_{T_0})| \leq \cperp
\end{align}
for a sufficiently small constant $\cperp$. Since $\xi_{T_0} / \sigma_{T_0} \geq 5$, the relations~\eqref{eq:rec-Gbound},~\eqref{eq:rec-sqbound}, and~\eqref{eq:rec-ratiobound} yield the bounds
\begin{align*}
G(\xi_{T_0}, \sigma_{T_0}) \leq 1, \quad [F(\xi_{T_0}, \sigma_{T_0})]^2 + [G(\xi_{T_0}, \sigma_{T_0})]^2 \geq [F(\xi_{T_0}, \sigma_{T_0})]^2 \geq 0.95 \quad 
\text{ and } \quad  
\frac{F(\xi_{T_0}, \sigma_{T_0})}{G(\xi_{T_0}, \sigma_{T_0})} \geq 6,
\end{align*}
respectively. Combining the first two bounds with the perturbation bound~\eqref{eq:pert-bound} yields the relations
\begin{align} \label{eq:first-two-GPR}
\sigma_{T_0 + 1} \leq 1.05 \qquad \text{ and } \xi_{T_0 + 1}^2 + \sigma^2_{T_0 + 1} \geq 0.9,
\end{align}
as desired. In order to prove a lower bound on the ratio $\xi_{T_0 + 1} / \sigma_{T_0 + 1}$, we first show an upper bound on the ratio 
$\xi_{T_0}/ \sigma_{T_0}$. Note that for each $(\xi, \sigma)$ pair, we have 
%
%Let us begin with the individual Gordon updates. We have 
\begin{subequations} \label{eq:double-eq}
\begin{align}
F(\xi, \sigma) \geq \frac{2}{\pi} \tan^{-1} (\xi/\sigma) \geq \frac{2}{\pi} \cdot \frac{\xi/\sigma}{\sqrt{1 + \left( \xi/\sigma \right)^2 }},
\end{align}
and
%where the last inequality follows from the lower bound $\xi_{T_0} / \sigma_{T_0} \leq 50$, and
\begin{align}
G(\xi, \sigma) \geq \sqrt{\frac{\delta - 2}{ \delta - 1}} \cdot \frac{2}{\pi} \cdot \sin^2 \alpha =  \sqrt{\frac{\delta - 2}{ \delta - 1}} \cdot \frac{2}{\pi} \cdot \frac{1}{1 + \left(\xi/\sigma \right)^2} \stackrel{(ii)}{\geq} \sqrt{\frac{8}{9}} \cdot \frac{2}{\pi} \cdot  \frac{1}{1 + \left(\xi/\sigma \right)^2},
\end{align}
\end{subequations}
where the final step follows for $\delta \geq C$.
Setting $(\xi, \sigma) = (\xi_{T_0 - 1}, \sigma_{T_0 - 1})$ and noting by definition of $T_0$ that $1/2 \leq \xi_{T_0 - 1}/\sigma_{T_0 - 1} \leq 5$, we have $F(\xi_{T_0 -1}, \sigma_{T_0 - 1}) \geq \frac{2}{\pi \sqrt{5}}$ and $G(\xi_{T_0 -1}, \sigma_{T_0 - 1}) \geq \frac{4 \sqrt{2}}{78 \pi}$. Moreover, Lemma~\ref{lem:ratio-jumps} yields $\frac{F(\xi_{T_0 -1}, \sigma_{T_0 - 1})}{G(\xi_{T_0 -1}, \sigma_{T_0 - 1})} \leq 50$, and combining the pieces with the perturbation relation guaranteed by the event $\mathcal{E}_{T_0}$ yields
$\xi_{T_0}/\sigma_{T_0} \leq 52$. Given that we have the upper bound $5 \leq \xi_{T_0}/\sigma_{T_0} \leq 52$ in hand, applying the same argument once again yields $F(\xi_{T_0}, \sigma_{T_0}) \geq c_1$ and $G(\xi_{T_0}, \sigma_{T_0}) \geq c_2$ for universal positive constants $c_1$ and $c_2$. Combining these with the above relation $F(\xi_{T_0}, \sigma_{T_0}) / G(\xi_{T_0}, \sigma_{T_0}) \geq 6$ and the perturbation bound~\eqref{eq:pert-bound}, we can choose $\cperp$ and $\cpar$ small enough to ensure that $\xi_{T_0 + 1} / \sigma_{T_0 + 1} \geq 5$. Putting this together with equation~\eqref{eq:first-two-GPR}, we see that $(\xi_{T_0 + 1}, \sigma_{T_0 + 1}) \in \GPR$, as desired. \qed

\iffalse
for a sufficiently small constant $c'$ that results from using the upper bound $\xi_0 / \sigma_0 \geq 5$
In step (ii), we use our lower bound $\delta \geq C$.

Now suppose $n$ is large enough to ensure that $\Deltaxi_n(\epsilon) \lor \Deltasigma_n(\epsilon) \leq 1/400$. Then owing to the above bounds, we have $\Fhat(\xi, \sigma) \geq \frac{80}{81} F(\xi, \sigma)$ and $\Ghat(\xi, \sigma) \leq \frac{10}{9} G(\xi, \sigma)$ with probability $1 - 2\epsilon$. 
Thus, on this event,
%Putting together the pieces with Lemma~\ref{lem:Gordon-AM-struct}(a), 
we have
\begin{align} \label{eq:ratio1}
\frac{\Fhat(\xi, \sigma)}{\Ghat(\xi, \sigma)} \geq \frac{9}{10} \cdot \frac{80}{81} \cdot \frac{F(\xi, \sigma)}{G(\xi,\sigma)} = \frac{8}{9} \cdot \frac{F(\xi, \sigma)}{G(\xi,\sigma)}.
\end{align}
It remains to relate the ratio $F(\xi, \sigma)/ G(\xi, \sigma)$ to $\xi/\sigma$, and we claim that if $1/2 \leq \xi/\sigma \leq 5$, then
\begin{align} \label{eq:ratio2}
\frac{F(\xi, \sigma)}{G(\xi, \sigma)} \geq \frac{8}{7} \cdot \frac{\xi}{\sigma}.
\end{align}
Indeed, the lemma follows directly by combining equations~\eqref{eq:ratio1} and~\eqref{eq:ratio2}, so we dedicate the rest of this proof to establishing claim~\eqref{eq:ratio2}.

\apcomment{Rest of this needs to be edited.}
\fi
\noindent It remains to prove Claim~\ref{clm:t-bound}.

\paragraph{Proof of Claim~\ref{clm:t-bound}(a):}
We will prove the stronger statement that on the event $\cap_{t = 0}^{\underline{t}} \mathcal{E}_t$, we have $\underline{T} \leq \underline{t}$. Suppose for the sake of contradiction that $\underline{T} > \underline{t}$. We prove (momentarily, by induction) that for all $1 \leq t \leq \underline{t}$,
\begin{align} \label{clm:ind}
\xi_{t} \geq (1.05)^{t-1} \cdot \xi_1 \qquad \text{ and } \qquad \sigma_{t} \leq 1.
\end{align}
But before this, note that on event $\mathcal{E}_0$, we have 
\begin{align*}
\xi_1 \geq F(\xi_0, \sigma_0) - \frac{\cpar}{\sqrt{d}} \geq  \frac{1.06}{100\sqrt{d}} - \frac{\cpar}{\sqrt{d}} \geq \frac{1}{100\sqrt{d}},
\end{align*}
where the first inequality follows from Lemma~\ref{lem:xi-jumps}, and the second inequality follows for small enough~$\cpar$. But putting together the above two displays, we have
\begin{align*}
\xi_{\underline{t}} \geq \frac{50 \sqrt{d}}{100 \sqrt{d}} = 1/2 \quad \text{ and } \quad \sigma_{\underline{t}} \leq 1,
\end{align*}
so that their ratio is greater than $1/2$. This provides the contradiction and proves the theorem. 

To prove claim~\eqref{clm:ind}, note that the base case $t = 1$ holds trivially. For the induction hypothesis, suppose that $\xi_t \geq (1.05)^t \cdot \xi_1 \geq \frac{1}{100 \sqrt{d}}$, and $\sigma_t \leq 1$. Note that $\xi_t / \sigma_t \leq 1/2$ by assumption. Then applying Lemma~\ref{lem:xi-jumps}, we have
\begin{align*}
\xi_{t + 1} \geq F(\xi_t, \sigma_t) - \frac{\cpar}{\sqrt{d}} \geq 1.06 \cdot \frac{\xi_t}{\sigma_t} - \frac{\cpar}{\sqrt{d}} \geq 1.05 \xi_t \geq (1.05)^t \cdot \xi_1.
\end{align*}
Lemma~\ref{lem:xi-jumps} also yields
\begin{align*}
\sigma_{t + 1} \leq G(\xi_t, \sigma_t) + \cperp \leq 0.95 + 0.05 \leq 1.
\end{align*}
This completes the induction step and hence proves the claim.
\qed
\iffalse
Furthermore, on event $\cap_{t = 0}^{\underline{t}} \mathcal{E}_t$, we have that for all $t \leq \underline{t}$, 
\begin{align} \label{eq:sigbound}
\sigma_{t+1} \leq G(\xi_t, \sigma_t) + 0.05,
\end{align}
where the last step follows since $\delta \geq C$ and $s^2 / \delta \leq c$.

, and fix some $1 \leq t \leq \underline{t}$. 
Since $\xi_t / \sigma_t < 1/2$ and owing to the bound~\eqref{eq:sigbound}, we may apply Lemma~\ref{lem:xi-jumps} to obtain
\begin{align*}
F(\xi_t, \sigma_t) \geq 1.06 \xi_t
\end{align*}

Let $\mathcal{E}_t$ denote the event guaranteed by Lemma~\ref{lem:xi-jumps} as applied to $(\xi,\sigma) = (\xi_t, \sigma_t)$, i.e.,
\[
\mathcal{E}_t = \{ \Fhat(\xi_t, \sigma_t) \geq (1 + c) \xi_t \quad \text{ and } \quad \Ghat(\xi_t, \sigma_t) \leq 0.05 \}. 
\]
Let $\underline{T} := \log (50 \sqrt{d}) + 1$, and define
$\underline{t} = \inf \left\{ t \mid \frac{\xi_t}{\sigma_t} \geq 1/2 \right\}$. 
\fi

\paragraph{Proof of Claim~\ref{clm:t-bound}(b):} 
%In order to prove this claim, it suffices to show that $\xi/\sigma \geq 5$ once $\log_{64/63} (10)$ iterations have passed after $\underline{t}$. 
We work on the event $\mathcal{E}$, and as before, we establish the claim by contradiction. Assume that $T_0 \geq t_0$, and note that $\xi_{\underline{t}}/\sigma_{\underline{t}} \geq 1/2$ by part (a) of the claim. We will show momentarily that for each $\underline{t} \leq t$, we have
\begin{align} \label{eq:ind2}
\frac{\xi_t}{\sigma_t} \geq \left( \frac{64}{63} \right)^{t - \underline{t}} \cdot \frac{\xi_{\underline{t}}}{\sigma_{\underline{t}}},
\end{align}
so that setting $t = t_0 - 1$, we obtain a contradiction since $\frac{\xi_t}{\sigma_t} \geq 10 \cdot \frac{1}{2} \geq 5$. 

To prove claim~\eqref{eq:ind2}, note once again that the base case in trivial. For the induction hypothesis, suppose that $\frac{\xi_t}{\sigma_t} \geq \left( \frac{64}{63} \right)^{t - \underline{t}} \cdot \frac{\xi_{\underline{t}}}{\sigma_{\underline{t}}} \geq 1/2$. By assumption, we have $\xi_t / \sigma_t \leq 5$, so that Lemma~\ref{lem:ratio-jumps} yields $\frac{F(\xi_t, \sigma_t)}{G(\xi_t, \sigma_t)} \geq \frac{8}{7}\cdot \frac{\xi_t}{\sigma_t}$. Since $1/2 \leq \xi_t/\sigma_t \leq 5$, the argument below equation~\eqref{eq:double-eq} yields the bounds $F(\xi_t, \sigma_t) \geq \frac{2}{\pi \sqrt{5}}$ and $G(\xi_t, \sigma_t) \geq \frac{4\sqrt{2}}{78\pi}$. Combining this with the bounds
\begin{align*}
|\xi_{t + 1} - F(\xi_t, \sigma_t)| \leq \frac{\cpar}{\sqrt{d}} \quad \text{ and } \quad |\sigma_{t + 1} - G(\xi_t, \sigma_t)| \leq \cperp,
\end{align*}
and choosing sufficiently small constants $(\cpar, \cperp)$, we have 
\[
\xi_{t + 1}/ \sigma_{t + 1} \geq \frac{8}{9} \cdot \frac{F(\xi_t, \sigma_t)}{G(\xi_t, \sigma_t)} \geq \frac{64}{63} \left( \frac{64}{63} \right)^{t - \underline{t}} \cdot \frac{\xi_{\underline{t}}}{\sigma_{\underline{t}}},
\]
thereby completing the inductive step.
\qed

\subsubsection{Proof of Lemma~\ref{lem:xi-jumps}}
Write $\beta = \pi/2 - \alpha = \tan^{-1} (\xi/\sigma)$. The expression~\eqref{eq:Gordon-AM-PR-xi} for the Gordon update yields
\begin{align*}
F(\xi, \sigma) = \frac{2 \beta + \sin 2\beta }{\pi}
\stackrel{(i)}{\geq} \frac{4\beta}{\pi} - \frac{4 \beta^3}{3\pi}
\stackrel{(ii)}{\geq} \frac{4}{\pi} \left( \frac{\xi}{\sigma} \right) - \frac{8}{3\pi} \left( \frac{\xi}{\sigma} \right)^3
\end{align*}
where in step (i), we have used the fact that $\sin x \geq x - \frac{x^3}{6}$ and in step (ii) we have used the Taylor expansion of the $\tan^{-1}$ function to conclude that $x - \frac{x^3}{3} \leq \tan^{-1} x \leq x$. Now using the facts that $\xi/\sigma \leq 1/2$ and $\sigma \leq 1$, respectively, we have
\begin{align*}
F(\xi, \sigma) \geq \frac{10}{3\pi} \left( \frac{\xi}{\sigma} \right) > 1.06 \cdot \frac{\xi}{\sigma}.
\end{align*}
We also have
\begin{align*}
[G(\xi, \sigma)]^2 \leq \frac{4}{\pi^2} \sin^4 \alpha + \frac{1}{\delta - 1} \left( 1 - [F(\xi, \sigma)]^2 s^2 \right) \leq \frac{4}{\pi^2} + \frac{1 + s^2}{\delta - 1} \leq 1, 
\end{align*}
where the final inequality holds for $\delta \geq C$ and $s^2 / \delta \leq c$.
%Finally, note that for a large enough constant $C_{\epsilon}$ depending on $\epsilon$ alone, we have $\Deltaxi_n(\epsilon) \leq 0.005 \xi$. Since $|\Fhat(\xi, \sigma) - F(\xi, \sigma)| \leq \Deltaxi_n(\epsilon)$ with probability greater than $1 - \epsilon$, we have on this event that
%$\Fhat(\xi, \sigma) \geq 1.005 \xi$,
%as desired.
\qed

\subsubsection{Proof of Lemma~\ref{lem:ratio-jumps}}

\iffalse %move to earlier
Let us begin with the individual Gordon updates. We have 
\begin{align*}
F(\xi, \sigma) \geq \frac{2}{\pi} \tan^{-1} (\xi/\sigma) \geq \frac{2}{\pi} \cdot \frac{\xi/\sigma}{\sqrt{1 + \left( \xi/\sigma \right)^2 }} \geq \frac{2}{\pi \sqrt{5}},
\end{align*}
where the final step holds since $\xi/\sigma \geq 1/2$ and the map $x \mapsto x / \sqrt{1 + x^2}$ is monotone. Moreover,
\begin{align*}
G(\xi, \sigma) \geq \sqrt{\frac{\delta - 2}{ \delta - 1}} \cdot \frac{2}{\pi} \cdot \sin^2 \alpha =  \sqrt{\frac{\delta - 2}{ \delta - 1}} \cdot \frac{2}{\pi} \cdot \frac{1}{1 + \left(\xi/\sigma \right)^2} \stackrel{(ii)}{\geq} \sqrt{\frac{8}{9}} \cdot \frac{2}{\pi} \cdot  \frac{1}{1 + \left(\xi/\sigma \right)^2} \stackrel{(iii)}{\geq} \frac{4 \sqrt{2}}{78\pi}.
\end{align*}
In step (ii), we use our lower bound $\delta \geq 10$, and in step (iii), we use the fact that the map $x \mapsto (1 + x^2)^{-1}$ is monotone decreasing for positive $x$, in conjunction with the assumption $\xi/\sigma \leq 5$.

Now suppose $n$ is large enough to ensure that $\Deltaxi_n(\epsilon) \lor \Deltasigma_n(\epsilon) \leq 1/400$. Then owing to the above bounds, we have $\Fhat(\xi, \sigma) \geq \frac{80}{81} F(\xi, \sigma)$ and $\Ghat(\xi, \sigma) \leq \frac{10}{9} G(\xi, \sigma)$ with probability $1 - 2\epsilon$. 
Thus, on this event,
%Putting together the pieces with Lemma~\ref{lem:Gordon-AM-struct}(a), 
we have
\begin{align} \label{eq:ratio1}
\frac{\Fhat(\xi, \sigma)}{\Ghat(\xi, \sigma)} \geq \frac{9}{10} \cdot \frac{80}{81} \cdot \frac{F(\xi, \sigma)}{G(\xi,\sigma)} = \frac{8}{9} \cdot \frac{F(\xi, \sigma)}{G(\xi,\sigma)}.
\end{align}
It remains to relate the ratio $F(\xi, \sigma)/ G(\xi, \sigma)$ to $\xi/\sigma$, and we claim that if $1/2 \leq \xi/\sigma \leq 5$, then
\begin{align} \label{eq:ratio2}
\frac{F(\xi, \sigma)}{G(\xi, \sigma)} \geq \frac{8}{7} \cdot \frac{\xi}{\sigma}.
\end{align}
Indeed, the lemma follows directly by combining equations~\eqref{eq:ratio1} and~\eqref{eq:ratio2}, so we dedicate the rest of this proof to establishing claim~\eqref{eq:ratio2}.
%The proof of this lemma involves showing some properties about the square of the ratio 
\fi
%We now split the proof into two cases:
%
%\noindent \underline{Case $\alpha \in [0, \pi/4]$:} 
Note that $\tan^{-1}(1/5) \leq \alpha \leq \tan^{-1}(2)$. We prove the upper and lower bounds separately. 
\paragraph{Proof of lower bound:} 
Write $H_{\delta} := \left( \frac{G(\xi, \sigma)}{F(\xi, \sigma)} \div \frac{\sigma}{\xi} \right)^2$, and note that the Gordon recursion~\eqref{eq:Gordon-AM-PR-restated} yields
\[
(\delta - 1) \cdot H_{\delta} = \frac{\cot^2 \alpha}{(\pi - 2 \alpha + \sin (2\alpha))^2} \cdot \left\{ 4 (\delta - 2) \sin^4 \alpha + \pi^2 - (\pi - 2 \alpha + \sin (2\alpha))^2 + s^2 \right\}.
\]
We now split this proof into two cases.

\noindent \underline{Case $\alpha \in [\tan^{-1}(1/5), \pi/4]$:} In this case, we make use of the easily-verified bounds
\begin{align*}
\cot^2 \alpha &\leq \alpha^{-2}, \\
(\pi - 2\alpha + \sin(2\alpha))^2 &\geq (1 + \pi/2)^2, \qquad \text{ and } \\
4(\delta - 2) \sin^4 \alpha + \pi^2 - (\pi - 2\alpha + \sin(2\alpha))^2 &\leq 4(\delta - 2) \alpha^4 + 2(2\alpha - \sin(2\alpha)) \\
& \leq 4(\delta - 2) \alpha^4 + \frac{8}{3} \alpha^3.
\end{align*}
Substituting above yields
\begin{align*}
(\delta - 1) \cdot H_{\delta}(\alpha) \leq \frac{4(\delta - 2) \alpha^2 + \frac{8}{3} \alpha + s^2 \alpha^{-2}}{(1 + \pi/2)^2} \leq \frac{\pi^2 (\delta - 2) }{(\pi + 2)^2}  + \frac{8\pi}{3(\pi + 2)^2} + \frac{4s^2}{\alpha^2 (\pi + 2)^2} \leq 0.5 \cdot (\delta - 1).
\end{align*}
The last inequality follows by the assumptions $\delta \geq C$ and $s^2/ \delta \leq c$.

\noindent \underline{Case $\alpha \in [\pi/4, 2\pi/5)$:} Let $\beta = \pi/2 - \alpha$, and note that for all $\beta \in [\pi/5, \pi/4]$, we have
\begin{align*}
\tan^2 \beta &\leq \frac{16}{\pi^2} \cdot \beta^2 \\
(2 \beta + \sin(2 \beta))^2 &\geq 4 (1 + 2/\pi)^2 \beta^2, \text{ and } \\
4(\delta - 2) \cos^4 \beta + \pi^2 - (2 \beta + \sin(2 \beta))^2 &\leq 4(\delta - 2) + \pi^2.
\end{align*}
Substituting above yields
\begin{align*}
(\delta - 1) \cdot H_{\delta}(\alpha) \leq \frac{4}{(\pi + 2)^2} \cdot (4(\delta - 2) + \pi^2 + s^2 ) \leq 0.7 \cdot (\delta - 1).
\end{align*}
Once again, the last inequality holds provided $\delta \geq C$ and $s^2 / \delta \leq c$.
\smallskip

\noindent Putting together the two cases, we have $\frac{F(\xi, \sigma)}{G(\xi, \sigma)} \geq \frac{1}{\sqrt{0.7}} \frac{\xi}{\sigma} \geq \frac{8}{7} \cdot \frac{\xi}{\sigma}$.

\paragraph{Proof of upper bound:} It suffices to bound from below the quantity
\begin{align}
\left( \frac{G(\xi, \sigma)}{F(\xi, \sigma)} \right)^2 &= \frac{1}{(\pi - 2 \alpha + \sin (2\alpha))^2} \cdot \left\{ \frac{4(\delta - 2)}{\delta - 1} \cdot \sin^4 \alpha + \frac{\pi^2 - (\pi - 2 \alpha + \sin (2\alpha))^2 + s^2}{\delta - 1} \right\} \notag \\
&\geq \frac{100}{26} \frac{\sin^4 \alpha}{(\pi - 2 \alpha + \sin (2\alpha))^2}, \label{eq:AM-ratio-bound}
\end{align}
where the inequality follows for $\delta \geq C$. Since the RHS is increasing in $\alpha$, we may set $\alpha = \tan^{-1} (1/5)$ and evaluate to obtain $\left( \frac{G(\xi, \sigma)}{F(\xi, \sigma)} \right)^2 \geq 50^{-2}$, as desired. \qed 

%\subsection{Step 4: Putting it all toghet}
\newpage

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Proof of Theorem~\ref{thm:GD-PR}: Subgradient descent for phase retrieval}

Once again, recall that the good region for phase retrieval is given by $\GPR$, the set of $\nu = (\xi, \sigma)$ satisfying $\sigma \leq 1.05$, $\xi/\sigma \geq 5$,  and $\xi^2 + \sigma^2 \geq 0.9$. Also recall our assumption that $\delta \geq C$ and $s^2 / \delta \leq c$ for universal constants $(c, C)$. This will be used in multiple steps of the proof.
 
For convenience, we first restate the Gordon state evolution for this case, with stepsize $\eta = 1/2$.
\begin{align} \label{eq:Gordon-GD-PR-restated}
\begin{split}
\xigordon &= 1 - \frac{1}{\pi} (2 \alpha - \sin(2 \alpha)), \text{ and } \\
\sigmagordon &= \Big(  \frac{4}{\pi^2} \sin^4 \alpha 
 + \frac{1}{\delta - 1} \Big\{ \xi^2 + \sigma^2 - 2\xi \left(1 - \frac{1}{\pi} (2 \alpha - \sin(2 \alpha)) \right) - 2\sigma \cdot \frac{2}{\pi} \sin^2 \alpha + 1 + s^2 \Big\} \Big)^{1/2}. 
\end{split}
\end{align}
Notice that the $\xigordon$ update is identical to the AM case~\eqref{eq:Gordon-AM-PR-restated}. As before, we denote the maps (in equation~\eqref{eq:Gordon-GD-PR-restated}) $(\xi, \sigma) \mapsto \xigordon$ and $(\xi, \sigma) \mapsto \sigmagordon$ by $F$ and $G$, respectively. It is also convenient to write the $\sigmagordon$ map as
\begin{align}
\sigmagordon &= \Bigg( \frac{\delta - 2}{\delta - 1} \cdot g^2 + \frac{1}{\delta - 1} \Big\{ (\xi - f)^2 + (\sigma - g)^2 + (1 - f^2) + s^2 \Big\} \Bigg)^{1/2}, \label{eq:conv-rearrange}
\end{align}
where $f = 1 - \frac{1}{\pi} (2 \alpha - \sin(2 \alpha))$ and $g = \frac{2}{\pi} \sin^2 \alpha$.


%As before, the rest of the proof proceeds in three steps. Steps 1, 2, and 3 are used to prove parts (a), (b), and (c) of the theorem, respectively.

\subsection{Step 1: Convergence of the Gordon update in the good region}

Once again, we prove this using two lemmas.
\begin{lemma} \label{lem:GD-PR-good-region}
Suppose $\delta \geq C$ and $s^2 / \delta \leq c$. If $\nu \in \GPR$, then $\mathcal{S}_{gor}(\nu) \in \GPR$.
\end{lemma}

\begin{lemma} \label{lem:GD-PR-convergence}
Suppose $\delta \geq C$ and $s^2 / \delta \leq c$. Then for each $\nu = (\xi, \sigma) \in \GPR$, we have
\begin{align*}
c_{\delta} \cdot [\DeltaSE(\nu)]^2 + \frac{s^2}{\delta - 1} \leq [\DeltaSE(\mathcal{S}_{gor}(\nu))]^2 \leq C_{\delta} \cdot [\DeltaSE(\nu)]^{2} + \frac{s^2}{\delta - 1}.
\end{align*}
Here $0 \leq c_{\delta} \leq C_{\delta} \leq 1$ are constants that depend solely on $\delta$.
\end{lemma}

\subsubsection{Proof of Theorem~\ref{thm:GD-PR}(a)}
Taken together, Lemmas~\ref{lem:GD-PR-good-region} and~\ref{lem:GD-PR-convergence} clearly establish part (a) of the theorem, since they ensure the two conditions of Definition~\ref{def:linear} are satisfied. \qed
%\apcomment{Add more detail.} \qed
\medskip

We now prove each lemma in turn. 

\subsubsection{Proof of Lemma~\ref{lem:GD-PR-good-region}}
We must show that if the pair $(\xi, \sigma)$ satisfies $\sigma \leq 1.05$, $\xi^2 + \sigma^2 \geq 0.9$, and $\xi/\sigma \geq 5$, then the Gordon state evolution~\eqref{eq:Gordon-AM-PR-restated} satisfies $G(\xi, \sigma) \leq 1.05$, $[F(\xi, \sigma)]^2 + [G(\xi, \sigma)]^2 \geq 0.9$, and $F(\xi, \sigma)/G(\xi, \sigma) \geq 5$. We show each of these bounds separately.

\paragraph{Bounding $F(\xi, \sigma)$:} This step is immediate just as in the AM case, since for all $\alpha \in [0, \pi/2]$, we have $F(\xi, \sigma) \in [0, 1]$.

\paragraph{Bounding $G(\xi, \sigma)$:} We have
\begin{align} 
[G(\xi, \sigma)]^2 &= \frac{4}{\pi^2} \sin^4 \alpha 
 + \frac{1}{\delta - 1} \Big\{ \xi^2 + \sigma^2 - 2\xi \left(1 - \frac{1}{\pi} (2 \alpha - \sin(2 \alpha)) \right) - 2\sigma \cdot \frac{2}{\pi} \sin^2 \alpha + 1 + s^2 \Big\} \label{eq:rec-Gbound-GD} \\
&\leq \frac{4}{\pi^2}  + \frac{1}{\delta - 1} \{ 1.15 + 1.15 + 1 + s^2 \} \leq 1, \notag
\end{align}
where the first inequality follows since $\xi \lor \sigma \leq 1.05$, and the final step holds for large enough $\delta$ and small enough $s^2 / \delta$.

\paragraph{Bounding $[F(\xi, \sigma)]^2 + [G(\xi, \sigma)]^2$:} Since the $F$ map coincides with that of the AM update, this bound follows directly from equation~\eqref{eq:rec-sqbound}.

\paragraph{Bounding $\frac{F(\xi/\sigma)}{G(\xi, \sigma)}$:}  As before, our goal is to prove that $\frac{[G(\xi, \sigma)]^2}{[F(\xi, \sigma)]^2} \leq 1/5^2$. Since $\alpha \leq 0.2$ in the good region, we know that
\begin{align*}
[F(\xi, \sigma)]^2 = (\pi - 2\alpha + \sin(2\alpha))^2 &\geq (1 + \pi/2)^2;
\end{align*} 
furthermore, equation~\eqref{eq:rec-Gbound-GD} yields
\begin{align*}
[G(\xi, \sigma)]^2 &\leq \frac{4}{\pi^2} \left( 1 / 5 \right)^4  + \frac{1}{\delta - 1} \Big\{ \xi^2 + \sigma^2 + 1 + s^2 \Big\} \leq 0.01 + \frac{1}{\delta - 1} \{ 1.11 + 1.11 + 1 + s^2 \} \leq 1/6,
\end{align*}
where the last inequality follows for $\delta \geq C$ and $s^2 / \delta \leq c$. Putting together the pieces, we have $\frac{[G(\xi, \sigma)]^2}{[F(\xi, \sigma)]^2} \leq 1/6^2$, as desired.
\qed
\iffalse
We have
\begin{align*}
(\delta - 1) \cdot \frac{[G(\xi, \sigma)]^2}{[F(\xi, \sigma)]^2} = \frac{4 (\delta - 2) \sin^4 \alpha + \pi^2 - (\pi - 2\alpha + \sin(2\alpha))^2 + s^2}{(\pi - 2\alpha + \sin(2\alpha))^2}
\end{align*}
Since $\alpha \leq 0.2$ in the good region, we have the easily verified bounds
\begin{align*}
(\pi - 2\alpha + \sin(2\alpha))^2 &\geq (1 + \pi/2)^2, \qquad \text{ and } \\
4(\delta - 2) \sin^4 \alpha + \pi^2 - (\pi - 2\alpha + \sin(2\alpha))^2 &\leq 4(\delta - 2) \alpha^4 + 2(2\alpha - \sin(2\alpha)) \\
& \leq 4(\delta - 2) \alpha^4 + \frac{8}{3} \alpha^3.
\end{align*} 
Putting together the pieces yields
\begin{align}
\frac{[G(\xi, \sigma)]^2}{[F(\xi, \sigma)]^2} &\leq \frac{\delta - 2}{\delta - 1} \cdot \alpha^4 + \frac{2}{3(\delta - 1)} \alpha^3 + \frac{s^2}{4(\delta - 1)} \notag \\
&\leq \frac{\delta - 2}{125(\delta - 1)} \alpha^2 + \frac{2}{15(\delta - 1)} \alpha^2 + \frac{s^2}{4(\delta - 1)} \leq 6^{-2},  \label{eq:rec-ratiobound}
\end{align}
where the final step holds for large enough $\delta$ and small enough $s^2 / \delta$.
\qed
\fi

\subsubsection{Proof of Lemma~\ref{lem:GD-PR-convergence}}
First, recall that any $(\xi, \sigma) \in \GPR$ satisfies $\xi \geq 0.93$ and $\xi^3 \geq 0.7$. We also have $\alpha \leq \sigma/ \xi \leq 1/5$.  We now prove the upper and lower bounds separately.

\paragraph{Proof of upper bound:} We have
\begin{align*}
[G(\xi, \sigma)]^2 &\leq \frac{\delta - 2}{\delta - 1} \cdot \frac{4}{\pi^2} \sin^4 \alpha + \frac{1}{\delta - 1} \left( 2 (1 - \xi)^2 +  2 (1 - f)^2 + 2 \sigma^2 + 2 g^2 + (1 - f)(1 + f) + s^2 \right) \\
&\leq \frac{\delta}{\delta - 1} \cdot \frac{4}{\pi^2} \sin^4 \alpha + \frac{1}{\delta - 1} \left( 2 (1 - \xi)^2 +  2\sigma^2 + 4 (1 - f)+ s^2 \right) \\
&\leq \frac{\delta}{\delta - 1} \cdot \frac{4}{\pi^2} \alpha^4 + \frac{32}{3 (\delta - 1)} \alpha^3 + \frac{2}{\delta - 1} \big( (1 - \xi)^2 + \sigma^2 \big) + \frac{s^2}{\delta - 1} \\
&\leq \frac{1}{2} \sigma^2 + \frac{2}{\delta - 1} \big( (1 - \xi)^2 + \sigma^2 \big) + \frac{s^2}{\delta - 1},
\end{align*}
where the last step holds for $\delta \geq C$.

From equation~\eqref{eq:xi-ineq}, we also have
$(1 - F(\xi, \sigma))^2 \leq \frac{1}{400} \sigma^2$,
so that putting together the pieces yields
\begin{align*}
[\DeltaSE(\mathcal{S}_{gor}(\nu))]^2 \leq \frac{1}{2} \sigma^2 + \frac{2}{\delta - 1} \big( (1 - \xi)^2 + \sigma^2 \big) + \frac{s^2}{\delta - 1} + \frac{\sigma^2}{400} \leq C_{\delta}  [\DeltaSE(\nu)]^2 + \frac{s^2}{\delta - 1},
\end{align*}
as desired.

\paragraph{Proof of lower bound:} From equation~\eqref{eq:conv-rearrange} and Young's inequality, we have
\begin{align*}
[G(\xi, \sigma)]^2 &\geq \frac{\delta - 2}{\delta - 1} \cdot g^2 + \frac{1}{\delta - 1} \left( \frac{1}{2} (1 - \xi)^2 - (1 - f)^2 + \frac{1}{2} \sigma^2 - g^2 + (1 - f)(1 + f) + s^2 \right) \\
&\geq \frac{\delta - 3}{\delta - 1} \cdot g^2 + \frac{1}{\delta - 1} \left( \frac{1}{2} (1 - \xi)^2 + \frac{1}{2} \sigma^2 + 2f(1 - f) + s^2 \right) \\
&\geq \frac{1}{2 (\delta - 1)} [\DeltaSE(\nu)]^2 + \frac{s^2}{\delta - 1},
\end{align*}
where the final inequality follows since $\delta \geq C$. The proof follows by noting that
$\DeltaSE(\mathcal{S}_{gor}(\nu)) \geq G(\xi, \sigma)$.
\qed



\subsection{Step 2: Empirical error is sharply tracked by Gordon state evolution}

Recall the following concentration bound relating the iterate maps to their Gordon counterparts, \apcomment{This needs to appear as lemma in one of the previous sections.} where we use the convenient shorthand
\begin{align*}
\Deltaxi_n(\epsilon) := \left( \frac{C\log^{3} (C/ \epsilon)}{n} \right)^{1/2} \qquad \text{ and } \qquad \Deltasigma_n(\epsilon) := \left( \frac{C \log(C n/ \epsilon )}{n} \right)^{1/2}.
\end{align*}
We have
\begin{align*}
\Pr \left\{ |\Fhat (\xi, \sigma) - F (\xi, \sigma) | \geq \Deltaxi_n(\epsilon) \right\} \leq \epsilon \quad \text{ and } \quad
\Pr \left\{ |\Ghat (\xi, \sigma) - G (\xi, \sigma) | \geq \Deltasigma_n(\epsilon) \right\} \leq \epsilon.
\end{align*}
The following lemma parallels Lemma~\ref{lem:elbow-right}, and we use the shorthand $\Delta_{n, \epsilon, T} := \Deltaxi_n(\epsilon/T) \lor \Deltasigma_n(\epsilon/T)$ as before.
\begin{lemma} \label{lem:elbow-right-GD}
Suppose that $\delta \geq C$, and that $(\xi, \sigma) \in \GPR$. There are universal positive constants $(c_1,c_2)$ such that if $n$ is large enough to ensure that $\Delta_{n, \epsilon, T} \leq c_1$, then for each $T \geq 1$, we have
\begin{align*}
\sup_{1 \leq t \leq T} \; | \Fhat^t(\xi, \sigma) - F^t(\xi, \sigma)| \lor | \Ghat^t(\xi, \sigma) - G^t(\xi, \sigma)| \leq c_2 \cdot \Delta_{n, \epsilon, T}
\end{align*}
with probability exceeding $1 - 2 \epsilon$.
\end{lemma}

\subsubsection{Proof of Theorem~\ref{thm:GD-PR}(b)}
The proof is identical to the AM case (see Section~\ref{sec:thm1bproof}), with Lemma~\ref{lem:elbow-right-GD} playing the role of Lemma~\ref{lem:elbow-right}. We omit it for the sake of brevity.
\qed

\subsubsection{Proof of Lemma~\ref{lem:elbow-right-GD}}
The proof of this lemma is almost identical to that of Lemma~\ref{lem:elbow-right}, and so we only sketch the differences. The proofs only differ in which technical lemmas are applied. In particular, instead of applying Lemmas~\ref{AM-PR-good-region} and~\ref{lem:Gordon-pert} for the AM case, we now apply Lemmas~\ref{lem:GD-PR-good-region} and~\ref{lem:Gordon-pert-GD}, respectively. The structure and logic of the proofs are otherwise identical.
\qed

\subsection{Step 3: Convergence of empirics from random initialization to good region}

Once again, the proof for this step is very similar to the AM case, with the following two lemmas replacing Lemmas~\ref{lem:xi-jumps} and~\ref{lem:ratio-jumps}. Note that the lemmas themselves are near-identical, with the only difference manifesting as an additional condition on $\xi$.
% and we do so by splitting the analysis into two parts that focus directly on the empirics. First, in Lemma~\ref{lem:xi-jumps}, we show that $\xi_t$ increases exponentially from its initial value $d^{-1/2}$ up until $\xi/\sigma \geq 1/2$. Then, in Lemma~\ref{lem:ratio-jumps}, we show that provided the initial ratio $\xi_0/\sigma_0$ is larger than $1/2$, the ratio $\xi_t/ \sigma_t$ at time $t$ gets exponentially larger until it is greater than $5$.

\begin{lemma} \label{lem:xi-jumps-GD}
Suppose the pair $(\xi, \sigma)$ satisfies $\xi \leq 1.05$ and $\frac{\xi}{\sigma} \leq 1/2$. Also suppose that $\delta \geq C$ and $s^2 / \delta \leq c$.
%There are universal positive constants $(c, C)$ such that if $n \geq C \cdot \log^{3}( 1/ \epsilon) \cdot \xi^{-2}$, then  on an event occuring with probability at least $1 - \epsilon$, we have
Then
\begin{align*}
F(\xi, \sigma) \geq 1.06 \cdot \frac{\xi}{\sigma} \quad \text{ and } \quad G(\xi, \sigma) \leq 0.95.
\end{align*}
%\begin{align*}
%\Fhat(\xi, \sigma) \geq (1 + c) \xi \quad \text{ and } \quad \Ghat(\xi, \sigma) \leq 1.
%\end{align*}
%with probability greater than $1 - \epsilon$.
\end{lemma}

%The previous lemma ensures that provided we initialize at random, we will have $\xi_t/\sigma_t \geq 1/2$ after $t = \mathcal{O}(\log d)$ iterations. It remains to boost this result to obtain an iterate in the ``good'' region covered by the previous section. Using the next lemma, we show that this happens after a constant number of further iterations.

\begin{lemma} \label{lem:ratio-jumps-GD}
Suppose $\delta \geq C$ and $s^2 /\delta \leq c$. 
%There is a constant $C_{\epsilon}$ depending only on $\epsilon$ and a universal positive constant $c$ such that if $n \geq C_\epsilon$, 
Then for all $(\xi, \sigma)$ pairs satisfying $\xi \leq 1.05$ and $1/2 \leq \xi/\sigma \leq 5$, we have 
\begin{align*}
\frac{8}{7} \cdot \frac{\xi}{\sigma} \leq \frac{F(\xi, \sigma)}{G(\xi, \sigma)} \leq 50.
\end{align*}
%\begin{align*}
%\frac{\Fhat(\xi, \sigma)}{\Ghat(\xi, \sigma)} \geq (1 + c) \cdot \frac{\xi}{\sigma}
%\end{align*}
%with probability greater than $1 - \epsilon$.
\end{lemma}

\subsubsection{Proof of Theorem~\ref{thm:GD-PR}(c)}
The proof of Theorem~\ref{thm:GD-PR}(c) follows in an almost identical fashion to that of Theorem~\ref{thm:AM-PR}(c).
The only difference is that we must ensure the condition $\xi_t \leq 1.05$ at each step, but this is immediate on the event $\mathcal{E}_t$ defined in the proof of Theorem~\ref{thm:AM-PR}(c), since $F(\xi, \sigma) \leq 1$ for all $(\xi, \sigma)$ pairs.
Thus, Lemmas~\ref{lem:xi-jumps-GD} and~\ref{lem:ratio-jumps-GD} can be applied instead of Lemmas~\ref{lem:xi-jumps} and~\ref{lem:ratio-jumps}, respectively. We direct the reader to Section~\ref{sec:thm1cproof} for the argument.
\qed

\subsubsection{Proof of Lemma~\ref{lem:xi-jumps-GD}}
Since the $F$ map is identical to the AM case, the first inequality follows from Lemma~\ref{lem:xi-jumps}. For the second inequality, note from inequality~\eqref{eq:rec-Gbound-GD} that
\begin{align*}
[G(\xi, \sigma)]^2 \leq \frac{4}{\pi^2} \sin^4 \alpha + \frac{1}{\delta - 1} \left( 3.3 + s^2 \right) \leq 0.95,
\end{align*}
where the final inequality follows for $\delta \geq C$ and $s^2 / \delta \leq c$.
\qed

\subsubsection{Proof of Lemma~\ref{lem:ratio-jumps-GD}}

As before, we prove the upper and lower bounds separately.
Note that $\tan^{-1} (1/5) \leq \alpha \leq \tan^{-1} (2)$. %We prove the upper and lower bounds separately. 
\paragraph{Proof of lower bound:} 
%\apcomment{Copied from AM, modify.}
Write $H_{\delta} := \left( \frac{G(\xi, \sigma)}{F(\xi, \sigma)} \div \frac{\sigma}{\xi} \right)^2$, and note that the Gordon recursion~\eqref{eq:Gordon-GD-PR-restated} in conjuction with inequality~\eqref{eq:rec-Gbound-GD} yields
\begin{align*}
(\delta - 1) \cdot H_{\delta} \leq \frac{\cot^2 \alpha}{(\pi - 2 \alpha + \sin (2\alpha))^2} \cdot \Big\{ 4 (\delta- 1) \sin^4 \alpha 
 + 3.3 \pi^2 + \pi^2 s^2 \Big\}.
\end{align*}
We now split this proof into two cases.

\noindent \underline{Case $\alpha \in [\tan^{-1} (1/5), \pi/4]$:} In this case, we make use of the easily-verified bounds
\begin{align*}
\cot^2 \alpha &\leq \alpha^{-2}, \\
(\pi - 2\alpha + \sin(2\alpha))^2 &\geq (1 + \pi/2)^2, \qquad \text{ and } \\
\sin^4 \alpha &\leq \alpha^4.
\end{align*}
Substituting above yields
\begin{align*}
(\delta - 1) \cdot H_{\delta}(\alpha) \leq \frac{4(\delta - 1) \alpha^2 + 3.3 \pi^2 \alpha^{-2} + s^2 \alpha^{-2}}{(1 + \pi/2)^2} \leq \frac{\pi^2 (\delta - 1) }{(\pi + 2)^2}  + \frac{14 \pi^2}{\alpha^2 (\pi + 2)^2} + \frac{4s^2}{\alpha^2 (\pi + 2)^2} \leq 0.5 \cdot (\delta - 1).
\end{align*}
The last inequality follows by the assumptions $\delta \geq C$ and $s^2/ \delta \leq c$.

\noindent \underline{Case $\alpha \in [\pi/4, \tan^{-1}(2)]$:} Let $\beta = \pi/2 - \alpha$, and note that for all $\beta \in [\pi/5, \pi/4]$, we have
\begin{align*}
\tan^2 \beta &\leq \frac{16}{\pi^2} \cdot \beta^2 \\
(2 \beta + \sin(2 \beta))^2 &\geq 4 (1 + 2/\pi)^2 \beta^2, \text{ and } \\
\cos^4 \beta &\leq 1.
\end{align*}
Substituting above yields
\begin{align*}
(\delta - 1) \cdot H_{\delta}(\alpha) \leq \frac{4}{(\pi + 2)^2} \cdot (4 (\delta - 1) + 3.3 \pi^2 + s^2) \leq 0.7 \cdot(\delta - 1).
\end{align*}
Once again, the last inequality holds provided $\delta \geq C$ and $s^2 / \delta \leq c$.
\smallskip

\noindent Putting together the two cases, we have $\frac{F(\xi, \sigma)}{G(\xi, \sigma)} \geq \frac{1}{\sqrt{0.7}} \frac{\xi}{\sigma} \geq \frac{8}{7} \cdot \frac{\xi}{\sigma}$.

\paragraph{Proof of upper bound:} This follows directly from our previous calculations, since the bound~\eqref{eq:AM-ratio-bound} still applies in this case to yield $\frac{F(\xi, \sigma)}{G(\xi, \sigma)} \leq 50$.
\qed

\newpage

\section{Proof of Theorem~\ref{thm:AM-MLR}: Alternating minimization for mixtures of regressions}

Recall that the good region for phase retrieval is given by $\GMR$, the set of $\nu = (\xi, \sigma)$ satisfying $\sigma \leq 1.05$, $\xi \geq 0.55$, and $\xi/\sigma \geq 5$. Also recall our assumption that $\delta \geq C$ and $s \leq c$ for universal constants $(c, C)$. We begin by restating the Gordon state evolution for this case.
\begin{align} \label{eq:Gordon-AM-MLR-restated}
\begin{split}
\xigordon &= 1 - A(\rho) + B(\rho), \text{ and } \\
\sigmagordon &= \sqrt{\rho^2 B(\rho)^2 + \frac{1}{\delta - 1}\left(1 + \noisestd^2 - (1 - A(\rho) + B(\rho))^2 - \rho^2 B(\rho)^2\right)},
\end{split}
\end{align}
where 
\begin{align*}
A(\rho) := \frac{2}{\pi}\tan^{-1}\left(\sqrt{\rho^2 + \noisestd^2 + \noisestd^2 \rho^2}\right) \quad \text{ and } \quad
B(\rho) := \frac{2}{\pi} \frac{\sqrt{\rho^2 + \noisestd^2 + \noisestd^2\rho^2}}{1 + \rho^2}.
\end{align*}
The rest of the proof proceeds in three steps as usual. We let $F_s$ and $G_s$ denote the maps $\xigordon$ and $\sigmagordon$, respectively.

\subsection{Step 1: Convergence of Gordon state evolution in good region}
As in the phase retrieval case, we prove this using two lemmas.
\begin{lemma} \label{lem:AM-MLR-good-region}
Suppose $\delta \geq C$ and $s^2 / \delta \leq c$. If $\nu \in \GPR$, then $\mathcal{S}_{gor}(\nu) \in \GMR$.
\end{lemma}

\begin{lemma} \label{lem:AM-MLR-convergence}
Suppose $\delta \geq C$ and $s \leq c$. Then for each $\nu = (\xi, \sigma) \in \GMR$, we have
\begin{align*}
c_{\delta} \cdot [\DeltaSE(\nu)]^2 + \frac{s^2}{\delta - 1} \leq [\DeltaSE(\mathcal{S}_{gor}(\nu))]^2 \leq C_{\delta} \cdot [\DeltaSE(\nu)]^{2} + \frac{s^2}{\delta - 1}.
\end{align*}
Here $0 \leq c_{\delta} \leq C_{\delta} \leq 1$ are constants that depend solely on $\delta$.
\end{lemma}

\subsubsection{Proof of Theorem~\ref{thm:AM-MLR}(a)}
Taken together, Lemmas~\ref{lem:AM-MLR-good-region} and~\ref{lem:AM-MLR-convergence} clearly establish part (a) of the theorem, since they ensure the two conditions of Definition~\ref{def:linear} are satisfied. \qed
%\apcomment{Add more detail.} \qed
\medskip

We now prove each lemma in turn. 

\subsubsection{Proof of Lemma~\ref{lem:AM-MLR-good-region}}
We must show that if the pair $(\xi, \sigma)$ satisfies $\sigma \leq 1.05$, $\xi \geq 0.55$, and $\xi/\sigma \geq 5$, then the Gordon state evolution~\eqref{eq:Gordon-AM-MLR-restated} satisfies $G_s(\xi, \sigma) \leq 1.05$, $F_s(\xi, \sigma) \geq 0.55$, and $F_s(\xi, \sigma)/G_s(\xi, \sigma) \geq 5$. We show each of these bounds separately.

\paragraph{Bounding $G_s(\xi, \sigma)$:} We have
\begin{align}  \label{eq:rec-Gbound-AM-MLR}
[G(\xi, \sigma)]^2 &\leq \rho^2 \cdot B^2(\rho) 
 + \frac{1}{\delta - 1} ( 1 + s^2 ) 
\leq \frac{4}{\pi^2} \rho^4 (1 + s^2) + \frac{4}{\pi^2} \rho^2 s^2 + \frac{1}{\delta - 1}( 1 + s^2 ) \leq 1,
\end{align}
where the final inequality follows since $\rho \leq 1/5$, $\delta \geq C$, and $s \leq c$.


\paragraph{Bounding $F_s(\xi, \sigma)$:} Note that $F_s$ is increasing in $s$, and so 
\[
F_s(\xi, \sigma) \geq F_0(\xi, \sigma) = 1 - \frac{1}{\pi} (2 \alpha - \sin(2 \alpha)). 
\]
By computation, we have $F_0(\xi, \sigma) \geq 0.95$ for all $\xi/\sigma \geq 5$.


\paragraph{Bounding $\frac{F_s(\xi/\sigma)}{G_s(\xi, \sigma)}$:}  As before, our goal is to prove that $\frac{[G_s(\xi, \sigma)]^2}{[F_s(\xi, \sigma)]^2} \leq 1/5^2$. But we know from the previous two calculations that for large enough $\delta$ and small enough $s$, we have $[G_s(\xi, \sigma)]^2 \leq 0.01$ and $F_s(\xi, \sigma) \geq 0.9$. Thus, we have $\frac{[G_s(\xi, \sigma)]^2}{[F_s(\xi, \sigma)]^2} \leq 1/6^2$, as desired.
\qed

\subsubsection{Proof of Lemma~\ref{lem:AM-MLR-convergence}}
We first present some useful inequalities, and then the upper and lower bounds, separately. First, note that
\begin{align}
G_s(\xi, \sigma) &= \sqrt{\rho^2 B(\rho)^2 \cdot \frac{\delta - 2}{\delta - 1} + \frac{1}{\delta - 1}\left(1 + \noisestd^2 - [F_s(\xi, \sigma)]^2 \right) } \notag \\
&= \sqrt{\rho^2 B(\rho)^2 \cdot \frac{\delta - 2}{\delta - 1} + \frac{s^2}{\delta - 1} + \frac{(1  - F_s(\xi, \sigma))(1 + F_s(\xi, \sigma))}{\delta - 1}  } \label{G-split}
\end{align}
Notice that the map $\rho \mapsto  1 - A(\rho) + B(\rho)$ is non-increasing for $\rho \geq 0$ so that 
\begin{align}
\label{ub:F}
F_s(\xi, \sigma) = 1 - A(\rho) + B(\rho) \leq 1 + \frac{2s^3}{3\pi},
\end{align}
where in the last inequality we have made use of the bound $\tan^{-1}(x) \geq x - \frac{x^3}{3}$. We also have
\begin{align} \label{Fbd-s0}
1 - F_s(\xi, \sigma) \leq 1 - F_0(\xi, \sigma) = \frac{2\alpha - \sin(2\alpha)}{\pi} \leq \frac{4}{3\pi} \rho^3,
\end{align}
where $\alpha = \tan^{-1} \rho$. Putting together inequalities~\eqref{G-split}-\eqref{Fbd-s0} and noting that $s \leq 0.5$ by assumption, we obtain the sandwich relation
\begin{align} \label{eq:sandwich-G-AM-MLR}
\frac{\rho}{2} \cdot B(\rho) \sqrt{\frac{\delta - 2}{\delta - 1}} + \frac{1}{4} \cdot \frac{s}{\sqrt{\delta - 1}} \leq G_s(\xi, \sigma) \leq \sqrt{\rho^2 B(\rho)^2 + \frac{s^2}{\delta - 1} + \frac{8 \rho^3}{3 \pi(\delta - 1)} \cdot \left( 1 + \frac{s^3}{3\pi} \right) }.
\end{align}

%

\paragraph{Proof of upper bound:} Using the upper bound in equation~\eqref{eq:sandwich-G-AM-MLR} in conjunction with the assumption $s \leq 0.5$ and the fact that $\rho \leq 1/5$ in $\GMR$, we obtain
\begin{align*}
G_s(\xi, \sigma) &\leq \rho B(\rho) + \frac{s}{\sqrt{\delta - 1}} + \frac{\rho}{\sqrt{\delta - 1}}
\end{align*}
where we have also used the inequality $\sqrt{a + b + c} \leq \sqrt{a} + \sqrt{b} + \sqrt{c}$, valid for any three non-negative scalars $(a, b, c)$. Putting this together with the definition of $F_s$ and the fact that $F_s \geq 0.95$ for all $\rho \leq 1/5$, we have
\begin{align*}
\frac{G_s}{F_s} \leq \rho \left( 1 - \frac{1 - A(\rho)}{1 + B(\rho) - A(\rho)} + \frac{1.1}{\sqrt{\delta - 1}}\right) + \frac{1.1s}{\sqrt{\delta - 1}} \leq \rho \left( 1 - \frac{1 - A(\rho)}{1 + B(\rho)} + \frac{1.1}{\sqrt{\delta - 1}}\right) + \frac{1.1s}{\sqrt{\delta - 1}}.
\end{align*}
Now note that if $s \leq 0.5$ and $\rho \leq 1/5$, then $A(\rho) \leq 0.6$ and $B(\rho) \leq \pi^{-1}$. Substituting above, we obtain
\begin{align*}
\frac{G_s}{F_s} &\leq \rho \left( 0.7 + \frac{1.1}{\sqrt{\delta - 1}}\right) + \frac{1.1s}{\sqrt{\delta - 1}} \leq \frac{4}{5} \cdot \frac{\sigma}{\xi} + \frac{1.1s}{\sqrt{\delta - 1}},
\end{align*}
where the final inequality uses the fact that $\delta \geq C$. Now note that if $a \leq 1$ then for all $x \leq 1$, we have $\tan^{-1} (ax + b) \leq a \tan^{-1} x + b$. Taking $\tan^{-1}$ on both sides of the above display completes the proof, since $\DeltaSEangle(\nu) = \tan^{-1} (\sigma/\xi)$ for an element $\nu = (\xi, \sigma)$ of the state-evolution.  %\apcomment{Come back and prove this carefully.}

\paragraph{Proof of lower bound:} Using the upper bound in equation~\eqref{eq:sandwich-G-AM-MLR} in conjunction with the assumption $\delta \geq C$ and equation~\eqref{ub:F}, we obtain
\begin{align*}
\frac{G_s(\xi, \sigma)}{F_s(\xi, \sigma)} &\geq \frac{\rho B(\rho)}{4} + \frac{s}{5\sqrt{\delta - 1}} \geq c s\rho + \frac{s}{5\sqrt{\delta - 1}}.
\end{align*}
In the first inequality, we have used the assumption $s \leq 0.5$, and the second inequality follows by noting that $B(\rho) \geq 4cs$ for all $\rho$ for some absolute constant $c > 0$. \apcomment{Finish by taking $\arctan$.}
\qed


\subsection{Step 2: Empirical error is sharply tracked by Gordon state evolution}

Recall the following concentration bound relating the iterate maps to their Gordon counterparts, \apcomment{This needs to appear as lemma in one of the previous sections.} where we use the convenient shorthand
\begin{align*}
\Deltaxi_n(\epsilon) := \left( \frac{C\log^{3} (C/ \epsilon)}{n} \right)^{1/2} \qquad \text{ and } \qquad \Deltasigma_n(\epsilon) := \left( \frac{C \log(C n/ \epsilon )}{n} \right)^{1/4}.
\end{align*}
We have
\begin{align*}
\Pr \left\{ |\Fhat (\xi, \sigma) - F (\xi, \sigma) | \geq \Deltaxi_n(\epsilon) \right\} \leq \epsilon \quad \text{ and } \quad
\Pr \left\{ |\Ghat (\xi, \sigma) - G (\xi, \sigma) | \geq \Deltasigma_n(\epsilon) \right\} \leq \epsilon.
\end{align*}
The following lemma parallels Lemma~\ref{lem:elbow-right}, and we use the shorthand $\Delta_{n, \epsilon, T} := \Deltaxi_n(\epsilon/T) \lor \Deltasigma_n(\epsilon/T)$ as before.
\begin{lemma} \label{lem:elbow-right-AM-MLR}
Suppose that $\delta \geq C$, and that $(\xi, \sigma) \in \GMR$. There are universal positive constants $(c_1,c_2)$ such that if $n$ is large enough to ensure that $\Delta_{n, \epsilon, T} \leq c_1$, then for each $T \geq 1$, we have
\begin{align*}
\sup_{1 \leq t \leq T} \; | \Fhat^t(\xi, \sigma) - F^t(\xi, \sigma)| \lor | \Ghat^t(\xi, \sigma) - G^t(\xi, \sigma)| \leq c_2 \cdot \Delta_{n, \epsilon, T}
\end{align*}
with probability exceeding $1 - 2 \epsilon$.
\end{lemma}

\subsubsection{Proof of Theorem~\ref{thm:AM-MLR}(b)}
The proof is identical to the AM case (see Section~\ref{sec:thm1bproof}), with Lemma~\ref{lem:elbow-right-GD} playing the role of Lemma~\ref{lem:elbow-right}.
\qed

\subsubsection{Proof of Lemma~\ref{lem:elbow-right-AM-MLR}}
The proof of this lemma is almost identical to that of Lemma~\ref{lem:elbow-right}, and only differ in which technical lemmas are applied. In particular, instead of applying Lemmas~\ref{AM-PR-good-region} and~\ref{lem:Gordon-pert} for the AM case, we now apply Lemmas~\ref{lem:AM-MLR-good-region} and~\ref{lem:Gordon-pert-AM-MLR}, respectively. The structure and logic of the proofs are otherwise identical.
\qed


\subsection{Step 3: Convergence of empirics from random initialization to good region}

Once again, the proof for this step is very similar to that of step 3 in the proof of Theorem~\ref{thm:AM-PR}, with the following two lemmas replacing Lemmas~\ref{lem:xi-jumps} and~\ref{lem:ratio-jumps}. Note that the lemmas themselves are near-identical, with the only difference manifesting in the scalar values.
% and we do so by splitting the analysis into two parts that focus directly on the empirics. First, in Lemma~\ref{lem:xi-jumps}, we show that $\xi_t$ increases exponentially from its initial value $d^{-1/2}$ up until $\xi/\sigma \geq 1/2$. Then, in Lemma~\ref{lem:ratio-jumps}, we show that provided the initial ratio $\xi_0/\sigma_0$ is larger than $1/2$, the ratio $\xi_t/ \sigma_t$ at time $t$ gets exponentially larger until it is greater than $5$.

\begin{lemma} \label{lem:xi-jumps-AM-MLR}
Suppose the pair $(\xi, \sigma)$ satisfies $\frac{\xi}{\sigma} \leq 1/2$. Also suppose that $\delta \geq C$ and $s \leq c$.
%There are universal positive constants $(c, C)$ such that if $n \geq C \cdot \log^{3}( 1/ \epsilon) \cdot \xi^{-2}$, then  on an event occuring with probability at least $1 - \epsilon$, we have
Then
\begin{align*}
F_s(\xi, \sigma) \geq 1.06 \cdot \frac{\xi}{\sigma} \quad \text{ and } \quad G_s(\xi, \sigma) \leq 0.95.
\end{align*}
%\begin{align*}
%\Fhat(\xi, \sigma) \geq (1 + c) \xi \quad \text{ and } \quad \Ghat(\xi, \sigma) \leq 1.
%\end{align*}
%with probability greater than $1 - \epsilon$.
\end{lemma}

%The previous lemma ensures that provided we initialize at random, we will have $\xi_t/\sigma_t \geq 1/2$ after $t = \mathcal{O}(\log d)$ iterations. It remains to boost this result to obtain an iterate in the ``good'' region covered by the previous section. Using the next lemma, we show that this happens after a constant number of further iterations.

\begin{lemma} \label{lem:ratio-jumps-AM-MLR}
Suppose $\delta \geq C$ and $s \leq c$. 
%There is a constant $C_{\epsilon}$ depending only on $\epsilon$ and a universal positive constant $c$ such that if $n \geq C_\epsilon$, 
Then for all $(\xi, \sigma)$ pairs satisfying $\sigma \leq 1$ and $1/4 \leq \xi/\sigma \leq 5$, we have 
\begin{align*}
\frac{8}{7} \cdot \frac{\xi}{\sigma} \leq \frac{F_s(\xi, \sigma)}{G_s(\xi, \sigma)} \leq 50.
\end{align*}
%\begin{align*}
%\frac{\Fhat(\xi, \sigma)}{\Ghat(\xi, \sigma)} \geq (1 + c) \cdot \frac{\xi}{\sigma}
%\end{align*}
%with probability greater than $1 - \epsilon$.
\end{lemma}

\subsubsection{Proof of Theorem~\ref{thm:AM-MLR}(c)}
The proof of Theorem~\ref{thm:AM-MLR}(c) follows in an almost identical fashion to that of Theorem~\ref{thm:AM-PR}(c), by adjusting constants.
%The only difference is that we must ensure the condition $\xi_t \leq 1.05$ at each step, but this is immediate on the event $\mathcal{E}_t$ defined in the proof of Theorem~\ref{thm:AM-PR}(c), since $F(\xi, \sigma) \leq 1$ for all $(\xi, \sigma)$ pairs.
%Thus, Lemmas~\ref{lem:xi-jumps-GD} and~\ref{lem:ratio-jumps-GD} can be applied instead of Lemmas~\ref{lem:xi-jumps} and~\ref{lem:ratio-jumps}, respectively. 
We direct the reader to Section~\ref{sec:thm1cproof} for the argument.
\qed

\subsubsection{Proof of Lemma~\ref{lem:xi-jumps-AM-MLR}}
Since $F_s(\xi, \sigma) \geq F_0(\xi, \sigma)$ for all $(\xi, \sigma)$ pairs, the first claim follows from Lemma~\ref{lem:xi-jumps}. For the second claim, note from inequality~\eqref{eq:sandwich-G-AM-MLR} that if $s \leq 0.5$, then
\begin{align*}
G_s(\xi, \sigma) \leq \rho B(\rho) + \frac{s}{\sqrt{\delta - 1}} + \frac{1.1}{\sqrt{\delta - 1}}.
\end{align*}
Now note that $\rho B(\rho) \leq \frac{2}{\pi} \sqrt{1 + s^2}$ and so if $\delta \geq C$ and $s \leq c$ for a sufficiently large constant $C$ and a sufficiently small constant $c$, we have $G_s(\xi, \sigma) \leq 0.95$.
\qed

\subsubsection{Proof of Lemma~\ref{lem:ratio-jumps-AM-MLR}}

As before, we prove the upper and lower bounds separately.
Note that $\tan^{-1} (1/5) \leq \alpha \leq \tan^{-1} (2)$. %We prove the upper and lower bounds separately. 
\paragraph{Proof of lower bound:} 
%\apcomment{Copied from AM, modify.}
Write $H_{\delta} := \left( \frac{G_s(\xi, \sigma)}{F_s(\xi, \sigma)} \div \frac{\sigma}{\xi} \right)^2$, and note that since $F_s \geq F_0$, we have
\begin{align*}
(\delta - 1) \cdot H_{\delta} \leq \frac{\cot^2 \alpha}{(\pi - 2 \alpha + \sin (2\alpha))^2} \cdot \Big\{ (\delta - 1) \cdot \rho^2 B(\rho)^2 + s^2 + 1.1 \Big\}.
\end{align*}
We now split this proof into two cases.

\noindent \underline{Case $\alpha \in [\tan^{-1} (1/5), \pi/4]$:} In this case, we make use of the easily-verified bounds
\begin{align*}
\cot^2 \alpha = \rho^{-2}, \quad  (\pi - 2\alpha + \sin(2\alpha))^2 \geq (1 + \pi/2)^2, \quad \text{ and }
\rho^2 B(\rho)^2 \leq \frac{\rho^2}{\pi^2},
\end{align*}
where the last bound holds since $s \leq 0.5$. Consequently,
\begin{align*}
(\delta - 1) \cdot H_{\delta}(\alpha) \leq \frac{(\delta - 1) \pi^{-2} + 1.1 \rho^{-2} + s^2 \rho^{-2}}{(1 + \pi/2)^2} \leq \frac{(\delta - 1) }{2(\pi + 2)^2}  + \frac{5}{\rho^2 (\pi + 2)^2} + \frac{4s^2}{\rho^2 (\pi + 2)^2} \leq 0.5 \cdot (\delta - 1).
\end{align*}
The last inequality follows by the assumptions $\delta \geq C$ and $s^2/ \delta \leq c$.

\noindent \underline{Case $\alpha \in [\pi/4, \tan^{-1}(2)]$:} Let $\beta = \pi/2 - \alpha$, and note that for all $\beta \in [\pi/5, \pi/4]$, we have
\begin{align*}
\tan^2 \beta \leq \frac{16}{\pi^2} \cdot \beta^2, \quad
(2 \beta + \sin(2 \beta))^2 \geq 4 (1 + 2/\pi)^2 \beta^2, \quad \text{ and } \quad
\rho^2 B(\rho)^2 \leq 1.
\end{align*}
Substituting above yields
\begin{align*}
(\delta - 1) \cdot H_{\delta}(\alpha) \leq \frac{4}{(\pi + 2)^2} \cdot ((\delta - 1) + 1.1 + s^2) \leq 0.7 \cdot(\delta - 1).
\end{align*}
Once again, the last inequality holds provided $\delta \geq C$ and $s^2 / \delta \leq c$.
\smallskip

\noindent Putting together the two cases, we have $\frac{F_s(\xi, \sigma)}{G_s(\xi, \sigma)} \geq \frac{1}{\sqrt{0.7}} \frac{\xi}{\sigma} \geq \frac{8}{7} \cdot \frac{\xi}{\sigma}$.

\paragraph{Proof of upper bound:} Combining the bounds~\eqref{ub:F} and the lower bound from equation~\eqref{eq:sandwich-G-AM-MLR}, we see that provided $s \leq 0.5$, we have
\begin{align*}
\frac{F_s(\xi, \sigma)}{G_s(\xi, \sigma)} \leq \frac{\left( 1 + \frac{2s^3}{\pi} \right)}{\sqrt{\frac{\delta - 2}{\delta - 1}} \rho B(\rho)} \leq \frac{1.1}{\rho B(\rho)} \leq \frac{1.1\pi (1 + \rho^2)}{2\rho^2},
\end{align*}
where in the first inequality, we have used the bounds $\delta \geq C$ and $s \leq c$, and in the final inequality, we have used the bound $B(\rho) \geq \frac{2}{\pi} \rho / (1 + \rho^2)$. Evaluating the RHS at $\rho = 1/5$ yields the desired result.
\qed

\newpage


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Proof of Theorem~\ref{thm:GD-MLR}: Subgradient descent for mixtures of regressions}

\subsection{Step 1: Convergence of the Gordon update in the good region}

\subsection{Step 2: Empirics lie in envelope around Gordon trajectory}

\subsection{Step 3: Parallel component $\xihat$ is boosted from random initialization}

\subsection{Step 4: Ratio $\xihat/\sigmahat$ is boosted until in good region}

==> sections/gordon/gd_optimal_conc_rate.tex <==
% ==================================================== %
Consider the gradient updates
\begin{align}
\thetanext &= \thetacur - \eta\cdot\frac{2}{n}\sum_{i=1}^n \omega\big(\inp{\x_i}{\thetacur},y_i\big)\cdot \bx_i.\label{eq:direct_gd}
\end{align}
For convenience, define (and with some abuse of notation) define $$\omegab_t=\omega(\X\thetacur,\y) = \omega\big(\X\thetacur,f(\X\theta^\star;\zb)+\epsb\big) \in\R^n.$$
In the previous section, we computed the statistics $\xi^{t+1},\alpha^{t+1}$ and $\beta^{t+1}$ of \eqref{eq:direct_gd} by first expressing the gradient update as the solution to a convex minimization problem and then using the CGMT machinery. Here, we compute the statistics directly from \eqref{eq:direct_gd}. \ct{Here, we will need to argue why this is not possible for quadratic methods.}

\vp
\noindent\textbf{Computation of $\beta^{t+1}$.}~
Recall that 
$$
\beta^{t+1} = \|P_{S^t}^{\perp}\thetanext\|_2 = \frac{2\eta}{n}\|P_{S^t}^{\perp}\X^T\omegab_t\|_2.
$$
In the second equality we used \eqref{eq:direct_gd} and $\thetacur\in S^t.$ Note  that $\omegab_t$ depends on $\X$ only via $\X\thetacur$ and $\X\thetastar$. But $\X\thetacur$ is independent of $\X P_{S^t}^\perp$. Thus, without loss of generality $\beta^{t+1}$ is distributed as $\frac{2\eta}{n}\|P_{S^t}^{\perp}\tilde\X^T\omegab_t\|_2$ for a standard Gaussian matrix $\tilde\X\in\R^{n\times p}$ independent of everything else. Further using rotational invariance of the Gaussian measure, this is in turn distributed as $\frac{2\eta}{n}\|P_{S^t}^{\perp}\h\|_2\|\omegab_t\|_2$ for a Gaussian vector $\h\sim\Nn(0,I_d)$ independent of everything else. 
%We studied concentration of exactly this term in \eqref{eq:AB}. 
To continue, recall the familiar notation
$$\gammab_1:=\X\frac{\thetastar}{\|\thetastar\|_2}\quad\text{and}\quad\gammab_2:=\X \frac{P_{\thetastar}^\perp\thetacur}{\|P_{\thetastar}^\perp\thetacur\|_2}$$
where recall that $\gammab_1\sim\Nn(0,\mathbf{I}_n),\gammab_2\sim\Nn(0,\mathbf{I}_n)$ and are independent of each other. Putting things together we have shown that
$$
\beta^{t+1}~\sim~\frac{2\eta}{n}\|P_{S^t}^{\perp}\h\|_2\big\|\omega\big(\xi_t\gammab_1+\sigma_t\gammab_2;f(R\gammab_1;\zb)+\eps)\big\|_2
$$


\vp
\noindent\textbf{Computation of $\alpha^{t+1}$.}~
Recall that 
$$
\alpha^{t+1} = \frac{1}{\sigma_t}\inp{\thetanext}{P_{\thetastar}^{\perp}\theta^{t}} = \frac{1}{\sigma_t}\left(\sigma_t^2 - \frac{2\eta}{n}\omegab_t^T\X P_{\thetastar}^{\perp}\theta^{t}\right),
$$
where we used that $\sigma_t^2 = \|P_{\thetastar}^{\perp}\theta^{t}\|_2^2 = \inp{\thetacur}{P_{\thetastar}^{\perp}\theta^{t}}$. We focus on the term $\omegab_t^T\X P_{\thetastar}^{\perp}\theta^{t}$ and we decompose
$$
\X =\frac{1}{R^2} \X \thetastar(\thetastar)^T + \X P_{\thetastar}^{\perp}.
$$
Thus, we write
\begin{align}
\omegab_t^T\X P_{\thetastar}^{\perp}\theta^{t} = \sigma_t\cdot\Big(\omega\big(\xi_t\X\frac{\thetastar}{R}+\sigma_t\X \frac{P_{\thetastar}^\perp\thetacur}{\|P_{\thetastar}^\perp\thetacur\|_2};f(R\X\frac{\thetastar}{R};\zb)+\epsb\big)\Big)^T\X \frac{P_{\thetastar}^{\perp}\theta^{t}}{\|P_{\thetastar}^\perp\thetacur\|_2}
\end{align}
Putting things together, we have shown that
$$
\alpha^{t+1} ~\sim~ \sigma_t - \frac{2\eta}{n}\gammab_2^T\omega\big(\xi_t\gammab_1+\sigma_t\gammab_2;f(R\gammab_1;\zb)+\eps).
$$
Thus, we recover the last equation in \eqref{eq:soln_n}.

\vp
\noindent\textbf{Computation of $\xi^{t+1}$.}~
Recall that
\begin{align}
\xi^{t+1} &= \frac{\inp{\thetanext}{\thetastar}}{\|\thetastar\|_2}=\xi_t - \frac{2\eta}{n}\omegab_t^T\X\frac{\thetastar}{R} \nn
\\
 &= \xi_t - \frac{2\eta}{n}\omega\big(\xi_t\X\frac{\thetastar}{R}+\sigma_t\X \frac{P_{\thetastar}^\perp\thetacur}{\|P_{\thetastar}^\perp\thetacur\|_2};f(R\X\frac{\thetastar}{R};\zb)+\epsb\big)^T\X\frac{\thetastar}{R}\nn
 \\
 &= \xi_t - \frac{2\eta}{n}\gammab_1^T\omega\big(\xi_t\gammab_1+\sigma_t\gammab_2;f(R\gammab_1;\zb)+\eps).
  \nn
\end{align}

\vp
\noindent\textbf{Concentration.}~
Compare the formulas derived above for the three statistics to the formulas we derived in Section \ref{sec:gd_ao}, i.e. \eqref{eq:soln_n}. It can be easily checked that the two sets of formulas have identical concentration properties.  Therefore, we can apply Lemma \ref{lem:conc_lemma} to conclude concentration of the three terms at a rate $n^{-1/2}.$


==> sections/gordon/gordon-alt/alt-gordon-proofs.tex <==
%!TEX root = ../../../convergence-gordon.tex

% ==================================================== %
%\subsection{Proofs of Lemmas}\label{sec:lem_proofs}
\subsection{Useful technical lemmas}
\begin{lemma}\label{lem:phi_tilde_aux}
	Let $A,B>0$ and vectors $\ab,\tb\in\R^n$. Assume that
	%\begin{align}\label{eq:u_opt_lem_cond}
	$
	\|A\left(\nicefrac{\ab}{\|\ab\|_2}\right)+\tb\|_2\leq B.
	$
	%\end{align}
	Then, the optimal cost of the quadratic program
	%\begin{align}\label{eq:u_opt_lem}
	$\Big\{\min_{\|\ub\|_2\leq B} \inp{\ab}{\ub}\quad\text{sub. to}~~\|\tb-\ub\|_2\leq A \Big\}$ is equal to  $-A\,\|\ab\|_2+\inp{\ab}{\tb}.$
	%\end{align}
\end{lemma}
\begin{proof}
	TBD
\end{proof}

\subsubsection{Proof of Lemma \ref{lem:minmax}}\label{sec:minmax_proof}
In the proof below $c,C,C_i$ are absolute positive constants whose values can change from line to line.

First, we prove that with probability $1-Ce^{-cn}$ and $C_1\geq 2 C_{\theta}$:
\begin{align}\label{eq:eqv1}
\min_{\theta\in\bar\Dc} \Lc_t(\theta) = \min_{\theta\in\bar\Dc\cap\Bc_2(C_1)} \Lc_t(\theta).
\end{align}
Start with the case $\bar\Dc=\R^d$, then the desired follows directly by Assumption \ref{ass:theta_bd}. Next, consider $\bar\Dc=\Sc_\eps^c$. For the sake of contradiction suppose that in the high probability event of Assumption \ref{ass:theta_bd} the following is true:
\begin{align}\label{eq:contra1}
\Lc_t(\theta_\eps) = \min_{\theta\in\bar\Sc_\eps^c} \Lc_t(\theta) < \min_{\theta\in\bar\Dc\cap\Sc_\eps^c} \Lc_t(\theta) = \Lc_t(\theta_c),
\end{align}
where the existence of $\theta_c$ is because of the extreme value theorem and of $\theta_\eps$ by {coercivity} of $\Lc$ as per Assumption \ref{ass:loss}. If this were true, then $\theta_\eps\not\in\Bc_2(C_1)$. Consider the unconstrained minimizer $\thetanext$. Since $\thetanext\in\Bc_2(C_1)$  there exists $\rho\in(0,1)$ such that $\theta_\rho=\rho\thetanext+(1-\rho)\theta_\eps\in\Bc_2(C_1)\cap\Sc_\eps^c$. But from  convexity of $\Lc_t$, optimality of $\theta_c$, contradiction assumption \eqref{eq:contra1} and $\rho>0$:
$$
\rho\Lc_t(\thetanext)+(1-\rho)\Lc_t(\theta_\eps) \geq \Lc_t(\theta_\rho) \geq \Lc_t(\theta_c) > \Lc_t(\theta_\eps) \implies \Lc_t(\thetanext)>\Lc_t(\theta_\eps),
$$
contradicting optimality of $\thetanext$. This proves \eqref{eq:eqv1}.

	
%\begin{align}\label{eq:eqv1}
%\min_{\theta\in\R^n} \Lc_t(\theta) = \min_{\|\theta\|\leq C_1} \Lc_t(\theta).
%\end{align}

Second, we prove that with the desired high probability:
\begin{align}\label{eq:eqv2}
\min_{\theta\in\bar\Dc\cap\Bc_2(C_1)} \Lc_t(\theta) = \min_{ \substack{\theta\in\bar\Dc\cap\Bc_2(C_1) \\ \|\ub\|_2\leq C_2\sqrt{n} } } \; \Fc_t(\ub,\theta) ~~\text{sub. to}\quad \ub=\X\theta.
\end{align}
For this, recall that $\Lc_t(\theta) = h(\theta, \thetacur) + \frac{1}{n} \sum_{i = 1}^n g(\langle \bx_i, \theta \rangle, \langle \bx_i, \thetacur \rangle; y_i) = \Fc_t(\langle \bx_i, \theta \rangle,\theta)$. To see why the ball constraint on the `dummy' variable $\ub\in\R^n$, note for any feasible $\theta\in\bar\Dc\cap\Bc_2(C_1) $ that with probability at least $1-Ce^{cn}$ (e.g. \cite[Cor.~7.3.3]{VerBook}):
\begin{align}
\|\X\theta\|_2\leq \|\X\|_2\|\theta\|_2 
\leq 2 \, C_1 \, \left(\sqrt{n}+\sqrt{d}\right)
= 4\, C_1 \sqrt{n} =: C_2\,\sqrt{n}.
\end{align}
%\ct{Fix the remaining of the proof to adjust for $\bar\Dc,\Dc$}
%Using this, \eqref{eq:eqv1} and recalling that $\Lc_t(\theta) = h(\theta, \thetacur) + \frac{1}{n} \sum_{i = 1}^n g(\langle \bx_i, \theta \rangle, \langle \bx_i, \thetacur \rangle; y_i)$, we can write
%\begin{align}\label{eq:eqv2}
%\min_{\theta\in\R^n} \Lc_t(\theta) = \min_{ \substack{\|\theta\|_2\leq C_1 \\ \|\ub\|_2\leq C_2\sqrt{n} } } \; \Fc_t(\ub,\theta) ~~\text{sub. to}\quad \ub=\X\theta.
%\end{align}

%\begin{lemma}
%Consider convex functions $f:\R^n\times\R^d\rightarrow\R$ and $g:\R^n\times\R^d\rightarrow\R^m$. Further assume that the function $f$ is L-Lipschitz. Then, the following is true:
%\begin{align}\label{eq:lemma_minmax_state}
%\Big\{\min_{\theta,\ub} f(\ub,\theta)\quad\text{sub. to}\quad g(\ub,\theta)\leq 0, ~i\in[m] \Big\}~=~\min_\x\max_{\vb_i} f(\x) + \sum_{i\in[m]}\inp{\vb_i}{g_i(\x)}
%\end{align}
%\end{lemma}
%\begin{proof}
%For convenience, let $L,R$ denote the LHS and RHS of \eqref{eq:lemma_minmax_state}, respectively.
%Clearly,
%\begin{align*}
%L~=~\min_\x\max_{\vb_i} f(\x) + \sum_{i\in[m]}\inp{\vb_i}{g_i(\x)}
%\geq R.
%\end{align*}
%Thus, it suffices to show that $R\leq L$.
%\end{proof}

To finish the proof, we will use Assumption \ref{ass:Lip} to prove that when \eqref{eq:eqv1} and \eqref{eq:eqv2} hold it is true that
\begin{align}\label{eq:eqv3}
\min_{\theta\in\bar\Dc} \Lc_t(\theta)
 = \,\, \min_{ \substack{\theta\in\bar\Dc\cap\Bc_2(C_1) \\ \|\ub\|_2\leq C_2\sqrt{n} } } \; \max_{\|\vb\|_2\leq  C_3 } \; \;\Fc_t(\ub,\theta) - \frac{1}{\sqrt{n}}\langle \vb, \ub - \X\theta\rangle\,,
\end{align}
with $C_3=C_3(R):=2C_L(R)$ where $C_L(R)/\sqrt{n}$ is the Lipschitzness constant in Assumption \ref{ass:Lip}. 

The first observations is that that
\begin{align*}
\text{LHS of  }\eqref{eq:eqv3} \stackrel{\eqref{eq:eqv1}}{=} \min_{\theta\in\bar\Dc\cap\Bc_2(C_1)} \Lc_t(\theta) &\stackrel{\eqref{eq:eqv2}}{=}  \min_{ \substack{\theta\in\bar\Dc\cap\Bc_2(C_1) \\ \|\ub\|_2\leq C_2\sqrt{n} } } \; \Fc_t(\ub,\theta) ~~\text{sub. to}\quad \ub=\X\theta\\
\\
&= \min_{ \substack{\theta\in\bar\Dc\cap\Bc_2(C_1) \\ \|\ub\|_2\leq C_2\sqrt{n} } } \; \max_{\vb } \; \;\Fc_t(\ub,\theta) - \frac{1}{\sqrt{n}}\langle \vb, \ub - \X\theta\rangle ~\geq~
\text{RHS of  }\eqref{eq:eqv3}
\end{align*}
Hence, it suffices to prove the reverse side of the inequality. The desired claim follows by the following chain of inequalities
\begin{align*}
&\text{RHS of  }\eqref{eq:eqv3} \stackrel{(\text{Ass. \ref{ass:Lip}})}{\geq}\min_{ \substack{\theta\in\bar\Dc\cap\Bc_2(C_1)  \\ \|\ub\|_2\leq C_2\sqrt{n} } } \; \max_{\|\vb\|_2\leq C_3 } \; \; \Fc_t(\X\theta,\theta) - \frac{C_L(R)}{\sqrt{n}}\|\ub-\X\theta\|_2 - \frac{1}{\sqrt{n}}\langle \vb, \ub - \X\theta\rangle\nn\\
&\qquad= \min_{ \substack{\theta\in\bar\Dc\cap\Bc_2(C_1)  \\ \|\ub\|_2\leq C_2\sqrt{n} } } \; \max_{0\leq \rho_\vb\leq C_3} \; \Lc_t(\theta) - \frac{C_L(R)}{\sqrt{n}}\|\ub-\X\theta\|_2 -  \frac{1}{\sqrt{n}}\min_{\|\vb\|_2=\rho_\vb} \; \; \langle \vb, \ub - \X\theta\rangle\nn\\
&\qquad= \min_{ \substack{\theta\in\bar\Dc\cap\Bc_2(C_1)  \\ \|\ub\|_2\leq C_2\sqrt{n} } } \; \max_{0\leq \rho_\vb\leq C_3} \;\Lc_t(\theta) + \big(\rho_\vb - C_L(R)\big)\frac{\|\ub-\X\theta\|_2 }{\sqrt{n}}\\
&\quad\stackrel{(C_3>C_L(R))}{\geq} \min_{\substack{\theta\in\bar\Dc\cap\Bc_2(C_1)  \\ \|\ub\|_2\leq C_2\sqrt{n} }} \Lc_t(\theta) = \min_{\theta\in\bar\Dc\cap\Bc_2(C_1) } \Lc_t(\theta)\\
&\qquad\stackrel{\eqref{eq:eqv1}}{=} \text{LHS of  }\eqref{eq:eqv3}
\end{align*}
%But clearly by evaluating the objective of the RHS of \eqref{eq:eqv3} at the feasible point $\theta=\thetanext,\ub=\X\thetanext$ it also holds that 
%$$
%\text{RHS of  }\eqref{eq:eqv3} \leq \min_{\theta\in\R^n} \Lc_t(\theta).
%$$
Combining the above two displays proves \eqref{eq:eqv3} completing the proof of the first statement of the lemma.

Next, we prove \eqref{eq:pro_bd}. We have the following chain of inequalities
 \begin{align}
 \Pro\left\{\thetanext\not\in\Sc_\eps \right\} &= \Pro\left\{ \min_{\theta\in\Sc_\eps^c} \Lc_t(\theta) \leq \min_{\theta\in\R^d} \Lc_t(\theta) \right\} \nn
\\
&\leq \Pro\left\{ \min_{\theta\in\Sc_\eps^c} \Lc_t(\theta) \leq \min_{\theta\in\R^d} \Lc_t(\theta) \,\big|\, 
 \Phi_{n,\Bc_2(C_1)} = \min_{\theta\in\R^d} \Lc_t(\theta),  \Phi_{n,\Bc_2(C_1)\cap\Sc_\eps^c} = \min_{\theta\in\Sc_\eps^c} \Lc_t(\theta) 
  \right\}  +  Ce^{-cn}.\nn\\
&=  \Pro\left\{  \Phi_{n,\Bc_2(C_1)\cap\Sc_\eps^c} \leq \Phi_{n,\Bc_2(C_1)}  \right\} \nn\\
  &= \Pro\left\{\hat\thetanext\not\in\Sc_\eps \right\} +  Ce^{-cn}.
\end{align}
This completes the proof of the lemma.

%\subsubsection{Proof of }
\subsubsection{Proof of \eqref{eq:conAO2}}
\label{sec:proof_unbd_v}

For convenience, let $A$ and $B$ denote the optimal costs of the constrained minimization in the RHS of \eqref{eq:conAO2} and of the min-max optimization in the RHS of \eqref{eq:sec_ao}. Clearly,
$$
A = \min_{ \substack{ (\xi,\alpha,\beta)\in\Dc_3 \\ \|\ub\|_2\leq C_2\sqrt{n} } }  \; \sup_{\rho_\vb\geq 0 }\Fc_t(\ub,\theta)+ \frac{\rho_\vb}{\sqrt{n}}\left(\Big\| \beta \g+ \X P_{S^t}\theta - \ub  \Big\|_2- \beta \|P^{\perp}_{S^t}\h\|_2\right).
$$
Thus, $A\geq B$. Now, we will show the other side of the inequality. 

For this let $\Oc\in\Dc_3\times \Bc_2(C_2\sqrt{n})$ denote the set of minimal values of the optimization in the RHS of \eqref{eq:sec_ao}. We assume that \emph{all} $(\xi,\alpha,\beta,\ub)\in\Oc$ are such that the constraint 
\begin{align}
f(\xi,\alpha,\beta,\ub) :=\Big\| \beta \g+ \X P_{S^t}\theta - \ub  \Big\|_2- \beta \|P^{\perp}_{S^t}\h\|_2 \leq 0\label{eq:f_con}
\end{align}
is \emph{not} satisfied, since otherwise it holds easily that $B\geq A$, as desired. 
Let then
$$
m_{\Oc} = \min_{(\xi,\alpha,\beta,\ub)\in\Oc}f(\xi,\alpha,\beta,\ub)>0,
$$
where the minimum is attained by the extreme value theorem.
%So, considering $(\xi,\alpha,\beta,\ub)\in\Oc$ such that $f(\xi,\alpha,\beta,\ub)>0$, we 

Now, fix arbitrary $(\xi,\alpha,\beta)\in\Dc_3$ and consider the set of $\ub\in\Bc(C_2\sqrt{n})$ that satisfy the constraint in \eqref{eq:f_con}. With probability at least $1-Ce^{-cn}$, this set is non-empty. To see this, note that with the same probability $\|\beta\g+ \X P_{S^t}\theta\|\leq C_2\sqrt{n}$ for large constant $C_2$.  Thus, for any $\ub\in\Bc(C_2\sqrt{n})$ let $\bar\ub(\xi,\alpha,\beta)$ denote the projection of $\ub$ on the (non-empty) constraint set in \eqref{eq:f_con}.

With this notation, it holds for any $(\xi,\alpha,\beta,\ub)\in\Oc$ that
\begin{align}
B &\stackrel{}{=} \Fc_t(\ub,\theta) + \max_{0\leq\rho_\vb\leq C_3}\frac{\rho_\vb}{\sqrt{n}} f(\xi,\alpha,\beta,\ub) \nn
\\
&\stackrel{(i)}{\geq} \Fc_t(\ub,\theta) + \frac{C_3}{\sqrt{n}} m_{\Oc} \nn
\\
&\stackrel{(ii)}{\geq} \Fc_t(\bar\ub(\xi,\alpha,\beta),\theta) - \frac{C_L}{\sqrt{n}}\|\bar\ub(\xi,\alpha,\beta)-\ub\|_2 + \frac{C_3}{\sqrt{n}} m_{\Oc} \nn
\\
&\stackrel{(iii)}{\geq} \Fc_t(\bar\ub(\xi,\alpha,\beta),\theta) - 2C_LC_2 + \frac{C_3}{\sqrt{n}} m_{\Oc}
\\
&\stackrel{(iv)}{\geq} A - 2C_LC_2 + \frac{C_3}{\sqrt{n}} m_{\Oc}
\end{align}
Specifically,  we used (i) the assumption that $f(\xi,\alpha,\beta,\ub)\geq m_\Oc>0$; (ii) Lipschitness of $\Fc_t$ as per Assumption \ref{ass:Lip}; (iii) the fact that $\ub,\bar\ub(\xi,\alpha,\beta)\in\Bc_2(C_2\sqrt{n})$; (iv) feasibility of $(\bar\ub(\xi,\alpha,\beta),\theta)$  in \eqref{eq:conAO2}, i.e. $f(\bar\ub(\xi,\alpha,\beta),\theta)\leq 0$.

Thus, we can always pick $C_3\geq 2C_LC_2\sqrt{n}/m_\Oc$ such that $B\geq A$ as desired.


\subsubsection{Proof of Lemma \ref{lem:phi_tilde_aux}}
\label{sec:phi_tilde_proof}\ct{To fix}

Recall from \eqref{eq:2min_u} that
\begin{align}
\phi_{n,\Dc} &= \min_{ \substack{(\xi,\alpha,\beta)\in\Dc_3 \\ \|\ub\|_2\leq C_2\sqrt{n} } }  \; \; \frac{1}{2}(\xi^2+\alpha^2+\beta^2) - \big(\xi\xi_t+\alpha\sigma_t\big) - \frac{2\eta}{n}\inp{\omegab_t}{\ub}\quad\text{sub. to}~\Big\|\beta\g+\xi\gammab_1+\alpha\gammab_2-\ub\Big\|_2\leq \beta\| P^{\perp}_{S^t}\h \|_2\end{align}
We will need the following auxiliary result to perform the constrained optimization of the linear form in $\ub$.
%\begin{lemma}\label{lem:phi_tilde_aux}
%Let $A,B>0$ and vectors $\ab,\tb\in\R^n$. Assume that
%\begin{align}\label{eq:u_opt_lem_cond}
%\|A\frac{\ab}{\|\ab\|_2}+\tb\|_2\leq B.
%\end{align}
% Then, it hold that
%\begin{align}\label{eq:u_opt_lem}
%\Big\{\min_{\|\ub\|_2\leq B}-\inp{\ab}{\ub}\quad\text{sub. to}~~\|\tb-\ub\|_2\leq A \Big\}= -A\,\|\ab\|_2-\inp{\ab}{\tb}.
%\end{align}
%\end{lemma}

Before proving Lemma \ref{lem:phi_tilde_aux}, we show how to conclude Lemma \ref{lem:phi_tilde} from it.  We see that the inner minimization over $\ub$ above is of the same form as the minimization in the LHS of \eqref{eq:u_opt_lem} with:
$$
\ab\leftarrow \frac{2\eta}{n}\omegab_t,\quad \tb\leftarrow\beta\g+\xi\gammab_1+\alpha\gammab_2,\quad A\leftarrow \beta\| P^{\perp}_{S^t}\h \|_2, \quad B\leftarrow C_2\sqrt{n}.
$$

%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Boundedness of omega %%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%From Assumption \ref{ass:omega}, for some absolute constant $\tilde C$:
%%%%%$
%%%%%\|\frac{\omegab(\xi,\sigma)}{\sqrt{\E\Omega^2}} - \sqrt{n}\|_{\psi_2} \leq \tilde{C}K_\omega^2
%%%%%$
%%%%%Hence,
%%%%%$$
%%%%%\Pro\left( \big\|\omegab(\xi,\sigma)\big\|_2 \geq 2\sqrt{\E\Omega^2}\sqrt{n} \right)\leq 2\exp(-cn/K_\omega^4).
%%%%%$$
%%%%%Also, 

Now, we will show that \eqref{eq:u_opt_lem_cond} holds for large enough constant $C_2$. 
First, from concentration of the norm of Gaussian isotropic vectors it holds that:
$$
\Pro\left( \max\left\{\|\g\|_2,\|\gammab_1\|_2,\|\gammab_2\|_2\right\} \geq 2\sqrt{n} \right)\leq C\exp(-cn).
$$
Hence, $\|\tb\|_2\leq 2\sqrt{n} $ with probability at least $1- C\exp(-cn)$. 
Second, the multivariate Gaussian $\x=P_{S_t}^\perp\h$ behaves as a $d-2$-dimensional isotropic Gaussian. Hence, from same arguments and using  $d-2<d\leq n$
$$
\Pro\left( \|P_{S_t}^\perp\h\|_2\geq 2\sqrt{n} \right) \leq C\exp(-cn).
$$
Putting these together, combining with the triangle inequality and using boundedness of $\xi,\alpha,\beta$ (cf. $\Dc_3\subset\Bc_2(C_1)$) we conclude that \eqref{eq:u_opt_lem_cond} holds with probability at least $1- C\exp(-cn)$ for sufficiently large constant $C_2$. 

Then, the desired follows directly from \eqref{eq:u_opt_lem}.

\begin{proof}[Proof of Lemma \ref{lem:phi_tilde_aux}]
We start by lower bounding the LHS of \eqref{eq:u_opt_lem} as follows:
\begin{align*}
\Big\{\min_{\|\ub\|_2\leq B}\,\,-\inp{\ab}{\ub}\quad\text{sub. to}~~\|\tb-\ub\|_2\leq A \Big\}&= \min_{{\|\ub\|_2\leq B}} \max_{\la\geq0}\,\, -\inp{\ab}{\ub}+\frac{\la}{2}\|\tb-\ub\|_2^2-\frac{\la}{2}A^2 \\
&\stackrel{(i)}{=}  \max_{\la\geq0} \min_{{\|\ub\|_2\leq B}}\,\, -\inp{\ab}{\ub}+\frac{\la}{2}\|\tb-\ub\|_2^2-\frac{\la}{2}A^2 \\
&\stackrel{(ii)}{\geq}  \max_{\la\geq0}\,\, \min_{\ub\in\R^n} -\inp{\ab}{\ub}+\frac{\la}{2}\|\tb-\ub\|_2^2-\frac{\la}{2}A^2 \\
&\stackrel{}{=}  \max_{\la\geq0}\,\, -\frac{1}{2\la}\|\ab\|_2^2 - \ab^T\tb -\frac{\la}{2}A^2\\
&\stackrel{}{=}  -A\,\|\ab\|_2- \ab^T\tb.
\end{align*}
Above, (i) holds because the minimization over $\ub$ is on a compact set and the objective is clearly convex in $\ub$ and concave in $\la$; (ii) is because the minimization set over $\ub$ is enlarged. 

Next, consider $\ub_\star=\frac{A}{\|\ab\|_2}\ab+\tb$. Clearly, $\ub_\star$ is feasible in the constrained minimization in \eqref{eq:u_opt_lem}. Thus, the LHS in \eqref{eq:u_opt_lem} is upper bounded by 
$$
-\inp{\ab}{\ub_\star} = A\|\ab\|_2-\ab^T\tb.
$$
Combining the above completes the proof of the lemma.
\end{proof}


\subsection{Probabilities of events in Equation  \eqref{eq:good_events_quad}}

\begin{lemma} Recall the definitions of $\A\in\R^{n\times 3}, \omegab_t\in\R^n, \vb_n\in\R^3$ in Section XXX. Further let Assumption \ref{ass:omega} hold. For large enough $n$, $\delta>c_\delta$ and any $\eta>0$ smaller than some constant, there exist constants $C,c,C'>0$ such that each one of the events $\Ec_i, i\in[4]$ in \eqref{eq:good_events_quad} holds with probability at least $1-Ce^{-cn\eta^2}$.
\end{lemma}
\begin{proof}
We will prove the following refined version of \eqref{eq:good_events_quad}.
\begin{subequations}
\begin{align}
\Ec_1&:=\left\{ \frac{1}{1+6n^{-1/2}+3\eta}\,\mathbf{I}_3 \preceq n(\A^T\A)^{-1} \preceq 
\frac{1}{1-6n^{-1/2}-3\eta}\,\mathbf{I}_3
\right\}
\\
\Ec_2&:=\left\{ \frac{1}{\delta}(1-\eta)-\frac{2}{n}\leq\|\vb_n\|_2^2\leq \frac{1}{\delta}(1+\eta)
\right\}\\
\Ec_3&:=\left\{ \left| \frac{\|\omegab_t\|_2^2}{n} - \E\Omega_t^2 \right|\leq \eta
\right\}
\\
\Ec_4&:=\left\{ \left| \frac{1}{n}\gammab_1^T\omegab_t - \E[G_1\Omega_t] \right| \vee 
\left| \frac{1}{n}\gammab_2^T\omegab_t - \E[G_2\Omega_t] \right| \vee
\left| \frac{1}{n}\g_1^T\omegab_t  \right|
\leq C'\eta\right\}
\\
\Ec_5&:=\left\{ \left| \frac{\|\A^T\omegab_t\|^2}{n^2} - \left(\E[G_1\Omega_t]\right)^2 - \left(\E[G_2\Omega_t]\right)^2 \right|\leq 3\eta^2 + 2\eta\left(\E[G_1\Omega_t]+\E[G_2\Omega_t]\right)\right\}
\end{align}
\end{subequations}
All these events hold with high-probability. Specifically,
\begin{subequations}
\begin{align}
\Pro(\Ec_1)\wedge\Pro(\Ec_2)&\geq 1 - Ce^{-c n \eta^2}
\\
\Pro(\Ec_3)&\geq 1 - 2e^{-cn\left(\frac{\eta^2}{K_\omega^4}\wedge\frac{\eta}{K_\omega^2}\right)}
\\
\Pro(\Ec_4)\wedge\Pro(\Ec_5)&\geq 1 - 2e^{-cn\frac{\eta^2}{K_\omega^2}}
\end{align}
\end{subequations}
\ct{From Assumption \ref{ass:omega}, $K_\omega<C$ and $\E[\Omega^2]<C$.}

Using $\E[G_1\Omega_t]\vee\E[G_2\Omega_t]\leq\sqrt{\E[\Omega_t^2]}$ and $\eta\in(0,1)$ on the event $\Ec$, we have that
\begin{align*}
\left| \frac{\|\A^T\omegab_t\|^2}{n^2} - \left(\E[G_1\Omega_t]\right)^2 - \left(\E[G_2\Omega_t]\right)^2 \right|&\leq \left(3 + 4\sqrt{\E[\Omega_t^2]}\right)\eta
%\\&\leq \left(3 + 4\sqrt{K_\omega}\right)\eta\leq C\left(1\vee \sqrt{K_\omega}\right)\eta\leq 
\leq C\eta,
\end{align*}
where we used Cauchy-Schwartz in the first inequality and $\E[\Omega_t^2]<C$ in the second inequality, respectively.


\end{proof}



\subsubsection{Proof of Lemma \ref{lem:conc_lemma}}
By Assumption \ref{ass:omega}, Gaussianity of $\gammab_1,\gammab_2$ and \cite{Ver}[Lemma 2.7.7] we have that the entries of $\inp{\gammab_1}{\omegab_t}$ and $\inp{\gammab_2}{\omegab_t}$ are independent sub-exponential random variables with sub-exponential constant at most $C K_\omega$ each and means $\E[G_1\cdot \Omega_t]$ and $\E[G_2\cdot \Omega_t]$, respectively. Thus, from Bernstein's inequality,
\begin{align}\label{eq:Bern_inp1}
\Pro\left\{ \max\left\{ \left| \xi_{\star,n} - \xi_{\star,t+1} \right|\,\,\left| \alpha_{\star,n} - \alpha_{\star,t+1} \right| \right\} \geq \eps \right\} \leq 4\exp\left(-c\,n\,\min\left(\eps^2/K_\omega^2,\eps/K_\omega\right)\right)\,.
\end{align}


For convenience, let us denote 
\begin{align*}
&A = \frac{1}{\sqrt{n}}\|P^{\perp}_{S^t}\h \|_2\quad\text{and}\quad \bar{A}=\sqrt{\frac{d-2}{n}}\\
&B = \frac{1}{\sqrt{n}}\|\omegab_t\|_2\quad\text{and}\quad \bar{B}=\sqrt{\E[\Omega^2]}.
\end{align*}

From subgaussianity of the entries of $\omegab_t$ (by Assumption \ref{ass:omega}) and the fact that $P^\perp_{S^t}\h$ is distributed as a $(d-2)$--dimensional isotropic Gaussian,  it holds  that  (e.g. \cite[Thm. 3.1.1]{Vershynin})
%$$
%\left\|  \frac{\|P^{\perp}_{S^t}\h \|_2}{\sqrt{n}} -  \sqrt{\frac{d-2}{n}} \right\|_{\psi_2}\leq \frac{C}{\sqrt{n}} \quad\text{and}\quad \left\|\frac{\|\omegab\|_2}{\sqrt{n}}-\sqrt{\E[\Omega^2]}\right\|_{\psi_2}  \leq \frac{CK_\omega}{\sqrt{n}}.
%$$ 
%\begin{align}
%\Pro\left\{ \Big|\frac{\|P^{\perp}_{S^t}\h \|_2^2}{{n}} -  \frac{d-2}{n}\Big| \geq\eps \right\}&\leq 2\exp\left(-c\,n\,\,\min(\eps^2,\eps)\right) \\
%\Pro\left\{ \Big|\frac{\|\omegab_t \|_2^2}{{n}} -  \E[\Omega^2]\Big| \geq\eps \right\}&\leq 2\exp\left(-c\,n\,\,\min(\eps^2/K_\omega^4,\eps/K_\omega^2)\right)\,.
%\end{align}
%\begin{align*}
%\Pro\left\{ \max\left\{ \left|  \frac{\|P^{\perp}_{S^t}\h \|_2}{\sqrt{n}} -  \frac{1}{\sqrt{\delta}} \right|\,,\, \left|\frac{\|\omegab\|_2}{\sqrt{n}}-\sqrt{\E[\Omega^2]}\right| \right\} \geq \eps \right\} \leq 4\exp\left(-c\eps^2n\right)
%\end{align*}
\begin{align*}
\Pro\left\{ \Big|A^2 -  \bar{A}^2\Big| \geq\eps \right\}&\leq 2\exp\left(-c\,n\,\,\min(\eps^2,\eps)\right) \\
\Pro\left\{ \Big|B^2-  \bar{B}^2\Big| \geq\eps \right\}&\leq 2\exp\left(-c\,n\,\,\min(\eps^2/K_\omega^4,\eps/K_\omega^2)\right)\,.
\end{align*}
Thus, (e.g. see \cite[Thm.~3.1.1]{Ver}), 
\begin{align}
\Pro\left\{ \big|{A} - \bar{A}\big| \geq \eps \right\} &\leq 2\exp\left(-c\,n\,\eps^2\right)\\
\Pro\left\{ \big|\frac{B}{\bar{B}} - 1\big| \geq \eps \right\} &\leq 2\exp\left(-c\,n\,\eps^2\bar{B}^4/K_\omega^4\right) \implies\Pro\left\{ \big|B- \bar{B}\big| \geq \eps\bar{B} \right\} \leq 2\exp\left(-c\,n\,\eps^2\bar{B}^4/K_\omega^4\right).
\end{align}

Now, conditioned on the event $\{|A-\bar A|\leq\eps,|B-\bar B|\}\leq \eps\bar B\}$ occurring with probability at least $1-4\exp\big(-c\,n\,\eps^2\min\{1,\bar{B}^4/K_\omega^4\}\big)$, it holds that
$$
|AB-\bar A\bar B|\leq C\bar{B}\max\{\eps^2,\eps\}.
$$
Above, we also used the facts that $\bar{A}\leq 1$ since $n>d$ and $\bar{B}\leq\sqrt{2}K_\omega$ by subgaussianity of the entries of $\omegab_t$ (e.g.  \cite[Prop.~2.5.2]{Ver}). 
Hence,
\begin{align}
\Pro\left\{|AB-\bar A\bar B|\geq \eps\right\}
&\leq C\exp\left(-c\,n\,\frac{\min\left(1,\bar{B}^4/K_\omega^4\right)}{\min(K_\omega,K_\omega^2)}\,\min\left(\eps,{\eps^2}\right)\right).\label{eq:AB}
\end{align}
For convenience, denote $C_\omega:=\frac{\min\left(1,\bar{B}^4/K_\omega^4\right)}{\min(K_\omega,K_\omega^2)}.$
%where the second inequality follows because: (i) $\bar A\leq 1$  since $n\geq d>d-2$; (ii) by sub-gaussianity of the entries of $\omegab_t$ it holds that $\bar B\leq \sqrt{2} K_\omega$ by \cite[Prop.~2.5.2]{Ver}.  

Finally, note that each entry of $\frac{1}{n}\inp{\g}{\omegab_t}$ is zero-mean subexponential with sub-exponential constant at most $CK_\omega/n$. Thus, by Bernestein's inequality
$$
\Pro(|\frac{1}{n}\inp{\g}{\omegab_t}|\geq \eps) \leq 2\exp\left(-c\,n\,\min\left(\eps^2/K_\omega^2,\eps/K_\omega\right)\right)
%\leq2\exp\left(-c\,n\,\frac{1}{1+K_\omega^2}\,\min\left(\eps^2,\eps\right)\right).
$$
Combining this with \eqref{eq:AB}, and further using the fact
\begin{align}
\bar{B}\big(\frac{1}{\sqrt{\delta}}-\frac{2\sqrt{\delta}}{n} \big) - \leq \bar{A}\bar{B} \leq \bar{B}\frac{1}{\sqrt{\delta}} \implies 
\bar{B}\frac{1}{\sqrt{\delta}}-\frac{C(\delta) K_\omega}{n} - \leq \bar{A}\bar{B} \leq \bar{B}\frac{1}{\sqrt{\delta}},
\end{align}
 we conclude with the desired:
%Now, note that
%$$
%2(AB-\bar A\bar B) = (A+B)^2 - (\bar A+\bar B)^2 - (A^2-\bar A ^2) - (B^2-\bar B ^2)
%$$
%Hence, $\beta_{\star,n}$ is subexponential with $\|\beta_{\star,n}\|_{\psi_1}\leq C/n$ and Bernstein's inequality gives \ct{Add some detail}
\begin{align}\label{eq:Bern_inp2}
\Pro\left\{ \abs{\beta_{\star,n}-\beta_{\star,t+1}} \geq \eps + \frac{\eta K_\omega \tilde C(\delta)} {n}\right\} \leq C\exp\left(-c\,C_\omega\,n\,\min\left(\eps,{\eps^2}\right)\right).
\end{align}

Now we will show that the unconstrained solution \eqref{eq:soln_n} of \eqref{eq:con_final_AO} is feasible (thus, optimal) when $\Dc:=\Bc_2(C_1)$. Here, recall that $C_1$ is a constant that can be made arbitrarily large without changing any of the results thus far. Specifically, it suffices from from \eqref{eq:Bern_inp1} and \eqref{eq:Bern_inp2} that
$$
C_1 > 2\sqrt{(\alpha_{\star,t+1}+\eps)^2+(\beta_{\star,t+1}+\eps)^2+(\xi_{\star,t+1}+\eps)^2}.
$$
(For example, $C_1^2=4(\alpha_{\star,t+1}^2+\beta_{\star,t+1}^2+\xi_{\star,t+1}^2)+12\eps^2+\frac{\eta^2K_\omega^2C^2}{n^2}$ suffices.) This guarantees that with the same probability as the RHS of \eqref{eq:Bern_inp2} 
%
% Hence, from \eqref{eq:Bern_inp1} and \eqref{eq:Bern_inp2}, letting $C_1 = 8 \max\{\alpha_{\star,t+1},\beta_{\star,t+1},\xi_{\star,t+1}\} > 2\sqrt{(\alpha_{\star,t+1}+\eps)^2+(\beta_{\star,t+1}+\eps)^2+(\xi_{\star,t+1}+\eps)^2}$ \ct{Need $\eps\leq \max\{\alpha_{\star,t+1},\beta_{\star,t+1},\xi_{\star,t+1}\}$} it holds with probability at least $1-C\exp\left(-c\,\min\left(n\eps^2,n\eps\right)\right)$ that 
 $\|\theta_n\|_2^2=\xi_{\star,n}^2+\alpha_{\star,n}^2+\beta_{\star,n}^2< C_1$, i.e. $(\xi_{\star,n},\alpha_{\star,n},\beta_{\star,n})$ is feasible in \eqref{eq:con_final_AO}. Hence, 
for large enough $C_1$, with the same probability:
\begin{align}
\wt\phi_{n,\Bc_2(C_1)} = -\frac{1}{2}\left(\alpha_{\star,n}^2+\beta_{\star,n}^2+\xi_{\star,n}^2\right).
\end{align}

When combined with \eqref{eq:Bern_inp1} and \eqref{eq:Bern_inp2}, these lead to the following for constants $C_4:=C_4(\delta,\eta,\alpha_{\star,t+1},\beta_{\star,t+1},\xi_{\star,t+1})$ and $C_5:=C_5(\delta,\eta,K_\omega,\beta_{\star,t+1})$:
\begin{align}\nn
\Pro\left\{\Big|\wt\phi_{n,\Bc_2(C_1)} - \bar\phi \Big| \geq {C_4} \max\{\eps,\eps^2\}+\frac{C_5}{n}\right\} \leq  C\exp\left(-c\,C_\omega\,n\,\min\left(\eps^2,\eps\right)\right),
%\max\left\{ \alpha_{\star,t+1}\, ,\,\beta_{\star,t+1}\, ,\,\xi_{\star,t+1}  \right\}\cdot 
\end{align}
with
\begin{align}\nn
\bar\phi:=-\frac{1}{2}\left(\alpha_{\star,t+1}^2+\beta_{\star,t+1}^2+\xi_{\star,t+1}^2\right)
\end{align}



==> sections/gordon/gordon-alt/gordon-alt.tex <==
%!TEX root = ../../../convergence-gordon.tex

This section is dedicated to a more general proposition that immediately implies Theorem~\ref{thm:one_step_main}(a), as well as weaker version of part (b). In the next section, we present the sharper analysis that leads to part (b) of the theorem. In this section, we let $\bt^{\sharp}$ denote the ``current'' iterate of the algorithm, with $(\parcomp^{\sharp}, \perpcomp^{\sharp}) = (\parcomp(\bt), \perpcomp(\bt))$. This frees up the tuple $(\bt, \parcomp, \perpcomp)$ to denote decision variables that will be used throughout the proof.
%
%
In order to state our general proposition, we require an expanded notion of the Gordon state evolution update, in which it is convenient to track a three-dimensional state evolution (cf. Definition~\ref{def:starnext_main}).


\begin{definition}[Expanded Gordon state evolution update]\label{def:expanded-gordon}
Recall the model~\eqref{eq:model}, and let $Q$ denote a random variable drawn from the latent variable distribution $\mathbb{Q}$. Let $(Z_1, Z_2, Z_3)$ denote a triplet of independent standard Gaussian random variables and let $\alpha^{\sharp} \in \mathbb{R}$ and $\beta^{\sharp} \in \mathbb{R}_{\geq 0}$ denote arbitrary scalars.  Let
\[
\Omega = \omega\big(\parcomp^{\sharp} Z_1 +\perpcomp^{\sharp} Z_2\,,\,f(Z_1; Q)+\noisestd Z_3 \big).
\]
\begin{itemize}
	\item[(a)] (Higher-order updates.)  If the loss function $\Lc$ is as in equation~\eqref{eq:sec_order_gen}, then define the scalars
\[
\alpha^{\gor} = \EE [ Z_1 \Omega], \qquad \mu^{\gor} = \EE[Z_2 \Omega], \qquad \text{ and } \qquad \nu^{\gor} = \sqrt{\frac{\EE[\Omega^2] - (\EE[Z_1 \Omega])^2 - (\EE[Z_2 \Omega])^2}{\kappa - 1}}.
\]
\item[(b)] (First-order updates.) If the loss function $\Lc$ is as in equation~\eqref{eq:GD_gen}, then define the scalars
\[
\alpha^{\gor} = \alpha^{\sharp} + 2\eta \cdot \EE[Z_1 \Omega], \qquad \perpone^{\gor} = \perpcomp^{\sharp} + 2\eta \cdot \EE[Z_2 \Omega], \qquad \text{ and } \qquad \perptwo^{\gor} = \frac{2 \eta}{\kappa} \cdot \sqrt{\EE[\Omega^2]}.
\]
\end{itemize}
\end{definition}
\iffalse
\kaccomment{Check this.  I think the denominator here is $1/\kappa$, not $1/(\kappa - 1)$.}
Note that from the above definition, one can easily recover the state evolution in Definition~\ref{def:starnext_main} from the relation
\[
\beta^{\gor} = \sqrt{(\mu^{\gor})^2 + (\nu^{\gor})^2}.
\]
\fi
With this expanded state evolution in hand, we state the following proposition.
\begin{proposition}
	\label{prop:gordon}
	There exists a universal triple of positive constants $(C_1, C_2, C_3)$ such that the following holds.  Let $\btsharp \in \mathbb{R}^d$ denote an arbitrary vector satisfying $\btsharp \in \mathbb{B}_2(C_1)$, let
	\[
	\parcomp^{\sharp} = \langle \btstar, \btsharp \rangle \qquad \text{ and } \qquad \perpcomp^{\sharp} = \| \proj_{\btstar}^{\perp} \btsharp \|_2,
	\]
	and define the subspace $S_{\sharp} = \mathsf{span}(\btstar, \btsharp)$.  Further, consider the general model~\eqref{eq:model} for the data and either type of update~\eqref{eq:sec_order_gen} or~\eqref{eq:GD_gen} and suppose that the the weight function $\omega$ satisfies Assumption~\ref{ass:omega}.  Consider the triple of scalars $(\parcomp^{\gor}, \perpone^{\gor}, \perptwo^{\gor})$ from Definition~\ref{def:expanded-gordon}.  If % both $n \geq C_2$ and 
	$\kappa \geq C_2$, then
	\[
	\Pro\biggl\{\max\Bigl(\lvert \langle \bt, \btstar \rangle - \alpha^{\gor} \rvert, \Bigl\lvert \frac{\langle \bt, \proj_{\btstar}^{\perp}\bt^{\sharp}\rangle}{\| \proj_{\btstar}^{\perp} \bt^{\sharp}\|_2} - \mu^{\gor} \Bigr\rvert, \lvert \| \proj_{S_{\sharp}}^{\perp} \bt \|_2 - \nu^{\gor} \rvert \Bigr) \geq C_3\Bigl(\frac{\log(1/\epsilon)}{n}\Bigr)^{1/4}\biggr\} \leq \epsilon.
	\]
\end{proposition}
In words, Proposition~\ref{prop:gordon} guarantees that the triple $(\parcompgordon, \perpone^{\gor}, \perptwo^{\gor})$ provides a reliable deterministic prediction---that is, up to fluctuations of $\ordertil(n^{-1/4})$ with high probability---of the triple
\begin{align*}
\langle \bt, \btstar \rangle, \qquad \frac{\langle \bt, \proj_{\btstar}^{\perp}\bt^{\sharp}\rangle}{\| \proj_{\btstar}^{\perp} \bt^{\sharp}\|_2}, \quad \text{ and } \quad \| \proj_{S_{\sharp}}^{\perp} \bt \|_2,
\end{align*}
respectively. Let us now prove Theorem~\ref{thm:one_step_main}(a) from this proposition.

\begin{proof}[Proof of Theorem~\ref{thm:one_step_main}(a)]
\apcomment{Insert.}
\end{proof}
\noindent It remains to prove Proposition~\ref{prop:gordon}. 

\begin{proof}[Proof of Proposition~\ref{prop:gordon}]
We present the proof according to the steps that were sketched in the recipe (see Section~\ref{subsec:heuristic-higher-order}), but with rigorous justifications for all the steps. We then put these pieces together to obtain Proposition~\ref{prop:gordon}.

\paragraph{Implementing step 1:} We implement this step under a general decomposability assumption on the loss function $\mathcal{L}$ as in equation~\eqref{eq:gordon_one_step}, which allows us to analyze first and second order methods under the same umbrella.
\begin{assumption}[Decomposability and convexity of Loss]\label{ass:loss}
	Consider a fixed vector $\bt^{\sharp} \in \mathbb{R}^d$ and a fixed matrix $\bX \in \mathbb{R}^{n \times d}$ and assume $\by$ is generated, given $\bX$ and $\btstar$, according to the generative model~\eqref{eq:model}.  Suppose each step of the iterative algorithm can be written in the form~\eqref{eq:opt_gen_intro}. The loss
	\[
	\Lc(\bt):={\mathcal{L}(\bt; \bt^{\sharp}, \bd{X}, \bd{y})}
	\]
	satisfies the following properties:
	\begin{enumerate}[label=(\alph*)]
		\item There is a pair of functions $g: \mathbb{R}^n \times \mathbb{R}^n \rightarrow \mathbb{R}$ and $h: \mathbb{R}^d \times \mathbb{R}^d \rightarrow \mathbb{R}$, and a (random) function
		\begin{align}
			\label{eq:Fc}
			F : \mathbb{R}^{n} \times \mathbb{R}^{d} &\rightarrow \mathbb{R} \nonumber\\
			F(\bu, \bt) &\mapsto g(\bu, \bX \bt^{\sharp}; \by) + h(\bt, \bt^{\sharp}),
		\end{align}	
		such that the loss function satisfies the equation
		\[
		\Lc(\bt) = F(\bX \bt, \bt).
		\]
		
		\item The functions $g$ and $h$ are convex in their first arguments.  Moreover, the function $F$ is $C_L/\sqrt{n}$-Lipschitz in its first argument.
		
		\item The function $h$ depends on $\bt$ only through its lower dimensional projections.  That is, there exists a function
		\begin{align*}
			\hscal: \mathbb{R}^3 \times \mathbb{R}^d &\rightarrow \mathbb{R}\\
			(\alpha, \mu, \nu), \bt^{\sharp} & \mapsto \hscal((\alpha, \mu, \nu), \bt^{\sharp}),
		\end{align*}
		such that 
		\[
		h(\bt, \bt') = \hscal\biggl(\langle \bt, \btstar\rangle, \frac{\langle \bt, \proj_{\btstar}^{\perp} \bt'\rangle}{\| \proj_{\btstar}^{\perp} \bt'\|_2}, \| \proj_{\mathsf{span}(\btstar, \bt')}^{\perp} \bt \|_2, \bt'
		\biggr)
		\]
		
		\item $\Lc(\bt)$ is coercive.  That is, $\Lc(\bt) \rightarrow \infty$ whenever $ \| \bt \|_2 \rightarrow \infty$.
	\end{enumerate}
\end{assumption}
Note that these assumptions encapsulate a set of loss functions more general than those we are interested in.  For instance, specifying
\begin{align*}
h(\bt, \bt^{\sharp}) = 0 \qquad  \text{ and } \qquad g(\bu, \bX \bt^{\sharp}; \by) = \frac{1}{\sqrt{n}}\| \omega(\bX \bt^{\sharp}, \by) - \bX \bt \|_2
\end{align*} 
recovers the higher-order loss functions~\eqref{eq:sec_order_gen}, whereas specifying 
\begin{align*}
h(\bt, \btsharp) = 1/2 \| \bt \|_2^2 - \langle \bt, \btsharp \rangle \qquad  \text{ and } \qquad g(\bu, \bX\btsharp; \by) = -2\eta/n \langle \bu, \omega(\bX \bt^{\sharp}, \by) \rangle
\end{align*}
recovers the first-order loss functions~\eqref{eq:GD_gen}.  The remaining properties (b)-(d) of the assumption can be straightforwardly verified for these two choices. Having written one step of each iterative algorithm of interest as a minimization of a convex loss, we are now ready to proceed to step 2.

\paragraph{Implementing step 2:} Next, we state a formal definition of the auxiliary loss function $\mathfrak{L}_n$.
% and $\bar{L}_n$ 
%from Section~\ref{sec:heuristic}.  %First, we define the auxiliary loss function.
\begin{definition}[Auxiliary loss]
\label{def:aux-gordon-loss}
Let $\bg \sim \mathsf{N}(0, \bI_n)$ and $\bh \sim \mathsf{N}(0, \bI_d)$ denote independent random vectors \apcomment{drawn independently of the pair $(\bX, \by)$?}, let $\btsharp \in \mathbb{R}^d$ denote an arbitrary vector and define the subspace $S_{\sharp} = \mathsf{span}(\btstar, \btsharp)$.  Further, let $\mathcal{L}$ denote an arbitrary loss function which satisfies Assumption~\ref{ass:loss} for functions $g$ and $h$.  Then, given a positive scalar $C_n$, %(which may scale with $n$), 
define the auxiliary loss function
\begin{align*}
%	\label{eq:intermediate-loss}
	\mathfrak{L}_n(\bt, \bu; C_n) := \max_{\bv \in \mathbb{B}_2(C_n)}\;\frac{1}{\sqrt{n}} \| \bv \|_2 \langle \proj_{S_{\sharp}}^{\perp} \bt, \bh \rangle + h(\bt, \bt^{\sharp}) + g(\bu, \bX \bt^{\sharp}; \by)  + \frac{1}{\sqrt{n}}\langle \bv, \bX \proj_{S_{\sharp}} \bt  + \| \proj_{S_{\sharp}}^{\perp} \bt \|_2 \bg - \bu\rangle.
\end{align*}
\end{definition}
The following lemma shows an equivalence between our original optimization over the loss function $\mathcal{L}$ to an auxiliary optimization $\mathfrak{L}_n$. 
\begin{lemma}
	\label{lem:bilinear}
	Let $\btsharp \in \mathbb{R}^d$, suppose that the loss function $\Lc(\bt; \btsharp, \bX, \by)$ satisfies Assumption~\ref{ass:loss}.  There exist universal positive constants $c, C, C'$ as well as a constant $C_n < \infty$ (which may scale with the sample size $n$), such that %with the auxiliary loss $\mathfrak{L}_n(\cdot, \cdot; C_n)$ from Definition~\ref{def:aux-gordon-loss}, 
	the following holds.  For any constant $C_1 \geq C$ and closed subset $D \subseteq \mathbb{B}_2(C_1)$, we have
		\[
		\Pro\Bigl\{ \min_{\bt \in D} \Lc(\bt) \geq t\Bigr\} \leq 2\Pro\Bigl\{\min_{\bt \in D, \bu \in \mathbb{B}_2(C') } \mathfrak{L}_n(\bt, \bu; C_n) \leq t\Bigr\} + Ce^{-cn}.
		\]
		If, in addition, $D$ is convex, then
		\[
		\Pro\Bigl\{\min_{\bt \in D} \mathcal{L}(\bt) \geq t\Bigr\} \leq 2\Pro\Bigl\{\min_{\bt \in D, \bu \in \mathbb{B}_2(C') } \mathfrak{L}_n(\bt, \bu; C_n) \geq t\Bigr\} + Ce^{-cn}.
		\]
\end{lemma}
\kaccomment{The constant $C$ can be made explicit in all three lemmas.} The proof of this lemma can be found in Subsection~\ref{subsec:proof-of-bilinear}, and involves the application of the CGMT (Proposition~\ref{thm:gordon}). Given that the minimization over $\mathcal{L}$ can be approximately written as a minimization over an auxiliary loss, we are now ready to proceed to step 3.


\paragraph{Implementing step 3:} Next, we define the scalarized auxiliary loss. Recall the definition of the convex conjugate of a function $g: \real^d \to \real$, given by $g^*(\bx) = \sup_{\bx' \in \real^d}\; \inprod{\bx'}{\bx} - g(\bx')$.
\begin{definition}[Scalarized auxiliary loss]
	Let $\bg \sim \mathsf{N}(0, \bI_n)$, $\bh \sim \mathsf{N}(0, \bI_d)$, $\bz_1 \sim \mathsf{N}(0, \bI_n)$, and $\bz_2 \sim \mathsf{N}(0, \bI_n)$ denote mutually independent random vectors \apcomment{Latter two are not chosen independently of the pair $(\bX, \by)$, right? Need to be more careful in defining.}, let $\btsharp \in \mathbb{R}^d$ denote an arbitrary vector and define the subspace $S_{\sharp} = \mathsf{span}(\btstar, \btsharp)$.  Further, let $\mathcal{L}$ denote an arbitrary loss function which satisfies Assumption~\ref{ass:loss} for functions $g$ and $h$ and associate with it the following \emph{scalarized auxiliary loss}
	\label{def:scalarized-ao}
	\[
	\bar{L}_n(\alpha, \mu, \nu; \btsharp) := \max_{\bv \in \mathbb{B}_2(C)} \hscal(\alpha, \mu, \nu, \btsharp) - g^{*}(\bv, \bX \btsharp; \by) - \nu \| \proj_{S_{\sharp}}^{\perp}\bh\|_2 \| \bv \|_2 + \langle \nu \bg + \alpha \bz_1 + \mu \bz_2, \bv \rangle,
	\]
	where $g^*$ denotes the convex conjugate of the function $g$ and $\hscal$ is as in part (c) of Assumption~\ref{ass:loss}.
\end{definition}
Our next lemma implements step 3, scalarizing the auxiliary loss $\mathfrak{L}_n$.  Before stating the lemma, we require the definition of a scalarized set and a deviation set. 
%\begin{definition}[Scalarized auxiliary loss]
%	Let $\bg \sim \mathsf{N}(0, \bI_n)$, $\bh \sim \mathsf{N}(0, \bI_d)$, $\bz_1 \sim \mathsf{N}(0, \bI_n)$, and $\bz_2 \sim \mathsf{N}(0, \bI_n)$ be independent random vectors, $\btsharp \in \mathbb{R}^d$ an arbitrary vector and let the subspace $S_{\sharp} = \mathsf{span}(\btstar, \btsharp)$.  Further, let $\mathcal{L}$ denote an arbitrary loss function which satisfies Assumption~\ref{ass:loss} for functions $g$ and $h$ and associate with it the following \emph{scalarized auxiliary loss}
%	\label{def:scalarized-ao}
%	\[
%	\bar{L}_n(\alpha, \mu, \nu; \btsharp) := \max_{\bv \in \mathbb{B}_2(C)} \hscal(\alpha, \mu, \nu, \btsharp) - g^{*}(\bv, \bX \btsharp; \by) - \nu \| \proj_{S_{\sharp}}^{\perp}\bh\|_2 \| \bv \|_2 + \langle \nu \bg + \alpha \bz_1 + \mu \bz_2, \bv \rangle,
%	\]
%	where $g^*$ denotes the convex conjugate of the function $g$ and $\hscal$ is as in part (c) of Assumption~\ref{ass:loss}.
%\end{definition}
\begin{definition}[Scalarized set]
	\label{def:scalarized-set}
Let $\btstar \in \mathbb{R}^d$ denote the ground truth, $\btsharp \in \mathbb{R}^d$ an arbitrary vector, and $S_{\sharp}$ the subspace $S_{\sharp} = \mathsf{span}(\btstar, \btsharp)$.  For any subset $D \subseteq \mathbb{R}^d$, define the scalarized set
	\[
\Pc(D) := \biggl\{(\alpha, \mu, \nu) \in \mathbb{R}^3: \bt \in D \text{ and } \alpha = \langle \bt, \btstar \rangle, \mu = \frac{\langle \bt, \proj_{\btstar}^{\perp}\bt^{\sharp}\rangle}{\| \proj_{\btstar}^{\perp} \bt^{\sharp}\|_2}, \nu = \| \proj_{S_{\sharp}}^{\perp} \bt \|_2\biggr\}.
\]
\end{definition}
\begin{definition}[Deviation set]
Define the deviation set
\begin{align}
	\label{eq:deviation-set}
	D_{\epsilon} := \{\bt \in \mathbb{R}^d: \max\Bigl(\lvert \langle \bt, \btstar \rangle - \alpha^{\gor} \rvert, \Bigl\lvert \frac{\langle \bt, \proj_{\btstar}^{\perp}\bt^{\sharp}\rangle}{\| \proj_{\btstar}^{\perp} \bt^{\sharp}\|_2} - \mu^{\gor} \Bigr\rvert, \lvert \| \proj_{S_{\sharp}}^{\perp} \bt \|_2 - \nu^{\gor} \rvert \Bigr) \geq \epsilon\}.
\end{align}
\end{definition}

We have the following lemma, whose proof we provide in Subsection~\ref{subsec:proof-scalarize-ao}.
\begin{lemma}
	\label{lem:scalarize-ao}
	Under the setting of Lemma~\ref{lem:bilinear}, let the scalarized auxiliary loss $\widebar{L}_n$ be as in Definition~\ref{def:scalarized-ao}.  Then, recalling the deviation set $D_{\epsilon}$~\eqref{eq:deviation-set}, there exists a universal positive constant $C$ such that for all constants $C_1 \geq C$ and for sets $D$ of the form
	\[
	(i.) \;\; D = \mathbb{B}_2(C_1) \qquad \text{ or } \qquad (ii.) \;\; D = D(\epsilon) \cap \mathbb{B}_2(C_1),
	\]
	the following holds. 
	\[
	\min_{\bt \in D, \bu \in \mathbb{B}_2(C_u \sqrt{n})}\; \mathfrak{L}_n(\bt, \bu) \;= \min_{(\alpha, \mu, \nu) \in \Pc(D)} \widebar{L}_n(\alpha, \mu, \nu; \btsharp),
	\]
	with probability at least $1 - Ce^{-cn}$.
\end{lemma}
Having (approximately) scalarized the problem, we are now ready to proceed to our final step of showing growth properties of the function $\bar{L}_n$.

\paragraph{Implementing step 4:} Our final lemma implements step 4, giving growth conditions on the function $\bar{L}_n$.  This is the only lemma which requires the loss function to be specialized to the form~\eqref{eq:sec_order_gen} or~\eqref{eq:GD_gen}.  We provide the proof for higher-order methods in Subsection~\ref{subsec:proof-ao-analysis-higher-order} and the proof for first-order methods in Subsection~\ref{subsec:proof-ao-analysis-first-order}.

\begin{lemma}
	\label{lem:ao-analysis}
	Suppose that the loss function $\mathcal{L}$ can be written in the form~\eqref{eq:GD_gen} or~\eqref{eq:sec_order_gen} and let the scalarized auxiliary loss $\widebar{L}_n$ be as in Definition~\ref{def:scalarized-ao}.  Define the constant $\bar{L}$ as 
	\[
	\bar{L} = \bar{L}^{\mathsf{so}} = \sqrt{\Bigl(1 - \frac{1}{\delta}\Bigr)\Bigl(\EE[\Omega^2] - (\EE[Z_1 \Omega])^2 - (\EE[Z_2 \Omega])^2\Bigr)},
	\]
	if the loss $\mathcal{L}$ is a higher-order loss~\eqref{eq:sec_order_gen} and
	\[
	\bar{L} = \bar{L}^{\mathsf{fo}} = -\frac{1}{2}((\alpha^{\gor})^2 + (\mu^{\gor})^2 + (\nu^{\gor})^2),
	\]
	if the loss $\mathcal{L}$ is a first-order loss~\eqref{eq:GD_gen}.  Then, there exist universal positive constants $c, C, C_1, C_2$ and $C_{\mathsf{sc}}$ such that for all $\kappa \geq C_1$, $n \geq C_1$, and $\epsilon > C_1/\sqrt{n}$, the following hold.
		\begin{enumerate}[label=(\alph*)]
		\item The minimizer
		\[
		(\alpha_n, \mu_n, \nu_n) = \argmin_{(\alpha, \mu, \nu) \in \Pc(\mathbb{B}_2(C_2))} \widebar{L}_n(\alpha, \mu, \nu), 
		\]
		is unique and satisfies both
		\[
		\max\bigl\{\lvert \alpha_n - \alpha^{\gor} \rvert, \lvert \mu_n - \mu^{\gor} \rvert, \lvert \nu_n - \nu^{\gor}\rvert\bigr\} \leq \epsilon,
		\]
		and 
		\[
		\biggl \lvert \widebar{L}_n^{\mathsf{so}}(\alpha_n, \mu_n, \nu_n) - \bar{L} \biggr \rvert \leq \epsilon,
		\]
		with probability at least $1 - Ce^{-cn\epsilon^2}$.
		\item The scalarized auxiliary loss $\bar{L}_n$ is $C_{\mathsf{sc}}$-strongly convex on the domain $\mathbb{B}_2(C_2)$ with probability at least $1 - Ce^{-cn}$.
%		
%		The following strong convexity property holds for the function $\widebar{L}_n$
%		\[
%		\min_{\|(\alpha, \mu, \nu) - (\alpha_n, \mu_n, \nu_n)\|_2 \geq \epsilon} \widebar{L}_n(\alpha, \mu, \nu) \geq \widebar{L}_n(\alpha_n, \mu_n, \nu_n) + C_{\mathsf{sc}}\epsilon^2,
%		\]
%		with probability at least $1 - Ce^{-Cn\epsilon^2}$.
	\end{enumerate}
\end{lemma}
With each of the individual steps completed, we can now put everything together.

\paragraph{Putting together the pieces:} For clarity, we include a schematic diagram of how each lemma is invoked to prove the proposition in Figure~\ref{fig:gordon-schematic}. 
We begin by introducing the convenient shorthand \apcomment{Not used here.}
\[
\bxi = [\parcomp, \perpone, \perptwo] \qquad \text{ and } \qquad \bxi^{\gor} = [\parcomp^{\gor}, \perpone^{\gor}, \perptwo^{\gor}].
\]
Note that our goal is to upper bound the probability
$\Pro\{\mathcal{T}_n(\btsharp) \in D_{\epsilon}\}$.
%The strategy is to implement the high-level steps outlined in Subsection~\ref{sec:high-level-steps}.  To this end, we state a sequence of lemmas, each of which implements a subset of these steps.  Our first lemma implements steps 1 and 2, showing an equivalence between our original optimization over the loss function $\mathcal{L}$ to an auxiliary optimization $\mathfrak{L}_n$.  
%
%  
%
%
%
%We take these lemmas as given and continue with the proof.   
%Now, recall the deviation set $D_{\epsilon}$~\eqref{eq:deviation-set} and 
Note that
\begin{align*}
	\Pro\{\mathcal{T}_n(\btsharp) \in D_{\epsilon} \} = \Pro\Bigl\{\argmin_{\bt \in \mathbb{R}^d} \mathcal{L}(\bt) \in D_{\epsilon}\Bigr\} \overset{\1}{=} \Pro\Bigl\{\argmin_{\bt \in \mathbb{B}_2(C')} \mathcal{L}(\bt) \in D_{\epsilon}\Bigr\} + Ce^{-cn},
\end{align*}
where step $\1$ occurs ... \kaccomment{This needs to be proved somewhere here! I forgot to include the proof.  In the same part where we do this, we need to verify Assumption~\ref{ass:loss} for the two methods considered.}
Subsequently let $\epsilon_1 > 0$ and apply the law of total probability to obtain the inequality 
\begin{align}
	\Pro\Bigl\{\argmin_{\bt \in \mathbb{B}_2(C')} \mathcal{L}(\bt) \in D_{\epsilon}\Bigr\} &\leq \Pro\Bigl\{\min_{\bt \in D_{\epsilon} \cap \mathbb{B}_2(C')} \mathcal{L}(\bt) \leq \min_{\bt \in \mathbb{B}_2(C')} \mathcal{L}(\bt) + \epsilon_1\Bigr\}\nonumber\\
	&\leq \Pro\Bigl\{\min_{\bt \in D_{\epsilon} \cap \mathbb{B}_2(C')} \mathcal{L}(\bt) \leq \bar{\mathsf{L}} + 2\epsilon_1\Bigr\} + \Pro\Bigl\{\min_{\bt \in \mathbb{B}_2(C')} \mathcal{L}(\bt) > \bar{\mathsf{L}} + \epsilon_1\Bigr\}.\label{ineq:step1-prop-gor}
\end{align}
Now, we apply Lemma~\ref{lem:bilinear}, which yields the pair of inequalities
\begin{subequations}\label{ineq:step2-prop-gor}
\begin{align}
	\Pro\Bigl\{\min_{\bt \in D_{\epsilon} \cap \mathbb{B}_2(C')} \mathcal{L}(\bt) \leq \bar{\mathsf{L}} + 2\epsilon_1\Bigr\} &\leq 2\Pro\Biggl\{\min_{\substack{\bt \in D_{\epsilon} \cap \mathbb{B}_2(C'),\\ \bu \in \mathbb{B}_2(C_u\sqrt{n})}}\mathfrak{L}_n(\bt, \bu) \leq \bar{\mathsf{L}} + 2\epsilon_1\Biggr\} + Ce^{-cn},\\
	\Pro\Bigl\{\min_{\bt \in \cap \mathbb{B}_2(C')} \mathcal{L}(\bt) > \bar{\mathsf{L}} + \epsilon_1\Bigr\} &\leq 2\Pro\Biggl\{\min_{\substack{\bt \in  \mathbb{B}_2(C'),\\ \bu \in \mathbb{B}_2(C_u\sqrt{n})}}\mathfrak{L}_n(\bt, \bu) > \bar{\mathsf{L}} + \epsilon_1\Biggr\} + Ce^{-cn}.
\end{align}
\end{subequations}
Subsequently, we apply Lemma~\ref{lem:scalarize-ao} to obtain the pair of inequalities
\begin{subequations}\label{ineq:step3-prop-gor}
	\begin{align}
		\Pro\Biggl\{\min_{\substack{\bt \in D_{\epsilon} \cap \mathbb{B}_2(C'),\\ \bu \in \mathbb{B}_2(C_u\sqrt{n})}}\mathfrak{L}_n(\bt, \bu) \leq \bar{\mathsf{L}} + 2\epsilon_1\Biggr\} &\leq \Pro\Bigl\{\min_{(\alpha, \mu, \nu) \in \Pc(D_{\epsilon} \cap \mathbb{B}_2(C'))}\bar{L}_n(\alpha, \mu, \nu) \leq \bar{\mathsf{L}} + 2\epsilon_1\Bigr\} + Ce^{-cn},\\
		\Pro\Biggl\{\min_{\substack{\bt \in  \mathbb{B}_2(C'),\\ \bu \in \mathbb{B}_2(C_u\sqrt{n})}}\mathfrak{L}_n(\bt, \bu) > \bar{\mathsf{L}} + \epsilon_1\Biggr\} &\leq \Pro\Bigl\{\min_{(\alpha, \mu, \nu) \in \Pc(\mathbb{B}_2(C))} \bar{L}_n(\alpha, \mu, \nu) > \bar{\mathsf{L}} + \epsilon_1\Bigr\} + Ce^{-Cn}. 
	\end{align}
\end{subequations}
Next, consider the two events
\begin{align*}
\mathcal{A}_1 = \Bigl\{\max\bigl\{\lvert \alpha_n - \alpha^{\gor} \rvert, \lvert \mu_n - \mu^{\gor} \rvert, \lvert \nu_n - \nu^{\gor}\rvert\bigr\} \leq \frac{\min(\epsilon, C_{\mathsf{sc}}\epsilon^2)}{2}\Bigr\},
\end{align*}
and
\begin{align*}
	\mathcal{A}_2 = \Bigl\{	\min_{\|(\alpha, \mu, \nu) - (\alpha_n, \mu_n, \nu_n)\|_2 \geq \epsilon\sqrt{3}/2} \widebar{L}_n^{\mathsf{so}}(\alpha, \mu, \nu) \geq \widebar{L}_n^{\mathsf{so}}(\alpha_n, \mu_n, \nu_n) + C_{\mathsf{sc}}\epsilon^2\Bigr\},
\end{align*}
where Lemma~\ref{lem:ao-analysis}(a) implies $\Pro\{\mathcal{A}_1\} \geq 1 - Ce^{-c\min(\epsilon^2, \epsilon^4)}$ and Lemma~\ref{lem:ao-analysis}(b) implies $\Pro\{\mathcal{A}_2\} \geq 1 - Ce^{-cn}$.  Thus, taking $\epsilon_1 = (3C_{\mathsf{sc}}/8) \cdot \epsilon^2$ and applying the law of total probability, we obtain the pair of inequalities
\begin{subequations}\label{ineq:step4-prop-gor}
	\begin{align}
			\Pro\Bigl\{\min_{(\alpha, \mu, \nu) \in \Pc(D_{\epsilon} \cap \mathbb{B}_2(C))}\bar{L}_n(\alpha, \mu, \nu) \leq \bar{\mathsf{L}} + 2\epsilon_1\Bigr\} &\leq C\exp\{-c\min(\epsilon^2, \epsilon^4)\},\\
			\Pro\Bigl\{\min_{(\alpha, \mu, \nu) \in \Pc(\mathbb{B}_2(C))} \bar{L}_n(\alpha, \mu, \nu) > \bar{\mathsf{L}} + \epsilon_1\Bigr\} &\leq C\exp\{-c\min(\epsilon^2, \epsilon^4)\}
	\end{align}
\end{subequations}
Combining the inequalities~\eqref{ineq:step1-prop-gor},~\eqref{ineq:step2-prop-gor},~\eqref{ineq:step3-prop-gor}, and~\eqref{ineq:step4-prop-gor}, we obtain the inequality
\[
\Pro\biggl\{\max\Bigl(\lvert \langle \bt, \btstar \rangle - \alpha^{\gor} \rvert, \Bigl\lvert \frac{\langle \bt, \proj_{\btstar}^{\perp}\bt^{\sharp}\rangle}{\| \proj_{\btstar}^{\perp} \bt^{\sharp}\|_2} - \mu^{\gor} \Bigr\rvert, \lvert \| \proj_{S_{\sharp}}^{\perp} \bt \|_2 - \nu^{\gor} \rvert \Bigr) \geq \epsilon\biggr\} \leq C\exp\{-C\min(\epsilon^2, \epsilon^4)\},
\]
and the proposition follows immediately \apcomment{by setting...}.
\end{proof}
\noindent It remains to prove the technical lemmas.

\begin{figure}[!htbp]
	\centering
	\input{figs/gordon-proof-fig.tex}
	\caption{Schematic diagram of the proof of Proposition~\ref{prop:gordon}, drawn for $\bt \in \mathbb{R}^3$.  The green curve denotes the original loss function $\Lc$, which admits the empirical update $\mathcal{T}_n(\btsharp)$ as its unique minimizer.  The black curve denotes the scalarized auxiliary loss $\bar{L}_n$ (see Definition~\ref{def:scalarized-ao}), which is strongly convex by Lemma~\ref{lem:ao-analysis}(b).  Its unique minimizer is the quantity $\bxi_n$.  The purple curve is the loss $\bar{L}$ which is the population loss corresponding to the empirical loss $\bar{L}_n$.  Its unique minimizer is the quantity $\bxi^{\gor}$.  Further, Lemma~\ref{lem:ao-analysis}(a) shows that $\bxi^{\gor}$ and $\bxi_n$ are at a distance of at most $C\epsilon^2$ from each other.  Lemmas~\ref{lem:bilinear} and~\ref{lem:scalarize-ao} show that the minima, over the sets $D = \mathbb{B}_{\infty}(\bxi^{\gor}; \epsilon)$ and $D = \mathbb{B}_2(C_1)$, of the loss $\Lc$ are the same as those of the loss $\bar{L}_n$.}
	\label{fig:gordon-schematic}
\end{figure}


\subsection{Proof of Lemma~\ref{lem:bilinear}}
\label{subsec:proof-of-bilinear}
We require two additional lemmas.  The first lemma, whose proof we provide in Subsection~\ref{subsec:proof-of-bilinear} shows that the optimization can be done over a compact set. 
\begin{lemma}
	\label{lem:bounded-optimization}
	Under the setting of Lemma~\ref{lem:bilinear}, there exists a universal positive constant $C$ such that for all constants $C_1 \geq C$ and closed subsets $D \subseteq \mathbb{B}_2(C_1)$, 
	\[
	\min_{\bt \in D} \Lc(\bt; \btsharp, \bX, \by) = \min_{\substack{\bt \in D, \\ \bu \in \mathbb{B}_2(C) }}\max_{\bv \in \mathbb{B}_2(C)} \frac{1}{\sqrt{n}} \langle \bv, \bX \bt - \bu \rangle + F(\bu, \bt),
	\]
	with probability at least $1 - Ce^{-Cn}$.  
\end{lemma}
The following lemma uses the bilinear characterization of Lemma~\ref{lem:bounded-optimization} and subsequently invokes Gordon's inequality to connect to the auxiliary loss $\mathfrak{L}_n$.
\begin{lemma}
	\label{lem:invoke-CGMT}
	Under the setting of Lemma~\ref{lem:bilinear}, there exists a universal positive constant $C$ such that for all constants $C_1 \geq C$ and any closed subset $D \subseteq \mathbb{B}_2(C_1)$, 
	\[
	\Pro\Biggl\{\min_{\substack{\bt \in D, \\ \bu \in \mathbb{B}_2(C) }}\max_{\bv \in \mathbb{B}_2(C)} \frac{1}{\sqrt{n}} \langle \bv, \bX \bt - \bu \rangle + F(\bu, \bt) \geq t\Biggr\} \leq 2\Pro\Biggl\{\min_{\substack{\bt \in D, \\ \bu \in \mathbb{B}_2(C) }} \mathfrak{L}(\bt; \bu) \geq t\Biggr\} + Ce^{-Cn}.
	\]
	If, in addition, $D$ is convex, then
		\[
	\Pro\Biggl\{\min_{\substack{\bt \in D, \\ \bu \in \mathbb{B}_2(C) }}\max_{\bv \in \mathbb{B}_2(C)} \frac{1}{\sqrt{n}} \langle \bv, \bX \bt - \bu \rangle + F(\bu, \bt) \leq t\Biggr\} \leq 2\Pro\Biggl\{\min_{\substack{\bt \in D, \\ \bu \in \mathbb{B}_2(C) }} \mathfrak{L}(\bt; \bu) \leq t\Biggr\} + Ce^{-Cn}.
	\]
\end{lemma}

Lemma~\ref{lem:bilinear} follows immediately upon combining Lemmas~\ref{lem:bounded-optimization} and~\ref{lem:invoke-CGMT}. \qed

\subsubsection{Proof of Lemma~\ref{lem:bounded-optimization}}
First, recall that Assumption~\ref{ass:loss} implies the existence of a function $F$ such that $\Lc(\bt) = F(\bX \bt, \bt)$.  Consequently, we obtain
\[
\min_{\bt \in D} \Lc(\bt) = \min_{\bt \in D, \bu \in \mathbb{R}^n} F(\bu, \bt) \quad \text{ s.t. } \quad \bu = \bX\bt.
\]
Applying the inequality~\cite[Corollary 7.3.3]{vershynin2018high} in conjunction with the assumption $D \subseteq \mathbb{B}_2(C_1)$ yields the inequality
\[
\| \bX\bt \|_2 \leq \| \bX\|_2 \| \bt \|_2 \leq C\sqrt{n},
\]
with probability at least $1 - 2e^{-n}$.  Thus,
\begin{align}
	\label{eq:bounded-optimization-intermediate}
\min_{\bt \in D} \Lc(\bt) &= \min_{\substack{\bt \in D, \\ \bu \in \mathbb{B}_2(C) }} F(\bu, \bt) \text{ s.t. } \bu = \bX\bt\nonumber\\
&= \min_{\substack{\bt \in D, \\ \bu \in \mathbb{B}_2(C) }} \max_{\bv \in \mathbb{R}^n} F(\bu, \bt) - \langle \bv, \bu - \bX \bt \rangle.
\end{align}
It remains only to prove that $\bv$ can further be constrained to the ball $\mathbb{B}_2(C\sqrt{n})$ for a large enough constant $C$.  To this end, recall that by Assumption~\ref{ass:loss}(b), the function $F(\bu, \bt)$ is $C_L/\sqrt{n}$-Lipschitz in its first argument.  We thus obtain the pair of inequalities
\begin{align*}
	 \min_{\substack{\bt \in D, \\ \bu \in \mathbb{B}_2(C) }} \max_{\bv \in \mathbb{B}_2(2C_L)} F(\bu, \bt) - \frac{1}{\sqrt{n}}\langle \bv, \bu - \bX \bt \rangle &\geq \min_{\substack{\bt \in D, \\ \bu \in \mathbb{B}_2(C) }} F(\bX \bt, \bt) + \max_{\bv \in \mathbb{B}_2(2C_L)}  \biggl(\frac{\| \bv \|_2}{\sqrt{n}} - \frac{C_L}{\sqrt{n}}\biggr)\| \bu - \bX\bt \|_2\\
	 	 \min_{\substack{\bt \in D, \\ \bu \in \mathbb{B}_2(C) }} \max_{\bv \in \mathbb{B}_2(2C_L)} F(\bu, \bt) - \frac{1}{\sqrt{n}}\langle \bv, \bu - \bX \bt \rangle &\leq \min_{\substack{\bt \in D, \\ \bu \in \mathbb{B}_2(C) }} F(\bX \bt, \bt) + \max_{\bv \in \mathbb{B}_2(2C_L)}  \biggl(\frac{\| \bv \|_2}{\sqrt{n}} + \frac{C_L}{\sqrt{n}}\biggr)\| \bu - \bX\bt \|_2.
\end{align*}
Note that the RHS of both inequalities takes the value $\min_{\bt \in D} F(\bX \bt, \bt)$ so that 
\[
\min_{\substack{\bt \in D, \\ \bu \in \mathbb{B}_2(C) }} \max_{\bv \in \mathbb{B}_2(2C_L)} F(\bu, \bt) - \frac{1}{\sqrt{n}}\langle \bv, \bu - \bX \bt \rangle  = \min_{\bt \in D} F(\bX\bt, \bt),
\]
which is the value of the unconstrained problem~\eqref{eq:bounded-optimization-intermediate}.  The proof is complete upon taking $C$ large enough.\qed

\subsubsection{Proof of Lemma~\ref{lem:invoke-CGMT}}
\label{subsec:proof-invoke-CGMT}
First, recall that by Assumption~\ref{ass:loss}, $F(\bu, \bt)$ can be decomposed as 
\[
F(\bu, \bt) = g(\bu,  \bX \btsharp; \by) + h(\bt, \btsharp).
\]
Next, recall the subspace $S_{\sharp} = \mathsf{span}(\btstar, \btsharp)$ and consider the orthogonal decomposition \\$\bt = \proj_{S_{\sharp}}\bt + \proj_{S_{\sharp}}^{\perp} \bt$.  Combining these two pieces, we obtain the representation
\begin{align*}
\frac{1}{\sqrt{n}} \langle \bv, \bX \bt - \bu \rangle + F(\bu, \bt) &= h(\bt, \btsharp) + g(\bu, \bX\btsharp; \by) - \frac{1}{\sqrt{n}} \langle \bv, \bu \rangle + \frac{1}{\sqrt{n}} \langle \bv, \bX \proj_{S_{\sharp}}\bt \rangle + \frac{1}{\sqrt{n}} \langle \bv, \bX\proj_{S_{\sharp}}^{\perp} \bt \rangle.
\end{align*}

Note that the Gaussian random variable $\langle \bv, \bX\proj_{S_{\sharp}}^{\perp} \bt \rangle$ is independent of all other randomness in the expression.  Thus, in that term, we replace the random matrix $\bX$ with an independent copy $\bG \in \mathbb{R}^{n \times d}$.  Turning to the variational problem of interest, we have
\begin{align*}
	&\min_{\substack{\bt \in D, \\ \bu \in \mathbb{B}_2(C) }}\max_{\bv \in \mathbb{B}_2(C)} h(\bt, \btsharp) + g(\bu, \bX\btsharp; \by) - \frac{1}{\sqrt{n}} \langle \bv, \bu \rangle + \frac{1}{\sqrt{n}} \langle \bv, \bX \proj_{S_{\sharp}}\bt \rangle + \frac{1}{\sqrt{n}} \langle \bv, \bX\proj_{S_{\sharp}}^{\perp} \bt \rangle \\
	\overset{(d)}{=}&\min_{\substack{\bt \in D, \\ \bu \in \mathbb{B}_2(C) }}\max_{\bv \in \mathbb{B}_2(C)} h(\bt, \btsharp) + g(\bu, \bX\btsharp; \by) - \frac{1}{\sqrt{n}} \langle \bv, \bu \rangle + \frac{1}{\sqrt{n}} \langle \bv, \bX \proj_{S_{\sharp}}\bt \rangle + \frac{1}{\sqrt{n}} \langle \bv, \bG\proj_{S_{\sharp}}^{\perp} \bt \rangle.
\end{align*}
At this juncture, we invoke the CGMT Proposition~\ref{thm:gordon} with
\[
P(\bG) = \min_{(\bt, \bu) \in D \times \mathbb{B}_2(C)}\max_{\bv \in \mathbb{B}_2(C)} h(\bt, \btsharp) + g(\bu, \bX\btsharp; \by) - \frac{1}{\sqrt{n}} \langle \bv, \bu \rangle + \frac{1}{\sqrt{n}} \langle \bv, \bX \proj_{S_{\sharp}}\bt \rangle + \frac{1}{\sqrt{n}} \langle \bv, \bG\proj_{S_{\sharp}}^{\perp} \bt \rangle
\]
and 
\[
A(\bg, \bh) = \min_{(\bt, \bu) \in D \times \mathbb{B}_2(C)}\max_{\bv \in \mathbb{B}_2(C)}\; \mathfrak{L}(\bt),
\]
which completes the proof. \qed



\subsection{Proof of Lemma~\ref{lem:scalarize-ao}}
\label{subsec:proof-scalarize-ao}
We begin by defining a few additional optimization problems. Under the setting of Lemma~\ref{lem:scalarize-ao}, recall the map $\Pc$ as defined in Definition~\ref{def:scalarized-set} and define the minimum of the variational problem
	\begin{align}\label{eq:def-phi-var}
		\phi_{\mathsf{var}} \;= &\min_{\substack{(\parcomp, \perpone, \perptwo) \in \Pc(D), \\ \bu \in \mathbb{B}_2(C_u\sqrt{n}) }} \; h_{\mathsf{scal}}(\parcomp, \perpone, \perptwo, \btsharp) + g(\bu, \bX \btsharp; \by) \notag \\
		& + \max_{0 \leq r \leq C_v}\; \frac{r}{\sqrt{n}} \cdot \Bigl( \| \perptwo \cdot  \bg + \parcomp \cdot \bz_1 + \perpone \cdot \bz_2 - \bu \|_2  - \perptwo \cdot  \| \proj_{S_{\sharp}}^{\perp} \bh \|_2 \Bigr).
	\end{align}
Next, define the minimum of the constrained problem
	\begin{align}\label{eq:def-phi-con}
		\phi_{\mathsf{con}} \;= &\min_{\substack{(\parcomp, \perpone, \perptwo) \in \Pc(D), \\ \bu \in \mathbb{B}_2(C\sqrt{n}) }}\; h_{\mathsf{scal}}(\parcomp, \perpone, \perptwo, \btsharp) + g(\bu, \bX \btsharp; \by) \notag \\
		&\;\;\;\;\;\;\; \mathrm{ s.t. }\;\;\;  \| \perptwo \cdot  \bg + \parcomp \cdot \bz_1 + \perpone \cdot \bz_2  - \bu \|_2  \leq  \perptwo \cdot  \| \proj_{S_{\sharp}}^{\perp} \bh \|_2.
	\end{align}
	Finally, define the minimum of the constrained problem
	\begin{align} \label{eq:def-phi-scal}
		\phi_{\mathsf{scal}} \;= &\min_{(\parcomp, \perpone, \perptwo) \in \Pc(D)} \max_{\bv \in \mathbb{R}^n} \;\; h_{\mathsf{scal}}(\parcomp, \perpone, \perptwo, \btsharp) - g^*(\bu, \bX \btsharp; \by) + \min_{\bu \in \mathbb{B}_2(C_u\sqrt{n}) } \langle \bu, \bv \rangle \nonumber\\
		&\;\;\;\;\;\;\; \mathrm{ s.t. }\;\;\;  \| \perptwo \cdot  \bg + \parcomp \cdot \bz_1 + \perpone \cdot \bz_2  - \bu \|_2  \leq  \perptwo \cdot  \| \proj_{S_{\sharp}}^{\perp} \bh \|_2.
	\end{align}


We now state two lemmas that will prove useful in the proof.
\begin{lemma}
	\label{lem:constrained-equivalence}
	% Under the setting of Lemma~\ref{lem:scalarize-ao}, recall the map $\Pc$ as defined in Definition~\ref{def:scalarized-set} and define the minimum of the variational problem
	% \begin{align}\label{eq:def-phi-var}
	% 	\phi_{\mathsf{var}} \;= &\min_{\substack{(\parcomp, \perpone, \perptwo) \in \Pc(D), \\ \bu \in \mathbb{B}_2(C_u\sqrt{n}) }} \; h_{\mathsf{scal}}(\parcomp, \perpone, \perptwo, \btsharp) + g(\bu, \bX \btsharp; \by) \\
	% 	& + \max_{0 \leq r \leq C_v}\; \frac{r}{\sqrt{n}} \cdot \Bigl( \| \perptwo \cdot  \bg + \parcomp \cdot \bz_1 + \perpone \cdot \bz_2 - \bu \|_2  - \perptwo \cdot  \| \proj_{S_{\sharp}}^{\perp} \bh \|_2 \Bigr),
	% \end{align}
	% as well as the minimum of the constrained problem
	% \begin{align}\label{eq:def-phi-con}
	% 	\phi_{\mathsf{con}} \;= &\min_{\substack{(\parcomp, \perpone, \perptwo) \in \Pc(D), \\ \bu \in \mathbb{B}_2(C\sqrt{n}) }}\; h_{\mathsf{scal}}(\parcomp, \perpone, \perptwo, \btsharp) + g(\bu, \bX \btsharp; \by) \\
	% 	&\;\;\;\;\;\;\; \mathrm{ s.t. }\;\;\;  \| \perptwo \cdot  \bg + \parcomp \cdot \bz_1 + \perpone \cdot \bz_2  - \bu \|_2  \leq  \perptwo \cdot  \| \proj_{S_{\sharp}}^{\perp} \bh \|_2.
	% \end{align}
	Under the setup above,
	there exists a universal positive constant $C$ such that 
	\[
	\Pro\Bigl\{\lvert \phi_{\mathsf{var}} - \phi_{\mathsf{con}}\rvert \leq \frac{C}{C_v}\Bigr\} \geq 1 - Ce^{-Cn}.
	\]
\end{lemma}

\begin{lemma}\label{lem:solve-constrained}
% 	Under the setting of Lemma~\ref{lem:scalarize-ao}, define the minimum of the constrained problem
% %	\[
% %	\phi_{\mathsf{scal}} = \min_{(\parcomp,\perpone,\perptwo)\in \Pc(D)}\max_{\bv \in \mathbb{R}^n} \; \hscal(\parcomp, \perpone, \perptwo, \btsharp) - g^*(\bv,\bX\btsharp;\by) -\perptwo \|\proj^{\perp}_{S_{\sharp}}\bh\|_2\|\bv\|_2+\langle \perptwo\bg+\parcomp\bz_1+\perpone\bz_2, \bv \rangle.
% %	\]
% 	\begin{align} \label{eq:def-phi-scal}
% 		\phi_{\mathsf{scal}} \;= &\min_{(\parcomp, \perpone, \perptwo) \in \Pc(D)} \max_{\bv \in \mathbb{R}^n} \;\; h_{\mathsf{scal}}(\parcomp, \perpone, \perptwo, \btsharp) - g^*(\bu, \bX \btsharp; \by) + \min_{\bu \in \mathbb{B}_2(C_u\sqrt{n}) } \langle \bu, \bv \rangle \nonumber\\
% 		&\;\;\;\;\;\;\; \mathrm{ s.t. }\;\;\;  \| \perptwo \cdot  \bg + \parcomp \cdot \bz_1 + \perpone \cdot \bz_2  - \bu \|_2  \leq  \perptwo \cdot  \| \proj_{S_{\sharp}}^{\perp} \bh \|_2.
% 	\end{align}
Under the setup above,
	there exists a universal positive constant $C$ such that 
	\[
	\Pro\biggl\{\phi_{\mathsf{con}} = \min_{(\parcomp,\perpone,\perptwo)\in \Pc(D)} \; \widebar{L}_n(\parcomp, \perpone, \perptwo; \btsharp)\biggr\} \geq 1 - Ce^{-Cn}.
	\]
\end{lemma}
Taking these lemmas as given, the proof of Lemma~\ref{lem:scalarize-ao} consists of three major steps, which we perform in sequence: (i.) we scalarize the maximization over $\bv$; (ii.) scalarize the minimization over $\bt$; and (iii.) optimize over $\bu$.  We proceed now to the execution of these steps.

\paragraph{Scalarize the maximization over $\bv$.}
Recall the auxiliary loss $\mathfrak{L}_n$ from Definition~\ref{def:aux-gordon-loss} and note that the Cauchy--Schwarz inequality implies that
\[
\min_{\substack{\bt \in D, \\ \bu \in \mathbb{B}_2(C_u \sqrt{n}) }}  \mathfrak{L}_n(\bt, \bu) = \min_{\substack{\bt \in D, \\ \bu \in \mathbb{B}_2(C_u\sqrt{n}) }} \max_{0 \leq r \leq C_v} F(\bu, \bt) + \frac{r}{\sqrt{n}} \cdot \Bigl(\langle \bh, \proj_{S_{\sharp}}^{\perp} \bt \rangle + \Bigl\| \| \proj_{S_{\sharp}}^{\perp} \bt \|_2 \cdot \bg + \bX\proj_{S_{\sharp}} \bt - \bu \Bigl\|_2 \Bigr).
\]

\paragraph{Scalarize the minimization in $\bt$.}
Note that by Assumption~\ref{ass:loss}, the function $F(\bu, \bt)$ only depends on the vector $\proj_{S_{\sharp}}^{\perp}$ through its norm.  Thus, since $D$ is either $\mathbb{B}_2(C_1)$ or $D(\epsilon) \cap \mathbb{B}_2(C_1)$ for $D(\epsilon)$ as in Definition XXX, and the objective in the preceding display depends on the direction of the vector $\proj_{S_{\sharp}}^{\perp}$ only through the linear term $\langle \bh, \proj_{S_{\sharp}}^{\perp} \bt \rangle$, we minimize the objective over the direction to obtain the characterization
\begin{align}
	\label{eq:scalarize-bt-characterization}
\min_{\substack{\bt \in D, \\ \bu \in \mathbb{B}_2(C_u \sqrt{n}) }}  \mathfrak{L}_n(\bt, \bu) = &\min_{\substack{\bt \in D, \\ \bu \in \mathbb{B}_2(C_u\sqrt{n}) }} \max_{0 \leq r \leq C_v} F(\bu, \bt)\nonumber\\ 
&+ \frac{r}{\sqrt{n}} \cdot \Bigl( \Bigl\| \| \proj_{S_{\sharp}}^{\perp} \bt \|_2 \cdot  \bg + \bX\proj_{S_{\sharp}} \bt - \bu \Bigl\|_2  - \| \proj_{S_{\sharp}}^{\perp} \bt \|_2\cdot  \| \bh \|_2 \Bigr).
\end{align}
Now, consider the independent random variables
\[
\bz_1  = \bX\btstar \qquad \text{ and } \qquad \bz_2 = \frac{\bX\proj_{\btstar}^{\perp} \btsharp}{\| \bX\proj_{\btstar}^{\perp} \btsharp \|_2},
\]
noting that both $\bz_1, \bz_2 \sim \mathsf{N}(0, \bI_n)$ since $\| \btstar \|_2 = 1$.  Using this notation, we write
\[
\by = f(\bz_1; \bq) + \beps \qquad \text{ and } \qquad \bX\btsharp = \alpha^{\sharp}\bz_1 + \beta^{\sharp} \bz_2.
\]
Now, consider the orthogonal decomposition
\[
\bt = \proj_{S_{\sharp}} \bt + \proj_{S_{\sharp}}^{\perp} \bt = \parcomp(\bt) \cdot \btstar + \perpone(\bt) \cdot \frac{\proj_{\btstar}^{\perp} \btsharp}{\| \proj_{\btstar}^{\perp} \btsharp \|_2} + \proj_{S_{\sharp}}^{\perp} \bt,
\]
where the second equality follows from the Gram--Schmidt orthogonalization.  Using this combined with the characterization~\eqref{eq:scalarize-bt-characterization}, we obtain
\begin{align}
	\label{eq:scalar-in-bt}
\min_{\substack{\bt \in D, \\ \bu \in \mathbb{B}_2(C_u\sqrt{n}) }} \mathfrak{L}_n(\bt, \bu) = &\min_{\substack{(\parcomp, \perpone, \perptwo) \in \Pc(D), \\ \bu \in \mathbb{B}_2(C_u\sqrt{n}) }} \; h_{\mathsf{scal}}(\parcomp, \perpone, \perptwo, \btsharp) + g(\bu, \bX \btsharp; \by)\nonumber\\
& + \max_{0 \leq r \leq C_v}\; \frac{r}{\sqrt{n}} \cdot \Bigl( \| \perptwo \cdot  \bg + \parcomp \cdot \bz_1 + \perpone \cdot \bz_2 - \bu \|_2  - \perptwo \cdot  \| \proj_{S_{\sharp}}^{\perp} \bh \|_2 \Bigr).
\end{align}

\paragraph{Optimize over $\bu$.}
Note that if the inner maximization over $r \geq 0$ were unbounded, the optimization problem in the display above would correspond to a constrained optimization problem.  To this end, we invoke Lemma~\ref{lem:constrained-equivalence}, taking $C_v$ arbitrarily large, in conjunction with the characterization~\eqref{eq:scalar-in-bt} to obtain the equation 
\begin{align*}
%	\label{eq:scalar-in-bt}
	\min_{\substack{\bt \in D, \\ \bu \in \mathbb{B}_2(C_u\sqrt{n}) }} \mathfrak{L}_n(\bt, \bu) = 
&\min_{\substack{(\parcomp, \perpone, \perptwo) \in \Pc(D), \\ \bu \in \mathbb{B}_2(C_u\sqrt{n}) }}\; h_{\mathsf{scal}}(\parcomp, \perpone, \perptwo, \btsharp) + g(\bu, \bX \btsharp; \by) \\
		&\;\;\;\;\;\;\; \mathrm{ s.t. }\;\;\;  \| \perptwo \cdot  \bg + \parcomp \cdot \bz_1 + \perpone \cdot \bz_2  - \bu \|_2  \leq  \perptwo \cdot  \| \proj_{S_{\sharp}}^{\perp} \bh \|_2),
\end{align*}
with probability at least $1 - Ce^{-Cn}$.  We continue by linearizing the constrained objective in the optimization variable $\bu$.  To this end, recall that $g$ is convex in its first argument and let $g^*$ denote its convex conjugate so that
\begin{align*}
			\min_{\substack{\bt \in D, \\ \bu \in \mathbb{B}_2(C_u\sqrt{n}) }} \mathfrak{L}_n(\bt, \bu) \;= &\min_{\substack{(\parcomp, \perpone, \perptwo) \in \Pc(D), \\ \bu \in \mathbb{B}_2(C_u\sqrt{n}) }}\max_{\bv \in \mathbb{R}^n}\; h_{\mathsf{scal}}(\parcomp, \perpone, \perptwo, \btsharp) - g^*(\bv, \bX \btsharp; \by) + \langle \bv, \bu \rangle \\
	&\;\;\;\;\;\;\; \mathrm{ s.t. }\;\;\;  \| \perptwo \cdot  \bg + \parcomp \cdot \bz_1 + \perpone \cdot \bz_2  - \bu \|_2  \leq  \perptwo \cdot  \| \proj_{S_{\sharp}}^{\perp} \bh \|_2.
\end{align*}
Now, we perform three steps in sequence: (i.) write the equivalent Lagrangian to the problem above; (ii.) note that the minimization over $\bu$ is of a convex function over a compact constraint and the maximization over $\bv$ is of a concave function and invoke Sion's minimax theorem to swap the minimization over $\bu$ with the maximization over $\bv$; and (iii.) re-write as a constrained optimization problem to obtain
	\begin{align*}
	\min_{\substack{\bt \in D, \\ \bu \in \mathbb{B}_2(C_u\sqrt{n}) }} \mathfrak{L}_n(\bt, \bu) \;= &\min_{(\parcomp, \perpone, \perptwo) \in \Pc(D)} \max_{\bv \in \mathbb{R}^n} \;\; h_{\mathsf{scal}}(\parcomp, \perpone, \perptwo, \btsharp) - g^*(\bu, \bX \btsharp; \by) + \min_{\bu \in \mathbb{B}_2(C_u\sqrt{n}) } \langle \bu, \bv \rangle\\
	&\;\;\;\;\;\;\; \mathrm{ s.t. }\;\;\;  \| \perptwo \cdot  \bg + \parcomp \cdot \bz_1 + \perpone \cdot \bz_2  - \bu \|_2  \leq  \perptwo \cdot  \| \proj_{S_{\sharp}}^{\perp} \bh \|_2.
\end{align*}
We complete the proof by invoking Lemma~\ref{lem:solve-constrained}. \qed


\subsubsection{Proof of Lemma~\ref{lem:constrained-equivalence}}
\label{subsec:proof-constrained-equivalence}
\kaccomment{note in definition of $\mathfrak{L}_n$ that $C_v$ can scale with $n$}
Note that $\phi_{\mathsf{con}}$ admits the variational representation 
	\begin{align*}
	\phi_{\mathsf{con}} \;= &\min_{\substack{(\parcomp, \perpone, \perptwo) \in \Pc(D), \\ \bu \in \mathbb{B}_2(C\sqrt{n}) }}\; h_{\mathsf{scal}}(\parcomp, \perpone, \perptwo, \btsharp) + g(\bu, \bX \btsharp; \by) \\
	& + \max_{r \geq 0}\; \frac{r}{\sqrt{n}} \cdot \Bigl( \| \perptwo \cdot  \bg + \parcomp \cdot \bz_1 + \perpone \cdot \bz_2 - \bu \|_2  - \perptwo \cdot  \| \proj_{S_{\sharp}}^{\perp} \bh \|_2 \Bigr),
\end{align*}
whence we obtain the inequality $\phi_{\mathsf{con}} \geq \phi_{\mathsf{var}}$.  The rest of the section is devoted to the proof of the reverse inequality $\phi_{\mathsf{var}} \leq \phi_{\mathsf{con}}$.  To this end, fix an arbitrary triple $(\parcomp, \perpone, \perptwo) \in \Pc(D)$.  Given this triple, define the constraint function
\[
\psi(\bu) = \| \perptwo \cdot  \bg + \parcomp \cdot \bz_1 + \perpone \cdot \bz_2 - \bu \|_2  - \perptwo \cdot  \| \proj_{S_{\sharp}}^{\perp} \bh \|_2,
\]
as well as the loss functions
\[
L_n^{\mathsf{var}}(\bu) = \max_{0 \leq r \leq C_v}h_{\mathsf{scal}}(\parcomp, \perpone, \perptwo, \btsharp) + g(\bu, \bX \btsharp; \by) + \frac{r}{\sqrt{n}} \cdot \psi(\bu),
\]
and 
\[
L_n^{\mathsf{con}}(\bu) = \max_{r \geq 0}\;h_{\mathsf{scal}}(\parcomp, \perpone, \perptwo, \btsharp) + g(\bu, \bX \btsharp; \by) + \frac{r}{\sqrt{n}} \cdot \psi(\bu).
\]
Let $\bu^{\var}$ denote an arbitrary minimizer of the loss function $L_n^{\mathsf{var}}$ and suppose that $\bu^{\var}$ does not satisfy the constraint $\psi(\bu^{\var}) \leq 0$---if any such minimizer does satisfy this constraint, then the desired inequality $\phi_{\mathsf{var}} \leq \phi_{\mathsf{con}}$ holds.  

Next, define the event
\[
\mathcal{A}_1 = \{ \| \bg \|_2 \leq 2\sqrt{n},\; \| \bz_1 \|_2 \leq 2\sqrt{n},\; \| \bz_2 \|_2 \leq 2\sqrt{n},\; \| \bh \|_2 \leq 2\},
\]
and note that applying~\cite[Theorem 3.1.1]{vershynin2018high} yields $\Pro\{\mathcal{A}_1\} \geq 1 - 8e^{-cn}$.  Working on this event, we note that we can take $C_u$ large enough so that the set
\begin{align}
	\label{def:S0-def}
S_{0} := \{\bu: \psi(\bu) \leq 0, \bu \in \mathbb{B}_2(C_u \sqrt{n})\} = \mathbb{B}_2\Bigl(\perptwo \cdot  \bg + \parcomp \cdot \bz_1 + \perpone \cdot \bz_2; \;\;\perptwo \cdot  \| \proj_{S_{\sharp}}^{\perp} \bh \|_2\Bigr) \cap \mathbb{B}_2(C_u \sqrt{n}),
\end{align}
is non-empty.  Thus, since $S_{0}$ is a non-empty closed, compact set, the projection onto $S_{0}$ is well-defined.  With this in hand, we require the following statement, whose proofs we defer to the end of the section:
\begin{align}
	\label{ineq:bound-psi-uvar}
	\psi(\bu^{\var}) \leq \frac{C\sqrt{n}}{C_v}. 
\end{align}

Now, note that the set
\[
S_R := \{\bu: \psi(\bu) \leq R\} = \mathbb{B}_2\Bigl(\perptwo \cdot  \bg + \parcomp \cdot \bz_1 + \perpone \cdot \bz_2; \;\;\perptwo \cdot  \| \proj_{S_{\sharp}}^{\perp} \bh \|_2 + R\Bigr).
\]
Thus, since $S_R$ and $S_{0}$ are concentric balls, if $\bu \in S_R$ and $\widetilde{\bu}$ denotes its projection onto $S_{0}$, the distance between the two points satisfies
\begin{align}
	\label{ineq:nested-balls}
\| \bu - \widetilde{\bu} \|_2 \leq R.
\end{align}
Now, let $R = C\sqrt{n}/C_v$ and let $\widetilde{\bu}^{\var}$ denote the projection of $\bu^{\var}$ (which is contained in $S_R$ due to the inequality~\eqref{ineq:bound-psi-uvar}) onto $S_0$.  We thus have 
\begin{align*}
	L_n^{\var} (\bu^{\var}) \overset{\1}{\geq} L_n^{\con}(\widetilde{\bu}^{\var}) - \frac{C_L \| \bu^{\var} - \widetilde{\bu}^{\var}\|_2}{\sqrt{n}} &\overset{\2}{\geq} L_n^{\con}(\bu^{\con}) - \frac{C_L \| \bu^{\var} - \widetilde{\bu}^{\var}\|_2}{\sqrt{n}}\\
	&\geq L_n^{\con}(\bu^{\con})  - \frac{C_L C}{C_v},
\end{align*}
where step $\1$ follows since $g$ is $C_L/\sqrt{n}$-Lipschitz in its first argument, step $\2$ follows by $L_n^{\con}$-minimality of $\bu^{\con}$, and the final inequality follows from the inequality~\eqref{ineq:nested-balls}.  Taking stock, since the above inequality holds for all values $(\parcomp, \perpone, \perptwo) \in \Pc(D)$, we have shown that 
\[
\lvert \phi^{\con} - \phi^{\var} \rvert \leq \frac{C}{C_v},
\]
for an absolute constant $C$.  Noting that $C_v < \infty$ was arbitrary, we make $C_v$ arbitrarily large to obtain the result.  \qed
\kaccomment{Check taking the limit in $C_v$ once more, also rename $C_v$ as it has a misleading name}

\paragraph{Proof of the inequality~\eqref{ineq:bound-psi-uvar}.}  Assume towards a contradiction that the inequality does not hold and let $\widetilde{\bu}^{\var}$ denote the projection of $\bu^{\var}$ onto the set $S_0$ (as defined in equation~\eqref{def:S0-def}).  Then, since the function $g$ is $C_L/\sqrt{n}$-Lipschitz in its first argument, we obtain the inequality
\[
L_n^{\var}(\bu^{\var}) \geq L_n^{\con}(\widetilde{\bu}^{\var}) - \frac{C_L \| \bu^{\var} - \widetilde{\bu}^{\var}\|_2}{\sqrt{n}} + \frac{C_v \psi(\bu^{\var})}{\sqrt{n}} > L_n^{\con}(\widetilde{\bu}^{\var})  - 2C_L C_u + C > L_n^{\con}(\widetilde{\bu}^{\var}),
\]
where the penultimate inequality follows since $\bu \in \mathbb{B}_2(C_u\sqrt{n})$ and the final inequality follows by taking $C$ large enough.  The above display contradicts $L_n^{\var}$-minimality of $\bu^{\var}$, whence we obtain the desired result.

\subsubsection{Proof of Lemma~\ref{lem:solve-constrained}}
\label{subsec:proof-solve-constrained}
Recall the value $\phi_{\mathsf{scal}}$~\eqref{eq:def-phi-scal}.  Now, we consider a fixed triplet $(\parcomp, \perpone, \perptwo) \in \Pc(D)$ and perform the minimization over $\bu$.  To this end, let
	\begin{align*}
	L_u = \; \min_{\bu \in \mathbb{B}_2(C_u\sqrt{n}) } \langle \bu, \bv \rangle \quad \mathrm{ s.t. } \quad \| \perptwo \cdot  \bg + \parcomp \cdot \bz_1 + \perpone \cdot \bz_2  - \bu \|_2  \leq  \perptwo \cdot  \| \proj_{S_{\sharp}}^{\perp} \bh \|_2.
\end{align*}
Then, introducing a Lagrange multiplier  and invoking Sion's minimax theorem to interchange minimization and maximization, we obtain
\begin{align*}
L_u &= \max_{\lambda \geq 0} \min_{\bu \in \mathbb{B}_2(C_u\sqrt{n})} \;\; \langle \bu, \bv \rangle + \frac{\lambda}{2} \| \perptwo \cdot  \bg + \parcomp \cdot \bz_1 + \perpone \cdot \bz_2  - \bu \|_2^2 - \frac{\lambda \nu^2}{2} \| \proj_{S_{\sharp}}^{\perp} \bh \|_2^2 \\
&\geq  \max_{\lambda \geq 0} \min_{\bu \in \mathbb{R}^n} \;\; \langle \bu, \bv \rangle + \frac{\lambda}{2} \| \perptwo \cdot  \bg + \parcomp \cdot \bz_1 + \perpone \cdot \bz_2  - \bu \|_2^2 - \frac{\lambda \nu^2}{2} \| \proj_{S_{\sharp}}^{\perp} \bh \|_2^2\\
&= \max_{\lambda \geq 0} \;\;\langle \perptwo \cdot  \bg + \parcomp \cdot \bz_1 + \perpone \cdot \bz_2, \bv \rangle - \frac{1}{2\lambda} \| \bv\|_2^2 - \frac{\lambda \nu^2}{2} \| \proj_{S_{\sharp}}^{\perp} \bh \|_2^2 \\
&= \langle \perptwo \cdot  \bg + \parcomp \cdot \bz_1 + \perpone \cdot \bz_2, \bv \rangle  - \perptwo \| \proj_{S_{\sharp}}^{\perp} \bh \|_2 \| \bv \|_2.
\end{align*}  
Conversely, let 
\[
\bar{\bu} = \perptwo \cdot  \bg + \parcomp \cdot \bz_1 + \perpone \cdot \bz_2 - \perptwo \| \proj_{S_{\sharp}}^{\perp} \bh \|_2 \cdot \frac{\bv}{\| \bv \|_2} ,
\]
which is feasible for large enough $C_u$.  Thus, we obtain
\[
L_u \leq \langle \bar{\bu}, \bv \rangle =  \langle \perptwo \cdot  \bg + \parcomp \cdot \bz_1 + \perpone \cdot \bz_2, \bv \rangle  - \perptwo \| \proj_{S_{\sharp}}^{\perp} \bh \|_2 \| \bv \|_2.
\]
Evidently, 
\[
L_u =  \langle \perptwo \cdot  \bg + \parcomp \cdot \bz_1 + \perpone \cdot \bz_2, \bv \rangle  - \perptwo \| \proj_{S_{\sharp}}^{\perp} \bh \|_2 \| \bv \|_2.
\]
Thus, we obtain
\begin{align*}
\phi_{\mathsf{scal}} &= \min_{(\parcomp, \perpone, \perptwo) \in \Pc(D)} \max_{\bv \in \mathbb{R}^n} \;\; h_{\mathsf{scal}}(\parcomp, \perpone, \perptwo, \btsharp) - g^*(\bu, \bX \btsharp; \by) + \langle \perptwo \cdot  \bg + \parcomp \cdot \bz_1 + \perpone \cdot \bz_2, \bv \rangle  - \perptwo \| \proj_{S_{\sharp}}^{\perp} \bh \|_2 \| \bv \|_2\\
&=\min_{(\parcomp,\perpone,\perptwo)\in \Pc(D)} \; \widebar{L}_n(\parcomp, \perpone, \perptwo; \btsharp),
\end{align*}
which concludes the proof. \qed



\subsection{Proof of Lemma~\ref{lem:ao-analysis}: Higher-order methods}
\label{subsec:proof-ao-analysis-higher-order}
In this subsection, we prove Lemma~\ref{lem:ao-analysis}, specialized to second order methods where the loss function~\eqref{eq:sec_order_gen} takes the form 
\[
\Lc(\bt; \btsharp, \bX, \by) = \frac{1}{\sqrt{n}} \| \omega(\bX\btsharp, \by) - \bX\bt \|_2,
\]
which corresponds to setting 
\[
F(\bu, \bt) = \| \omega(\bX\btsharp, \by) - \bu \|_2, \qquad h(\bt, \btsharp) = 0, \qquad \text{ and } \qquad g(\bu, \bX \btsharp; \by) = \| \omega(\bX\btsharp, \by) - \bu \|_2.
\]
We now state several lemmas, which we will invoke in sequence.  The first specializes the scalarized auxiliary loss $\bar{L}_n$ when the loss corresponds to a higher-order method.
\begin{lemma}
	\label{lem:remove-positive-restriction}
	Under the setting of Lemma~\ref{lem:ao-analysis}, let the loss $\Lc$ correspond to a higher-order method as in equation~\eqref{eq:sec_order_gen}.  There exists a universal positive constant $c$ such that with probability at least $1 - 6e^{-cn}$, \apcomment{Weirdly stated. Is this a definition or a lemma? Also need to be expicit about dependence between $(\bz_1, \bz_2)$ and $(\bX, \by)$.}
	\[
	\bar{L}_n(\parcomp, \perpone, \perptwo; \btsharp) = \frac{1}{\sqrt{n}} \| \perptwo \cdot \bg + \parcomp \cdot \bz_1 + \perpone \cdot \bz_2 - \omega(\bX \btsharp, \by) \|_2 - \perptwo \frac{\| \proj_{S_{\sharp}}^{\perp} \bh \|_2}{\sqrt{n}}.
	\]
\end{lemma}
Proved in Subsection~\ref{subsec:proof-lemma-remove-positive-restriction}.
Before stating the next lemma, we introduce the shorthand 
\[
\sqrt{\kappa_n} := \frac{\| \proj^{\perp}_{S_{\sharp}} \bh\|_2}{\sqrt{n}}, \qquad \bA:= [\bz_1, \bz_2, \bg] \in \mathbb{R}^{n \times 3}, \qquad \text{ and } \qquad \bv_n := [0, 0, \sqrt{\kappa_n}]^{\top} \in \mathbb{R}^3,
\]
so that letting $\bxi = [\parcomp, \perpone, \perptwo]$ and invoking Lemma~\ref{lem:remove-positive-restriction}, we obtain
\[
\bar{L}_n(\bxi; \btsharp) = \frac{1}{\sqrt{n}} \| \bA \bxi - \omega(\bX \btsharp, \by) \|_2 - \langle \bv_n, \bxi \rangle.
\]
Now, introduce the variable $\tau$ and write the above display in the form
\[
\bar{L}_n(\bxi; \btsharp) = \inf_{\tau > 0} \widetilde{L}_n(\bxi, \tau)\; \frac{\tau}{2} + \frac{1}{2\tau n} \| \bA \bxi - \omega(\bX \btsharp, \by) \|_2^2 - \langle \bv_n, \bxi \rangle 
\]
\begin{lemma}
	\label{lem:row-space-A}
	There exists a universal positive constants $c$ and $c'$ such that with probability at least $1 - 10e^{-cn}$, the following inequality holds 
	\[
	\frac{1}{n} \| \bA\bxi - \omega(\bX\btsharp, \by) \|_2^2 > c',
	\]
	for all $\bxi \in \mathbb{R}^3$.
\end{lemma}
Proved in Subsection~\ref{subsec:proof-lemma-row-space-A}.

\begin{lemma}
	\label{lem:minimize-lbar-higher-order}
	There exists a universal positive constant $c$ such that with probability at least $ 1 - 10e^{-cn}$, 
	\begin{subequations}
	\begin{align}\label{eq:interchange-inf-min}
	\min_{\bxi \in \Pc(\mathbb{B}_2(C))} \inf_{\tau > 0}\; \widetilde{L}_n(\bxi, \tau) = \inf_{\tau > 0}	\min_{\bxi \in \Pc(\mathbb{B}_2(C))}\; \widetilde{L}_n(\bxi, \tau)
	\end{align}
	and the optimization problem on the RHS of equation~\eqref{eq:interchange-inf-min} admits unique minimizers
	\begin{align} \label{eq:unique-empirical-xi}
	\bxi_n(\tau) = (\bA^{\top} \bA)^{-1} \bA^{\top} \omega(\bX\btsharp, \by) + \tau \cdot n \cdot (\bA^{\top} \bA)^{-1} \bv_n,
	\end{align}
	and 
	\begin{align} \label{eq:unique-empirical-tau}
	\tau_n = \frac{\frac{1}{\sqrt{n}}\|(\bI_n - \bA(\bA^{\top} \bA)^{-1}\bA^{\top})\omega(\bX \btsharp, \by) \|_2}{\sqrt{1 - n\cdot \bv_n^{\top} (\bA^{\top} \bA)^{-1} \bv_n}}.
	\end{align}
	\end{subequations}
\end{lemma}
Proved in Subsection~\ref{subsec:proof-lemma-minimize-lbar}.

\subsubsection{Proof of Lemma~\ref{lem:ao-analysis}(a): Higher-order methods} 
The first part of the statement---uniqueness of the minimizer--- is an immediate consequence of Lemma~\ref{lem:minimize-lbar-higher-order}; moreover, the unique minimizer is given by $\xi_n(\tau_n)$.  It remains to prove the concentration properties.  As a preliminary step, we show that the dual variable $\tau_n$ concentrates around a deterministic quantity 
\[
\tau^{\gor} = \sqrt{\Bigl(\frac{\kappa}{\kappa - 1} \Bigr) (\EE\{ \Omega^2\} - (\EE\{ Z_1 \Omega\})^2 - (\EE\{ Z_2 \Omega\})^2)}.
\]
To this end, consider the event
\[
\Ac_1 = \Bigl\{(1 - C\epsilon)\bI_3 \preceq \frac{1}{n} \bA^{\top} \bA \preceq (1 +C\epsilon)\bI_3\Bigr\},
\]
and apply~\cite[Theorem 6.1]{wainwright2019high} to obtain $\Pro\{\Ac_1\} \geq 1 - 2e^{-cn\epsilon^2}$.  We note that on the event $\Ac_1$, we obtain the sandwich relation
\[
(1 - C\epsilon/2) \bI_3 \preceq n (\bA^{\top} \bA)^{-1} \preceq (1 + C\epsilon/2) \bI_3.
\]

\paragraph{Bounding $\tau_n$~\eqref{eq:unique-empirical-tau}.} We proceed in three steps.  First, we bound the numberator; second, we bound the denominator; and finally we combine the two bounds.\\

\noindent\underline{Bounding the numerator.}
First, let $\bomega_{\sharp} = \omega(\bX \btsharp, \by)$ and expand the norm to obtain
\[
\frac{1}{\sqrt{n}}\|(\bI_n - \bA(\bA^{\top} \bA)^{-1}\bA^{\top})\omega(\bX \btsharp, \by) \|_2 = \sqrt{ \frac{1}{n}\| \bomega_{\sharp}\|_2^2 - \frac{1}{n}(\bA^{\top}\bomega_{\sharp})^{\top}(\bA^{\top} \bA)^{-1} (\bA^{\top} \bomega_{\sharp})}.
\]
Now, on the event $\Ac_1$, we obtain the sandwich relation
\[
A_L \leq \sqrt{ \frac{1}{n}\| \bomega_{\sharp}\|_2^2 - \frac{1}{n}(\bA^{\top}\bomega_{\sharp})^{\top}(\bA^{\top} \bA)^{-1} (\bA^{\top} \bomega_{\sharp})} \leq A_U,
\]
where we have let
\begin{align*}
	A_L &= \sqrt{ \frac{1}{n}\| \bomega_{\sharp}\|_2^2 - \frac{1 + C\epsilon/2}{n^2}\|\bA\bomega_{\sharp}\|_2^2} =  \sqrt{ \frac{1}{n}\| \bomega_{\sharp}\|_2^2 - \frac{1 + C\epsilon/2}{n^2}(\langle \bg, \bomega_{\sharp}\rangle^2 + \langle \bz_1, \bomega_{\sharp}\rangle^2 + \langle \bz_2, \bomega_{\sharp} \rangle^2)}\\
	A_U &= \sqrt{ \frac{1}{n}\| \bomega_{\sharp}\|_2^2 - \frac{1 - C\epsilon/2}{n^2}\|\bA\bomega_{\sharp}\|_2^2} =\sqrt{ \frac{1}{n}\| \bomega_{\sharp}\|_2^2 - \frac{1 - C\epsilon/2}{n^2}(\langle \bg, \bomega_{\sharp}\rangle^2 + \langle \bz_1, \bomega_{\sharp}\rangle^2 + \langle \bz_2, \bomega_{\sharp} \rangle^2)}, 
\end{align*}
where the last equality in both lines follows by recalling that $\bA^{\top}\bomega_{\sharp} = [\langle \bz_1, \bomega_{\sharp} \rangle, \langle \bz_2, \bomega_{\sharp}\rangle, \langle \bg, \bomega_{\sharp}]$  Now, consider the two events
\begin{align*}
	\Ac_2 = \Bigl\{\frac{1}{n^2}\lvert \langle \bg, \bomega_{\sharp} \rangle \rvert^2 \vee \Bigl\lvert \frac{1}{n^2}\langle \bz_1, \bomega_{\sharp}\rangle^2 - (\EE \{ Z_1 \Omega \})^2\Bigr\rvert \vee \Bigl\lvert \frac{1}{n^2}\langle \bz_2, \bomega_{\sharp} \rangle^2 - (\EE\{Z_2 \Omega \})^2 \Bigr \rvert \leq C\epsilon\Bigr\},
\end{align*}
and 
\begin{align*}
	\Ac_3 &= \Bigl\{\Bigl\lvert \frac{1}{n} \| \bomega_{\sharp} \|_2^2 - \EE\{\Omega^2\} \Bigr\rvert \leq C\epsilon \Bigr\}.
\end{align*}
Next, recall that by Assumption~\ref{ass:omega}, we have the bound $\| \bomega_{\sharp} \|_{\psi_2} \leq K$.  Thus, we apply Bernstein's inequality to obtain the inequality
\[
\Pro\Bigl\{ \Bigl \lvert \frac{1}{n} \langle \bz_1, \bomega_{\sharp} \rangle - \EE\{ Z_1 \Omega\}\Bigr\rvert \geq C\epsilon \Bigr\} \leq 2e^{-cn\epsilon^2}.
\]
Consequently, with probability at least $1 - 2e^{-cn\epsilon^2}$,  
\[
\Bigl\lvert\frac{1}{n^2}\langle \bz_1, \bomega_{\sharp}\rangle^2 - (\EE \{ Z_1 \Omega \})^2\Bigr\rvert = \Bigl \lvert \frac{1}{n} \langle \bz_1, \bomega_{\sharp} \rangle - \EE\{ Z_1 \Omega\}\Bigr\rvert \cdot \Bigl \lvert \frac{1}{n} \langle \bz_1, \bomega_{\sharp} \rangle + \EE\{ Z_1 \Omega\}\Bigr\rvert \overset{\1}{\leq} \frac{C\epsilon}{3},
\]
where step $\1$ additionally used the fact that $\EE\{Z_1 \Omega\} \leq C$.  Bounding the other terms similarly and applying the union bound, we obtain $\Pro\{\Ac_2\} \geq 1 - 6e^{-cn\epsilon^2}$.  Finally, we apply Bernstein's inequality once more to obtain the inequality $\Pro\{ \Ac_3 \} \geq 1 - 2e^{-cn\epsilon^2}$.  Thus, on the event $\Ac_2 \cap \Ac_3$, we obtain 
\[
A_L \geq \sqrt{(\EE\{\Omega^2\} - (\EE\{Z_1 \Omega\})^2 - (\EE\{Z_2 \Omega\})^2 - C\epsilon} \overset{\1}{\geq}  \sqrt{(\EE\{\Omega^2\} - (\EE\{Z_1 \Omega\})^2 - (\EE\{Z_2 \Omega\})^2} - C'\epsilon, 
\]
where step $\1$ follows since by Assumption~\ref{ass:omega}, the first terrm on the RHS is at least a small positive constant.  We additionally emphasize that the constant $C$ has changed from line to line.  Proceeding similarly, we obtain the upper bound
\[
A_U \leq \sqrt{(\EE\{\Omega^2\} - (\EE\{Z_1 \Omega\})^2 - (\EE\{Z_2 \Omega\})^2} + C'\epsilon.
\]
Putting the pieces together, we see that with probability at least $1 - 10e^{-cn\epsilon^2}$, 
\[
\Bigl\lvert \frac{1}{\sqrt{n}}\|(\bI_n - \bA(\bA^{\top} \bA)^{-1}\bA^{\top})\omega(\bX \btsharp, \by) \|_2 -  \sqrt{(\EE\{\Omega^2\} - (\EE\{Z_1 \Omega\})^2 - (\EE\{Z_2 \Omega\})^2} \Bigr\rvert \leq C'\epsilon
\]

\noindent\underline{Bounding the denominator.} On the event $\Ac_1$, we note the sandwich relation
\[
D_L \leq \sqrt{1 - n\cdot \bv_n^{\top} (\bA^{\top} \bA)^{-1} \bv_n} \leq D_U,
\]
where we have let
\begin{align*}
	D_L &= \sqrt{1 - (1 + C\epsilon) \|\bv_n\|_2^2}, \qquad \text{ and } \qquad D_U = \sqrt{1 - (1 - C\epsilon) \|\bv_n\|_2^2}.
\end{align*}
Now, consider the event
\[
\Ac_4 = \bigl\{\bigl\lvert \| \bv_n \|_2^2 - \kappa^{-1} \bigr \rvert \leq C\epsilon \bigr\},
\]
noting that an application of Bernstein's inequality implies $\Pro\{\Ac_4\} \geq 1 - 2e^{-cn\epsilon^2}$.  Now, on the event $\Ac_4$, we further obtain the bounds
\[
D_L \geq \sqrt{1 - \kappa^{-1}} - C'\epsilon, \qquad \text{ and } \qquad D_U \leq \sqrt{1 - \kappa^{-1}} + C'\epsilon.
\]

\noindent\underline{Putting the pieces together to control $\tau_n$.}  Now, we combine the two-sided bounds on both the numerator and denominator to obtain the inequality
\begin{align}\label{ineq:probabalistic-control-taun}
\Pro\bigl\{\bigl \lvert \tau_n - \tau^{\gor} \bigr \rvert \leq C\epsilon \bigr\} \geq 1 - 10e^{-cn\epsilon^2}.
\end{align}

\paragraph{Bounding the minimizer $\bxi_n(\tau_n)$~\eqref{eq:unique-empirical-xi}.} First, let $\be_1$ denote the first elementary vector and consider the quantity
\[
\lvert \langle \be_1, \bxi_n(\tau_n) \rangle - \parcomp^{\gor} \rvert = \lvert \langle \be_1, (\bA^{\top} \bA)^{-1} \bA^{\top} \omega(\bX\btsharp, \by) + \tau \cdot n \cdot (\bA^{\top} \bA)^{-1} \bv_n\rangle - \parcomp^{\gor} \rvert.
\]
First, note that on the event $\Ac_1$, we can write $n\cdot (\bA^{\top} \bA)^{-1} = \bI_3 + \bB$, where $\| \bB \|_{\mathsf{op}} \leq C\epsilon$.  We thus obtain the decomposition
\[
\lvert \langle \be_1, (\bA^{\top} \bA)^{-1} \bA^{\top} \omega(\bX\btsharp, \by) + \tau_n \cdot n \cdot (\bA^{\top} \bA)^{-1} \bv_n\rangle - \parcomp^{\gor} \rvert \leq A_1 + A_2,
\]
where
\begin{align*}
	A_1 &= \Bigl \lvert \frac{1}{n} \langle \be_1, \bA^{\top} \omega(\bX\btsharp, \by) \rangle + \tau_n \langle \be_1, \bv_n \rangle  - \alpha^{\gor}\Bigr\rvert\\
	A_2 &= \Bigl \lvert  \frac{1}{n} \langle \be_1, \bB  \bA^{\top} \omega(\bX\btsharp, \by) \rangle + \tau_n \cdot \langle \be_1, \bB \bv_n \rangle \Bigr\rvert.
\end{align*}
Now, consider the two events
\begin{align*}
	\Ac_5 = \Bigl\{\frac{1}{n}\lvert \langle \bg, \bomega_{\sharp} \rangle \rvert \vee \Bigl\lvert \frac{1}{n}\langle \bz_1, \bomega_{\sharp}\rangle - \EE \{ Z_1 \Omega \}\Bigr\rvert \vee \Bigl\lvert \frac{1}{n}\langle \bz_2, \bomega_{\sharp} \rangle - \EE\{Z_2 \Omega \} \Bigr \rvert \leq C\epsilon\Bigr\},
\end{align*}
and 
\begin{align*}
	\Ac_6 = \{\lvert \tau_n - \tau^{\gor}\rvert \leq C\epsilon\}.
\end{align*}
Note that by the inequality~\eqref{ineq:probabalistic-control-taun}, $\Pro\{\Ac_6\} \geq 1 - 10e^{-cn\epsilon^2}$ and further by applying Bernstein's inequality, $\Pro\{\Ac_5\} \geq 1 - 6e^{-cn\epsilon^2}$.  Working on the event $\Ac_5 \cap \Ac_6$ and applying the triangle inequality, we obtain the upper bound
\[
A_1 \leq \lvert \EE\{Z_1 \Omega\} - \parcomp^{\gor} \rvert + C\epsilon.
\]
Further noting that $\| \bB \|_{\mathsf{op}} \leq C\epsilon$ and noting that $\EE\{Z_1 \Omega\} \leq C$, we obtain the bound
\[
A_2 \leq \frac{1}{n}\| \bB\|_{\mathsf{op}}  \| \bA^{\top} \omega(\bX\btsharp, \by) \|_2 \leq C\epsilon.
\]
Summarizing, we have shown that
\begin{subequations}\label{ineq:bound-minimizers-scalarized-ao}
\begin{align}
\Pro\{\lvert \langle \be_1, \bxi_n(\tau_n) \rangle - \parcomp^{\gor} \rvert \leq C\epsilon\} \geq 1 - 16e^{-cn\epsilon^2}.
\end{align}
Proceeding in a parallel manner, we obtain the two bounds
\begin{align}
\Pro\{\lvert \langle \be_2, \bxi_n(\tau_n) \rangle - \perpone^{\gor} \rvert \leq C\epsilon\} \geq 1 - 16e^{-cn\epsilon^2},
\end{align} 
\begin{align}
	 \Pro\{\lvert \langle \be_1, \bxi_n(\tau_n) \rangle - \perptwo^{\gor} \rvert \leq C\epsilon\} \geq 1 - 16e^{-cn\epsilon^2}.
\end{align}
\end{subequations}

\paragraph{Bounding the minimum $\bar{L}_n(\bxi_n(\tau_n), \btsharp)$.}  Note that 
\[
\bar{L}_n(\bxi_n(\tau_n); \btsharp) = \frac{1}{\sqrt{n}} \| \bA\bxi_n(\tau_n) - \omega(\bX \btsharp, \by) \|_2 - \langle \bv_n, \bxi_n(\tau_n) \rangle.
\]
Now, consider the event
\[
\Ac_7 = \{\|\xi_n(\tau_n) - \bxi^{\gor}\|_{\infty} \leq C\epsilon\},
\]
noting that the inequality~\eqref{ineq:bound-minimizers-scalarized-ao} implies $\Pro\{\Ac_7\} \geq 1 - 16e^{-cn\epsilon^2}$.  For the remainder of the proof, we will work on the event $\mathcal{A} = \bigcap_{k=1}^{7} \Ac_k$.  Adding and subtracting the quantity $\xi^{\gor}$ yields
\begin{align*}
	\bar{L}_n(\bxi_n(\tau_n); \btsharp) = \frac{1}{\sqrt{n}} \| \bA\bxi^{\gor} + \bA (\bxi_n(\tau_n) - \bxi^{\gor}) - \omega(\bX \btsharp, \by) \|_2 - \langle \bv_n, \bxi^{\gor} \rangle - \langle \bv_n, \bxi_n(\tau_n) - \bxi^{\gor} \rangle.
\end{align*}
Thus, on the event $\Ac$, we obtain the inequality
\[
\Bigl \lvert \bar{L}_n(\bxi_n(\tau_n); \btsharp)  - \frac{1}{\sqrt{n}} \| \bA\bxi^{\gor} - \omega(\bX \btsharp, \by) \|_2 + \langle \bv_n, \bxi^{\gor} \rangle \Bigr\rvert \leq C\epsilon.
\]
Now, on the event $\Ac$, we obtain the inequality
\[
\biggl \lvert\frac{1}{\sqrt{n}} \| \bA\bxi^{\gor} - \omega(\bX \btsharp, \by) \|_2 - \langle \bv_n, \bxi^{\gor} \rangle - \sqrt{\Bigl(1 - \frac{1}{\kappa}\Bigr)\Bigl(\EE[\Omega^2] - (\EE[Z_1 \Omega])^2 - (\EE[Z_2 \Omega])^2\Bigr)} \biggr \rvert \leq C\epsilon.
\]
We obtain the result upon combining the two displays above. \qed

\subsubsection{Proof of Lemma~\ref{lem:ao-analysis}(b): Higher-order methods}
We begin by defining the three events
\[
\Ac_1 = \Bigl\{\min_{\bxi \in \mathbb{R}^3} \frac{1}{\sqrt{n}}\| \bA \bxi - \omega(\bX \btsharp, \by) \|_2 \geq c\Bigr\},
\]
\[
 \Ac_2 = \Bigl\{ \frac{1}{2} \bI_3 \preceq \frac{1}{n} \bA^{\top} \bA \preceq 2 \bI_3\Bigr\}, \qquad \text{ and } \qquad \Ac_3 = \Bigl\{\frac{1}{\sqrt{n}}\| \omega(\bX \btsharp, \by)\|_2 \leq C\Bigr\},
\]
and note that on the event $\Ac_2 \cap \Ac_3$, we obtain the inequality
\begin{align}\label{ineq:upper-bound-quadratic}
\max_{\bxi \in \mathbb{B}_2(C')} \frac{1}{\sqrt{n}}\| \bA \bxi - \omega(\bX \btsharp, \by)\|_2 \leq C.
\end{align}
Applying Lemma~\ref{lem:row-space-A} yields the inequality $\Pro\{\Ac_1\} \geq 1 - 10e^{-cn}$; applying~\cite[Theorem 6.1]{wainwright2019high} yields $\Pro\{\Ac_2\} \geq 1 - 2e^{-cn}$; and applying Bernstein's inequality (as each component of $\omega(\bX \btsharp, \by)$ is $K$-sub-Gaussian by Assumption~\ref{ass:omega}) implies $\Pro\{\Ac_3\} \geq 2e^{-cn}$.  

Note that on the event $\Ac_1$, $\bar{L}_n$ is twice continuously differentiable.  Thus, our strategy is to bound the minimum eigenvalue of the Hessian $\nabla^2 \bar{L}_n$.  We compute
\begin{align*}
\nabla^2 \bar{L}_n(\bxi; \btsharp) &= \frac{1}{\| \bA\bxi - \omega(\bX \btsharp, \by) \|_2} \cdot \frac{1}{\sqrt{n}} \cdot \Bigl( \bA^{\top} \bA - \frac{\bA^{\top} (\bA \bxi - \omega(\bX \btsharp, \by)(\bA \bxi - \omega(\bX\btsharp, \by))^{\top}\bA}{\| \bA\bxi - \omega(\bX \btsharp, \by) \|_2^2}\Bigr)\\
&\overset{\1}{\succeq} \frac{1}{Cn} \cdot \Bigl( \bA^{\top} \bA - \frac{\bA^{\top} (\bA \bxi - \omega(\bX \btsharp, \by)(\bA \bxi - \omega(\bX\btsharp, \by))^{\top}\bA}{\| \bA\bxi - \omega(\bX \btsharp, \by) \|_2^2}\Bigr),
\end{align*}
where step $\1$ follows on the event $\Ac_2 \cap \Ac_3$.  Subsequently, we utilize the variational characterization of eigenvalues to obtain
\begin{align}\label{ineq:lower-bound-mineig}
	\lambda_{\min}(\nabla^2 \bar{L}_n(\bxi; \btsharp) ) &\geq \frac{1}{Cn} \min_{\| \bv \|_2 = 1} \langle \bv, \bA^{\top} \bA\bv \rangle - \frac{\langle \bv, \bA^{\top} (\bA \bxi - \omega(\bX \btsharp, \by)(\bA \bxi - \omega(\bX\btsharp, \by))^{\top}\bA\bv \rangle}{\| \bA\bxi - \omega(\bX \btsharp, \by) \|_2^2}\nonumber\\
	&= \frac{1}{Cn} \min_{\| \bv \|_2 = 1} \| \bA \bv \|_2^2 - \frac{\langle \bA \bv, \bA \bxi - \omega(\bX \btsharp, \by) \rangle^2}{\| \bA\bxi - \omega(\bX \btsharp, \by) \|_2^2}.
\end{align}
Next, consider the orthogonal decomposition
\[
\omega(\bX \btsharp, \by) = \bA \bomega + \bomega^{\perp},
\]
where $\bA \bomega$ denotes an element in the row space of the random matrix $\bA$ and $\bomega^{\perp}$ is orthogonal to the row space of $\bA$.  Thus, 
\begin{align}\label{eq:variational-characterization}
	\min_{\| \bv \|_2 = 1} \| \bA \bv \|_2^2 - \frac{\langle \bA \bv, \bA \bxi - \omega(\bX \btsharp, \by) \rangle^2}{\| \bA\bxi - \omega(\bX \btsharp, \by) \|_2^2} &= \min_{\| \bv \|_2 = 1} \| \bA \bv \|_2^2 - \frac{\langle \bA \bv, \bA (\bxi - \bomega) - \bomega^{\perp}\rangle^2}{\| \bA(\bxi - \bomega)\|_2^2 + \| \bomega^{\perp} \|_2^2}\nonumber\\
	&= \min_{\| \bv \|_2 = 1} \| \bA \bv \|_2^2 - \frac{\langle \bA \bv, \bA (\bxi - \bomega)\rangle^2}{\| \bA(\bxi - \bomega)\|_2^2 + \| \bomega^{\perp} \|_2^2}\nonumber\\
	&\overset{\1}{=}  \min_{\| \bv \|_2 = 1} \| \bA \bv \|_2^2 - \frac{\| \bA \bv\|_2^2 \cdot \| \bA (\bxi - \bomega)\|_2^2}{\| \bA(\bxi - \bomega)\|_2^2 + \| \bomega^{\perp} \|_2^2},
\end{align}
where step $\1$ follows by applying the Cauchy--Schwarz inequality.  Now, 
\begin{align} \label{ineq:lower-bound-variational}
	\min_{\| \bv \|_2 = 1} \| \bA \bv \|_2^2 - \frac{\| \bA \bv\|_2^2 \cdot \| \bA (\bxi - \bomega)\|_2^2}{\| \bA(\bxi - \bomega)\|_2^2 + \| \bomega^{\perp} \|_2^2} \overset{\1}{\geq} \frac{n}{2} \cdot \frac{\| \bomega^{\perp} \|_2^2}{\| \bA(\bxi - \bomega)\|_2^2 + \| \bomega^{\perp} \|_2^2} \overset{\2}{\geq} cn
\end{align}
where step $\1$ follows on the event $\Ac_2$ and step $\2$ follows on the event $\Ac_1$.  Finally, combining the lower bound~\eqref{ineq:lower-bound-mineig}, the equation~\eqref{eq:variational-characterization}, and the lower bound~\eqref{ineq:lower-bound-variational}, we obtain the inequality
\[
\lambda_{\min}(\nabla^2 \bar{L}_n(\bxi; \btsharp) ) \geq c,
\]
on the event $\Ac_1 \cap \Ac_2 \cap \Ac_3$, which occurs with probability at least $1 - 14e^{-cn}$.\qed

\subsubsection{Proof of Lemma~\ref{lem:remove-positive-restriction}}
\label{subsec:proof-lemma-remove-positive-restriction}
Recall the loss function $\Lc$~\eqref{eq:sec_order_gen}:
\[
\Lc(\bt; \btsharp, \bX, \by) = \frac{1}{\sqrt{n}} \| \omega(\bX\btsharp, \by) - \bX\bt \|_2,
\]
which corresponds to setting 
\[
F(\bu, \bt) = \| \omega(\bX\btsharp, \by) - \bu \|_2, \qquad h(\bt, \btsharp) = 0, \qquad \text{ and } \qquad g(\bu, \bX \btsharp; \by) = \| \omega(\bX\btsharp, \by) - \bu \|_2.
\]
Additionally, note that the convex conjugate is given by
\[
g^*(\bv, \bX\btsharp; \by) = \begin{cases}\langle \bv, \omega(\bX\btsharp, \by) \rangle & \text{ if } \| \bv \|_2 \leq \frac{1}{\sqrt{n}},\\
	+\infty & \text{ otherwise.} \end{cases}
\]
Substituting into the definition of the scalarized auxiliary loss $\bar{L}_n$ (see Definition~\ref{def:scalarized-ao}), we obtain
\[
\bar{L}_n(\alpha, \mu, \nu; \btsharp) = \biggl(\frac{1}{\sqrt{n}} \| \perptwo \cdot \bg + \parcomp \cdot \bz_1 + \perpone \cdot \bz_2 - \omega(\bX \btsharp, \by) \|_2 - \perptwo \frac{\| \proj_{S_{\sharp}}^{\perp} \bh \|_2}{\sqrt{n}}\biggr)_{+}.
\]
Now, consider the shorthand
\[
\bq = \parcomp \cdot \bz_1 + \perpone \cdot \bz_2 - \omega(\bX \btsharp, \by),
\]
and define the three events
\[
\Ac_1 = \Bigl\{\frac{1}{n}\lvert \langle \perptwo \cdot \bg, \bq\rangle \rvert \leq \frac{4\perptwo}{5\sqrt{n}}\|\bq\|_2\Bigr\}, \qquad \Ac_2 = \Bigl\{\| \bg \|_2^2 \geq 4n/5\}, \qquad \text{ and } \qquad \Ac_3 = \{\| \bh \|_2^2 \leq 36d/25\}.
\]
Next, apply Bernstein's inequality to bound the quantity $\Pro\{\Ac_1^c\}$, Hoeffding's inequality to bound the quantities $\Pro\{\Ac_2^c\}$ and $\Pro\{\Ac_3\}$, and the union bound to obtain the inequality 
\[\Pro\{\Ac_1 \cap \Ac_2 \cap \Ac_3\} \geq 1 - 6e^{-cn}.
\]
Working on the intersection of these three events, we obtain
\begin{align*}
	\frac{1}{\sqrt{n}} \| \perptwo \cdot \bg + \bq \|_2  &= \sqrt{ \frac{4 \perptwo^2}{5n}\| \bg \|_2^2 + \frac{\perptwo^2}{5n} \| \bg \|_2^2 + \frac{1}{n}\langle \perptwo \cdot \bg, \bq \rangle + \frac{1}{n} \| \bq \|_2^2 }\\
	&\geq \sqrt{ \frac{16 \perptwo^2}{25} + \frac{4\perptwo^2}{25} - \frac{4\perptwo}{5\sqrt{n}}\| \bq \|_2 + \frac{1}{n} \| \bq \|_2^2 } = \sqrt{\frac{16 \perptwo^2}{25}  + \Bigl(\frac{2\perptwo}{5} - \frac{\| \bq \|_2}{\sqrt{n}}\Bigr)^2} \geq \frac{4\perptwo}{5}.
\end{align*}
Thus, we obtain
\[
\frac{1}{\sqrt{n}} \| \perptwo \cdot \bg + \bq \|_2 - \perptwo \frac{\| \proj_{S_{\sharp}}^{\perp} \bh \|_2}{\sqrt{n}} \geq \frac{4\perptwo}{5} - \frac{6\perptwo}{5\sqrt{\kappa}} \geq 0, 
\]
where the last inequality holds for $\kappa \geq C$ with $C$ a large enough constant.  Summarizing, we see that 
\[
\frac{1}{\sqrt{n}} \| \perptwo \cdot \bg + \parcomp \cdot \bz_1 + \perpone \cdot \bz_2 - \omega(\bX \btsharp, \by) \|_2 - \perptwo \frac{\| \proj_{S_{\sharp}}^{\perp} \bh \|_2}{\sqrt{n}} \geq 0,
\]
whence 
\[
\bar{L}_n(\alpha, \mu, \nu; \btsharp)  = \frac{1}{\sqrt{n}} \| \perptwo \cdot \bg + \parcomp \cdot \bz_1 + \perpone \cdot \bz_2 - \omega(\bX \btsharp, \by) \|_2 - \perptwo \frac{\| \proj_{S_{\sharp}}^{\perp} \bh \|_2}{\sqrt{n}}.
\]
\qed

\subsubsection{Proof of Lemma~\ref{lem:row-space-A}}
\label{subsec:proof-lemma-row-space-A}
We begin by introducing the shorthand
\[
\bomega_{\sharp} = \omega(\bX\btsharp, \by).
\]
Now, note the inequality
\begin{align*}
	\frac{1}{n} \| \bA\bxi - \bomega_{\sharp} \|_2^2 &\overset{\1}{\geq} \frac{1}{n} \| (\bI_n - \bA(\bA^{\top}\bA)^{-1}\bA^{\top})\bomega_{\sharp} \|_2^2\\
	&= \frac{1}{n}\| \bomega_{\sharp}\|_2^2 - \frac{1}{n}(\bA\bomega_{\sharp})^{\top}(\bA^{\top} \bA)^{-1} (\bA \bomega_{\sharp}),
\end{align*}
where step $\1$ follows by minimizing the LHS in $\bxi$.  Next, let $0 < c' < 1$ be a small constant and define the event 
\begin{align*}
	\Ac_1 &= \Bigl\{(1 - c') \bI_3 \preceq \frac{1}{n} \bA^{\top} \bA \preceq (1 + c') \bI_3 \Bigr\},
\end{align*}
and note that on the event $\Ac_1$, we further obtain the inequality
\begin{align}
	\label{ineq:row-space-ineq1}
	\frac{1}{n} \| \bA\bxi - \bomega_{\sharp} \|_2^2 \geq \frac{1}{n}\| \bomega_{\sharp}\|_2^2 - \frac{1 + c''}{n^2}\|\bA\bomega_{\sharp}\|_2^2 \overset{\1}{=} \frac{1}{n}\| \bomega_{\sharp}\|_2^2 - \frac{1 + c''}{n^2}\Bigl(\langle \bg, \bomega_{\sharp}\rangle^2 + \langle \bz_1, \bomega_{\sharp}\rangle^2 + \langle \bz_2, \bomega_{\sharp}\rangle^2\Bigr),
\end{align}
where step $\1$ follows by recalling that $\bA\bomega_{\sharp} = [\langle \bg, \bomega_{\sharp} \rangle, \langle \bz_1, \bomega_{\sharp}\rangle, \langle \bz_2, \bomega_{\sharp} \rangle]$
and consider the two events
\begin{align*}
	\Ac_2 = \Bigl\{\frac{1}{n^2}\lvert \langle \bg, \bomega_{\sharp} \rangle \rvert^2 \vee \Bigl\lvert \frac{1}{n^2}\langle \bz_1, \bomega_{\sharp}\rangle^2 - (\EE \{ Z_1 \Omega \})^2\Bigr\rvert \vee \Bigl\lvert \frac{1}{n^2}\langle \bz_2, \bomega_{\sharp} \rangle^2 - (\EE\{Z_2 \Omega \})^2 \Bigr \rvert \leq c'\Bigr\},
\end{align*}
and 
\begin{align*}
	\Ac_3 &= \Bigl\{\Bigl\lvert \frac{1}{n} \| \bomega_{\sharp} \|_2^2 - \EE\{\Omega^2\} \Bigr\rvert \leq c' \Bigr\}.
\end{align*}
%\begin{align*}
%	\Ac_1 &= \Bigl\{\Bigl\lvert \frac{1}{n} \| \bomega_{\sharp} \|_2^2 - \EE\{\Omega^2\} \Bigr\rvert \leq c' \Bigr\}, \qquad 	&&\Ac_2 = \Bigl\{\frac{1}{n^2}\lvert \langle \bg, \bomega_{\sharp} \rangle \rvert^2 \leq c'\Bigr\},\\ 
%	\Ac_3 &= \Bigl\{ \Bigl\lvert \frac{1}{n^2}\langle \bz_1, \bomega_{\sharp}\rangle - (\EE \{ Z_1 \Omega \})^2\Bigr\rvert \leq c'\Bigr\}, \qquad \text{ and } \qquad &&\Ac_4 = \Bigl\{\Bigl\lvert \frac{1}{n^2}\langle \bz_2, \bomega_{\sharp} \rangle - (\EE\{Z_2 \Omega \})^2 \Bigr \rvert \leq c'\Bigr\}.
%\end{align*}
Working on the intersection of the above two events, we further lower bound the RHS of the inequality~\eqref{ineq:row-space-ineq1} to obtain the inequality 
\[
\frac{1}{n} \| \bA\bxi - \bomega_{\sharp} \|_2^2 \geq \EE\{ \Omega^2\} - \EE\{ Z_1 \Omega\}^2 - \EE\{ Z_2 \Omega\}^2 - c'\cdot (1 + 3c'') \overset{\1}{\geq} c > 0,
\]
where step $\1$ follows by Assumption~\ref{ass:omega}.  

The proof is complete upon bounding the probability $\Pro\{\Ac_1 \cap \Ac_2 \cap \Ac_3\}$.  First, we apply~\cite[Theorem 6.1]{wainwright2019high} to control the minimum and maximum singular values of the Wishart matrix $\bA$ in conjunction with the assumption that $n \geq C$ to obtain $\Pro\{\Ac_1\} \geq 1 - 2e^{-cn}$.  Next, recall that by Assumption~\ref{ass:omega}, we have the bound $\| \bomega_{\sharp} \|_{\psi_2} \leq K$.  Thus, we apply Bernstein's inequality to obtain the bound
\[
\Pro\Bigl\{ \Bigl \lvert \frac{1}{n} \langle \bz_1, \bomega_{\sharp} \rangle - \EE\{ Z_1 \Omega\}\Bigr\rvert \geq \frac{c'}{C} \Bigr\} \leq 2e^{-cn}.
\]
Consequently, with probability at least $1 - 2e^{-cn}$,  
\[
\Bigl\lvert\frac{1}{n^2}\langle \bz_1, \bomega_{\sharp}\rangle^2 - (\EE \{ Z_1 \Omega \})^2\Bigr\rvert = \Bigl \lvert \frac{1}{n} \langle \bz_1, \bomega_{\sharp} \rangle - \EE\{ Z_1 \Omega\}\Bigr\rvert \cdot \Bigl \lvert \frac{1}{n} \langle \bz_1, \bomega_{\sharp} \rangle + \EE\{ Z_1 \Omega\}\Bigr\rvert \overset{\1}{\leq} \frac{c'}{3},
\]
where step $\1$ additionally used the fact that $\EE\{Z_1 \Omega\} \leq C$.  Bounding the other terms similarly and applying the union bound, we obtain $\Pro\{\Ac_2\} \geq 1 - 6e^{-cn}$.  Finally, we apply Bernstein's inequality once more to obtain the inequality $\Pro\{ \Ac_3 \} \geq 1 - 2e^{-cn}$.  Putting the pieces together, we obtain the result. \qed

\subsubsection{Proof of Lemma~\ref{lem:minimize-lbar-higher-order}}
\label{subsec:proof-lemma-minimize-lbar}
We note the following characterization
\begin{align}
	\label{eq:tau-characterization}
	\min_{\bxi \in \Pc(\mathbb{B}_2(C) )} \bar{L}_n(\bxi; \btsharp) &= \min_{\bxi \in \Pc(\mathbb{B}_2(C) )} \inf_{\tau > 0}\; \frac{\tau}{2} + \frac{1}{2\tau n} \| \bA \bxi - \omega(\bX \btsharp, \by) \|_2^2 - \langle \bv_n, \bxi \rangle \nonumber \\
	&=  \inf_{\tau > 0}\min_{\bxi \in \Pc(\mathbb{B}_2(C) )}\; \frac{\tau}{2} + \frac{1}{2\tau n} \| \bA \bxi - \omega(\bX \btsharp, \by) \|_2^2 - \langle \bv_n, \bxi \rangle,
\end{align}
where the interchange follows as Lemma~\ref{lem:row-space-A} implies that the infimum over $\tau$ is achieved.  Next, we note that the inner minimization admits the unique minimizer
\[
\bxi_n(\tau) = (\bA^{\top} \bA)^{-1} \bA^{\top} \omega(\bX\btsharp, \by) + \tau \cdot n \cdot (\bA^{\top} \bA)^{-1} \bv_n.
\]
Substituting this value into the RHS of the optimization problem~\eqref{eq:tau-characterization} yields
\begin{align}
	\label{eq:opt-tau}
	\min_{\bxi \in \Pc(\mathbb{B}_2(C) )} \bar{L}_n(\bxi; \btsharp) &= \inf_{\tau > 0} \frac{\tau}{2} + \frac{1}{2\tau n} \| \bA \bxi_n(\tau) - \omega(\bX \btsharp, \by) \|_2^2 - \langle \bv_n, \bxi_n(\tau) \rangle\nonumber\\
	&=\inf_{\tau > 0}\;\frac{1}{2\tau n}\|(\bI_n-\bA(\bA^{\top}\bA)^{-1}\bA^{\top})\omega(\bX \btsharp, \by)\|_2^2 + \frac{\tau}{2}(1-n\cdot\bv_n^{\top}(\bA^{\top}\bA)^{-1}\bv_n)\nonumber\\
	&\qquad\;\;\;-\bv_n^{\top}(\bA^{\top}\bA)^{-1}\bA\omega(\bX \btsharp, \by).
\end{align}
Consider the events
\[
\Ac_1 = \{ \| \bh \|_2^2 \leq 36d/25\} \qquad \text{ and } \qquad \Ac_2 = \Bigl\{(1 - c') \bI_3 \preceq \frac{1}{n} \bA^{\top} \bA \preceq (1 + c') \bI_3 \Bigr\},
\]
where we apply Bernstein's inequality to obtain $\Pro\{\Ac_1\} \geq 1 - 2e^{-cn}$ and apply~\cite[Theorem 6.1]{wainwright2019high} to obtain $\Pro\{\Ac_2\} \geq 1 - 2e^{-cn}$.  On the event $\Ac_1 \cap \Ac_2$, note that 
\[
1 - n\cdot\bv_n^{\top}(\bA^{\top}\bA)^{-1}\bv_n \geq 1 - (1 + c'/2) \| \bv_n \|_2^2 \geq 1 - (1 + c'/2) \cdot \frac{6}{5 \kappa} > 0.
\]
Thus, the optimization problem~\eqref{eq:opt-tau} admits a unique minimizer
\[
\tau_n = \frac{\frac{1}{\sqrt{n}}\|(\bI_n - \bA(\bA^{\top} \bA)^{-1}\bA^{\top})\omega(\bX \btsharp, \by) \|_2}{\sqrt{1 - n\cdot \bv_n^{\top} (\bA^{\top} \bA)^{-1} \bv_n}}.
\]

\subsection{Proof of Lemma~\ref{lem:ao-analysis}: First-order methods}
\label{subsec:proof-ao-analysis-first-order}
In this subsection, we prove Lemma~\ref{lem:ao-analysis}, specialized to first-order methods.  To this end, consider the a first order loss as in equation~\eqref{eq:GD_gen}
\[
\Lc(\bt; \btsharp, \bX, \by) = \frac{1}{2} \| \bt \|_2^2 - \langle \bt, \btsharp \rangle - \frac{2\eta}{n} \sum_{i=1}^{n} \omega(\langle \bx_i, \btsharp \rangle, y_i) \cdot \langle \bx_i, \bt \rangle,
\]
which corresponds to setting
\[
h(\bt, \btsharp) = \frac{1}{2} \| \bt\|_2^2 - \langle \bt, \btsharp \rangle, \qquad \hscal(\parcomp, \perpone, \perptwo) = \frac{1}{2}(\parcomp^2 + \perpone^2 + \perptwo^2) - (\parcomp \parcomp_{\sharp} + \perpone \perpcomp_{\sharp}),
\]
and 
\[
g(\bu, \bX \btsharp; \by) = -\frac{2\eta}{n} \langle \bu, \omega(\bX \btsharp, \by) \rangle.
\]
Note that 
\[
g^*(\bv, \bX\btsharp; \by) = \begin{cases} 0 & \text{ if } \bv = \frac{2\eta}{n}\cdot \omega(\bX\btsharp, \by), \\
	+\infty & \text{ otherwise}.\end{cases}
\]
Consequently, we obtain
\begin{align} \label{eq:Lbar-first-order}
\bar{L}_n(\parcomp, \perpone, \perptwo) = \;&\frac{\parcomp^2 + \perpone^2 + \perptwo^2}{2} - (\parcomp \parcomp_{\sharp} + \perpone \perpcomp_{\sharp}) - \frac{2\eta}{n} \cdot \langle \omega(\bX\btsharp, \by), \perptwo \bg + \parcomp \bz_1 + \perpone \bz_2 \rangle \nonumber\\
&- \frac{2 \eta \perptwo}{n} \cdot \| \proj_{S_{\sharp}}^{\perp} \bh\|_2 \cdot \| \omega(\bX\btsharp, \by) \|_2.
\end{align}
Note that part (b) of the lemma is evident from the expression above, so we focus our attention on part (a) in the next subsection.

\subsubsection{Proof of Lemma~\ref{lem:ao-analysis}(a): First-order methods}
Evidently, $\bar{L}_n$~\eqref{eq:Lbar-first-order} is strongly convex and continuously differentiable.  The optimizers are given by the first order conditions
\begin{subequations}
	\begin{align}\label{eq:first-order-minimizers}
		\parcomp_n &= \parcomp_{\sharp} + \frac{2\eta}{n} \cdot \langle \bz_1, \omega(\bX\btsharp, \by) \rangle \\
		\perpone_n &= \perpcomp_{\sharp} + \frac{2 \eta}{n} \cdot \langle \bz_2, \omega(\bX \btsharp, \by) \rangle \\
		\perptwo_n &= \frac{2\eta}{n} \cdot \langle \bg, \omega(\bX\btsharp, \by) \rangle + \frac{2\eta}{n} \cdot \| \proj_{S_{\sharp}}^{\perp} \bh\|_2 \cdot \| \omega(\bX \btsharp, \by) \|_2.
	\end{align}
\end{subequations}
Now, consider the events
\[
\Ac_1 = \Bigl\{\Bigl \lvert \frac{1}{n} \langle \bg, \omega(\bX \btsharp, \by) \rangle \Bigr \rvert  \vee \Bigl \lvert \frac{1}{n} \langle \bz_1, \omega(\bX \btsharp, \by) \rangle - \EE\{ Z_1 \Omega\} \Bigr \rvert \vee \Bigl \lvert \frac{1}{n} \langle \bz_2, \omega(\bX \btsharp, \by) \rangle - \EE\{ Z_2 \Omega\} \Bigr \rvert  \leq \epsilon \Bigr\},
\]
and 
\[
\Ac_2 = \Bigl\{\Bigl \lvert \frac{1}{\sqrt{n}} \| \proj_{S_{\sharp}}^{\perp} \bh \|_2 - \kappa^{-1/2} \Bigr \rvert \vee \Bigl \lvert \frac{1}{\sqrt{n}} \| \omega(\bX\btsharp, \by) \|_2 - \sqrt{\EE\{\Omega^2\}} \Bigr\rvert \leq \epsilon\}, 
\]
and apply Bernstein's inequality to obtain the bound $\Pro\{\Ac_1 \cap \Ac_2\} \geq 1 - 10e^{-cn\epsilon^2}$.  Consequently, on the event $\Ac_1 \cap \Ac_2$, we obtain 
\[
\Pro\{ \| [\parcomp_n, \perpone_n, \perptwo_n] - [\parcomp^{\gor}, \perpone^{\gor}, \perptwo^{\gor}]\|_{\infty} \leq C\epsilon\} \geq 1 - 20e^{-cn\epsilon^2}
\]
Additionally, substitute the empirical minimizers~\eqref{eq:first-order-minimizers} into the loss $\bar{L}_n$~\eqref{eq:Lbar-first-order} to obtain
\[
\bar{L}_n(\parcomp_n, \perpone_n, \perptwo_n) =\; - \frac{1}{2}\cdot (\parcomp_n^2 + \perpone_n^2 + \perptwo_n^2).
\]
Now, define the constant
\[
\bar{L} = - \frac{1}{2}\cdot ((\parcomp^{\gor})^2 + (\perpone^{\gor})^2 + (\perptwo^{\gor})^2),
\]
and note that on the event $\Ac_1 \cap \Ac_2$, we obtain
\[
\lvert \bar{L}_n(\parcomp_n, \perpone_n, \perptwo_n) - \bar{L}\rvert \leq \frac{\epsilon}{2}\Bigl(\lvert \parcomp_n + \parcomp^{\gor} \rvert + \lvert \perpone_n + \perpone^{\gor} \rvert + \lvert \perptwo_n + \perptwo^{\gor} \rvert \Bigr) \leq C\epsilon.
\]
This completes the proof. \qed

==> sections/gordon/gordon-alt/gordon-alt2-backup-Sep1.tex <==
%!TEX root = ../../../convergence-gordon.tex

In this section, we prove part (a) of both Theorem~\ref{thm:one_step_main_HO} and Theorem~\ref{thm:one_step_main_FO}. The structure of the proof follows the recipe sketched in Section~\ref{sec:heuristic}. We proceed by carrying out steps 1--3 of the recipe for a broader class of algorithms (captured by one-step updates satisfying Assumption~\ref{ass:loss} to follow), and derive a general Proposition~\ref{prop:first-three-steps}. With this proposition in hand, we then carry out step 4 of the recipe for higher-order methods in Section~\ref{sec:growth-HO} to prove Theorem~\ref{thm:one_step_main_HO}(a) and for first-order methods in Section~\ref{sec:growth-FO} to prove Theorem~\ref{thm:one_step_main_FO}(a).

%is dedicated to a more general proposition that immediately implies Theorem~\ref{thm:one_step_main}(a), as well as weaker version of part (b). In the next section, we present the sharper analysis that leads to part (b) of the theorem. In 


Throughout this section, we let $\bt^{\sharp}$ denote the ``current'' iterate of the algorithm, with $(\parcomp^{\sharp}, \perpcomp^{\sharp}) = (\parcomp(\btsharp), \perpcomp(\btsharp))$. This frees up the tuple $(\bt, \parcomp, \perpcomp)$ to denote decision variables that will be used throughout the proof.  In addition, as in the heuristic derivation in Section~\ref{subsec:heuristic-second-order}, it is useful in the proof to track a three dimensional state evolution $(\parcomp, \perpone, \perptwo)$, where
\begin{align}
	\label{eq:gordon-3D-state}
\parcomp = \langle \bt, \thetastar \rangle, \qquad \perpone = \frac{\langle \bt, \proj_{\thetastar}^{\perp}\btsharp\rangle}{\| \proj_{\thetastar}^{\perp}\btsharp \|_2}, \qquad \text{and}\qquad \perptwo = \| \proj_{S_\#}^{\perp} \bt \|_2, 
\end{align}
where $S_{\#} = \mathsf{span}(\thetastar, \btsharp)$ and $\proj^\perp_{S_\#}$ is the projection matrix onto the orthogonal complement of this subspace.
Finally, define the independent random variables
\begin{align} \label{eq:zone-ztwo}
\bz_1  = \bX\btstar \qquad \text{ and } \qquad \bz_2 = \frac{\bX\proj_{\btstar}^{\perp} \btsharp}{\| \bX\proj_{\btstar}^{\perp} \btsharp \|_2},
\end{align}
noting that both $\bz_1, \bz_2 \sim \mathsf{N}(0, \bI_n)$ since $\| \btstar \|_2 = 1$. 
We are now ready to rigorously implement each step of the recipe.

\subsection{General result from steps 1--3 of recipe}
%
%
Our general result is derived by implementing steps 1--3 in a setting involving a general decomposability assumption on the one-step loss function $\mathcal{L}$~\eqref{eq:gordon_one_step}. 
%Our goal is to show that the minimum over $\mathcal{L}$ is approximately equal to the minimum over a suitably defined loss

\subsubsection{Implementing step 1: One-step convex optimization} 

Our general assumption takes the following form: \apcomment{Notation $g,h$ for functions is not related to $\bg, \bh$. Could be confusing.}
\begin{assumption}[Decomposability and convexity of loss]\label{ass:loss}
	Consider a fixed vector $\bt^{\sharp} \in \mathbb{R}^d$ and a Gaussian random matrix $\bX \in \mathbb{R}^{n \times d}$ and assume $\by$ is generated, given $\bX$ and $\btstar$, according to the generative model~\eqref{eq:model}.  Then each step of the iterative algorithm can be written in the form~\eqref{eq:opt_gen_intro}, where the loss
	\[
	\Lc(\bt):={\mathcal{L}(\bt; \bt^{\sharp}, \bd{X}, \bd{y})}
	\]
	satisfies the following properties:
	\begin{enumerate}[label=(\alph*)]
		\item There is a pair of functions $g: \mathbb{R}^n \times \mathbb{R}^n \rightarrow \mathbb{R}$ and $h: \mathbb{R}^d \times \mathbb{R}^d \rightarrow \mathbb{R}$, and a (random) function
		\begin{align}
			\label{eq:Fc}
			F : \mathbb{R}^{n} \times \mathbb{R}^{d} &\rightarrow \mathbb{R} \nonumber\\
			F(\bu, \bt) &\mapsto g(\bu, \bX \bt^{\sharp}; \by) + h(\bt, \bt^{\sharp}),
		\end{align}	
		such that
		\begin{align*}
		\Lc(\bt) = F(\bX \bt, \bt) \qquad \text{ for all } \bt \in \real^d.
		\end{align*}
		
		\item The functions $g$ and $h$ are convex in their first arguments.  Moreover, the function $F$ is $C_L/\sqrt{n}$-Lipschitz in its first argument.
		
		\item The function $h$ depends on $\bt$ only through its lower dimensional projections.  That is, there exists a function
		\begin{align*}
			\hscal: \mathbb{R}^3 \times \mathbb{R}^d &\rightarrow \mathbb{R}\\
			(\alpha, \mu, \nu), \bt^{\sharp} & \mapsto \hscal((\alpha, \mu, \nu), \bt^{\sharp}),
		\end{align*}
		such that 
		\[
		h(\bt, \bt') = \hscal\biggl(\langle \bt, \btstar\rangle, \frac{\langle \bt, \proj_{\btstar}^{\perp} \bt'\rangle}{\| \proj_{\btstar}^{\perp} \bt'\|_2}, \| \proj_{\mathsf{span}(\btstar, \bt')}^{\perp} \bt \|_2, \bt'
		\biggr)
		\]
		
		\item $\Lc(\bt)$ is coercive.  That is, $\Lc(\bt) \rightarrow \infty$ whenever $ \| \bt \|_2 \rightarrow \infty$.
	\end{enumerate}
\end{assumption}
%Note that these assumptions encapsulate a set of loss functions more general than those we are interested in.  For instance, s
Note that specifying
\begin{align*}
h(\bt, \bt^{\sharp}) = 0 \qquad  \text{ and } \qquad g(\bu, \bX \bt^{\sharp}; \by) = \frac{1}{\sqrt{n}}\| \omega(\bX \bt^{\sharp}, \by) - \ub  \|_2
\end{align*} 
recovers the higher-order loss functions~\eqref{eq:sec_order_gen}, whereas specifying 
\begin{align*}
h(\bt, \btsharp) = 1/2 \| \bt \|_2^2 - \langle \bt, \btsharp \rangle \qquad  \text{ and } \qquad g(\bu, \bX\btsharp; \by) = -2\eta/n \langle \bu, \omega(\bX \bt^{\sharp}, \by) \rangle
\end{align*}
recovers the first-order loss functions~\eqref{eq:GD_gen}.  The remaining properties (b)-(d) of the assumption can be straightforwardly verified for these two choices. Thus, Assumption~\ref{ass:loss} captures both the special cases corresponding to Theorems~\ref{thm:one_step_main_HO} and~\ref{thm:one_step_main_FO}. Having written one step of the iterative algorithm of interest as a minimization of a convex loss, we are now ready to proceed to step 2 of the recipe.

\subsubsection{Implementing step 2: The auxiliary optimization problem} 
Next, we state a formal definition of the auxiliary loss function $\mathfrak{L}_n$.
% and $\widebar{L}_n$ 
%from Section~\ref{sec:heuristic}.  %First, we define the auxiliary loss function.
\begin{definition}[Auxiliary loss]
\label{def:aux-gordon-loss}
Let $\bg \sim \mathsf{N}(0, \bI_n)$ and $\bh \sim \mathsf{N}(0, \bI_d)$ denote independent random vectors drawn independently of the pair $(\bX, \by)$, let $\btsharp \in \mathbb{R}^d$ denote an arbitrary vector and define the subspace $S_{\sharp} = \mathsf{span}(\btstar, \btsharp)$.  Further, let $\mathcal{L}$ denote an arbitrary loss function which satisfies Assumption~\ref{ass:loss} for functions $g$ and $h$.  Then, given a positive scalar $C_n$, %(which may scale with $n$), 
define the auxiliary loss function
\begin{align*}
%	\label{eq:intermediate-loss}
	\mathfrak{L}_n(\bt, \bu; C_n) := \max_{\bv \in \mathbb{B}_2(C_n)}\;\frac{1}{\sqrt{n}} \| \bv \|_2 \langle \proj_{S_{\sharp}}^{\perp} \bt, \bh \rangle + h(\bt, \bt^{\sharp}) + g(\bu, \bX \bt^{\sharp}; \by)  + \frac{1}{\sqrt{n}}\langle \bv, \bX \proj_{S_{\sharp}} \bt  + \| \proj_{S_{\sharp}}^{\perp} \bt \|_2 \bg - \bu\rangle.
\end{align*}
\end{definition}
The following lemma shows that our original optimization problem over the loss function $\mathcal{L}$ is essentially equivalent to an auxiliary optimization problem involving the loss $\mathfrak{L}_n$. 
\begin{lemma}
	\label{lem:bilinear}
	Let $\btsharp \in \mathbb{R}^d$, suppose that the loss function $\Lc(\bt; \btsharp, \bX, \by)$ satisfies Assumption~\ref{ass:loss}.  There exist universal positive constants $c, C, C'$ as well as a constant $C_n < \infty$ (which may scale with the sample size $n$), such that %with the auxiliary loss $\mathfrak{L}_n(\cdot, \cdot; C_n)$ from Definition~\ref{def:aux-gordon-loss}, 
	the following holds.  For any constant $C_1 \geq C$ and closed subset $D \subseteq \mathbb{B}_2(C_1)$, we have
		\[
		\Pro\Bigl\{ \min_{\bt \in D} \Lc(\bt) \geq t\Bigr\} \leq 2\Pro\Bigl\{\min_{\bt \in D, \bu \in \mathbb{B}_2(C') } \mathfrak{L}_n(\bt, \bu; C_n) \leq t\Bigr\} + Ce^{-cn}.
		\]
		If, in addition, $D$ is convex, then
		\[
		\Pro\Bigl\{\min_{\bt \in D} \mathcal{L}(\bt) \geq t\Bigr\} \leq 2\Pro\Bigl\{\min_{\bt \in D, \bu \in \mathbb{B}_2(C') } \mathfrak{L}_n(\bt, \bu; C_n) \geq t\Bigr\} + Ce^{-cn}.
		\]
\end{lemma}
\kaccomment{The constant $C$ can be made explicit in all three lemmas.} \apcomment{Quantifiers here are confusing to me. Check comment after Lemma 5.} The proof of this lemma can be found in Subsection~\ref{subsec:proof-of-bilinear}, and involves the application of the CGMT (Proposition~\ref{thm:gordon}). Given that the minimization over $\mathcal{L}$ can be approximately written as a minimization over an auxiliary loss, we are now ready to proceed to step 3.


\subsubsection{Implementing step 3: Scalarization} 
Next, we define the scalarized auxiliary loss. Recall the definition of the convex conjugate of a function $g: \real^d \to \real$, given by $g^*(\bx) = \sup_{\bx' \in \real^d}\; \inprod{\bx'}{\bx} - g(\bx')$.
\begin{definition}[Scalarized auxiliary loss]
	Let $\bg \sim \mathsf{N}(0, \bI_n)$, $\bh \sim \mathsf{N}(0, \bI_d)$, $\bz_1 \sim \mathsf{N}(0, \bI_n)$, and $\bz_2 \sim \mathsf{N}(0, \bI_n)$ denote mutually independent random vectors, with the pair $(\bz_1, \bz_2)$ chosen according to equation~\eqref{eq:zone-ztwo}. Let $\btsharp \in \mathbb{R}^d$ denote an arbitrary vector and define the subspace $S_{\sharp} = \mathsf{span}(\btstar, \btsharp)$.  Further, let $\mathcal{L}$ denote an arbitrary loss function that satisfies Assumption~\ref{ass:loss} for functions $g$ and $h$. Associate with it the following \emph{scalarized auxiliary loss}
	\label{def:scalarized-ao}
	\[
	\widebar{L}_n(\alpha, \mu, \nu; \btsharp) := \max_{\bv \in \mathbb{B}_2(C)} \hscal(\alpha, \mu, \nu, \btsharp) - g^{*}(\bv, \bX \btsharp; \by) - \nu \| \proj_{S_{\sharp}}^{\perp}\bh\|_2 \| \bv \|_2 + \langle \nu \bg + \alpha \bz_1 + \mu \bz_2, \bv \rangle,
	\]
	where $g^*$ denotes the convex conjugate of the function $g$ and $\hscal$ is as in part (c) of Assumption~\ref{ass:loss}.
\end{definition}
Our next lemma implements step 3, scalarizing the auxiliary loss $\mathfrak{L}_n$.  Before stating the lemma, we require the definition of a scalarized set. 
%\begin{definition}[Scalarized auxiliary loss]
%	Let $\bg \sim \mathsf{N}(0, \bI_n)$, $\bh \sim \mathsf{N}(0, \bI_d)$, $\bz_1 \sim \mathsf{N}(0, \bI_n)$, and $\bz_2 \sim \mathsf{N}(0, \bI_n)$ be independent random vectors, $\btsharp \in \mathbb{R}^d$ an arbitrary vector and let the subspace $S_{\sharp} = \mathsf{span}(\btstar, \btsharp)$.  Further, let $\mathcal{L}$ denote an arbitrary loss function which satisfies Assumption~\ref{ass:loss} for functions $g$ and $h$ and associate with it the following \emph{scalarized auxiliary loss}
%	\label{def:scalarized-ao}
%	\[
%	\widebar{L}_n(\alpha, \mu, \nu; \btsharp) := \max_{\bv \in \mathbb{B}_2(C)} \hscal(\alpha, \mu, \nu, \btsharp) - g^{*}(\bv, \bX \btsharp; \by) - \nu \| \proj_{S_{\sharp}}^{\perp}\bh\|_2 \| \bv \|_2 + \langle \nu \bg + \alpha \bz_1 + \mu \bz_2, \bv \rangle,
%	\]
%	where $g^*$ denotes the convex conjugate of the function $g$ and $\hscal$ is as in part (c) of Assumption~\ref{ass:loss}.
%\end{definition}
\begin{definition}[Scalarized set]
	\label{def:scalarized-set}
Let $\btstar \in \mathbb{R}^d$ denote the ground truth, $\btsharp \in \mathbb{R}^d$ an arbitrary vector, and $S_{\sharp}$ the subspace $S_{\sharp} = \mathsf{span}(\btstar, \btsharp)$.  For any subset $D \subseteq \mathbb{R}^d$, define the scalarized set
	\[
\Pc(D) := \biggl\{(\alpha, \mu, \nu) \in \mathbb{R}^3: \bt \in D \text{ and } \alpha = \langle \bt, \btstar \rangle, \mu = \frac{\langle \bt, \proj_{\btstar}^{\perp}\bt^{\sharp}\rangle}{\| \proj_{\btstar}^{\perp} \bt^{\sharp}\|_2}, \nu = \| \proj_{S_{\sharp}}^{\perp} \bt \|_2\biggr\}.
\]
A \emph{product} scalarized set is one that can be written as the product $S_1 \times S_2 \times S_3$, where $S_1, S_2, S_3$ are open subsets of the real line $\mathbb{R}$.
\end{definition}

\iffalse
\begin{definition}[Deviation set]
Define the deviation set
\begin{align}
	\label{eq:deviation-set}
	D_{\epsilon} := \{\bt \in \mathbb{R}^d: \max\Bigl(\lvert \langle \bt, \btstar \rangle - \alpha^{\gor} \rvert, \Bigl\lvert \frac{\langle \bt, \proj_{\btstar}^{\perp}\bt^{\sharp}\rangle}{\| \proj_{\btstar}^{\perp} \bt^{\sharp}\|_2} - \mu^{\gor} \Bigr\rvert, \lvert \| \proj_{S_{\sharp}}^{\perp} \bt \|_2 - \nu^{\gor} \rvert \Bigr) \geq \epsilon\}.
\end{align}
\end{definition}
\fi

We have the following lemma, whose proof we provide in Subsection~\ref{subsec:proof-scalarize-ao}.
\begin{lemma}
	\label{lem:scalarize-ao}
	Under the setting of Lemma~\ref{lem:bilinear}, let the scalarized auxiliary loss $\widebar{L}_n$ be as in Definition~\ref{def:scalarized-ao}.  Also suppose that $D = \bar{D} \cap \mathbb{B}_2(C)$ is any set in $\mathbb{R}^d$ such that $\mathcal{P}(\bar{D})$ is a product scalarized set and $C$ is a nonnegative scalar.
%
%	Then, recalling the deviation set $D_{\epsilon}$~\eqref{eq:deviation-set}, there exists a universal positive constant $C$ such that for all constants $C_1 \geq C$ and for sets $D$ of the form
%	\[
%	(i.) \;\; D = \mathbb{B}_2(C_1) \qquad \text{ or } \qquad (ii.) \;\; D = D(\epsilon) \cap \mathbb{B}_2(C_1),
%	\]
%	the following holds. 
Then
	\[
	\min_{ \substack{\bt \in D \\ \bu \in \mathbb{B}_2(C_u \sqrt{n})}}\; \mathfrak{L}_n(\bt, \bu) \;= \min_{(\alpha, \mu, \nu) \in \Pc(D)} \widebar{L}_n(\alpha, \mu, \nu; \btsharp)
	\]
	with probability at least $1 - Ce^{-cn}$.
\end{lemma}
%Having (approximately) scalarized the problem, we are now ready to proceed to our final step of showing growth properties of the function $\widebar{L}_n$.

\ct{We went from $C'$ in Lemma 1 to $C_u\sqrt{n}$ here. }

\subsubsection{Putting together steps 1--3}

We are now in a position to put the pieces together and prove a formal equivalence between the original minimization problem over the loss $\mathcal{L}$ and a low-dimensional minimization problem over the loss $\widebar{L}_n$.
\begin{proposition} \label{prop:first-three-steps}
For each set $\bar{D} \subseteq \real^d$ such that $\mathcal{P}(\bar{D})$ is product scalarized, and scalars $\mathsf{L}$ and $C', \epsilon' > 0$, we have
\begin{align*}
\Pro\Bigl\{\argmin_{\bt \in \mathbb{B}_2(C')} \mathcal{L}(\bt) \in \bar{D} \Bigr\} &\leq 2 \Pro\Bigl\{\min_{(\alpha, \mu, \nu) \in \Pc( \bar{D} \cap \mathbb{B}_2(C'))}\widebar{L}_n(\alpha, \mu, \nu) \leq \mathsf{L} + 2\epsilon' \Bigr\} \\
&\quad  + 2 \Pro\Bigl\{\min_{(\alpha, \mu, \nu) \in \Pc(\mathbb{B}_2(C'))} \widebar{L}_n(\alpha, \mu, \nu) > \mathsf{L} + \epsilon' \Bigr\} + 8 e^{-n/2}.
\end{align*}
\apcomment{Constants in exponential are placeholders.}
\end{proposition}
\begin{proof}
%
Applying the law of total probability, we obtain 
\begin{align}
	\Pro\Bigl\{\argmin_{\bt \in \mathbb{B}_2(C')} \mathcal{L}(\bt) \in \bar{D} \Bigr\} &\leq \Pro\Bigl\{\min_{\bt \in \bar{D} \cap \mathbb{B}_2(C')} \mathcal{L}(\bt) \leq \min_{\bt \in \mathbb{B}_2(C')} \mathcal{L}(\bt) + \epsilon' \Bigr\}\nonumber\\
	&\leq \Pro\Bigl\{\min_{\bt \in \bar{D} \cap \mathbb{B}_2(C')} \mathcal{L}(\bt) \leq \mathsf{L} + 2\epsilon'\Bigr\} + \Pro\Bigl\{\min_{\bt \in \mathbb{B}_2(C')} \mathcal{L}(\bt) > \mathsf{L} + \epsilon' \Bigr\}. \label{ineq:step1-prop-gor}
\end{align}
Now, we apply Lemma~\ref{lem:bilinear}, \apcomment{$C_u$ stuff.} which yields the pair of inequalities
\begin{subequations}\label{ineq:step2-prop-gor}
\begin{align}
	\Pro\Bigl\{\min_{\bt \in \bar{D} \cap \mathbb{B}_2(C')} \mathcal{L}(\bt) \leq \mathsf{L} + 2\epsilon' \Bigr\} &\leq 2\Pro\Biggl\{\min_{\substack{\bt \in \bar{D} \cap \mathbb{B}_2(C'),\\ \bu \in \mathbb{B}_2(C_u\sqrt{n})}}\mathfrak{L}_n(\bt, \bu) \leq \mathsf{L} + 2\epsilon' \Biggr\} + 2e^{-cn},\\
	\Pro\Bigl\{\min_{\bt \in \cap \mathbb{B}_2(C')} \mathcal{L}(\bt) > \mathsf{L} + \epsilon' \Bigr\} &\leq 2\Pro\Biggl\{\min_{\substack{\bt \in  \mathbb{B}_2(C'),\\ \bu \in \mathbb{B}_2(C_u\sqrt{n})}}\mathfrak{L}_n(\bt, \bu) > \mathsf{L} + \epsilon' \Biggr\} + 2e^{-cn}.
\end{align}
\end{subequations}
Subsequently, noting that $\mathcal{P}(\bar{D})$ is a product scalarized set and applying Lemma~\ref{lem:scalarize-ao} yields
\begin{subequations}\label{ineq:step3-prop-gor}
	\begin{align}
		\Pro\Biggl\{\min_{\substack{\bt \in \bar{D} \cap \mathbb{B}_2(C'),\\ \bu \in \mathbb{B}_2(C_u\sqrt{n})}}\mathfrak{L}_n(\bt, \bu) \leq \mathsf{L} + 2\epsilon' \Biggr\} &\leq \Pro\Bigl\{\min_{(\alpha, \mu, \nu) \in \Pc(\bar{D} \cap \mathbb{B}_2(C'))}\widebar{L}_n(\alpha, \mu, \nu) \leq \mathsf{L} + 2\epsilon' \Bigr\} + 2e^{-cn},\\
		\Pro\Biggl\{\min_{\substack{\bt \in  \mathbb{B}_2(C'),\\ \bu \in \mathbb{B}_2(C_u\sqrt{n})}}\mathfrak{L}_n(\bt, \bu) > \mathsf{L} + \epsilon' \Biggr\} &\leq \Pro\Bigl\{\min_{(\alpha, \mu, \nu) \in \Pc(\mathbb{B}_2(C'))} \widebar{L}_n(\alpha, \mu, \nu) > \mathsf{L} + \epsilon' \Bigr\} + 2e^{-Cn}. 
	\end{align}
\end{subequations}
Putting together equations~\eqref{ineq:step1-prop-gor}--\eqref{ineq:step3-prop-gor} completes the proof.
\end{proof}
Having established steps 1--3 of the recipe under the general Assumption~\ref{ass:loss} on the one-step loss function, we now carry out step 4 of the recipe individually for each theorem. For clarity, we include a schematic diagram of the various ingredients in Figure~\ref{fig:gordon-schematic}. 

\begin{figure}[!htbp]
	\centering
	\input{figs/gordon-proof-fig.tex}
	\caption{Schematic diagram of the proof of Proposition~\ref{prop:gordon}, drawn for $\bt \in \mathbb{R}^3$.  The green curve denotes the original loss function $\Lc$, which admits the empirical update $\mathcal{T}_n(\btsharp)$ as its unique minimizer.  The black curve denotes the scalarized auxiliary loss $\widebar{L}_n$ (see Definition~\ref{def:scalarized-ao}), which is strongly convex by Lemma~\ref{lem:ao-analysis}(b).  Its unique minimizer is the quantity $\bxi_n$.  The purple curve is the loss $\bar{L}$ which is the population loss corresponding to the empirical loss $\widebar{L}_n$.  Its unique minimizer is the quantity $\bxi^{\gor}$.  Further, Lemma~\ref{lem:ao-analysis}(a) shows that $\bxi^{\gor}$ and $\bxi_n$ are at a distance of at most $C\epsilon^2$ from each other.  Lemmas~\ref{lem:bilinear} and~\ref{lem:scalarize-ao} show that the minima, over the sets $D = \mathbb{B}_{\infty}(\bxi^{\gor}; \epsilon)$ and $D = \mathbb{B}_2(C_1)$, of the loss $\Lc$ are the same as those of the loss $\widebar{L}_n$.}
	\label{fig:gordon-schematic}
\end{figure}

\subsection{Proof of Theorem~\ref{thm:one_step_main_HO}(a)}

%Given Proposition XXX, the only remaining task is to implement step 4 and combine the pieces. Before, doing so, 
First, let us define the following expanded Gordon state evolution update for higher-order methods.

\begin{definition}[Expanded Gordon state evolution update: Higher-order methods] \label{def:expanded-gordon-HO}
Recall the model~\eqref{eq:model}, and let $Q$ denote a random variable drawn from the latent variable distribution $\mathbb{Q}$. Suppose that the loss function $\Lc$ takes the form~\eqref{eq:sec_order_gen}. Let $(Z_1, Z_2, Z_3)$ denote a triplet of independent standard Gaussian random variables and let $\alpha^{\sharp} \in \mathbb{R}$ and $\beta^{\sharp} \in \mathbb{R}_{\geq 0}$ denote arbitrary scalars.  Let
\[
\Omega = \omega\big(\parcomp^{\sharp} Z_1 +\perpcomp^{\sharp} Z_2\,,\,f(Z_1; Q)+\noisestd Z_3 \big).
\]
Then define the scalars
\[
\alpha^{\gor} = \EE [ Z_1 \Omega], \qquad \mu^{\gor} = \EE[Z_2 \Omega], \qquad \text{ and } \qquad \nu^{\gor} = \sqrt{\frac{\EE[\Omega^2] - (\EE[Z_1 \Omega])^2 - (\EE[Z_2 \Omega])^2}{\kappa - 1}}.
\]
\end{definition}

With this definition in hand, note that in order to prove Theorem~\ref{thm:one_step_main_HO}(a) it suffices to show that for a parameter $c_K$ depending only on the pair $(K_1, K_2)$ in Assumptions~\ref{ass:omega} and~\ref{ass:omega-lb}, we have
\begin{align} \label{eq:equiv-thm1a}
\Pro \left\{ \max \left( \left| \frac{\inprod{\mathcal{T}_n(\btsharp)}{\proj^{\perp}_{\thetastar} \btsharp}}{ \| \proj^{\perp}_{\thetastar} \btsharp \|_2} - \perpone^{\gor} \right|, \left| \| \proj^{\perp}_{S_{\#}} \mathcal{T}_n(\btsharp) \|_2 - \perptwo^{\gor} \right| \right) > \epsilon \right\} \leq C \exp \left( -c_K n \epsilon^4 \right).
\end{align}
%for each $\epsilon \geq n^{-1/4}$. 
%
Indeed, setting $\epsilon = \epsilon_0 := \left( \frac{\log (C/\delta)}{c_K \cdot n} \right)^{1/4}$, we have
\begin{align*}
\Pro \left\{ \max \left( \left| \frac{\inprod{\mathcal{T}_n(\btsharp)}{\proj^{\perp}_{\thetastar} \btsharp}}{ \| \proj^{\perp}_{\thetastar} \btsharp \|_2} - \perpone^{\gor} \right|, \left| \| \proj^{\perp}_{S_{\#}} \mathcal{T}_n(\btsharp) \|_2 - \perptwo^{\gor} \right| \right) > \epsilon_0 \right\} \leq \delta.
\end{align*}
Note that $(\perpcomp^+)^2 = \frac{\inprod{\mathcal{T}_n(\btsharp)}{\proj^{\perp}_{\thetastar} \btsharp}^2}{ \| \proj^{\perp}_{\thetastar} \btsharp \|^2_2} + \| \proj^{\perp}_{S_{\#}} \mathcal{T}_n(\btsharp) \|_2^2$ and $(\perpcompgordon)^2 = (\perpone^{\gor})^2 + (\perptwo^\gor)^2$. Applying the triangle inequality and adjusting constant factors, we have $\Pro( |\beta^+ - \beta^\gor| \geq c \epsilon_0) \leq \delta$, as desired. Consequently, we dedicate our effort toward establishing inequality~\eqref{eq:equiv-thm1a}.

\subsubsection{Implementing step 4: Growth properties of $\widebar{L}_n$} 
The following lemma guarantees growth conditions on the function $\widebar{L}_n$ when the one-step loss function takes the form~\eqref{eq:sec_order_gen}.  
%We provide the proof for higher-order methods in Subsection~\ref{subsec:proof-ao-analysis-higher-order} and the proof for first-order methods in Subsection~\ref{subsec:proof-ao-analysis-first-order}.

\begin{lemma}
	\label{lem:ao-analysis}
	Suppose that the loss function $\mathcal{L}$ can be written in the form %~\eqref{eq:GD_gen} or
	\eqref{eq:sec_order_gen} and let the scalarized auxiliary loss $\widebar{L}_n$ be as in Definition~\ref{def:scalarized-ao}.  Define the constant 
	\[
	\bar{\mathsf{L}} =  \sqrt{\Bigl(1 - \frac{1}{\delta}\Bigr)\Bigl(\EE[\Omega^2] - (\EE[Z_1 \Omega])^2 - (\EE[Z_2 \Omega])^2\Bigr)},
	\]
	and let the tuple $(\parcompgordon, \perpone^{\gor}, \perptwo^{\gor})$ be as in Definition~\ref{def:expanded-gordon-HO}.
	Suppose that Assumptions~\ref{ass:omega} and~\ref{ass:omega-lb} hold with parameters $K_1$ and~$K_2$, respectively.
	Then, there exist parameters $(c_{K_1}, C_{K_2}) > 0$ depending only on $K_1$ and $K_2$ respectively, and universal positive constants $c, C, C_1, C_2$  such that for all $\kappa \geq C_1$, the following hold:
		\begin{enumerate}[label=(\alph*)]
		\item The minimizer
		\[
		(\alpha_n, \mu_n, \nu_n) = \argmin_{(\alpha, \mu, \nu) \in \Pc(\mathbb{B}_2(C_2))} \widebar{L}_n(\alpha, \mu, \nu) 
		\]
		is unique and satisfies both
		\[
		\max\bigl\{\lvert \alpha_n - \alpha^{\gor} \rvert, \lvert \mu_n - \mu^{\gor} \rvert, \lvert \nu_n - \nu^{\gor}\rvert\bigr\} \leq \epsilon,
		\]
		and 
		\[
		\biggl \lvert \widebar{L}_n^{\mathsf{so}}(\alpha_n, \mu_n, \nu_n) - \bar{\mathsf{L}} \biggr \rvert \leq \epsilon,
		\]
		with probability at least $1 - C \exp \{ -c_{K_1} \cdot n\epsilon^2 \} - Ce^{-cn}$.
		\item The scalarized auxiliary loss $\widebar{L}_n$ is $C_{K_2}$-strongly convex on the domain $\mathbb{B}_2(C_2)$ with probability at least $1 - Ce^{-cn}$.
%		
%		The following strong convexity property holds for the function $\widebar{L}_n$
%		\[
%		\min_{\|(\alpha, \mu, \nu) - (\alpha_n, \mu_n, \nu_n)\|_2 \geq \epsilon} \widebar{L}_n(\alpha, \mu, \nu) \geq \widebar{L}_n(\alpha_n, \mu_n, \nu_n) + C_{\mathsf{sc}}\epsilon^2,
%		\]
%		with probability at least $1 - Ce^{-Cn\epsilon^2}$.
	\end{enumerate}
\end{lemma}
With each of the individual steps of the recipe completed, we can now put everything together to prove equation~\eqref{eq:equiv-thm1a}.

\subsubsection{Combining the pieces} 

Let the tuple $(\parcompgordon, \perpone^{\gor}, \perptwo^{\gor})$ be as in Definition~\ref{def:expanded-gordon-HO}. For each nonnegative scalar $\epsilon$, define the deviation set
\begin{align}
	\label{eq:deviation-set}
	D_{\epsilon} := \{\bt \in \mathbb{R}^d: \max\Bigl(\lvert \langle \bt, \btstar \rangle - \alpha^{\gor} \rvert, \Bigl\lvert \frac{\langle \bt, \proj_{\btstar}^{\perp}\bt^{\sharp}\rangle}{\| \proj_{\btstar}^{\perp} \bt^{\sharp}\|_2} - \mu^{\gor} \Bigr\rvert, \lvert \| \proj_{S_{\sharp}}^{\perp} \bt \|_2 - \nu^{\gor} \rvert \Bigr) \geq \epsilon\}.
\end{align}
Note that it suffices to bound $\Pro\{\mathcal{T}_n (\btsharp) \in D_\epsilon \}$.
\iffalse
We begin by introducing the convenient shorthand \apcomment{Not used here.}
\[
\bxi = [\parcomp, \perpone, \perptwo] \qquad \text{ and } \qquad \bxi^{\gor} = [\parcomp^{\gor}, \perpone^{\gor}, \perptwo^{\gor}].
\]
Note that our goal is to upper bound the probability
$\Pro\{\mathcal{T}_n(\btsharp) \in D_{\epsilon}\}$.
\fi
%The strategy is to implement the high-level steps outlined in Subsection~\ref{sec:high-level-steps}.  To this end, we state a sequence of lemmas, each of which implements a subset of these steps.  Our first lemma implements steps 1 and 2, showing an equivalence between our original optimization over the loss function $\mathcal{L}$ to an auxiliary optimization $\mathfrak{L}_n$.  
%
%  
%
%
%
%We take these lemmas as given and continue with the proof.   
%Now, recall the deviation set $D_{\epsilon}$~\eqref{eq:deviation-set} and 
We have
\begin{align*}
	\Pro\{\mathcal{T}_n(\btsharp) \in D_{\epsilon} \} = \Pro\Bigl\{\argmin_{\bt \in \mathbb{R}^d} \mathcal{L}(\bt) \in D_{\epsilon}\Bigr\} \overset{\1}{=} \Pro\Bigl\{\argmin_{\bt \in \mathbb{B}_2(C')} \mathcal{L}(\bt) \in D_{\epsilon}\Bigr\} + Ce^{-cn},
\end{align*}
where step $\1$ occurs ... \kaccomment{This needs to be proved somewhere here! I forgot to include the proof.  In the same part where we do this, we need to verify Assumption~\ref{ass:loss} for the two methods considered.}
With $C_{K_2}$ and $C_1$ as defined in Lemma~\ref{lem:ao-analysis}, fix $\epsilon > C_1/\sqrt{n}$ and define the events
\begin{align*}
\mathcal{A}_1 = \Bigl\{\max\bigl\{\lvert \alpha_n - \alpha^{\gor} \rvert, \lvert \mu_n - \mu^{\gor} \rvert, \lvert \nu_n - \nu^{\gor}\rvert\bigr\} \leq \frac{\min(\epsilon, C_{K_2} \epsilon^2)}{2}\Bigr\},
\end{align*}
and
\begin{align*}
	\mathcal{A}_2 = \Bigl\{	\min_{\|(\alpha, \mu, \nu) - (\alpha_n, \mu_n, \nu_n)\|_2 \geq \epsilon\sqrt{3}/2} \widebar{L}_n^{\mathsf{so}}(\alpha, \mu, \nu) \geq \widebar{L}_n^{\mathsf{so}}(\alpha_n, \mu_n, \nu_n) + C_{K}\epsilon^2\Bigr\}.
\end{align*}
Now Lemma~\ref{lem:ao-analysis}(a) implies $\Pro\{\mathcal{A}_1\} \geq 1 - Ce^{-cn \min(\epsilon^2, C_K^2 \epsilon^4)}$ and Lemma~\ref{lem:ao-analysis}(b) implies $\Pro\{\mathcal{A}_2\} \geq 1 - Ce^{-cn}$.  Thus, taking $\epsilon_1 = (3C_{K}/8) \cdot \epsilon^2$ and applying the law of total probability, we obtain the pair of inequalities \apcomment{Make the folowing steps clearer with proper dependence on $C_K$ parameters.}
\begin{subequations}\label{ineq:step4-prop-gor}
	\begin{align}
			\Pro\Bigl\{\min_{(\alpha, \mu, \nu) \in \Pc(D_{\epsilon} \cap \mathbb{B}_2(C))}\widebar{L}_n(\alpha, \mu, \nu) \leq \bar{\mathsf{L}} + 2\epsilon_1\Bigr\} &\leq C\exp\{-cn\min(\epsilon^2, \epsilon^4)\} \text{ and }\\
			\Pro\Bigl\{\min_{(\alpha, \mu, \nu) \in \Pc(\mathbb{B}_2(C))} \widebar{L}_n(\alpha, \mu, \nu) > \bar{\mathsf{L}} + \epsilon_1\Bigr\} &\leq C\exp\{-cn\min(\epsilon^2, \epsilon^4)\}.
	\end{align}
\end{subequations}
Finally, since $\mathcal{P}(D_\epsilon)$ is a product scalarized set (see Definition~\ref{def:scalarized-set}), Proposition~\ref{prop:first-three-steps} applies to yield
\begin{align} \label{eq:final-prop-ineq-HO}
\Pro\Bigl\{\argmin_{\bt \in \mathbb{B}_2(C')} \mathcal{L}(\bt) \in D_{\epsilon}\Bigr\} &\leq 2 \Pro\Bigl\{\min_{(\alpha, \mu, \nu) \in \Pc( \bar{D} \cap \mathbb{B}_2(C'))}\widebar{L}_n(\alpha, \mu, \nu) \leq \bar{\mathsf{L}} + 2\epsilon_1 \Bigr\} \notag \\
&\quad  + 2 \Pro\Bigl\{\min_{(\alpha, \mu, \nu) \in \Pc(\mathbb{B}_2(C'))} \widebar{L}_n(\alpha, \mu, \nu) > \bar{\mathsf{L}} + \epsilon_1 \Bigr\} + 8 e^{-n/2}.
\end{align}
Combining the inequalities~\eqref{ineq:step4-prop-gor} and \eqref{eq:final-prop-ineq-HO}, we obtain
\[
\Pro\biggl\{\max\Bigl(\lvert \langle \bt, \btstar \rangle - \alpha^{\gor} \rvert, \Bigl\lvert \frac{\langle \bt, \proj_{\btstar}^{\perp}\bt^{\sharp}\rangle}{\| \proj_{\btstar}^{\perp} \bt^{\sharp}\|_2} - \mu^{\gor} \Bigr\rvert, \lvert \| \proj_{S_{\sharp}}^{\perp} \bt \|_2 - \nu^{\gor} \rvert \Bigr) \geq \epsilon\biggr\} \leq C\exp\{-Cn\min(\epsilon^2, \epsilon^4)\},
\]
and the theorem follows immediately. \qed
%\end{proof}

\subsection{Proof of Theorem~\ref{thm:one_step_main_FO}(a)}

We begin by defining the first-order analog of the expanded Gordon state evolution update.

%\apcomment{Should the $2\eta / \kappa$ term for $\nu^\gor$ below be $2\eta / \sqrt{\kappa}$?}
\begin{definition}[Expanded Gordon state evolution update: First-order methods]\label{def:expanded-gordon-FO}
Recall the model~\eqref{eq:model}, and let $Q$ denote a random variable drawn from the latent variable distribution $\mathbb{Q}$. Suppose the loss function $\Lc$ takes the form~\eqref{eq:GD_gen}. Let $(Z_1, Z_2, Z_3)$ denote a triplet of independent standard Gaussian random variables and let $\alpha^{\sharp} \in \mathbb{R}$ and $\beta^{\sharp} \in \mathbb{R}_{\geq 0}$ denote arbitrary scalars.  Let
\[
\Omega = \omega\big(\parcomp^{\sharp} Z_1 +\perpcomp^{\sharp} Z_2\,,\,f(Z_1; Q)+\noisestd Z_3 \big).
\]
Then define the scalars
\[
\alpha^{\gor} = \alpha^{\sharp} + 2\eta \cdot \EE[Z_1 \Omega], \qquad \perpone^{\gor} = \perpcomp^{\sharp} + 2\eta \cdot \EE[Z_2 \Omega], \qquad \text{ and } \qquad \perptwo^{\gor} = \frac{2 \eta}{\sqrt{\kappa}} \cdot \sqrt{\EE[\Omega^2]}.
\]
\end{definition}
As before, it suffices to show that for a parameter $c_K$ depending only on $K_1$ from Assumption~\ref{ass:omega}, we have
\begin{align} \label{eq:equiv-thm2a}
\Pro \left\{ \max \left( \left| \frac{\inprod{\mathcal{T}_n(\btsharp)}{\proj^{\perp}_{\thetastar} \btsharp}}{ \| \proj^{\perp}_{\thetastar} \btsharp \|_2} - \perpone^{\gor} \right|, \left| \| \proj^{\perp}_{S_{\#}} \mathcal{T}_n(\btsharp) \|_2 - \perptwo^{\gor} \right| \right) > \epsilon \right\} \leq C \exp \left( -c_K n \epsilon^4 \right).
\end{align}
%for each $\epsilon \geq n^{-1/4}$. 

\subsubsection{Implementing step 4: Growth properties of $\widebar{L}_n$}

The following lemma guarantees growth conditions on the function $\widebar{L}_n$ when the one-step loss function takes the form~\eqref{eq:GD_gen}.  
%We provide the proof for higher-order methods in Subsection~\ref{subsec:proof-ao-analysis-higher-order} and the proof for first-order methods in Subsection~\ref{subsec:proof-ao-analysis-first-order}.

\begin{lemma}
	\label{lem:ao-analysis-FO}
	Suppose that the loss function $\mathcal{L}$ takes the form %~\eqref{eq:GD_gen} or
	\eqref{eq:GD_gen} and let the scalarized auxiliary loss $\widebar{L}_n$ be as in Definition~\ref{def:scalarized-ao}.  Define the constant 
	\[
	\bar{\mathsf{L}} = -\frac{1}{2}((\alpha^{\gor})^2 + (\mu^{\gor})^2 + (\nu^{\gor})^2),
	\]
	and let the tuple $(\parcompgordon, \perpone^{\gor}, \perptwo^{\gor})$ be as in Definition~\ref{def:expanded-gordon-FO}.
	Suppose that Assumption~\ref{ass:omega} holds with parameter $K_1$.
	Then, there exists $c_{K_1} > 0$ depending only on $K_1$ and universal positive constants $c, C, C_1, C_2$  such that for all $\kappa \geq C_1$, the following hold:
		\begin{enumerate}[label=(\alph*)]
		\item The minimizer
		\[
		(\alpha_n, \mu_n, \nu_n) = \argmin_{(\alpha, \mu, \nu) \in \Pc(\mathbb{B}_2(C_2))} \widebar{L}_n(\alpha, \mu, \nu) 
		\]
		is unique and satisfies both
		\[
		\max\bigl\{\lvert \alpha_n - \alpha^{\gor} \rvert, \lvert \mu_n - \mu^{\gor} \rvert, \lvert \nu_n - \nu^{\gor}\rvert\bigr\} \leq \epsilon,
		\]
		and 
		\[
		\biggl \lvert \widebar{L}_n^{\mathsf{so}}(\alpha_n, \mu_n, \nu_n) - \bar{\mathsf{L}} \biggr \rvert \leq \epsilon,
		\]
		with probability at least $1 - C \exp\{ -c_{K_1} \cdot n \epsilon^2 \} - C e^{-cn}$.
		\item The scalarized auxiliary loss $\widebar{L}_n$ is $2$-strongly convex on the domain $\mathbb{B}_2(C_2)$ with probability at least $1 - Ce^{-cn}$.
%	
%		The following strong convexity property holds for the function $\widebar{L}_n$
%		\[
%		\min_{\|(\alpha, \mu, \nu) - (\alpha_n, \mu_n, \nu_n)\|_2 \geq \epsilon} \widebar{L}_n(\alpha, \mu, \nu) \geq \widebar{L}_n(\alpha_n, \mu_n, \nu_n) + C_{\mathsf{sc}}\epsilon^2,
%		\]
%		with probability at least $1 - Ce^{-Cn\epsilon^2}$.
	\end{enumerate}
\end{lemma}
Note that the strong convexity constant here is absolute (equal to $2$) instead of dependent on Assumption~\ref{ass:omega-lb} like in higher-order methods. We can now put everything together exactly like before.

\subsubsection{Combining the pieces}
The calculations here are very similar to before, so we only sketch the differences. With the tuple $(\parcompgordon, \perpone^{\gor}, \perptwo^{\gor})$ as in Definition~\ref{def:expanded-gordon-FO}, define the events \apcomment{Need $C_K$ dependence here?}
\begin{align*}
\mathcal{A}_1 &= \Bigl\{\max\bigl\{\lvert \alpha_n - \alpha^{\gor} \rvert, \lvert \mu_n - \mu^{\gor} \rvert, \lvert \nu_n - \nu^{\gor}\rvert\bigr\} \leq \min(\epsilon, \epsilon^2) \Bigr\} \text{ and } \\
	\mathcal{A}_2 &= \Bigl\{	\min_{\|(\alpha, \mu, \nu) - (\alpha_n, \mu_n, \nu_n)\|_2 \geq \epsilon\sqrt{3}/2} \widebar{L}_n^{\mathsf{so}}(\alpha, \mu, \nu) \geq \widebar{L}_n^{\mathsf{so}}(\alpha_n, \mu_n, \nu_n) + \epsilon^2\Bigr\}.
\end{align*}
Carrying out the proof exactly as before but now with $\epsilon_1 = 3\epsilon^2/4$ leads to the desired result.
\qed

\subsection{Proofs of technical lemmas in steps 1--3}

In this subsection, we prove each of our technical lemmas used in the proof of Proposition~\ref{prop:first-three-steps}.

\subsubsection{Proof of Lemma~\ref{lem:bilinear}}
\label{subsec:proof-of-bilinear}
We require two additional lemmas that are proved at the end of this subsection.  The first lemma shows that the optimization can be done over a compact set. \apcomment{Switched quantifiers here, earlier version didn't make sense to me. (It is commented out in Tex file.)} 
% Modified quantifiers from before.
% \begin{lemma}
% 	\label{lem:bounded-optimization}
% 	Under the setting of Lemma~\ref{lem:bilinear}, there exists a universal positive constant $C$ such that for all constants $C_1 \geq C$ and closed subsets $D \subseteq \mathbb{B}_2(C_1)$, 
% 	\[
% 	\min_{\bt \in D} \Lc(\bt; \btsharp, \bX, \by) = \min_{\substack{\bt \in D \\ \bu \in \mathbb{B}_2(C) }}\max_{\bv \in \mathbb{B}_2(C)} \frac{1}{\sqrt{n}} \langle \bv, \bX \bt - \bu \rangle + F(\bu, \bt),
% 	\]
% 	with probability at least $1 - Ce^{-Cn}$.  
% \end{lemma}
\begin{lemma}
	\label{lem:bounded-optimization}
	Suppose $\kappa > 1$ and that we operate under the setting of Lemma~\ref{lem:bilinear}. There are universal constants $c, C > 0$ such that the following is true. For each $R > 0$, there exists a positive $C_n$ (that may depend on $n$ and $R$) such that for all %constants $C_1 \geq C$ and 
	closed subsets $D \subseteq \mathbb{B}_2(R)$, 
	\[
	\min_{\bt \in D} \Lc(\bt; \btsharp, \bX, \by) = \min_{\substack{\bt \in D \\ \bu \in \mathbb{B}_2(C_n) }}\max_{\bv \in \mathbb{B}_2(C_n)} \frac{1}{\sqrt{n}} \langle \bv, \bX \bt - \bu \rangle + F(\bu, \bt),
	\]
	with probability at least $1 - Ce^{-cn}$.  
\end{lemma}
The following lemma uses the bilinear characterization of Lemma~\ref{lem:bounded-optimization} and subsequently invokes the CGMT to connect to the auxiliary loss $\mathfrak{L}_n$.
\begin{lemma}
	\label{lem:invoke-CGMT}
	Under the setting of Lemma~\ref{lem:bilinear}, there exists a universal positive constant $C$ such that for all constants $C_1 \geq C$ and any closed subset $D \subseteq \mathbb{B}_2(C_1)$,  \apcomment{Quantifiers here look weird to me. What is $C_1$?}
	\[
	\Pro\Biggl\{\min_{\substack{\bt \in D \\ \bu \in \mathbb{B}_2(C) }}\max_{\bv \in \mathbb{B}_2(C)} \frac{1}{\sqrt{n}} \langle \bv, \bX \bt - \bu \rangle + F(\bu, \bt) \geq t\Biggr\} \leq 2\Pro\Biggl\{\min_{\substack{\bt \in D \\ \bu \in \mathbb{B}_2(C) }} \mathfrak{L}(\bt; \bu) \geq t\Biggr\} + Ce^{-Cn}.
	\]
	If, in addition, $D$ is convex, then
		\[
	\Pro\Biggl\{\min_{\substack{\bt \in D \\ \bu \in \mathbb{B}_2(C) }}\max_{\bv \in \mathbb{B}_2(C)} \frac{1}{\sqrt{n}} \langle \bv, \bX \bt - \bu \rangle + F(\bu, \bt) \leq t\Biggr\} \leq 2\Pro\Biggl\{\min_{\substack{\bt \in D \\ \bu \in \mathbb{B}_2(C) }} \mathfrak{L}(\bt; \bu) \leq t\Biggr\} + Ce^{-Cn}.
	\]
\end{lemma}

Lemma~\ref{lem:bilinear} follows immediately upon combining Lemmas~\ref{lem:bounded-optimization} and~\ref{lem:invoke-CGMT}. \qed

\paragraph{Proof of Lemma~\ref{lem:bounded-optimization}}
First, recall that Assumption~\ref{ass:loss} implies the existence of a function $F$ such that $\Lc(\bt) = F(\bX \bt, \bt)$.  Consequently, we obtain
\[
\min_{\bt \in D} \Lc(\bt) = \min_{\bt \in D, \bu \in \mathbb{R}^n} F(\bu, \bt) \quad \text{ s.t. } \quad \bu = \bX\bt.
\]
Applying~\citet[Corollary 7.3.3]{vershynin2018high} in conjunction with the assumptions $\kappa > 1$ and $D \subseteq \mathbb{B}_2(R)$ yields that the event
\[
\mathcal{A} = \{ \| \bX\bt \|_2 \leq 2R \sqrt{n} \}
\]
occurs with probability at least $1 - 2e^{-n}$.  We carry out the rest of the proof on this event, obtaining
\begin{align}
	\label{eq:bounded-optimization-intermediate}
\min_{\bt \in D} \Lc(\bt) &= \min_{\substack{\bt \in D \\ \bu \in \mathbb{B}_2(2R \sqrt{n}) }} F(\bu, \bt) \quad \text{ s.t. }\quad \bu = \bX\bt\nonumber\\
&= \min_{\substack{\bt \in D \\ \bu \in \mathbb{B}_2(2R \sqrt{n}) }} \max_{\bv \in \mathbb{R}^n} \; F(\bu, \bt) - \langle \bv, \bu - \bX \bt \rangle.
\end{align}
It remains only to prove that $\bv$ can further be constrained to the ball $\mathbb{B}_2(C\sqrt{n})$ for a large enough $C$.  To this end, recall that by Assumption~\ref{ass:loss}(b), the function $F(\bu, \bt)$ is $C_L/\sqrt{n}$-Lipschitz in its first argument.  We thus obtain the pair of inequalities \apcomment{Unclear, discuss.}
\begin{align*}
	 \min_{\substack{\bt \in D \\ \bu \in \mathbb{B}_2(C) }} \max_{\bv \in \mathbb{B}_2(2C_L)} F(\bu, \bt) - \frac{1}{\sqrt{n}}\langle \bv, \bu - \bX \bt \rangle &\geq \min_{\substack{\bt \in D \\ \bu \in \mathbb{B}_2(C) }} F(\bX \bt, \bt) + \max_{\bv \in \mathbb{B}_2(2C_L)}  \biggl(\frac{\| \bv \|_2}{\sqrt{n}} - \frac{C_L}{\sqrt{n}}\biggr)\| \bu - \bX\bt \|_2\\
	 	 \min_{\substack{\bt \in D \\ \bu \in \mathbb{B}_2(C) }} \max_{\bv \in \mathbb{B}_2(2C_L)} F(\bu, \bt) - \frac{1}{\sqrt{n}}\langle \bv, \bu - \bX \bt \rangle &\leq \min_{\substack{\bt \in D \\ \bu \in \mathbb{B}_2(C) }} F(\bX \bt, \bt) + \max_{\bv \in \mathbb{B}_2(2C_L)}  \biggl(\frac{\| \bv \|_2}{\sqrt{n}} + \frac{C_L}{\sqrt{n}}\biggr)\| \bu - \bX\bt \|_2.
\end{align*}
Note that the RHS of both inequalities takes the value $\min_{\bt \in D} F(\bX \bt, \bt)$ so that 
\[
\min_{\substack{\bt \in D \\ \bu \in \mathbb{B}_2(C) }} \max_{\bv \in \mathbb{B}_2(2C_L)} F(\bu, \bt) - \frac{1}{\sqrt{n}}\langle \bv, \bu - \bX \bt \rangle  = \min_{\bt \in D} F(\bX\bt, \bt),
\]
which is the value of the unconstrained problem~\eqref{eq:bounded-optimization-intermediate}.  The proof is complete upon taking $C$ large enough.\qed

\paragraph{Proof of Lemma~\ref{lem:invoke-CGMT}}
%\label{subsec:proof-invoke-CGMT}
First, recall that by Assumption~\ref{ass:loss}, $F(\bu, \bt)$ can be decomposed as 
\[
F(\bu, \bt) = g(\bu,  \bX \btsharp; \by) + h(\bt, \btsharp).
\]
Next, recall the subspace $S_{\sharp} = \mathsf{span}(\btstar, \btsharp)$ and consider the orthogonal decomposition \\$\bt = \proj_{S_{\sharp}}\bt + \proj_{S_{\sharp}}^{\perp} \bt$.  Combining these two pieces, we obtain the representation
\begin{align*}
\frac{1}{\sqrt{n}} \langle \bv, \bX \bt - \bu \rangle + F(\bu, \bt) &= h(\bt, \btsharp) + g(\bu, \bX\btsharp; \by) - \frac{1}{\sqrt{n}} \langle \bv, \bu \rangle + \frac{1}{\sqrt{n}} \langle \bv, \bX \proj_{S_{\sharp}}\bt \rangle + \frac{1}{\sqrt{n}} \langle \bv, \bX\proj_{S_{\sharp}}^{\perp} \bt \rangle.
\end{align*}

Note that the Gaussian random variable $\langle \bv, \bX\proj_{S_{\sharp}}^{\perp} \bt \rangle$ is independent of all other randomness in the expression.  Thus, in that term, we replace the random matrix $\bX$ with an independent copy $\bG \in \mathbb{R}^{n \times d}$.  Turning to the variational problem of interest, we have
\begin{align*}
	&\min_{\substack{\bt \in D \\ \bu \in \mathbb{B}_2(C) }}\max_{\bv \in \mathbb{B}_2(C)} h(\bt, \btsharp) + g(\bu, \bX\btsharp; \by) - \frac{1}{\sqrt{n}} \langle \bv, \bu \rangle + \frac{1}{\sqrt{n}} \langle \bv, \bX \proj_{S_{\sharp}}\bt \rangle + \frac{1}{\sqrt{n}} \langle \bv, \bX\proj_{S_{\sharp}}^{\perp} \bt \rangle \\
	\overset{(d)}{=}&\min_{\substack{\bt \in D \\ \bu \in \mathbb{B}_2(C) }}\max_{\bv \in \mathbb{B}_2(C)} h(\bt, \btsharp) + g(\bu, \bX\btsharp; \by) - \frac{1}{\sqrt{n}} \langle \bv, \bu \rangle + \frac{1}{\sqrt{n}} \langle \bv, \bX \proj_{S_{\sharp}}\bt \rangle + \frac{1}{\sqrt{n}} \langle \bv, \bG\proj_{S_{\sharp}}^{\perp} \bt \rangle.
\end{align*}
At this juncture, we invoke the CGMT Proposition~\ref{thm:gordon} with
\[
P(\bG) = \min_{(\bt, \bu) \in D \times \mathbb{B}_2(C)}\max_{\bv \in \mathbb{B}_2(C)} h(\bt, \btsharp) + g(\bu, \bX\btsharp; \by) - \frac{1}{\sqrt{n}} \langle \bv, \bu \rangle + \frac{1}{\sqrt{n}} \langle \bv, \bX \proj_{S_{\sharp}}\bt \rangle + \frac{1}{\sqrt{n}} \langle \bv, \bG\proj_{S_{\sharp}}^{\perp} \bt \rangle
\]
and 
\[
A(\bg, \bh) = \min_{(\bt, \bu) \in D \times \mathbb{B}_2(C)}\max_{\bv \in \mathbb{B}_2(C)}\; \mathfrak{L}(\bt),
\]
which completes the proof. \qed



\subsubsection{Proof of Lemma~\ref{lem:scalarize-ao}}
\label{subsec:proof-scalarize-ao}
We begin by defining a few additional optimization problems. Under the setting of Lemma~\ref{lem:scalarize-ao}, recall the map $\Pc$ as defined in Definition~\ref{def:scalarized-set}, and the random vectors $\bz_1$ and $\bz_2$~\eqref{eq:zone-ztwo}. Define the minimum of the variational problem \apcomment{$C_u, C_v$ notation.}
	\begin{align}\label{eq:def-phi-var}
		\phi_{\mathsf{var}} \;= &\min_{\substack{(\parcomp, \perpone, \perptwo) \in \Pc(D), \\ \bu \in \mathbb{B}_2(C_u\sqrt{n}) }} \; h_{\mathsf{scal}}(\parcomp, \perpone, \perptwo, \btsharp) + g(\bu, \bX \btsharp; \by) \notag \\
		& + \max_{0 \leq r \leq C_v}\; \frac{r}{\sqrt{n}} \cdot \Bigl( \| \perptwo \cdot  \bg + \parcomp \cdot \bz_1 + \perpone \cdot \bz_2 - \bu \|_2  - \perptwo \cdot  \| \proj_{S_{\sharp}}^{\perp} \bh \|_2 \Bigr).
	\end{align}
Next, define the minimum of the constrained problem
	\begin{align}\label{eq:def-phi-con}
		\phi_{\mathsf{con}} \;= &\min_{\substack{(\parcomp, \perpone, \perptwo) \in \Pc(D), \\ \bu \in \mathbb{B}_2(C\sqrt{n}) }}\; h_{\mathsf{scal}}(\parcomp, \perpone, \perptwo, \btsharp) + g(\bu, \bX \btsharp; \by) \notag \\
		&\;\;\;\;\;\;\; \mathrm{ s.t. }\;\;\;  \| \perptwo \cdot  \bg + \parcomp \cdot \bz_1 + \perpone \cdot \bz_2  - \bu \|_2  \leq  \perptwo \cdot  \| \proj_{S_{\sharp}}^{\perp} \bh \|_2.
	\end{align}
	Finally, define the minimum of the constrained problem
	\begin{align} \label{eq:def-phi-scal}
		\phi_{\mathsf{scal}} \;= &\min_{(\parcomp, \perpone, \perptwo) \in \Pc(D)} \max_{\bv \in \mathbb{R}^n} \;\; h_{\mathsf{scal}}(\parcomp, \perpone, \perptwo, \btsharp) - g^*(\bv, \bX \btsharp; \by) + \min_{\bu \in \mathbb{B}_2(C_u\sqrt{n}) } \langle \bu, \bv \rangle \nonumber\\
		&\;\;\;\;\;\;\; \mathrm{ s.t. }\;\;\;  \| \perptwo \cdot  \bg + \parcomp \cdot \bz_1 + \perpone \cdot \bz_2  - \bu \|_2  \leq  \perptwo \cdot  \| \proj_{S_{\sharp}}^{\perp} \bh \|_2.
	\end{align}


We now state two lemmas that will prove useful in the proof.
\begin{lemma}
	\label{lem:constrained-equivalence}
	% Under the setting of Lemma~\ref{lem:scalarize-ao}, recall the map $\Pc$ as defined in Definition~\ref{def:scalarized-set} and define the minimum of the variational problem
	% \begin{align}\label{eq:def-phi-var}
	% 	\phi_{\mathsf{var}} \;= &\min_{\substack{(\parcomp, \perpone, \perptwo) \in \Pc(D), \\ \bu \in \mathbb{B}_2(C_u\sqrt{n}) }} \; h_{\mathsf{scal}}(\parcomp, \perpone, \perptwo, \btsharp) + g(\bu, \bX \btsharp; \by) \\
	% 	& + \max_{0 \leq r \leq C_v}\; \frac{r}{\sqrt{n}} \cdot \Bigl( \| \perptwo \cdot  \bg + \parcomp \cdot \bz_1 + \perpone \cdot \bz_2 - \bu \|_2  - \perptwo \cdot  \| \proj_{S_{\sharp}}^{\perp} \bh \|_2 \Bigr),
	% \end{align}
	% as well as the minimum of the constrained problem
	% \begin{align}\label{eq:def-phi-con}
	% 	\phi_{\mathsf{con}} \;= &\min_{\substack{(\parcomp, \perpone, \perptwo) \in \Pc(D), \\ \bu \in \mathbb{B}_2(C\sqrt{n}) }}\; h_{\mathsf{scal}}(\parcomp, \perpone, \perptwo, \btsharp) + g(\bu, \bX \btsharp; \by) \\
	% 	&\;\;\;\;\;\;\; \mathrm{ s.t. }\;\;\;  \| \perptwo \cdot  \bg + \parcomp \cdot \bz_1 + \perpone \cdot \bz_2  - \bu \|_2  \leq  \perptwo \cdot  \| \proj_{S_{\sharp}}^{\perp} \bh \|_2.
	% \end{align}
	Under the setup above,
	there exists a universal positive constant $C$ such that 
	\[
	\Pro\Bigl\{\lvert \phi_{\mathsf{var}} - \phi_{\mathsf{con}}\rvert \leq \frac{C}{C_v}\Bigr\} \geq 1 - Ce^{-Cn}.
	\]
\end{lemma}

\begin{lemma}\label{lem:solve-constrained}
% 	Under the setting of Lemma~\ref{lem:scalarize-ao}, define the minimum of the constrained problem
% %	\[
% %	\phi_{\mathsf{scal}} = \min_{(\parcomp,\perpone,\perptwo)\in \Pc(D)}\max_{\bv \in \mathbb{R}^n} \; \hscal(\parcomp, \perpone, \perptwo, \btsharp) - g^*(\bv,\bX\btsharp;\by) -\perptwo \|\proj^{\perp}_{S_{\sharp}}\bh\|_2\|\bv\|_2+\langle \perptwo\bg+\parcomp\bz_1+\perpone\bz_2, \bv \rangle.
% %	\]
% 	\begin{align} \label{eq:def-phi-scal}
% 		\phi_{\mathsf{scal}} \;= &\min_{(\parcomp, \perpone, \perptwo) \in \Pc(D)} \max_{\bv \in \mathbb{R}^n} \;\; h_{\mathsf{scal}}(\parcomp, \perpone, \perptwo, \btsharp) - g^*(\bu, \bX \btsharp; \by) + \min_{\bu \in \mathbb{B}_2(C_u\sqrt{n}) } \langle \bu, \bv \rangle \nonumber\\
% 		&\;\;\;\;\;\;\; \mathrm{ s.t. }\;\;\;  \| \perptwo \cdot  \bg + \parcomp \cdot \bz_1 + \perpone \cdot \bz_2  - \bu \|_2  \leq  \perptwo \cdot  \| \proj_{S_{\sharp}}^{\perp} \bh \|_2.
% 	\end{align}
Under the setup above,
	there exists a universal positive constant $C$ such that 
	\[
	\Pro\biggl\{\phi_{\mathsf{con}} = \min_{(\parcomp,\perpone,\perptwo)\in \Pc(D)} \; \widebar{L}_n(\parcomp, \perpone, \perptwo; \btsharp)\biggr\} \geq 1 - Ce^{-Cn},
	\]
	where $\widebar{L}_n$ is the scalarized loss from Definition~\ref{def:scalarized-ao}.
\end{lemma}

Taking these lemmas as given, the proof of Lemma~\ref{lem:scalarize-ao} consists of three major steps, which we perform in sequence: we (i) scalarize the maximization over $\bv$; (ii) scalarize the minimization over $\bt$; and (iii) optimize over $\bu$.  We proceed now to the execution of these steps.
\medskip

\noindent \underline{Scalarize the maximization over $\bv$.}
Recall the auxiliary loss $\mathfrak{L}_n$ from Definition~\ref{def:aux-gordon-loss} and note that the Cauchy--Schwarz inequality implies that
\[
\min_{\substack{\bt \in D \\ \bu \in \mathbb{B}_2(C_u \sqrt{n}) }}  \mathfrak{L}_n(\bt, \bu) = \min_{\substack{\bt \in D \\ \bu \in \mathbb{B}_2(C_u\sqrt{n}) }} \max_{0 \leq r \leq C_v} F(\bu, \bt) + \frac{r}{\sqrt{n}} \cdot \Bigl(\langle \bh, \proj_{S_{\sharp}}^{\perp} \bt \rangle + \Bigl\| \| \proj_{S_{\sharp}}^{\perp} \bt \|_2 \cdot \bg + \bX\proj_{S_{\sharp}} \bt - \bu \Bigl\|_2 \Bigr).
\]
\medskip

\noindent \underline{Scalarize the minimization in $\bt$.}
Note that by Assumption~\ref{ass:loss}, the function $F(\bu, \bt)$ only depends on the vector $\proj_{S_{\sharp}}^{\perp} \bt$ through its norm.  Thus, since $D = \bar{D} \cap \mathbb{B}_2(C_1)$ with $\mathcal{P}(\bar{D})$ product scalarized, and the objective in the preceding display depends on the direction of the vector $\proj_{S_{\sharp}}^{\perp} \bt$ only through the linear term $\langle \bh, \proj_{S_{\sharp}}^{\perp} \bt \rangle$, we may minimize the objective over the direction to obtain the characterization
\begin{align}
	\label{eq:scalarize-bt-characterization}
\min_{\substack{\bt \in D \\ \bu \in \mathbb{B}_2(C_u \sqrt{n}) }}  \mathfrak{L}_n(\bt, \bu) = &\min_{\substack{\bt \in D \\ \bu \in \mathbb{B}_2(C_u\sqrt{n}) }} \max_{0 \leq r \leq C_v} F(\bu, \bt)\nonumber\\ 
&+ \frac{r}{\sqrt{n}} \cdot \Bigl( \Bigl\| \| \proj_{S_{\sharp}}^{\perp} \bt \|_2 \cdot  \bg + \bX\proj_{S_{\sharp}} \bt - \bu \Bigl\|_2  - \| \proj_{S_{\sharp}}^{\perp} \bt \|_2\cdot  \| \bh \|_2 \Bigr).
\end{align}
Recalling the independent random variables $\bz_1$ and $\bz_2$~\eqref{eq:zone-ztwo},
%\[
%\bz_1  = \bX\btstar \qquad \text{ and } \qquad \bz_2 = \frac{\bX\proj_{\btstar}^{\perp} \btsharp}{\| \bX\proj_{\btstar}^{\perp} \btsharp \|_2},
%\]
%noting that both $\bz_1, \bz_2 \sim \mathsf{N}(0, \bI_n)$ since $\| \btstar \|_2 = 1$.  Using this notation, we 
write
\[
\by = f(\bz_1; \bq) + \beps \qquad \text{ and } \qquad \bX\btsharp = \alpha^{\sharp}\bz_1 + \beta^{\sharp} \bz_2.
\]
We have the orthogonal decomposition
\[
\bt = \proj_{S_{\sharp}} \bt + \proj_{S_{\sharp}}^{\perp} \bt = \parcomp(\bt) \cdot \btstar + \perpone(\bt) \cdot \frac{\proj_{\btstar}^{\perp} \btsharp}{\| \proj_{\btstar}^{\perp} \btsharp \|_2} + \nu(\bt) \cdot \frac{\proj_{S_{\sharp}}^{\perp} \bt}{\| \proj_{S_{\sharp}}^{\perp} \bt \|_2},
\]
where the second equality follows from the Gram--Schmidt orthogonalization.  Using this combined with the characterization~\eqref{eq:scalarize-bt-characterization}, we obtain
\begin{align}
	\label{eq:scalar-in-bt}
\min_{\substack{\bt \in D \\ \bu \in \mathbb{B}_2(C_u\sqrt{n}) }} \mathfrak{L}_n(\bt, \bu) = &\min_{\substack{(\parcomp, \perpone, \perptwo) \in \Pc(D), \\ \bu \in \mathbb{B}_2(C_u\sqrt{n}) }} \; h_{\mathsf{scal}}(\parcomp, \perpone, \perptwo, \btsharp) + g(\bu, \bX \btsharp; \by)\nonumber\\
& + \max_{0 \leq r \leq C_v}\; \frac{r}{\sqrt{n}} \cdot \Bigl( \| \perptwo \cdot  \bg + \parcomp \cdot \bz_1 + \perpone \cdot \bz_2 - \bu \|_2  - \perptwo \cdot  \| \proj_{S_{\sharp}}^{\perp} \bh \|_2 \Bigr).
\end{align}
\medskip

\noindent \underline{Optimize over $\bu$.}
Note that if the inner maximization over $r \geq 0$ were unbounded, the optimization problem in the display above would correspond to a constrained optimization problem.  To this end, we invoke Lemma~\ref{lem:constrained-equivalence}, taking $C_v$ arbitrarily large, in conjunction with the characterization~\eqref{eq:scalar-in-bt} to obtain the equation \apcomment{Unclear, discuss}
\begin{align*}
%	\label{eq:scalar-in-bt}
	\min_{\substack{\bt \in D \\ \bu \in \mathbb{B}_2(C_u\sqrt{n}) }} \mathfrak{L}_n(\bt, \bu) = 
&\min_{\substack{(\parcomp, \perpone, \perptwo) \in \Pc(D), \\ \bu \in \mathbb{B}_2(C_u\sqrt{n}) }}\; h_{\mathsf{scal}}(\parcomp, \perpone, \perptwo, \btsharp) + g(\bu, \bX \btsharp; \by) \\
		&\;\;\;\;\;\;\; \mathrm{ s.t. }\;\;\;  \| \perptwo \cdot  \bg + \parcomp \cdot \bz_1 + \perpone \cdot \bz_2  - \bu \|_2  \leq  \perptwo \cdot  \| \proj_{S_{\sharp}}^{\perp} \bh \|_2),
\end{align*}
with probability at least $1 - Ce^{-Cn}$.  We continue by linearizing the constrained objective in the optimization variable $\bu$.  To this end, recall that $g$ is convex in its first argument and let $g^*$ denote its convex conjugate so that
\begin{align*}
			\min_{\substack{\bt \in D \\ \bu \in \mathbb{B}_2(C_u\sqrt{n}) }} \mathfrak{L}_n(\bt, \bu) \;= &\min_{\substack{(\parcomp, \perpone, \perptwo) \in \Pc(D), \\ \bu \in \mathbb{B}_2(C_u\sqrt{n}) }}\max_{\bv \in \mathbb{R}^n}\; h_{\mathsf{scal}}(\parcomp, \perpone, \perptwo, \btsharp) - g^*(\bv, \bX \btsharp; \by) + \langle \bv, \bu \rangle \\
	&\;\;\;\;\;\;\; \mathrm{ s.t. }\;\;\;  \| \perptwo \cdot  \bg + \parcomp \cdot \bz_1 + \perpone \cdot \bz_2  - \bu \|_2  \leq  \perptwo \cdot  \| \proj_{S_{\sharp}}^{\perp} \bh \|_2.
\end{align*}
Next, we perform three steps in sequence: (i) write the equivalent Lagrangian to the problem above; (ii) note that the minimization over $\bu$ is of a convex function over a compact constraint and the maximization over $\bv$ is of a concave function and invoke Sion's minimax theorem to swap the minimization over $\bu$ with the maximization over $\bv$; and (iii) re-write as a constrained optimization problem to obtain
	\begin{align*}
	\min_{\substack{\bt \in D \\ \bu \in \mathbb{B}_2(C_u\sqrt{n}) }} \mathfrak{L}_n(\bt, \bu) \;= &\min_{(\parcomp, \perpone, \perptwo) \in \Pc(D)} \max_{\bv \in \mathbb{R}^n} \;\; h_{\mathsf{scal}}(\parcomp, \perpone, \perptwo, \btsharp) - g^*(\bu, \bX \btsharp; \by) + \min_{\bu \in \mathbb{B}_2(C_u\sqrt{n}) } \langle \bu, \bv \rangle\\
	&\;\;\;\;\;\;\; \mathrm{ s.t. }\;\;\;  \| \perptwo \cdot  \bg + \parcomp \cdot \bz_1 + \perpone \cdot \bz_2  - \bu \|_2  \leq  \perptwo \cdot  \| \proj_{S_{\sharp}}^{\perp} \bh \|_2.
\end{align*}
We complete the proof by invoking Lemma~\ref{lem:solve-constrained}. \qed


\paragraph{Proof of Lemma~\ref{lem:constrained-equivalence}}
%\label{subsec:proof-constrained-equivalence}
\kaccomment{note in definition of $\mathfrak{L}_n$ that $C_v$ can scale with $n$}
Note that $\phi_{\mathsf{con}}$ admits the variational representation 
	\begin{align*}
	\phi_{\mathsf{con}} \;= &\min_{\substack{(\parcomp, \perpone, \perptwo) \in \Pc(D), \\ \bu \in \mathbb{B}_2(C\sqrt{n}) }}\; h_{\mathsf{scal}}(\parcomp, \perpone, \perptwo, \btsharp) + g(\bu, \bX \btsharp; \by) \\
	& + \max_{r \geq 0}\; \frac{r}{\sqrt{n}} \cdot \Bigl( \| \perptwo \cdot  \bg + \parcomp \cdot \bz_1 + \perpone \cdot \bz_2 - \bu \|_2  - \perptwo \cdot  \| \proj_{S_{\sharp}}^{\perp} \bh \|_2 \Bigr),
\end{align*}
whence we obtain the inequality $\phi_{\mathsf{con}} \geq \phi_{\mathsf{var}}$.  The rest of the section is devoted to the proof of the reverse inequality $\phi_{\mathsf{var}} \leq \phi_{\mathsf{con}}$.  To this end, fix an arbitrary triple $(\parcomp, \perpone, \perptwo) \in \Pc(D)$.  Given this triple, define the constraint function
\[
\psi(\bu) = \| \perptwo \cdot  \bg + \parcomp \cdot \bz_1 + \perpone \cdot \bz_2 - \bu \|_2  - \perptwo \cdot  \| \proj_{S_{\sharp}}^{\perp} \bh \|_2,
\]
as well as the loss functions
\[
L_n^{\mathsf{var}}(\bu) = \max_{0 \leq r \leq C_v}h_{\mathsf{scal}}(\parcomp, \perpone, \perptwo, \btsharp) + g(\bu, \bX \btsharp; \by) + \frac{r}{\sqrt{n}} \cdot \psi(\bu),
\]
and 
\[
L_n^{\mathsf{con}}(\bu) = \max_{r \geq 0}\;h_{\mathsf{scal}}(\parcomp, \perpone, \perptwo, \btsharp) + g(\bu, \bX \btsharp; \by) + \frac{r}{\sqrt{n}} \cdot \psi(\bu).
\]
Let $\bu^{\var}$ denote an arbitrary minimizer of the loss function $L_n^{\mathsf{var}}$ and suppose that $\bu^{\var}$ does not satisfy the constraint $\psi(\bu^{\var}) \leq 0$---if any such minimizer does satisfy this constraint, then the desired inequality $\phi_{\mathsf{var}} \leq \phi_{\mathsf{con}}$ holds.  

Next, define the event
\[
\mathcal{A}_1 = \{ \| \bg \|_2 \leq 2\sqrt{n},\; \| \bz_1 \|_2 \leq 2\sqrt{n},\; \| \bz_2 \|_2 \leq 2\sqrt{n},\; \| \bh \|_2 \leq 2\},
\]
and note that applying~\citet[Theorem 3.1.1]{vershynin2018high} yields $\Pro\{\mathcal{A}_1\} \geq 1 - 8e^{-cn}$.  Working on this event, we note that we can take $C_u$ large enough so that the set
\begin{align}
	\label{def:S0-def}
S_{0} := \{\bu: \psi(\bu) \leq 0, \bu \in \mathbb{B}_2(C_u \sqrt{n})\} = \mathbb{B}_2\Bigl(\perptwo \cdot  \bg + \parcomp \cdot \bz_1 + \perpone \cdot \bz_2; \;\;\perptwo \cdot  \| \proj_{S_{\sharp}}^{\perp} \bh \|_2\Bigr) \cap \mathbb{B}_2(C_u \sqrt{n}),
\end{align}
is non-empty.  Thus, since $S_{0}$ is a non-empty closed, compact set, the projection onto $S_{0}$ is well-defined.  With this in hand, we require the following statement, whose proof we defer to the end of the section:
\begin{align}
	\label{ineq:bound-psi-uvar}
	\psi(\bu^{\var}) \leq \frac{C\sqrt{n}}{C_v}. 
\end{align}

Now, note that the set
\[
S_R := \{\bu: \psi(\bu) \leq R\} = \mathbb{B}_2\Bigl(\perptwo \cdot  \bg + \parcomp \cdot \bz_1 + \perpone \cdot \bz_2; \;\;\perptwo \cdot  \| \proj_{S_{\sharp}}^{\perp} \bh \|_2 + R\Bigr).
\]
Thus, since $S_R$ and $S_{0}$ are concentric balls, if $\bu \in S_R$ and $\widetilde{\bu}$ denotes its projection onto $S_{0}$, the distance between the two points satisfies
\begin{align}
	\label{ineq:nested-balls}
\| \bu - \widetilde{\bu} \|_2 \leq R.
\end{align}
Now, let $R = C\sqrt{n}/C_v$ and let $\widetilde{\bu}^{\var}$ denote the projection of $\bu^{\var}$ (which is contained in $S_R$ due to the inequality~\eqref{ineq:bound-psi-uvar}) onto $S_0$.  We thus have 
\begin{align*}
	L_n^{\var} (\bu^{\var}) \overset{\1}{\geq} L_n^{\con}(\widetilde{\bu}^{\var}) - \frac{C_L \| \bu^{\var} - \widetilde{\bu}^{\var}\|_2}{\sqrt{n}} &\overset{\2}{\geq} L_n^{\con}(\bu^{\con}) - \frac{C_L \| \bu^{\var} - \widetilde{\bu}^{\var}\|_2}{\sqrt{n}}\\
	&\geq L_n^{\con}(\bu^{\con})  - \frac{C_L C}{C_v},
\end{align*}
where step $\1$ follows since $g$ is $C_L/\sqrt{n}$-Lipschitz in its first argument, step $\2$ follows by $L_n^{\con}$-minimality of $\bu^{\con}$, and the final inequality follows from the inequality~\eqref{ineq:nested-balls}.  Taking stock, since the above inequality holds for all values $(\parcomp, \perpone, \perptwo) \in \Pc(D)$, we have shown that 
\[
\lvert \phi^{\con} - \phi^{\var} \rvert \leq \frac{C}{C_v},
\]
for an absolute constant $C$.  Noting that $C_v < \infty$ was arbitrary, we make $C_v$ arbitrarily large to obtain the result.  \qed
\kaccomment{Check taking the limit in $C_v$ once more, also rename $C_v$ as it has a misleading name}
\medskip

\noindent \underline{Proof of the inequality~\eqref{ineq:bound-psi-uvar}.}  Assume for the sake contradiction that the inequality does not hold and let $\widetilde{\bu}^{\var}$ denote the projection of $\bu^{\var}$ onto the set $S_0$ (as defined in equation~\eqref{def:S0-def}).  Then, since the function $g$ is $C_L/\sqrt{n}$-Lipschitz in its first argument, we obtain the inequality
\[
L_n^{\var}(\bu^{\var}) \geq L_n^{\con}(\widetilde{\bu}^{\var}) - \frac{C_L \| \bu^{\var} - \widetilde{\bu}^{\var}\|_2}{\sqrt{n}} + \frac{C_v \psi(\bu^{\var})}{\sqrt{n}} > L_n^{\con}(\widetilde{\bu}^{\var})  - 2C_L C_u + C > L_n^{\con}(\widetilde{\bu}^{\var}),
\]
where the penultimate inequality follows since $\bu \in \mathbb{B}_2(C_u\sqrt{n})$ and the final inequality follows by taking $C$ large enough.  The above display contradicts $L_n^{\var}$-minimality of $\bu^{\var}$, whence we obtain the desired result.

\paragraph{Proof of Lemma~\ref{lem:solve-constrained}}
%\label{subsec:proof-solve-constrained}
Recall the value $\phi_{\mathsf{scal}}$~\eqref{eq:def-phi-scal}.  Now, we consider a fixed triplet $(\parcomp, \perpone, \perptwo) \in \Pc(D)$ and perform the minimization over $\bu$.  To this end, let
	\begin{align*}
	L_u = \; \min_{\bu \in \mathbb{B}_2(C_u\sqrt{n}) } \langle \bu, \bv \rangle \quad \mathrm{ s.t. } \quad \| \perptwo \cdot  \bg + \parcomp \cdot \bz_1 + \perpone \cdot \bz_2  - \bu \|_2  \leq  \perptwo \cdot  \| \proj_{S_{\sharp}}^{\perp} \bh \|_2.
\end{align*}
Then, introducing a Lagrange multiplier  and invoking Sion's minimax theorem to interchange minimization and maximization, we obtain
\begin{align*}
L_u &= \max_{\lambda \geq 0} \min_{\bu \in \mathbb{B}_2(C_u\sqrt{n})} \;\; \langle \bu, \bv \rangle + \frac{\lambda}{2} \| \perptwo \cdot  \bg + \parcomp \cdot \bz_1 + \perpone \cdot \bz_2  - \bu \|_2^2 - \frac{\lambda \nu^2}{2} \| \proj_{S_{\sharp}}^{\perp} \bh \|_2^2 \\
&\geq  \max_{\lambda \geq 0} \min_{\bu \in \mathbb{R}^n} \;\; \langle \bu, \bv \rangle + \frac{\lambda}{2} \| \perptwo \cdot  \bg + \parcomp \cdot \bz_1 + \perpone \cdot \bz_2  - \bu \|_2^2 - \frac{\lambda \nu^2}{2} \| \proj_{S_{\sharp}}^{\perp} \bh \|_2^2\\
&= \max_{\lambda \geq 0} \;\;\langle \perptwo \cdot  \bg + \parcomp \cdot \bz_1 + \perpone \cdot \bz_2, \bv \rangle - \frac{1}{2\lambda} \| \bv\|_2^2 - \frac{\lambda \nu^2}{2} \| \proj_{S_{\sharp}}^{\perp} \bh \|_2^2 \\
&= \langle \perptwo \cdot  \bg + \parcomp \cdot \bz_1 + \perpone \cdot \bz_2, \bv \rangle  - \perptwo \| \proj_{S_{\sharp}}^{\perp} \bh \|_2 \| \bv \|_2.
\end{align*}  
Conversely, let 
\[
\bar{\bu} = \perptwo \cdot  \bg + \parcomp \cdot \bz_1 + \perpone \cdot \bz_2 - \perptwo \| \proj_{S_{\sharp}}^{\perp} \bh \|_2 \cdot \frac{\bv}{\| \bv \|_2} ,
\]
which is feasible for large enough $C_u$.  Thus, we obtain
\[
L_u \leq \langle \bar{\bu}, \bv \rangle =  \langle \perptwo \cdot  \bg + \parcomp \cdot \bz_1 + \perpone \cdot \bz_2, \bv \rangle  - \perptwo \| \proj_{S_{\sharp}}^{\perp} \bh \|_2 \| \bv \|_2.
\]
Evidently, 
\[
L_u =  \langle \perptwo \cdot  \bg + \parcomp \cdot \bz_1 + \perpone \cdot \bz_2, \bv \rangle  - \perptwo \| \proj_{S_{\sharp}}^{\perp} \bh \|_2 \| \bv \|_2.
\]
Thus, we obtain
\begin{align*}
\phi_{\mathsf{scal}} &= \min_{(\parcomp, \perpone, \perptwo) \in \Pc(D)} \max_{\bv \in \mathbb{R}^n} \;\; h_{\mathsf{scal}}(\parcomp, \perpone, \perptwo, \btsharp) - g^*(\bu, \bX \btsharp; \by) + \langle \perptwo \cdot  \bg + \parcomp \cdot \bz_1 + \perpone \cdot \bz_2, \bv \rangle  - \perptwo \| \proj_{S_{\sharp}}^{\perp} \bh \|_2 \| \bv \|_2\\
&=\min_{(\parcomp,\perpone,\perptwo)\in \Pc(D)} \; \widebar{L}_n(\parcomp, \perpone, \perptwo; \btsharp),
\end{align*}
which concludes the proof. \qed

%\subsection{Proofs of technical lemmas in step 4}

\subsection{Establishing growth conditions for higher-order methods} \label{sec:growth-HO}
%\label{subsec:proof-ao-analysis-higher-order}
In this subsection, we prove Lemma~\ref{lem:ao-analysis}, specialized to second order methods where the loss function~\eqref{eq:sec_order_gen} takes the form 
\[
\Lc(\bt; \btsharp, \bX, \by) = \frac{1}{\sqrt{n}} \| \omega(\bX\btsharp, \by) - \bX\bt \|_2,
\]
which corresponds to setting 
\[
F(\bu, \bt) = \| \omega(\bX\btsharp, \by) - \bu \|_2, \qquad h(\bt, \btsharp) = 0, \qquad \text{ and } \qquad g(\bu, \bX \btsharp; \by) = \| \omega(\bX\btsharp, \by) - \bu \|_2.
\]
We now state several lemmas, which we will invoke in sequence.  The first specializes the scalarized auxiliary loss $\widebar{L}_n$ when the loss corresponds to a higher-order method.
\begin{lemma}
	\label{lem:remove-positive-restriction}
	Under the setting of Lemma~\ref{lem:ao-analysis}, let the loss $\Lc$ correspond to a higher-order method as in equation~\eqref{eq:sec_order_gen}, and let $\widebar{L}_n$ denote the corresponding scalarized loss given by Definition~\ref{def:scalarized-ao}. Also recall the pair of random vectors $(\bz_1, \bz_2)$ from equation~\eqref{eq:zone-ztwo}.
	  There exists a universal positive constant $c$ such that with probability at least $1 - 6e^{-cn}$, \apcomment{Need to state a bit better to make clear that the functions are equivalent whp, not just the value at a particular argument.}
	  %\apcomment{Weirdly stated. Is this a definition or a lemma? Also need to be expicit about dependence between $(\bz_1, \bz_2)$ and $(\bX, \by)$.}
	\[
	\widebar{L}_n(\parcomp, \perpone, \perptwo; \btsharp) = \frac{1}{\sqrt{n}} \| \perptwo \cdot \bg + \parcomp \cdot \bz_1 + \perpone \cdot \bz_2 - \omega(\bX \btsharp, \by) \|_2 - \perptwo \frac{\| \proj_{S_{\sharp}}^{\perp} \bh \|_2}{\sqrt{n}}.
	\]
\end{lemma}
This lemma is proved in Subsection~\ref{subsec:proof-lemma-remove-positive-restriction}.
Before stating the next lemma, we introduce the shorthand \apcomment{Is $\kappa_n$ ever used after?}
\[
\sqrt{\kappa_n} := \frac{\| \proj^{\perp}_{S_{\sharp}} \bh\|_2}{\sqrt{n}}, \qquad \bA:= [\bz_1, \bz_2, \bg] \in \mathbb{R}^{n \times 3}, \qquad \text{ and } \qquad \bv_n := [0, 0, \sqrt{\kappa_n}]^{\top} \in \mathbb{R}^3,
\]
so that letting $\bxi = [\parcomp, \perpone, \perptwo]$ and invoking Lemma~\ref{lem:remove-positive-restriction}, we obtain
\[
\widebar{L}_n(\bxi; \btsharp) = \frac{1}{\sqrt{n}} \| \bA \bxi - \omega(\bX \btsharp, \by) \|_2 - \langle \bv_n, \bxi \rangle.
\]
Now, introduce the variable $\tau$ and write the above display in the form
\[
\widebar{L}_n(\bxi; \btsharp) = \inf_{\tau > 0} \; \underbrace{\frac{\tau}{2} + \frac{1}{2\tau n} \| \bA \bxi - \omega(\bX \btsharp, \by) \|_2^2 - \langle \bv_n, \bxi \rangle}_{\widetilde{L}_n(\bxi, \tau)}.
\]
Next, recall the parameters $(K_1, K_2)$ from Assumptions~\ref{ass:omega} and~\ref{ass:omega-lb} and fix $\epsilon > 0$. For a universal constant $C > 0$, a parameter $C_{K_1} > 0$ depending only on $K_1$, define the events
\begin{subequations} \label{eq:three-events}
\begin{align} \label{eq:event1}
\Ac_1 = \Bigl\{(1 - C\epsilon) \cdot \bI_3 \preceq \frac{1}{n} \bA^{\top} \bA \preceq (1 +C\epsilon) \cdot \bI_3\Bigr\},
\end{align}
\begin{align} \label{eq:event2}
	\Ac_2 = \Bigl\{\frac{1}{n^2}\lvert \langle \bg, \bomega_{\sharp} \rangle \rvert^2 \vee \Bigl\lvert \frac{1}{n^2}\langle \bz_1, \bomega_{\sharp}\rangle^2 - (\EE \{ Z_1 \Omega \})^2\Bigr\rvert \vee \Bigl\lvert \frac{1}{n^2}\langle \bz_2, \bomega_{\sharp} \rangle^2 - (\EE\{Z_2 \Omega \})^2 \Bigr \rvert \leq C_{K_1} \cdot \epsilon\Bigr\},
\end{align}
and 
\begin{align} \label{eq:event3}
	\Ac_3 &= \Bigl\{\Bigl\lvert \frac{1}{n} \| \bomega_{\sharp} \|_2^2 - \EE\{\Omega^2\} \Bigr\rvert \leq C\epsilon \Bigr\}.
\end{align}
\end{subequations}
Finally, note that $\min_{\bxi \in \real^3} \| \bA\bxi - \omega(\bX\btsharp, \by) \|_2 = \| \left( \bI - \bA (\bA^\top \bA)^{-1} \bA^\top \right) \cdot \omega(\bX\btsharp, \by) \|_2$.
\begin{lemma}
	\label{lem:row-space-A}
	%Recall the parameter $K_2$ from Assumption~\ref{ass:omega-lb}. 
	Under the setup above, there exists a parameter $c_{K_1}$ depending only on $K_1$ and universal positive constants $c, C$ such that for all $\epsilon > 0$, \\%with probability at least $1 - 10e^{-cn}$, the following inequality holds 
	(a) On the event $\Ac_1 \cap \Ac_2 \cap \Ac_3$, we have
	\[
	\Bigl\lvert \frac{1}{\sqrt{n}} \| \left( \bI - \bA (\bA^\top \bA)^{-1} \bA^\top \right) \cdot \omega(\bX\btsharp, \by) \|_2 - \sqrt{(\EE\{\Omega^2\} - (\EE\{Z_1 \Omega\})^2 - (\EE\{Z_2 \Omega\})^2} \Bigr\rvert \leq C \cdot C_{K_1} \cdot \epsilon.
	\]
	(b) We have $\Pro \{ \Ac_1 \cap \Ac_2 \cap \Ac_3 \} \geq 1 - C e^{-cn \epsilon^2}$. 
\end{lemma}
This lemma is proved in Subsection~\ref{subsec:proof-lemma-row-space-A}.

\begin{lemma}
	\label{lem:minimize-lbar-higher-order}
	There exists a universal positive constant $c$ such that the following holds. There is an event holding with probability at least $ 1 - 10e^{-cn}$ such that on this event, the following statements hold. \\
	(a) For each $C > 0$, we have the equivalence
	\begin{subequations}
	\begin{align}\label{eq:interchange-inf-min}
	\min_{\bxi \in \Pc(\mathbb{B}_2(C))} \inf_{\tau > 0}\; \widetilde{L}_n(\bxi, \tau) = \inf_{\tau > 0}	\min_{\bxi \in \Pc(\mathbb{B}_2(C))}\; \widetilde{L}_n(\bxi, \tau).
	\end{align}
	(b) The optimization problem on the RHS of equation~\eqref{eq:interchange-inf-min} admits unique minimizers
	\begin{align} \label{eq:unique-empirical-xi}
	\bxi_n(\tau) = (\bA^{\top} \bA)^{-1} \bA^{\top} \omega(\bX\btsharp, \by) + \tau \cdot n \cdot (\bA^{\top} \bA)^{-1} \bv_n,
	\end{align}
	and 
	\begin{align} \label{eq:unique-empirical-tau}
	\tau_n = \frac{\frac{1}{\sqrt{n}}\|(\bI_n - \bA(\bA^{\top} \bA)^{-1}\bA^{\top}) \cdot \omega(\bX \btsharp, \by) \|_2}{\sqrt{1 - n\cdot \bv_n^{\top} (\bA^{\top} \bA)^{-1} \bv_n}}.
	\end{align}
	\end{subequations}
\end{lemma}
We prove this lemma in Subsection~\ref{subsec:proof-lemma-minimize-lbar}.

\subsubsection{Proof of Lemma~\ref{lem:ao-analysis}(a)} 
The first part of the statement---uniqueness of the minimizer---is an immediate consequence of Lemma~\ref{lem:minimize-lbar-higher-order}; moreover, the unique minimizer is given by $\bxi_n(\tau_n)$.  It remains to prove the concentration properties.  As a preliminary step, we show that the dual variable $\tau_n$ concentrates around a deterministic quantity 
\[
\tau^{\gor} = \sqrt{\Bigl(\frac{\kappa}{\kappa - 1} \Bigr) (\EE\{ \Omega^2\} - (\EE\{ Z_1 \Omega\})^2 - (\EE\{ Z_2 \Omega\})^2)}.
\]
To this end, consider the events $\Ac_1, \Ac_2, \Ac_3$ from equation~\eqref{eq:three-events}, and note that Lemma~\ref{lem:row-space-A}(b) implies that $\Ac_1 \cap \Ac_2 \cap \Ac_3$ occurs with probability greater than $1 - C e^{-cn \epsilon^2}$. We carry out the proof on this event.
%\[
%\Ac_1 = \Bigl\{(1 - C\epsilon) \cdot \bI_3 \preceq \frac{1}{n} \bA^{\top} \bA \preceq (1 +C\epsilon) \cdot \bI_3\Bigr\},
%\]
%
\iffalse
Apply~\citet[Theorem 6.1]{wainwright2019high} to obtain $\Pro\{\Ac_1\} \geq 1 - 2e^{-cn\epsilon^2}$.  We note that on the event $\Ac_1$, we obtain the sandwich relation
\[
(1 - C\epsilon/2) \cdot \bI_3 \preceq n (\bA^{\top} \bA)^{-1} \preceq (1 + C\epsilon/2) \cdot \bI_3.
\]
\fi

\paragraph{Bounding $\tau_n$~\eqref{eq:unique-empirical-tau}.} We proceed in three steps.  First, we bound the numerator; second, we bound the denominator; and finally we combine the two bounds.\\

\noindent\underline{Bounding the numerator.}
This step is immediate, since Lemma~\ref{lem:row-space-A}(a) yields
\[
\Bigl\lvert \frac{1}{\sqrt{n}} \| \left( \bI - \bA (\bA^\top \bA)^{-1} \bA^\top \right) \cdot \omega(\bX\btsharp, \by) \|_2 - \sqrt{(\EE\{\Omega^2\} - (\EE\{Z_1 \Omega\})^2 - (\EE\{Z_2 \Omega\})^2} \Bigr\rvert \leq C \cdot C_{K_1} \cdot \epsilon.
\]

\iffalse %Put in proof of Lemma 10
First, let $\bomega_{\sharp} = \omega(\bX \btsharp, \by)$ and expand the norm to obtain
\[
\frac{1}{\sqrt{n}}\|(\bI_n - \bA(\bA^{\top} \bA)^{-1}\bA^{\top}) \cdot \omega(\bX \btsharp, \by) \|_2 = \sqrt{ \frac{1}{n}\| \bomega_{\sharp}\|_2^2 - \frac{1}{n}(\bA^{\top}\bomega_{\sharp})^{\top}(\bA^{\top} \bA)^{-1} (\bA^{\top} \bomega_{\sharp})}.
\]
Now, on the event $\Ac_1$, we obtain the sandwich relation
\[
A_L \leq \sqrt{ \frac{1}{n}\| \bomega_{\sharp}\|_2^2 - \frac{1}{n}(\bA^{\top}\bomega_{\sharp})^{\top}(\bA^{\top} \bA)^{-1} (\bA^{\top} \bomega_{\sharp})} \leq A_U,
\]
where we have let
\begin{align*}
	A_L &= \sqrt{ \frac{1}{n}\| \bomega_{\sharp}\|_2^2 - \frac{1 + C\epsilon/2}{n^2}\|\bA\bomega_{\sharp}\|_2^2} =  \sqrt{ \frac{1}{n}\| \bomega_{\sharp}\|_2^2 - \frac{1 + C\epsilon/2}{n^2}(\langle \bg, \bomega_{\sharp}\rangle^2 + \langle \bz_1, \bomega_{\sharp}\rangle^2 + \langle \bz_2, \bomega_{\sharp} \rangle^2)}\\
	A_U &= \sqrt{ \frac{1}{n}\| \bomega_{\sharp}\|_2^2 - \frac{1 - C\epsilon/2}{n^2}\|\bA\bomega_{\sharp}\|_2^2} =\sqrt{ \frac{1}{n}\| \bomega_{\sharp}\|_2^2 - \frac{1 - C\epsilon/2}{n^2}(\langle \bg, \bomega_{\sharp}\rangle^2 + \langle \bz_1, \bomega_{\sharp}\rangle^2 + \langle \bz_2, \bomega_{\sharp} \rangle^2)}, 
\end{align*}
where the last equality in both lines follows by recalling that $\bA^{\top}\bomega_{\sharp} = [\langle \bz_1, \bomega_{\sharp} \rangle, \langle \bz_2, \bomega_{\sharp}\rangle, \langle \bg, \bomega_{\sharp}]$  Now, consider the two events
\begin{align*}
	\Ac_2 = \Bigl\{\frac{1}{n^2}\lvert \langle \bg, \bomega_{\sharp} \rangle \rvert^2 \vee \Bigl\lvert \frac{1}{n^2}\langle \bz_1, \bomega_{\sharp}\rangle^2 - (\EE \{ Z_1 \Omega \})^2\Bigr\rvert \vee \Bigl\lvert \frac{1}{n^2}\langle \bz_2, \bomega_{\sharp} \rangle^2 - (\EE\{Z_2 \Omega \})^2 \Bigr \rvert \leq C\epsilon\Bigr\},
\end{align*}
and 
\begin{align*}
	\Ac_3 &= \Bigl\{\Bigl\lvert \frac{1}{n} \| \bomega_{\sharp} \|_2^2 - \EE\{\Omega^2\} \Bigr\rvert \leq C\epsilon \Bigr\}.
\end{align*}
Next, recall that by Assumption~\ref{ass:omega}, we have the bound $\| \bomega_{\sharp} \|_{\psi_2} \leq K$.  Thus, we apply Bernstein's inequality to obtain the inequality
\[
\Pro\Bigl\{ \Bigl \lvert \frac{1}{n} \langle \bz_1, \bomega_{\sharp} \rangle - \EE\{ Z_1 \Omega\}\Bigr\rvert \geq C\epsilon \Bigr\} \leq 2e^{-cn\epsilon^2}.
\]
Consequently, with probability at least $1 - 2e^{-cn\epsilon^2}$,  
\[
\Bigl\lvert\frac{1}{n^2}\langle \bz_1, \bomega_{\sharp}\rangle^2 - (\EE \{ Z_1 \Omega \})^2\Bigr\rvert = \Bigl \lvert \frac{1}{n} \langle \bz_1, \bomega_{\sharp} \rangle - \EE\{ Z_1 \Omega\}\Bigr\rvert \cdot \Bigl \lvert \frac{1}{n} \langle \bz_1, \bomega_{\sharp} \rangle + \EE\{ Z_1 \Omega\}\Bigr\rvert \overset{\1}{\leq} \frac{C\epsilon}{3},
\]
where step $\1$ additionally used the fact that $\EE\{Z_1 \Omega\} \leq C$.  Bounding the other terms similarly and applying the union bound, we obtain $\Pro\{\Ac_2\} \geq 1 - 6e^{-cn\epsilon^2}$.  Finally, we apply Bernstein's inequality once more to obtain the inequality $\Pro\{ \Ac_3 \} \geq 1 - 2e^{-cn\epsilon^2}$.  Thus, on the event $\Ac_2 \cap \Ac_3$, we obtain 
\[
A_L \geq \sqrt{(\EE\{\Omega^2\} - (\EE\{Z_1 \Omega\})^2 - (\EE\{Z_2 \Omega\})^2 - C\epsilon} \overset{\1}{\geq}  \sqrt{(\EE\{\Omega^2\} - (\EE\{Z_1 \Omega\})^2 - (\EE\{Z_2 \Omega\})^2} - C'\epsilon, 
\]
where step $\1$ follows since by Assumption~\ref{ass:omega}, the first terrm on the RHS is at least a small positive constant.  We additionally emphasize that the constant $C$ has changed from line to line.  Proceeding similarly, we obtain the upper bound
\[
A_U \leq \sqrt{(\EE\{\Omega^2\} - (\EE\{Z_1 \Omega\})^2 - (\EE\{Z_2 \Omega\})^2} + C'\epsilon.
\]
Putting the pieces together, we see that with probability at least $1 - 10e^{-cn\epsilon^2}$, 
\[
\Bigl\lvert \frac{1}{\sqrt{n}}\|(\bI_n - \bA(\bA^{\top} \bA)^{-1}\bA^{\top}) \cdot \omega(\bX \btsharp, \by) \|_2 -  \sqrt{(\EE\{\Omega^2\} - (\EE\{Z_1 \Omega\})^2 - (\EE\{Z_2 \Omega\})^2} \Bigr\rvert \leq C'\epsilon
\]
\fi

\noindent\underline{Bounding the denominator.} On the event $\Ac_1$, we note the sandwich relation
\[
D_L \leq \sqrt{1 - n\cdot \bv_n^{\top} (\bA^{\top} \bA)^{-1} \bv_n} \leq D_U,
\]
where we have let
\begin{align*}
	D_L &= \sqrt{1 - (1 + C\epsilon) \|\bv_n\|_2^2}, \qquad \text{ and } \qquad D_U = \sqrt{1 - (1 - C\epsilon) \|\bv_n\|_2^2}.
\end{align*}
Now, consider the event
\[
\Ac_4 = \bigl\{\bigl\lvert \| \bv_n \|_2^2 - \kappa^{-1} \bigr \rvert \leq C\epsilon \bigr\},
\]
noting that an application of Bernstein's inequality implies $\Pro\{\Ac_4\} \geq 1 - 2e^{-cn\epsilon^2}$.  Now, on the event $\Ac_4$, we further obtain the bounds
\[
D_L \geq \sqrt{1 - \kappa^{-1}} - C'\epsilon, \qquad \text{ and } \qquad D_U \leq \sqrt{1 - \kappa^{-1}} + C'\epsilon.
\]

\noindent\underline{Putting the pieces together to control $\tau_n$.}  Now, we combine the two-sided bounds on both the numerator and denominator to obtain the inequality
\begin{align}\label{ineq:probabalistic-control-taun}
\Pro\bigl\{\bigl \lvert \tau_n - \tau^{\gor} \bigr \rvert \leq C_{K_1} \cdot \epsilon \bigr\} \geq 1 - Ce^{-cn\epsilon^2}.
\end{align}

\paragraph{Bounding the minimizer $\bxi_n(\tau_n)$~\eqref{eq:unique-empirical-xi}.} First, let $\be_1$ denote the first standard basis vector in $\real^3$ and consider the quantity
\[
\lvert \langle \be_1, \bxi_n(\tau_n) \rangle - \parcomp^{\gor} \rvert = \lvert \langle \be_1, (\bA^{\top} \bA)^{-1} \bA^{\top} \omega(\bX\btsharp, \by) + \tau \cdot n \cdot (\bA^{\top} \bA)^{-1} \bv_n\rangle - \parcomp^{\gor} \rvert.
\]
First, note that on the event $\Ac_1$, we can write $n\cdot (\bA^{\top} \bA)^{-1} = \bI_3 + \bB$, where $\| \bB \|_{\mathsf{op}} \leq C\epsilon$.  We thus obtain the decomposition
\[
\lvert \langle \be_1, (\bA^{\top} \bA)^{-1} \bA^{\top} \omega(\bX\btsharp, \by) + \tau_n \cdot n \cdot (\bA^{\top} \bA)^{-1} \bv_n\rangle - \parcomp^{\gor} \rvert \leq A_1 + A_2,
\]
where
\begin{align*}
	A_1 &= \Bigl \lvert \frac{1}{n} \langle \be_1, \bA^{\top} \omega(\bX\btsharp, \by) \rangle + \tau_n \langle \be_1, \bv_n \rangle  - \alpha^{\gor}\Bigr\rvert\\
	A_2 &= \Bigl \lvert  \frac{1}{n} \langle \be_1, \bB  \bA^{\top} \omega(\bX\btsharp, \by) \rangle + \tau_n \cdot \langle \be_1, \bB \bv_n \rangle \Bigr\rvert.
\end{align*}
Now, consider the event
\begin{align*}
	\Ac_5 = \Bigl\{\frac{1}{n}\lvert \langle \bg, \bomega_{\sharp} \rangle \rvert \vee \Bigl\lvert \frac{1}{n}\langle \bz_1, \bomega_{\sharp}\rangle - \EE \{ Z_1 \Omega \}\Bigr\rvert \vee \Bigl\lvert \frac{1}{n}\langle \bz_2, \bomega_{\sharp} \rangle - \EE\{Z_2 \Omega \} \Bigr \rvert \leq C'_{K_1} \epsilon\Bigr\},
\end{align*}
and note that on $\Ac_1 \cap \Ac_2 \cap \Ac_3$, we have
\begin{align*}
	\lvert \tau_n - \tau^{\gor}\rvert \leq C_{K_1} \cdot \epsilon
\end{align*}
for a pair $(C_{K_1}, C'_{K_1})$ depending only on $K_1$. In the following lines, we note that $C_{K_1}$ may change from line to line, but always depends only on $K_1$.
Note that %by Lemma~\ref{}, $\Pro\{\Ac_1 \cap \Ac_2 \cap \Ac_3 \} \geq 1 - C e^{-cn\epsilon^2}$ and further 
by applying Bernstein's inequality,  we obtain $\Pro\{\Ac_5\} \geq 1 - 6e^{-cn\epsilon^2}$.  Working on the event $\Ac_5 \cap \Ac_1 \cap \Ac_2 \cap \Ac_3$ and applying the triangle inequality, we obtain the upper bound
\[
A_1 \leq \lvert \EE\{Z_1 \Omega\} - \parcomp^{\gor} \rvert + C_{K_1} \cdot \epsilon.
\]
Further, noting that $\| \bB \|_{\mathsf{op}} \leq C\epsilon$ and that $\EE\{Z_1 \Omega\} \leq (\EE\{Z_1^2\} \cdot \EE\{ \Omega^2 \} )^{1/2}\leq C_{K_1}$, we obtain the bound
\[
A_2 \leq \frac{1}{n}\| \bB\|_{\mathsf{op}}  \| \bA^{\top} \omega(\bX\btsharp, \by) \|_2 \leq C_{K_1} \cdot \epsilon.
\]
Summarizing, we have shown that
\begin{subequations}\label{ineq:bound-minimizers-scalarized-ao}
\begin{align}
\Pro\{\lvert \langle \be_1, \bxi_n(\tau_n) \rangle - \parcomp^{\gor} \rvert \leq C_{K_1} \cdot \epsilon\} \geq 1 - 16e^{-cn\epsilon^2}.
\end{align}
Proceeding in a parallel manner, we obtain the two bounds
\begin{align}
\Pro\{\lvert \langle \be_2, \bxi_n(\tau_n) \rangle - \perpone^{\gor} \rvert \leq C_{K_1} \cdot \epsilon\} \geq 1 - 16e^{-cn\epsilon^2},
\end{align} 
\begin{align}
	 \Pro\{\lvert \langle \be_1, \bxi_n(\tau_n) \rangle - \perptwo^{\gor} \rvert \leq  C_{K_1} \cdot \epsilon\} \geq 1 - 16e^{-cn\epsilon^2}.
\end{align}
\end{subequations}

\paragraph{Bounding the minimum $\widebar{L}_n(\bxi_n(\tau_n), \btsharp)$.}  Note that 
\[
\widebar{L}_n(\bxi_n(\tau_n); \btsharp) = \frac{1}{\sqrt{n}} \| \bA\bxi_n(\tau_n) - \omega(\bX \btsharp, \by) \|_2 - \langle \bv_n, \bxi_n(\tau_n) \rangle.
\]
Now, consider the event
\[
\Ac_6 = \{\|\bxi_n(\tau_n) - \bxi^{\gor}\|_{\infty} \leq C_{K_1} \cdot \epsilon\},
\]
noting that the inequality~\eqref{ineq:bound-minimizers-scalarized-ao} implies $\Pro\{\Ac_6\} \geq 1 - 16e^{-cn\epsilon^2}$.  For the remainder of the proof, we will work on the event $\mathcal{A} = \bigcap_{k=1}^{6} \Ac_k$.  Adding and subtracting the quantity $\xi^{\gor}$ yields
\begin{align*}
	\widebar{L}_n(\bxi_n(\tau_n); \btsharp) = \frac{1}{\sqrt{n}} \| \bA\bxi^{\gor} + \bA (\bxi_n(\tau_n) - \bxi^{\gor}) - \omega(\bX \btsharp, \by) \|_2 - \langle \bv_n, \bxi^{\gor} \rangle - \langle \bv_n, \bxi_n(\tau_n) - \bxi^{\gor} \rangle.
\end{align*}
Thus, on the event $\Ac$, we obtain the inequality
\[
\Bigl \lvert \widebar{L}_n(\bxi_n(\tau_n); \btsharp)  - \frac{1}{\sqrt{n}} \| \bA\bxi^{\gor} - \omega(\bX \btsharp, \by) \|_2 + \langle \bv_n, \bxi^{\gor} \rangle \Bigr\rvert \leq C_{K_1} \cdot \epsilon.
\]
Furthermore, on the event $\Ac$, we obtain the inequality \apcomment{Needs more explanation.}
\[
\biggl \lvert\frac{1}{\sqrt{n}} \| \bA\bxi^{\gor} - \omega(\bX \btsharp, \by) \|_2 - \langle \bv_n, \bxi^{\gor} \rangle - \sqrt{\Bigl(1 - \frac{1}{\kappa}\Bigr)\Bigl(\EE[\Omega^2] - (\EE[Z_1 \Omega])^2 - (\EE[Z_2 \Omega])^2\Bigr)} \biggr \rvert \leq C_{K_1} \cdot \epsilon.
\]
We obtain the desired result upon combining the two displays above. \qed

\subsubsection{Proof of Lemma~\ref{lem:ao-analysis}(b)}
We begin by defining the events
\begin{align} \label{eq:prime-event1}
\Ac'_1 = \Bigl\{\min_{\bxi \in \mathbb{R}^3} \frac{1}{\sqrt{n}}\| \bA \bxi - \omega(\bX \btsharp, \by) \|_2 \geq c_{K} \Bigr\},
\end{align}
\[
 \Ac'_2 = \Bigl\{ \frac{1}{2} \bI_3 \preceq \frac{1}{n} \bA^{\top} \bA \preceq 2 \bI_3\Bigr\}, \qquad \text{ and } \qquad \Ac'_3 = \Bigl\{\frac{1}{\sqrt{n}}\| \omega(\bX \btsharp, \by)\|_2 \leq C_{K_1} \Bigr\},
\]
where $c_K$ is a constant depending only on $(K_1, K_2)$.
Note that on the event $\Ac'_2 \cap \Ac'_3$, we obtain the inequality
\begin{align}\label{ineq:upper-bound-quadratic}
\max_{\bxi \in \mathbb{B}_2(C')} \frac{1}{\sqrt{n}}\| \bA \bxi - \omega(\bX \btsharp, \by)\|_2 \leq C_{K_1}.
\end{align}
Applying Lemma~\ref{lem:row-space-A} for small enough $\epsilon$ in conjunction with Assumption~\ref{ass:omega-lb} yields the inequality $\Pro\{\Ac'_1\} \geq 1 - Ce^{-c'_K \cdot n}$; applying~\citet[Theorem 6.1]{wainwright2019high} yields $\Pro\{\Ac'_2\} \geq 1 - 2e^{-cn}$; and applying Bernstein's inequality (as each component of $\omega(\bX \btsharp, \by)$ is $K$-sub-Gaussian by Assumption~\ref{ass:omega}) implies $\Pro\{\Ac'_3\} \geq 2e^{-cn}$. For the rest of the proof, we work on the event $\Ac'_1 \cap \Ac'_2 \cap \Ac'_3$. 

Note that on the event $\Ac'_1$, the function $\widebar{L}_n$ is twice continuously differentiable.  Thus, our strategy is to bound the minimum eigenvalue of the Hessian $\nabla^2 \widebar{L}_n$.  We compute
\begin{align*}
\nabla^2 \widebar{L}_n(\bxi; \btsharp) &= \frac{1}{\| \bA\bxi - \omega(\bX \btsharp, \by) \|_2} \cdot \frac{1}{\sqrt{n}} \cdot \Bigl( \bA^{\top} \bA - \frac{\bA^{\top} (\bA \bxi - \omega(\bX \btsharp, \by)(\bA \bxi - \omega(\bX\btsharp, \by))^{\top}\bA}{\| \bA\bxi - \omega(\bX \btsharp, \by) \|_2^2}\Bigr)\\
&\overset{\1}{\succeq} \frac{1}{Cn} \cdot \Bigl( \bA^{\top} \bA - \frac{\bA^{\top} (\bA \bxi - \omega(\bX \btsharp, \by)(\bA \bxi - \omega(\bX\btsharp, \by))^{\top}\bA}{\| \bA\bxi - \omega(\bX \btsharp, \by) \|_2^2}\Bigr),
\end{align*}
where step $\1$ follows on the event $\Ac'_2 \cap \Ac'_3$.  Subsequently, we utilize the variational characterization of eigenvalues to obtain
\begin{align}\label{ineq:lower-bound-mineig}
	\lambda_{\min}(\nabla^2 \widebar{L}_n(\bxi; \btsharp) ) &\geq \frac{1}{Cn} \min_{\| \bv \|_2 = 1} \langle \bv, \bA^{\top} \bA\bv \rangle - \frac{\langle \bv, \bA^{\top} (\bA \bxi - \omega(\bX \btsharp, \by)(\bA \bxi - \omega(\bX\btsharp, \by))^{\top}\bA\bv \rangle}{\| \bA\bxi - \omega(\bX \btsharp, \by) \|_2^2}\nonumber\\
	&= \frac{1}{Cn} \min_{\| \bv \|_2 = 1} \| \bA \bv \|_2^2 - \frac{\langle \bA \bv, \bA \bxi - \omega(\bX \btsharp, \by) \rangle^2}{\| \bA\bxi - \omega(\bX \btsharp, \by) \|_2^2}.
\end{align}
Next, consider the orthogonal decomposition
\[
\omega(\bX \btsharp, \by) = \bA \bxi_0 + \bomega^{\perp},
\]
where $\bA \bxi_0$ denotes an element in the row space of the random matrix $\bA$ and $\bomega^{\perp}$ is orthogonal to the row space of $\bA$.  Thus, 
\begin{align}\label{eq:variational-characterization}
	\min_{\| \bv \|_2 = 1} \| \bA \bv \|_2^2 - \frac{\langle \bA \bv, \bA \bxi - \omega(\bX \btsharp, \by) \rangle^2}{\| \bA\bxi - \omega(\bX \btsharp, \by) \|_2^2} &= \min_{\| \bv \|_2 = 1} \| \bA \bv \|_2^2 - \frac{\langle \bA \bv, \bA (\bxi - \bxi_0) - \bomega^{\perp}\rangle^2}{\| \bA(\bxi - \bxi_0)\|_2^2 + \| \bomega^{\perp} \|_2^2}\nonumber\\
	&= \min_{\| \bv \|_2 = 1} \| \bA \bv \|_2^2 - \frac{\langle \bA \bv, \bA (\bxi - \bxi_0)\rangle^2}{\| \bA(\bxi - \bxi_0)\|_2^2 + \| \bomega^{\perp} \|_2^2}\nonumber\\
	&\overset{\1}{=}  \min_{\| \bv \|_2 = 1} \| \bA \bv \|_2^2 - \frac{\| \bA \bv\|_2^2 \cdot \| \bA (\bxi - \bxi_0)\|_2^2}{\| \bA(\bxi - \bxi_0)\|_2^2 + \| \bomega^{\perp} \|_2^2},
\end{align}
where step $\1$ follows by applying the Cauchy--Schwarz inequality.  Now, 
\begin{align} \label{ineq:lower-bound-variational}
	\min_{\| \bv \|_2 = 1} \| \bA \bv \|_2^2 - \frac{\| \bA \bv\|_2^2 \cdot \| \bA (\bxi - \bxi_0)\|_2^2}{\| \bA(\bxi - \bxi_0)\|_2^2 + \| \bomega^{\perp} \|_2^2} \overset{\1}{\geq} \frac{n}{2} \cdot \frac{\| \bomega^{\perp} \|_2^2}{\| \bA(\bxi - \bxi_0)\|_2^2 + \| \bomega^{\perp} \|_2^2} \overset{\2}{\geq} c_K \cdot n
\end{align}
where step $\1$ follows on the event $\Ac'_2$ and step $\2$ follows on the event $\Ac'_1$.  Finally, combining the lower bound~\eqref{ineq:lower-bound-mineig}, the equation~\eqref{eq:variational-characterization}, and the lower bound~\eqref{ineq:lower-bound-variational}, we obtain the inequality
\[
\lambda_{\min}(\nabla^2 \widebar{L}_n(\bxi; \btsharp) ) \geq c_K,
\]
on the event $\Ac'_1 \cap \Ac'_2 \cap \Ac'_3$, which occurs with probability at least $1 - 14e^{-c'_K \cdot n}$.\qed

\subsubsection{Proof of Lemma~\ref{lem:remove-positive-restriction}}
\label{subsec:proof-lemma-remove-positive-restriction}
Recall the loss function $\Lc$~\eqref{eq:sec_order_gen}:
\[
\Lc(\bt; \btsharp, \bX, \by) = \frac{1}{\sqrt{n}} \| \omega(\bX\btsharp, \by) - \bX\bt \|_2,
\]
which corresponds to setting 
\[
F(\bu, \bt) = \| \omega(\bX\btsharp, \by) - \bu \|_2, \qquad h(\bt, \btsharp) = 0, \qquad \text{ and } \qquad g(\bu, \bX \btsharp; \by) = \| \omega(\bX\btsharp, \by) - \bu \|_2.
\]
Additionally, note that the convex conjugate is given by
\[
g^*(\bv, \bX\btsharp; \by) = \begin{cases}\langle \bv, \omega(\bX\btsharp, \by) \rangle & \text{ if } \| \bv \|_2 \leq \frac{1}{\sqrt{n}},\\
	+\infty & \text{ otherwise.} \end{cases}
\]
Substituting into the definition of the scalarized auxiliary loss $\widebar{L}_n$ (see Definition~\ref{def:scalarized-ao}), we obtain
\[
\widebar{L}_n(\alpha, \mu, \nu; \btsharp) = \biggl(\frac{1}{\sqrt{n}} \| \perptwo \cdot \bg + \parcomp \cdot \bz_1 + \perpone \cdot \bz_2 - \omega(\bX \btsharp, \by) \|_2 - \perptwo \frac{\| \proj_{S_{\sharp}}^{\perp} \bh \|_2}{\sqrt{n}}\biggr)_{+}.
\]
Now, consider the shorthand
\[
\bw = \parcomp \cdot \bz_1 + \perpone \cdot \bz_2 - \omega(\bX \btsharp, \by),
\]
and define the three events
\[
\Ec_1 = \Bigl\{\frac{1}{n}\lvert \langle \perptwo \cdot \bg, \bw\rangle \rvert \leq \frac{4\perptwo}{5\sqrt{n}}\|\bw\|_2\Bigr\}, \quad \Ec_2 = \Bigl\{\| \bg \|_2^2 \geq 4n/5\}, \quad \text{ and } \quad \Ec_3 = \{\| \bh \|_2^2 \leq 36d/25\}.
\]
Next, apply Bernstein's inequality to bound the quantity $\Pro\{\Ec_1^c\}$, Hoeffding's inequality to bound the quantities $\Pro\{\Ec_2^c\}$ and $\Pro\{\Ec_3\}$, and the union bound to obtain the inequality 
\[\Pro\{\Ec_1 \cap \Ec_2 \cap \Ec_3\} \geq 1 - 6e^{-cn}.
\]
Working on the intersection of these three events, we obtain
\begin{align*}
	\frac{1}{\sqrt{n}} \| \perptwo \cdot \bg + \bw \|_2  &= \sqrt{ \frac{4 \perptwo^2}{5n}\| \bg \|_2^2 + \frac{\perptwo^2}{5n} \| \bg \|_2^2 + \frac{1}{n}\langle \perptwo \cdot \bg, \bw \rangle + \frac{1}{n} \| \bw \|_2^2 }\\
	&\geq \sqrt{ \frac{16 \perptwo^2}{25} + \frac{4\perptwo^2}{25} - \frac{4\perptwo}{5\sqrt{n}}\| \bw \|_2 + \frac{1}{n} \| \bw \|_2^2 } = \sqrt{\frac{16 \perptwo^2}{25}  + \Bigl(\frac{2\perptwo}{5} - \frac{\| \bw \|_2}{\sqrt{n}}\Bigr)^2} \geq \frac{4\perptwo}{5}.
\end{align*}
Thus, we obtain
\[
\frac{1}{\sqrt{n}} \| \perptwo \cdot \bg + \bw \|_2 - \perptwo \frac{\| \proj_{S_{\sharp}}^{\perp} \bh \|_2}{\sqrt{n}} \geq \frac{4\perptwo}{5} - \frac{6\perptwo}{5\sqrt{\kappa}} \geq 0, 
\]
where the last inequality holds for $\kappa \geq C$ with $C$ a large enough constant.  Summarizing, we see that 
\[
\frac{1}{\sqrt{n}} \| \perptwo \cdot \bg + \parcomp \cdot \bz_1 + \perpone \cdot \bz_2 - \omega(\bX \btsharp, \by) \|_2 - \perptwo \frac{\| \proj_{S_{\sharp}}^{\perp} \bh \|_2}{\sqrt{n}} \geq 0,
\]
whence 
\[
\widebar{L}_n(\alpha, \mu, \nu; \btsharp)  = \frac{1}{\sqrt{n}} \| \perptwo \cdot \bg + \parcomp \cdot \bz_1 + \perpone \cdot \bz_2 - \omega(\bX \btsharp, \by) \|_2 - \perptwo \frac{\| \proj_{S_{\sharp}}^{\perp} \bh \|_2}{\sqrt{n}}
\]
as desired.
\qed

\subsubsection{Proof of Lemma~\ref{lem:row-space-A}}
\label{subsec:proof-lemma-row-space-A}

%\apcomment{Need to modify this proof given above change.}
Recall the three events~\eqref{eq:three-events}. We prove each part of the lemma in turn.

\paragraph{Proof of part (a):} First, let $\bomega_{\sharp} = \omega(\bX \btsharp, \by)$ and expand the norm to obtain
\[
\frac{1}{\sqrt{n}}\|(\bI_n - \bA(\bA^{\top} \bA)^{-1}\bA^{\top})\omega(\bX \btsharp, \by) \|_2 = \sqrt{ \frac{1}{n}\| \bomega_{\sharp}\|_2^2 - \frac{1}{n}(\bA^{\top}\bomega_{\sharp})^{\top}(\bA^{\top} \bA)^{-1} (\bA^{\top} \bomega_{\sharp})}.
\]
Now, on the event $\Ac_1$, we obtain the sandwich relation
\[
A_L \leq \sqrt{ \frac{1}{n}\| \bomega_{\sharp}\|_2^2 - \frac{1}{n}(\bA^{\top}\bomega_{\sharp})^{\top}(\bA^{\top} \bA)^{-1} (\bA^{\top} \bomega_{\sharp})} \leq A_U,
\]
where we have let
\begin{align*}
	A_L &= \sqrt{ \frac{1}{n}\| \bomega_{\sharp}\|_2^2 - \frac{1 + C\epsilon/2}{n^2}\|\bA\bomega_{\sharp}\|_2^2} =  \sqrt{ \frac{1}{n}\| \bomega_{\sharp}\|_2^2 - \frac{1 + C\epsilon/2}{n^2}(\langle \bg, \bomega_{\sharp}\rangle^2 + \langle \bz_1, \bomega_{\sharp}\rangle^2 + \langle \bz_2, \bomega_{\sharp} \rangle^2)}\\
	A_U &= \sqrt{ \frac{1}{n}\| \bomega_{\sharp}\|_2^2 - \frac{1 - C\epsilon/2}{n^2}\|\bA\bomega_{\sharp}\|_2^2} =\sqrt{ \frac{1}{n}\| \bomega_{\sharp}\|_2^2 - \frac{1 - C\epsilon/2}{n^2}(\langle \bg, \bomega_{\sharp}\rangle^2 + \langle \bz_1, \bomega_{\sharp}\rangle^2 + \langle \bz_2, \bomega_{\sharp} \rangle^2)}, 
\end{align*}
where the last equality in both lines follows by recalling that $\bA^{\top}\bomega_{\sharp} = [\langle \bz_1, \bomega_{\sharp} \rangle, \langle \bz_2, \bomega_{\sharp}\rangle, \langle \bg, \bomega_{\sharp} \rangle ]$. 
On the event $\Ac_2 \cap \Ac_3$, we obtain 
\[
A_L \geq \sqrt{(\EE\{\Omega^2\} - (\EE\{Z_1 \Omega\})^2 - (\EE\{Z_2 \Omega\})^2 - C_{K_1} \epsilon} \overset{\1}{\geq}  \sqrt{(\EE\{\Omega^2\} - (\EE\{Z_1 \Omega\})^2 - (\EE\{Z_2 \Omega\})^2} - C_K \cdot \epsilon, 
\]
where step $\1$ follows since by Assumption~\ref{ass:omega-lb}, the first term on the RHS is at least $K_2$.  
%We additionally emphasize that the constant $C$ has changed from line to line.  
Proceeding similarly, we obtain the upper bound
\[
A_U \leq \sqrt{(\EE\{\Omega^2\} - (\EE\{Z_1 \Omega\})^2 - (\EE\{Z_2 \Omega\})^2} + C'_K \epsilon.
\]
Putting the pieces together, we see that with probability at least $1 - 10e^{-cn\epsilon^2}$, 
\[
\Bigl\lvert \frac{1}{\sqrt{n}}\|(\bI_n - \bA(\bA^{\top} \bA)^{-1}\bA^{\top}) \cdot \omega(\bX \btsharp, \by) \|_2 -  \sqrt{(\EE\{\Omega^2\} - (\EE\{Z_1 \Omega\})^2 - (\EE\{Z_2 \Omega\})^2} \Bigr\rvert \leq C_K \epsilon,
\]
as claimed. \qed

\paragraph{Proof of part (b):} From~\citet[Theorem 6.1]{wainwright2019high}, we directly have $\Pro\{ \Ac_1 \} \geq 1 - C e^{-cn\epsilon^2}$. Next, recall for convenience the other two events
\begin{align*}
	\Ac_2 = \Bigl\{\frac{1}{n^2}\lvert \langle \bg, \bomega_{\sharp} \rangle \rvert^2 \vee \Bigl\lvert \frac{1}{n^2}\langle \bz_1, \bomega_{\sharp}\rangle^2 - (\EE \{ Z_1 \Omega \})^2\Bigr\rvert \vee \Bigl\lvert \frac{1}{n^2}\langle \bz_2, \bomega_{\sharp} \rangle^2 - (\EE\{Z_2 \Omega \})^2 \Bigr \rvert \leq C_{K_1} \cdot \epsilon\Bigr\},
\end{align*}
and 
\begin{align*}
	\Ac_3 &= \Bigl\{\Bigl\lvert \frac{1}{n} \| \bomega_{\sharp} \|_2^2 - \EE\{\Omega^2\} \Bigr\rvert \leq C_{K_1} \cdot \epsilon \Bigr\}.
\end{align*}
Next, recall that by Assumption~\ref{ass:omega}, we have the bound $\| \bomega_{\sharp} \|_{\psi_2} \leq K_1$.  Thus, we apply Bernstein's inequality to obtain 
\[
\Pro\Bigl\{ \Bigl \lvert \frac{1}{n} \langle \bz_1, \bomega_{\sharp} \rangle - \EE\{ Z_1 \Omega\}\Bigr\rvert \geq C_{K_1} \cdot \epsilon \Bigr\} \leq 2e^{-cn\epsilon^2}.
\]
Consequently, with probability at least $1 - 2e^{-cn\epsilon^2}$,  
\[
\Bigl\lvert\frac{1}{n^2}\langle \bz_1, \bomega_{\sharp}\rangle^2 - (\EE \{ Z_1 \Omega \})^2\Bigr\rvert = \Bigl \lvert \frac{1}{n} \langle \bz_1, \bomega_{\sharp} \rangle - \EE\{ Z_1 \Omega\}\Bigr\rvert \cdot \Bigl \lvert \frac{1}{n} \langle \bz_1, \bomega_{\sharp} \rangle + \EE\{ Z_1 \Omega\}\Bigr\rvert \overset{\1}{\leq} C_{K_1} \cdot \epsilon,
\]
where step $\1$ additionally used the fact that $\EE\{Z_1 \Omega\} \leq C_{K_1}$.  Bounding the other terms similarly and applying a union bound, we obtain $\Pro\{\Ac_2\} \geq 1 - 6e^{-cn\epsilon^2}$.  Finally, we apply Bernstein's inequality once more to obtain the inequality $\Pro\{ \Ac_3 \} \geq 1 - 2e^{-cn\epsilon^2}$. \qed

\iffalse
\apcomment{Old.}
We begin by introducing the shorthand
\[
\bomega_{\sharp} = \omega(\bX\btsharp, \by).
\]
Now, note the inequality
\begin{align*}
	\frac{1}{n} \| \bA\bxi - \bomega_{\sharp} \|_2^2 &\overset{\1}{\geq} \frac{1}{n} \| (\bI_n - \bA(\bA^{\top}\bA)^{-1}\bA^{\top})\bomega_{\sharp} \|_2^2\\
	&= \frac{1}{n}\| \bomega_{\sharp}\|_2^2 - \frac{1}{n}(\bA\bomega_{\sharp})^{\top}(\bA^{\top} \bA)^{-1} (\bA \bomega_{\sharp}),
\end{align*}
where step $\1$ follows by minimizing the LHS in $\bxi$.  Next, let $0 < c' < 1$ be a small constant and define the event 
\begin{align*}
	\Ac_1 &= \Bigl\{(1 - c') \bI_3 \preceq \frac{1}{n} \bA^{\top} \bA \preceq (1 + c') \bI_3 \Bigr\},
\end{align*}
and note that on the event $\Ac_1$, we further obtain the inequality
\begin{align}
	\label{ineq:row-space-ineq1}
	\frac{1}{n} \| \bA\bxi - \bomega_{\sharp} \|_2^2 \geq \frac{1}{n}\| \bomega_{\sharp}\|_2^2 - \frac{1 + c''}{n^2}\|\bA\bomega_{\sharp}\|_2^2 \overset{\1}{=} \frac{1}{n}\| \bomega_{\sharp}\|_2^2 - \frac{1 + c''}{n^2}\Bigl(\langle \bg, \bomega_{\sharp}\rangle^2 + \langle \bz_1, \bomega_{\sharp}\rangle^2 + \langle \bz_2, \bomega_{\sharp}\rangle^2\Bigr),
\end{align}
where step $\1$ follows by recalling that $\bA\bomega_{\sharp} = [\langle \bg, \bomega_{\sharp} \rangle, \langle \bz_1, \bomega_{\sharp}\rangle, \langle \bz_2, \bomega_{\sharp} \rangle]$
and consider the two events
\begin{align*}
	\Ac_2 = \Bigl\{\frac{1}{n^2}\lvert \langle \bg, \bomega_{\sharp} \rangle \rvert^2 \vee \Bigl\lvert \frac{1}{n^2}\langle \bz_1, \bomega_{\sharp}\rangle^2 - (\EE \{ Z_1 \Omega \})^2\Bigr\rvert \vee \Bigl\lvert \frac{1}{n^2}\langle \bz_2, \bomega_{\sharp} \rangle^2 - (\EE\{Z_2 \Omega \})^2 \Bigr \rvert \leq c'\Bigr\},
\end{align*}
and 
\begin{align*}
	\Ac_3 &= \Bigl\{\Bigl\lvert \frac{1}{n} \| \bomega_{\sharp} \|_2^2 - \EE\{\Omega^2\} \Bigr\rvert \leq c' \Bigr\}.
\end{align*}
%\begin{align*}
%	\Ac_1 &= \Bigl\{\Bigl\lvert \frac{1}{n} \| \bomega_{\sharp} \|_2^2 - \EE\{\Omega^2\} \Bigr\rvert \leq c' \Bigr\}, \qquad 	&&\Ac_2 = \Bigl\{\frac{1}{n^2}\lvert \langle \bg, \bomega_{\sharp} \rangle \rvert^2 \leq c'\Bigr\},\\ 
%	\Ac_3 &= \Bigl\{ \Bigl\lvert \frac{1}{n^2}\langle \bz_1, \bomega_{\sharp}\rangle - (\EE \{ Z_1 \Omega \})^2\Bigr\rvert \leq c'\Bigr\}, \qquad \text{ and } \qquad &&\Ac_4 = \Bigl\{\Bigl\lvert \frac{1}{n^2}\langle \bz_2, \bomega_{\sharp} \rangle - (\EE\{Z_2 \Omega \})^2 \Bigr \rvert \leq c'\Bigr\}.
%\end{align*}
Working on the intersection of the above two events, we further lower bound the RHS of the inequality~\eqref{ineq:row-space-ineq1} to obtain the inequality 
\[
\frac{1}{n} \| \bA\bxi - \bomega_{\sharp} \|_2^2 \geq \EE\{ \Omega^2\} - \EE\{ Z_1 \Omega\}^2 - \EE\{ Z_2 \Omega\}^2 - c'\cdot (1 + 3c'') \overset{\1}{\geq} c > 0,
\]
where step $\1$ follows by Assumption~\ref{ass:omega}.  

The proof is complete upon bounding the probability $\Pro\{\Ac_1 \cap \Ac_2 \cap \Ac_3\}$.  First, we apply~\cite[Theorem 6.1]{wainwright2019high} to control the minimum and maximum singular values of the Wishart matrix $\bA$ in conjunction with the assumption that $n \geq C$ to obtain $\Pro\{\Ac_1\} \geq 1 - 2e^{-cn}$.  Next, recall that by Assumption~\ref{ass:omega}, we have the bound $\| \bomega_{\sharp} \|_{\psi_2} \leq K$.  Thus, we apply Bernstein's inequality to obtain the bound
\[
\Pro\Bigl\{ \Bigl \lvert \frac{1}{n} \langle \bz_1, \bomega_{\sharp} \rangle - \EE\{ Z_1 \Omega\}\Bigr\rvert \geq \frac{c'}{C} \Bigr\} \leq 2e^{-cn}.
\]
Consequently, with probability at least $1 - 2e^{-cn}$,  
\[
\Bigl\lvert\frac{1}{n^2}\langle \bz_1, \bomega_{\sharp}\rangle^2 - (\EE \{ Z_1 \Omega \})^2\Bigr\rvert = \Bigl \lvert \frac{1}{n} \langle \bz_1, \bomega_{\sharp} \rangle - \EE\{ Z_1 \Omega\}\Bigr\rvert \cdot \Bigl \lvert \frac{1}{n} \langle \bz_1, \bomega_{\sharp} \rangle + \EE\{ Z_1 \Omega\}\Bigr\rvert \overset{\1}{\leq} \frac{c'}{3},
\]
where step $\1$ additionally used the fact that $\EE\{Z_1 \Omega\} \leq C$.  Bounding the other terms similarly and applying the union bound, we obtain $\Pro\{\Ac_2\} \geq 1 - 6e^{-cn}$.  Finally, we apply Bernstein's inequality once more to obtain the inequality $\Pro\{ \Ac_3 \} \geq 1 - 2e^{-cn}$.  Putting the pieces together, we obtain the result. \qed
\fi

\subsubsection{Proof of Lemma~\ref{lem:minimize-lbar-higher-order}}
\label{subsec:proof-lemma-minimize-lbar}
We note the following characterization
\begin{align}
	\label{eq:tau-characterization}
	\min_{\bxi \in \Pc(\mathbb{B}_2(C) )} \widebar{L}_n(\bxi; \btsharp) &= \min_{\bxi \in \Pc(\mathbb{B}_2(C) )} \inf_{\tau > 0}\; \frac{\tau}{2} + \frac{1}{2\tau n} \| \bA \bxi - \omega(\bX \btsharp, \by) \|_2^2 - \langle \bv_n, \bxi \rangle \nonumber \\
	&=  \inf_{\tau > 0}\min_{\bxi \in \Pc(\mathbb{B}_2(C) )}\; \frac{\tau}{2} + \frac{1}{2\tau n} \| \bA \bxi - \omega(\bX \btsharp, \by) \|_2^2 - \langle \bv_n, \bxi \rangle,
\end{align}
where the interchange follows on event $\Ac'_1$~\eqref{eq:prime-event1}, which implies that the infimum over $\tau$ is achieved.  Next, we note that the inner minimization admits the unique minimizer
\[
\bxi_n(\tau) = (\bA^{\top} \bA)^{-1} \bA^{\top} \omega(\bX\btsharp, \by) + \tau \cdot n \cdot (\bA^{\top} \bA)^{-1} \bv_n.
\]
Substituting this value into the RHS of the optimization problem~\eqref{eq:tau-characterization} yields
\begin{align}
	\label{eq:opt-tau}
	\min_{\bxi \in \Pc(\mathbb{B}_2(C) )} \widebar{L}_n(\bxi; \btsharp) &= \inf_{\tau > 0} \; \frac{\tau}{2} + \frac{1}{2\tau n} \| \bA \bxi_n(\tau) - \omega(\bX \btsharp, \by) \|_2^2 - \langle \bv_n, \bxi_n(\tau) \rangle\nonumber\\
	&=\inf_{\tau > 0}\;\frac{1}{2\tau n}\|(\bI_n-\bA(\bA^{\top}\bA)^{-1}\bA^{\top})\omega(\bX \btsharp, \by)\|_2^2 + \frac{\tau}{2}(1-n\cdot\bv_n^{\top}(\bA^{\top}\bA)^{-1}\bv_n)\nonumber\\
	&\qquad\;\;\;-\bv_n^{\top}(\bA^{\top}\bA)^{-1}\bA\omega(\bX \btsharp, \by).
\end{align}
Consider the events
\[
\Ac''_1 = \{ \| \bh \|_2^2 \leq 36d/25\} \qquad \text{ and } \qquad \Ac''_2 = \Bigl\{(1 - c') \bI_3 \preceq \frac{1}{n} \bA^{\top} \bA \preceq (1 + c') \bI_3 \Bigr\}.
\]
Apply Bernstein's inequality to obtain $\Pro\{\Ac''_1\} \geq 1 - 2e^{-cn}$ and apply~\citet[Theorem 6.1]{wainwright2019high} to obtain $\Pro\{\Ac''_2\} \geq 1 - 2e^{-cn}$.  On the event $\Ac''_1 \cap \Ac''_2$, note that 
\[
1 - n\cdot\bv_n^{\top}(\bA^{\top}\bA)^{-1}\bv_n \geq 1 - (1 + c'/2) \| \bv_n \|_2^2 \geq 1 - (1 + c'/2) \cdot \frac{6}{5 \kappa} > 0.
\]
Thus, on the event $\Ac'_1 \cap \Ac''_1 \cap \Ac''_2$, the optimization problem~\eqref{eq:opt-tau} admits the unique minimizer
\[
\tau_n = \frac{\frac{1}{\sqrt{n}}\|(\bI_n - \bA(\bA^{\top} \bA)^{-1}\bA^{\top}) \cdot \omega(\bX \btsharp, \by) \|_2}{\sqrt{1 - n\cdot \bv_n^{\top} (\bA^{\top} \bA)^{-1} \bv_n}}.
\]
\qed

\subsection{Establishing growth conditions for first-order methods} \label{sec:growth-FO}
%\label{subsec:proof-ao-analysis-first-order}
In this subsection, we prove Lemma~\ref{lem:ao-analysis-FO}. Note that the events in this section are unrelated to
events defined in Section~\ref{sec:growth-HO}. Also note that universal constants, as well as those depending on $(K_1, K_2)$
may change from line to line.
%specialized to first-order methods.  To this end, 
Consider the first order loss as in equation~\eqref{eq:GD_gen}
\[
\Lc(\bt; \btsharp, \bX, \by) = \frac{1}{2} \| \bt \|_2^2 - \langle \bt, \btsharp \rangle - \frac{2\eta}{n} \sum_{i=1}^{n} \omega(\langle \bx_i, \btsharp \rangle, y_i) \cdot \langle \bx_i, \bt \rangle,
\]
which corresponds to setting
\[
h(\bt, \btsharp) = \frac{1}{2} \| \bt\|_2^2 - \langle \bt, \btsharp \rangle, \qquad \hscal(\parcomp, \perpone, \perptwo) = \frac{1}{2}(\parcomp^2 + \perpone^2 + \perptwo^2) - (\parcomp \parcomp_{\sharp} + \perpone \perpcomp_{\sharp}),
\]
and 
\[
g(\bu, \bX \btsharp; \by) = -\frac{2\eta}{n} \langle \bu, \omega(\bX \btsharp, \by) \rangle.
\]
Note that 
\[
g^*(\bv, \bX\btsharp; \by) = \begin{cases} 0 & \text{ if } \bv = \frac{2\eta}{n}\cdot \omega(\bX\btsharp, \by), \\
	+\infty & \text{ otherwise}.\end{cases}
\]
Consequently, we obtain
\begin{align} \label{eq:Lbar-first-order}
\widebar{L}_n(\parcomp, \perpone, \perptwo) = \;&\frac{\parcomp^2 + \perpone^2 + \perptwo^2}{2} - (\parcomp \parcomp_{\sharp} + \perpone \perpcomp_{\sharp}) - \frac{2\eta}{n} \cdot \langle \omega(\bX\btsharp, \by), \perptwo \bg + \parcomp \bz_1 + \perpone \bz_2 \rangle \nonumber\\
&- \frac{2 \eta \perptwo}{n} \cdot \| \proj_{S_{\sharp}}^{\perp} \bh\|_2 \cdot \| \omega(\bX\btsharp, \by) \|_2.
\end{align}
Note that the $2$-strong convexity claimed in part (b) of the lemma is evident from the expression above, so we focus our attention on proving part (a) in the next subsection.

\subsubsection{Proof of Lemma~\ref{lem:ao-analysis-FO}(a)}
Evidently, $\widebar{L}_n$~\eqref{eq:Lbar-first-order} is strongly convex and continuously differentiable.  The optimizers are given by the first order conditions
\begin{subequations}
	\begin{align}\label{eq:first-order-minimizers}
		\parcomp_n &= \parcomp_{\sharp} + \frac{2\eta}{n} \cdot \langle \bz_1, \omega(\bX\btsharp, \by) \rangle \\
		\perpone_n &= \perpcomp_{\sharp} + \frac{2 \eta}{n} \cdot \langle \bz_2, \omega(\bX \btsharp, \by) \rangle \\
		\perptwo_n &= \frac{2\eta}{n} \cdot \langle \bg, \omega(\bX\btsharp, \by) \rangle + \frac{2\eta}{n} \cdot \| \proj_{S_{\sharp}}^{\perp} \bh\|_2 \cdot \| \omega(\bX \btsharp, \by) \|_2.
	\end{align}
\end{subequations}
Now, consider the events
\[
\Ac_1 = \Bigl\{\Bigl \lvert \frac{1}{n} \langle \bg, \omega(\bX \btsharp, \by) \rangle \Bigr \rvert  \vee \Bigl \lvert \frac{1}{n} \langle \bz_1, \omega(\bX \btsharp, \by) \rangle - \EE\{ Z_1 \Omega\} \Bigr \rvert \vee \Bigl \lvert \frac{1}{n} \langle \bz_2, \omega(\bX \btsharp, \by) \rangle - \EE\{ Z_2 \Omega\} \Bigr \rvert  \leq C_{K_1} \cdot \epsilon \Bigr\},
\]
and 
\[
\Ac_2 = \Bigl\{\Bigl \lvert \frac{1}{\sqrt{n}} \| \proj_{S_{\sharp}}^{\perp} \bh \|_2 - \kappa^{-1/2} \Bigr \rvert \vee \Bigl \lvert \frac{1}{\sqrt{n}} \| \omega(\bX\btsharp, \by) \|_2 - \sqrt{\EE\{\Omega^2\}} \Bigr\rvert \leq C_{K_1} \cdot \epsilon\}, 
\]
and apply Bernstein's inequality to obtain the bound $\Pro\{\Ac_1 \cap \Ac_2\} \geq 1 - 10e^{-cn\epsilon^2}$.  Consequently, on the event $\Ac_1 \cap \Ac_2$, we obtain 
\[
\Pro\{ \| [\parcomp_n, \perpone_n, \perptwo_n] - [\parcomp^{\gor}, \perpone^{\gor}, \perptwo^{\gor}]\|_{\infty} \leq C_{K_1} \cdot \epsilon\} \geq 1 - 20e^{-cn\epsilon^2}
\]
Additionally, substitute the empirical minimizers~\eqref{eq:first-order-minimizers} into the loss $\widebar{L}_n$~\eqref{eq:Lbar-first-order} to obtain
\[
\widebar{L}_n(\parcomp_n, \perpone_n, \perptwo_n) =\; - \frac{1}{2}\cdot (\parcomp_n^2 + \perpone_n^2 + \perptwo_n^2).
\]
Now, define the constant
\[
\bar{\mathsf{L}} = - \frac{1}{2}\cdot ((\parcomp^{\gor})^2 + (\perpone^{\gor})^2 + (\perptwo^{\gor})^2),
\]
and note that on the event $\Ac_1 \cap \Ac_2$, we obtain
\[
\lvert \widebar{L}_n(\parcomp_n, \perpone_n, \perptwo_n) - \bar{L}\rvert \leq \frac{C_{K_1} \cdot \epsilon}{2}\Bigl(\lvert \parcomp_n + \parcomp^{\gor} \rvert + \lvert \perpone_n + \perpone^{\gor} \rvert + \lvert \perptwo_n + \perptwo^{\gor} \rvert \Bigr) \leq C'_{K_1} \cdot  \epsilon,
\]
where the final line follows since $\alpha^\gor \vee \mu^\gor \vee \nu^\gor \leq C_{K_1}$. \apcomment{Justify?}
This completes the proof. \qed

==> sections/gordon/gordon-proofs.tex <==
% ==================================================== %
%\subsection{Proofs of Lemmas}\label{sec:lem_proofs}

\subsubsection{Proof of Lemma \ref{lem:minmax}}\label{sec:minmax_proof}
In the proof below $c,C,C_i$ are absolute positive constants whose values can change from line to line.

First, we prove that with probability $1-Ce^{-cn}$ and $C_1\geq 2 C_{\theta}$:
\begin{align}\label{eq:eqv1}
\min_{\theta\in\bar\Dc} \Lc_t(\theta) = \min_{\theta\in\bar\Dc\cap\Bc_2(C_1)} \Lc_t(\theta).
\end{align}
Start with the case $\bar\Dc=\R^d$, then the desired follows directly by Assumption \ref{ass:theta_bd}. Next, consider $\bar\Dc=\Sc_\eps^c$. For the sake of contradiction suppose that in the high probability event of Assumption \ref{ass:theta_bd} the following is true:
\begin{align}\label{eq:contra1}
\Lc_t(\theta_\eps) = \min_{\theta\in\bar\Sc_\eps^c} \Lc_t(\theta) < \min_{\theta\in\bar\Dc\cap\Sc_\eps^c} \Lc_t(\theta) = \Lc_t(\theta_c),
\end{align}
where the existence of $\theta_c$ is because of the extreme value theorem and of $\theta_\eps$ by {coercivity} of $\Lc$ as per Assumption \ref{ass:loss}. If this were true, then $\theta_\eps\not\in\Bc_2(C_1)$. Consider the unconstrained minimizer $\thetanext$. Since $\thetanext\in\Bc_2(C_1)$  there exists $\rho\in(0,1)$ such that $\theta_\rho=\rho\thetanext+(1-\rho)\theta_\eps\in\Bc_2(C_1)\cap\Sc_\eps^c$. But from  convexity of $\Lc_t$, optimality of $\theta_c$, contradiction assumption \eqref{eq:contra1} and $\rho>0$:
$$
\rho\Lc_t(\thetanext)+(1-\rho)\Lc_t(\theta_\eps) \geq \Lc_t(\theta_\rho) \geq \Lc_t(\theta_c) > \Lc_t(\theta_\eps) \implies \Lc_t(\thetanext)>\Lc_t(\theta_\eps),
$$
contradicting optimality of $\thetanext$. This proves \eqref{eq:eqv1}.

	
%\begin{align}\label{eq:eqv1}
%\min_{\theta\in\R^n} \Lc_t(\theta) = \min_{\|\theta\|\leq C_1} \Lc_t(\theta).
%\end{align}

Second, we prove that with the desired high probability:
\begin{align}\label{eq:eqv2}
\min_{\theta\in\bar\Dc\cap\Bc_2(C_1)} \Lc_t(\theta) = \min_{ \substack{\theta\in\bar\Dc\cap\Bc_2(C_1) \\ \|\ub\|_2\leq C_2\sqrt{n} } } \; \Fc_t(\ub,\theta) ~~\text{sub. to}\quad \ub=\X\theta.
\end{align}
For this, recall that $\Lc_t(\theta) = h(\theta, \thetacur) + \frac{1}{n} \sum_{i = 1}^n g(\langle \bx_i, \theta \rangle, \langle \bx_i, \thetacur \rangle; y_i) = \Fc_t(\langle \bx_i, \theta \rangle,\theta)$. To see why the ball constraint on the `dummy' variable $\ub\in\R^n$, note for any feasible $\theta\in\bar\Dc\cap\Bc_2(C_1) $ that with probability at least $1-Ce^{cn}$ (e.g. \cite[Cor.~7.3.3]{VerBook}):
\begin{align}
\|\X\theta\|_2\leq \|\X\|_2\|\theta\|_2 
\leq 2 \, C_1 \, \left(\sqrt{n}+\sqrt{d}\right)
= 4\, C_1 \sqrt{n} =: C_2\,\sqrt{n}.
\end{align}
%\ct{Fix the remaining of the proof to adjust for $\bar\Dc,\Dc$}
%Using this, \eqref{eq:eqv1} and recalling that $\Lc_t(\theta) = h(\theta, \thetacur) + \frac{1}{n} \sum_{i = 1}^n g(\langle \bx_i, \theta \rangle, \langle \bx_i, \thetacur \rangle; y_i)$, we can write
%\begin{align}\label{eq:eqv2}
%\min_{\theta\in\R^n} \Lc_t(\theta) = \min_{ \substack{\|\theta\|_2\leq C_1 \\ \|\ub\|_2\leq C_2\sqrt{n} } } \; \Fc_t(\ub,\theta) ~~\text{sub. to}\quad \ub=\X\theta.
%\end{align}

%\begin{lemma}
%Consider convex functions $f:\R^n\times\R^d\rightarrow\R$ and $g:\R^n\times\R^d\rightarrow\R^m$. Further assume that the function $f$ is L-Lipschitz. Then, the following is true:
%\begin{align}\label{eq:lemma_minmax_state}
%\Big\{\min_{\theta,\ub} f(\ub,\theta)\quad\text{sub. to}\quad g(\ub,\theta)\leq 0, ~i\in[m] \Big\}~=~\min_\x\max_{\vb_i} f(\x) + \sum_{i\in[m]}\inp{\vb_i}{g_i(\x)}
%\end{align}
%\end{lemma}
%\begin{proof}
%For convenience, let $L,R$ denote the LHS and RHS of \eqref{eq:lemma_minmax_state}, respectively.
%Clearly,
%\begin{align*}
%L~=~\min_\x\max_{\vb_i} f(\x) + \sum_{i\in[m]}\inp{\vb_i}{g_i(\x)}
%\geq R.
%\end{align*}
%Thus, it suffices to show that $R\leq L$.
%\end{proof}

To finish the proof, we will use Assumption \ref{ass:Lip} to prove that when \eqref{eq:eqv1} and \eqref{eq:eqv2} hold it is true that
\begin{align}\label{eq:eqv3}
\min_{\theta\in\bar\Dc} \Lc_t(\theta)
 = \,\, \min_{ \substack{\theta\in\bar\Dc\cap\Bc_2(C_1) \\ \|\ub\|_2\leq C_2\sqrt{n} } } \; \max_{\|\vb\|_2\leq  C_3 } \; \;\Fc_t(\ub,\theta) - \frac{1}{\sqrt{n}}\langle \vb, \ub - \X\theta\rangle\,,
\end{align}
with $C_3=C_3(R):=2C_L(R)$ where $C_L(R)/\sqrt{n}$ is the Lipschitzness constant in Assumption \ref{ass:Lip}. 

The first observations is that that
\begin{align*}
\text{LHS of  }\eqref{eq:eqv3} \stackrel{\eqref{eq:eqv1}}{=} \min_{\theta\in\bar\Dc\cap\Bc_2(C_1)} \Lc_t(\theta) &\stackrel{\eqref{eq:eqv2}}{=}  \min_{ \substack{\theta\in\bar\Dc\cap\Bc_2(C_1) \\ \|\ub\|_2\leq C_2\sqrt{n} } } \; \Fc_t(\ub,\theta) ~~\text{sub. to}\quad \ub=\X\theta\\
\\
&= \min_{ \substack{\theta\in\bar\Dc\cap\Bc_2(C_1) \\ \|\ub\|_2\leq C_2\sqrt{n} } } \; \max_{\vb } \; \;\Fc_t(\ub,\theta) - \frac{1}{\sqrt{n}}\langle \vb, \ub - \X\theta\rangle ~\geq~
\text{RHS of  }\eqref{eq:eqv3}
\end{align*}
Hence, it suffices to prove the reverse side of the inequality. The desired claim follows by the following chain of inequalities
\begin{align*}
&\text{RHS of  }\eqref{eq:eqv3} \stackrel{(\text{Ass. \ref{ass:Lip}})}{\geq}\min_{ \substack{\theta\in\bar\Dc\cap\Bc_2(C_1)  \\ \|\ub\|_2\leq C_2\sqrt{n} } } \; \max_{\|\vb\|_2\leq C_3 } \; \; \Fc_t(\X\theta,\theta) - \frac{C_L(R)}{\sqrt{n}}\|\ub-\X\theta\|_2 - \frac{1}{\sqrt{n}}\langle \vb, \ub - \X\theta\rangle\nn\\
&\qquad= \min_{ \substack{\theta\in\bar\Dc\cap\Bc_2(C_1)  \\ \|\ub\|_2\leq C_2\sqrt{n} } } \; \max_{0\leq \rho_\vb\leq C_3} \; \Lc_t(\theta) - \frac{C_L(R)}{\sqrt{n}}\|\ub-\X\theta\|_2 -  \frac{1}{\sqrt{n}}\min_{\|\vb\|_2=\rho_\vb} \; \; \langle \vb, \ub - \X\theta\rangle\nn\\
&\qquad= \min_{ \substack{\theta\in\bar\Dc\cap\Bc_2(C_1)  \\ \|\ub\|_2\leq C_2\sqrt{n} } } \; \max_{0\leq \rho_\vb\leq C_3} \;\Lc_t(\theta) + \big(\rho_\vb - C_L(R)\big)\frac{\|\ub-\X\theta\|_2 }{\sqrt{n}}\\
&\quad\stackrel{(C_3>C_L(R))}{\geq} \min_{\substack{\theta\in\bar\Dc\cap\Bc_2(C_1)  \\ \|\ub\|_2\leq C_2\sqrt{n} }} \Lc_t(\theta) = \min_{\theta\in\bar\Dc\cap\Bc_2(C_1) } \Lc_t(\theta)\\
&\qquad\stackrel{\eqref{eq:eqv1}}{=} \text{LHS of  }\eqref{eq:eqv3}
\end{align*}
%But clearly by evaluating the objective of the RHS of \eqref{eq:eqv3} at the feasible point $\theta=\thetanext,\ub=\X\thetanext$ it also holds that 
%$$
%\text{RHS of  }\eqref{eq:eqv3} \leq \min_{\theta\in\R^n} \Lc_t(\theta).
%$$
Combining the above two displays proves \eqref{eq:eqv3} completing the proof of the first statement of the lemma.

Next, we prove \eqref{eq:pro_bd}. We have the following chain of inequalities
 \begin{align}
 \Pro\left\{\thetanext\not\in\Sc_\eps \right\} &= \Pro\left\{ \min_{\theta\in\Sc_\eps^c} \Lc_t(\theta) \leq \min_{\theta\in\R^d} \Lc_t(\theta) \right\} \nn
\\
&\leq \Pro\left\{ \min_{\theta\in\Sc_\eps^c} \Lc_t(\theta) \leq \min_{\theta\in\R^d} \Lc_t(\theta) \,\big|\, 
 \Phi_{n,\Bc_2(C_1)} = \min_{\theta\in\R^d} \Lc_t(\theta),  \Phi_{n,\Bc_2(C_1)\cap\Sc_\eps^c} = \min_{\theta\in\Sc_\eps^c} \Lc_t(\theta) 
  \right\}  +  Ce^{-cn}.\nn\\
&=  \Pro\left\{  \Phi_{n,\Bc_2(C_1)\cap\Sc_\eps^c} \leq \Phi_{n,\Bc_2(C_1)}  \right\} \nn\\
  &= \Pro\left\{\hat\thetanext\not\in\Sc_\eps \right\} +  Ce^{-cn}.
\end{align}
This completes the proof of the lemma.

%\subsubsection{Proof of }
\subsubsection{Proof of \eqref{eq:conAO2}}
\label{sec:proof_unbd_v}

For convenience, let $A$ and $B$ denote the optimal costs of the constrained minimization in the RHS of \eqref{eq:conAO2} and of the min-max optimization in the RHS of \eqref{eq:sec_ao}. Clearly,
$$
A = \min_{ \substack{ (\xi,\alpha,\beta)\in\Dc_3 \\ \|\ub\|_2\leq C_2\sqrt{n} } }  \; \sup_{\rho_\vb\geq 0 }\Fc_t(\ub,\theta)+ \frac{\rho_\vb}{\sqrt{n}}\left(\Big\| \beta \g+ \X P_{S^t}\theta - \ub  \Big\|_2- \beta \|P^{\perp}_{S^t}\h\|_2\right).
$$
Thus, $A\geq B$. Now, we will show the other side of the inequality. 

For this let $\Oc\in\Dc_3\times \Bc_2(C_2\sqrt{n})$ denote the set of minimal values of the optimization in the RHS of \eqref{eq:sec_ao}. We assume that \emph{all} $(\xi,\alpha,\beta,\ub)\in\Oc$ are such that the constraint 
\begin{align}
f(\xi,\alpha,\beta,\ub) :=\Big\| \beta \g+ \X P_{S^t}\theta - \ub  \Big\|_2- \beta \|P^{\perp}_{S^t}\h\|_2 \leq 0\label{eq:f_con}
\end{align}
is \emph{not} satisfied, since otherwise it holds easily that $B\geq A$, as desired. 
Let then
$$
m_{\Oc} = \min_{(\xi,\alpha,\beta,\ub)\in\Oc}f(\xi,\alpha,\beta,\ub)>0,
$$
where the minimum is attained by the extreme value theorem.
%So, considering $(\xi,\alpha,\beta,\ub)\in\Oc$ such that $f(\xi,\alpha,\beta,\ub)>0$, we 

Now, fix arbitrary $(\xi,\alpha,\beta)\in\Dc_3$ and consider the set of $\ub\in\Bc(C_2\sqrt{n})$ that satisfy the constraint in \eqref{eq:f_con}. With probability at least $1-Ce^{-cn}$, this set is non-empty. To see this, note that with the same probability $\|\beta\g+ \X P_{S^t}\theta\|\leq C_2\sqrt{n}$ for large constant $C_2$.  Thus, for any $\ub\in\Bc(C_2\sqrt{n})$ let $\bar\ub(\xi,\alpha,\beta)$ denote the projection of $\ub$ on the (non-empty) constraint set in \eqref{eq:f_con}.

With this notation, it holds for any $(\xi,\alpha,\beta,\ub)\in\Oc$ that
\begin{align}
B &\stackrel{}{=} \Fc_t(\ub,\theta) + \max_{0\leq\rho_\vb\leq C_3}\frac{\rho_\vb}{\sqrt{n}} f(\xi,\alpha,\beta,\ub) \nn
\\
&\stackrel{(i)}{\geq} \Fc_t(\ub,\theta) + \frac{C_3}{\sqrt{n}} m_{\Oc} \nn
\\
&\stackrel{(ii)}{\geq} \Fc_t(\bar\ub(\xi,\alpha,\beta),\theta) - \frac{C_L}{\sqrt{n}}\|\bar\ub(\xi,\alpha,\beta)-\ub\|_2 + \frac{C_3}{\sqrt{n}} m_{\Oc} \nn
\\
&\stackrel{(iii)}{\geq} \Fc_t(\bar\ub(\xi,\alpha,\beta),\theta) - 2C_LC_2 + \frac{C_3}{\sqrt{n}} m_{\Oc}
\\
&\stackrel{(iv)}{\geq} A - 2C_LC_2 + \frac{C_3}{\sqrt{n}} m_{\Oc}
\end{align}
Specifically,  we used (i) the assumption that $f(\xi,\alpha,\beta,\ub)\geq m_\Oc>0$; (ii) Lipschitness of $\Fc_t$ as per Assumption \ref{ass:Lip}; (iii) the fact that $\ub,\bar\ub(\xi,\alpha,\beta)\in\Bc_2(C_2\sqrt{n})$; (iv) feasibility of $(\bar\ub(\xi,\alpha,\beta),\theta)$  in \eqref{eq:conAO2}, i.e. $f(\bar\ub(\xi,\alpha,\beta),\theta)\leq 0$.

Thus, we can always pick $C_3\geq 2C_LC_2\sqrt{n}/m_\Oc$ such that $B\geq A$ as desired.


\subsubsection{Proof of Lemma \ref{lem:phi_tilde_aux}}
\label{sec:phi_tilde_proof}\ct{To fix}

Recall from \eqref{eq:2min_u} that
\begin{align}
\phi_{n,\Dc} &= \min_{ \substack{(\xi,\alpha,\beta)\in\Dc_3 \\ \|\ub\|_2\leq C_2\sqrt{n} } }  \; \; \frac{1}{2}(\xi^2+\alpha^2+\beta^2) - \big(\xi\xi_t+\alpha\sigma_t\big) - \frac{2\eta}{n}\inp{\omegab_t}{\ub}\quad\text{sub. to}~\Big\|\beta\g+\xi\gammab_1+\alpha\gammab_2-\ub\Big\|_2\leq \beta\| P^{\perp}_{S^t}\h \|_2\end{align}
We will need the following auxiliary result to perform the constrained optimization of the linear form in $\ub$.
%\begin{lemma}\label{lem:phi_tilde_aux}
%Let $A,B>0$ and vectors $\ab,\tb\in\R^n$. Assume that
%\begin{align}\label{eq:u_opt_lem_cond}
%\|A\frac{\ab}{\|\ab\|_2}+\tb\|_2\leq B.
%\end{align}
% Then, it hold that
%\begin{align}\label{eq:u_opt_lem}
%\Big\{\min_{\|\ub\|_2\leq B}-\inp{\ab}{\ub}\quad\text{sub. to}~~\|\tb-\ub\|_2\leq A \Big\}= -A\,\|\ab\|_2-\inp{\ab}{\tb}.
%\end{align}
%\end{lemma}

Before proving Lemma \ref{lem:phi_tilde_aux}, we show how to conclude Lemma \ref{lem:phi_tilde} from it.  We see that the inner minimization over $\ub$ above is of the same form as the minimization in the LHS of \eqref{eq:u_opt_lem} with:
$$
\ab\leftarrow \frac{2\eta}{n}\omegab_t,\quad \tb\leftarrow\beta\g+\xi\gammab_1+\alpha\gammab_2,\quad A\leftarrow \beta\| P^{\perp}_{S^t}\h \|_2, \quad B\leftarrow C_2\sqrt{n}.
$$

%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Boundedness of omega %%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%From Assumption \ref{ass:omega}, for some absolute constant $\tilde C$:
%%%%%$
%%%%%\|\frac{\omegab(\xi,\sigma)}{\sqrt{\E\Omega^2}} - \sqrt{n}\|_{\psi_2} \leq \tilde{C}K_\omega^2
%%%%%$
%%%%%Hence,
%%%%%$$
%%%%%\Pro\left( \big\|\omegab(\xi,\sigma)\big\|_2 \geq 2\sqrt{\E\Omega^2}\sqrt{n} \right)\leq 2\exp(-cn/K_\omega^4).
%%%%%$$
%%%%%Also, 

Now, we will show that \eqref{eq:u_opt_lem_cond} holds for large enough constant $C_2$. 
First, from concentration of the norm of Gaussian isotropic vectors it holds that:
$$
\Pro\left( \max\left\{\|\g\|_2,\|\gammab_1\|_2,\|\gammab_2\|_2\right\} \geq 2\sqrt{n} \right)\leq C\exp(-cn).
$$
Hence, $\|\tb\|_2\leq 2\sqrt{n} $ with probability at least $1- C\exp(-cn)$. 
Second, the multivariate Gaussian $\x=P_{S_t}^\perp\h$ behaves as a $d-2$-dimensional isotropic Gaussian. Hence, from same arguments and using  $d-2<d\leq n$
$$
\Pro\left( \|P_{S_t}^\perp\h\|_2\geq 2\sqrt{n} \right) \leq C\exp(-cn).
$$
Putting these together, combining with the triangle inequality and using boundedness of $\xi,\alpha,\beta$ (cf. $\Dc_3\subset\Bc_2(C_1)$) we conclude that \eqref{eq:u_opt_lem_cond} holds with probability at least $1- C\exp(-cn)$ for sufficiently large constant $C_2$. 

Then, the desired follows directly from \eqref{eq:u_opt_lem}.

\begin{proof}[Proof of Lemma \ref{lem:phi_tilde_aux}]
We start by lower bounding the LHS of \eqref{eq:u_opt_lem} as follows:
\begin{align*}
\Big\{\min_{\|\ub\|_2\leq B}\,\,-\inp{\ab}{\ub}\quad\text{sub. to}~~\|\tb-\ub\|_2\leq A \Big\}&= \min_{{\|\ub\|_2\leq B}} \max_{\la\geq0}\,\, -\inp{\ab}{\ub}+\frac{\la}{2}\|\tb-\ub\|_2^2-\frac{\la}{2}A^2 \\
&\stackrel{(i)}{=}  \max_{\la\geq0} \min_{{\|\ub\|_2\leq B}}\,\, -\inp{\ab}{\ub}+\frac{\la}{2}\|\tb-\ub\|_2^2-\frac{\la}{2}A^2 \\
&\stackrel{(ii)}{\geq}  \max_{\la\geq0}\,\, \min_{\ub\in\R^n} -\inp{\ab}{\ub}+\frac{\la}{2}\|\tb-\ub\|_2^2-\frac{\la}{2}A^2 \\
&\stackrel{}{=}  \max_{\la\geq0}\,\, -\frac{1}{2\la}\|\ab\|_2^2 - \ab^T\tb -\frac{\la}{2}A^2\\
&\stackrel{}{=}  -A\,\|\ab\|_2- \ab^T\tb.
\end{align*}
Above, (i) holds because the minimization over $\ub$ is on a compact set and the objective is clearly convex in $\ub$ and concave in $\la$; (ii) is because the minimization set over $\ub$ is enlarged. 

Next, consider $\ub_\star=\frac{A}{\|\ab\|_2}\ab+\tb$. Clearly, $\ub_\star$ is feasible in the constrained minimization in \eqref{eq:u_opt_lem}. Thus, the LHS in \eqref{eq:u_opt_lem} is upper bounded by 
$$
-\inp{\ab}{\ub_\star} = A\|\ab\|_2-\ab^T\tb.
$$
Combining the above completes the proof of the lemma.
\end{proof}


\subsection{Probabilities of events in Equation  \eqref{eq:good_events_quad}}

\begin{lemma} Recall the definitions of $\A\in\R^{n\times 3}, \omegab_t\in\R^n, \vb_n\in\R^3$ in Section XXX. Further let Assumption \ref{ass:omega} hold. For large enough $n$, $\delta>c_\delta$ and any $\eta>0$ smaller than some constant, there exist constants $C,c,C'>0$ such that each one of the events $\Ec_i, i\in[4]$ in \eqref{eq:good_events_quad} holds with probability at least $1-Ce^{-cn\eta^2}$.
\end{lemma}
\begin{proof}
We will prove the following refined version of \eqref{eq:good_events_quad}.
\begin{subequations}
\begin{align}
\Ec_1&:=\left\{ \frac{1}{1+6n^{-1/2}+3\eta}\,\mathbf{I}_3 \preceq n(\A^T\A)^{-1} \preceq 
\frac{1}{1-6n^{-1/2}-3\eta}\,\mathbf{I}_3
\right\}
\\
\Ec_2&:=\left\{ \frac{1}{\delta}(1-\eta)-\frac{2}{n}\leq\|\vb_n\|_2^2\leq \frac{1}{\delta}(1+\eta)
\right\}\\
\Ec_3&:=\left\{ \left| \frac{\|\omegab_t\|_2^2}{n} - \E\Omega_t^2 \right|\leq \eta
\right\}
\\
\Ec_4&:=\left\{ \left| \frac{1}{n}\gammab_1^T\omegab_t - \E[G_1\Omega_t] \right| \vee 
\left| \frac{1}{n}\gammab_2^T\omegab_t - \E[G_2\Omega_t] \right| \vee
\left| \frac{1}{n}\g_1^T\omegab_t  \right|
\leq C'\eta\right\}
\\
\Ec_5&:=\left\{ \left| \frac{\|\A^T\omegab_t\|^2}{n^2} - \left(\E[G_1\Omega_t]\right)^2 - \left(\E[G_2\Omega_t]\right)^2 \right|\leq 3\eta^2 + 2\eta\left(\E[G_1\Omega_t]+\E[G_2\Omega_t]\right)\right\}
\end{align}
\end{subequations}
All these events hold with high-probability. Specifically,
\begin{subequations}
\begin{align}
\Pro(\Ec_1)\wedge\Pro(\Ec_2)&\geq 1 - Ce^{-c n \eta^2}
\\
\Pro(\Ec_3)&\geq 1 - 2e^{-cn\left(\frac{\eta^2}{K_\omega^4}\wedge\frac{\eta}{K_\omega^2}\right)}
\\
\Pro(\Ec_4)\wedge\Pro(\Ec_5)&\geq 1 - 2e^{-cn\frac{\eta^2}{K_\omega^2}}
\end{align}
\end{subequations}
\ct{From Assumption \ref{ass:omega}, $K_\omega<C$ and $\E[\Omega^2]<C$.}

Using $\E[G_1\Omega_t]\vee\E[G_2\Omega_t]\leq\sqrt{\E[\Omega_t^2]}$ and $\eta\in(0,1)$ on the event $\Ec$, we have that
\begin{align*}
\left| \frac{\|\A^T\omegab_t\|^2}{n^2} - \left(\E[G_1\Omega_t]\right)^2 - \left(\E[G_2\Omega_t]\right)^2 \right|&\leq \left(3 + 4\sqrt{\E[\Omega_t^2]}\right)\eta
%\\&\leq \left(3 + 4\sqrt{K_\omega}\right)\eta\leq C\left(1\vee \sqrt{K_\omega}\right)\eta\leq 
\leq C\eta,
\end{align*}
where we used Cauchy-Schwartz in the first inequality and $\E[\Omega_t^2]<C$ in the second inequality, respectively.


\end{proof}



\subsubsection{Proof of Lemma \ref{lem:conc_lemma}}
By Assumption \ref{ass:omega}, Gaussianity of $\gammab_1,\gammab_2$ and \cite{Ver}[Lemma 2.7.7] we have that the entries of $\inp{\gammab_1}{\omegab_t}$ and $\inp{\gammab_2}{\omegab_t}$ are independent sub-exponential random variables with sub-exponential constant at most $C K_\omega$ each and means $\E[G_1\cdot \Omega_t]$ and $\E[G_2\cdot \Omega_t]$, respectively. Thus, from Bernstein's inequality,
\begin{align}\label{eq:Bern_inp1}
\Pro\left\{ \max\left\{ \left| \xi_{\star,n} - \xi_{\star,t+1} \right|\,\,\left| \alpha_{\star,n} - \alpha_{\star,t+1} \right| \right\} \geq \eps \right\} \leq 4\exp\left(-c\,n\,\min\left(\eps^2/K_\omega^2,\eps/K_\omega\right)\right)\,.
\end{align}


For convenience, let us denote 
\begin{align*}
&A = \frac{1}{\sqrt{n}}\|P^{\perp}_{S^t}\h \|_2\quad\text{and}\quad \bar{A}=\sqrt{\frac{d-2}{n}}\\
&B = \frac{1}{\sqrt{n}}\|\omegab_t\|_2\quad\text{and}\quad \bar{B}=\sqrt{\E[\Omega^2]}.
\end{align*}

From subgaussianity of the entries of $\omegab_t$ (by Assumption \ref{ass:omega}) and the fact that $P^\perp_{S^t}\h$ is distributed as a $(d-2)$--dimensional isotropic Gaussian,  it holds  that  (e.g. \cite[Thm. 3.1.1]{Vershynin})
%$$
%\left\|  \frac{\|P^{\perp}_{S^t}\h \|_2}{\sqrt{n}} -  \sqrt{\frac{d-2}{n}} \right\|_{\psi_2}\leq \frac{C}{\sqrt{n}} \quad\text{and}\quad \left\|\frac{\|\omegab\|_2}{\sqrt{n}}-\sqrt{\E[\Omega^2]}\right\|_{\psi_2}  \leq \frac{CK_\omega}{\sqrt{n}}.
%$$ 
%\begin{align}
%\Pro\left\{ \Big|\frac{\|P^{\perp}_{S^t}\h \|_2^2}{{n}} -  \frac{d-2}{n}\Big| \geq\eps \right\}&\leq 2\exp\left(-c\,n\,\,\min(\eps^2,\eps)\right) \\
%\Pro\left\{ \Big|\frac{\|\omegab_t \|_2^2}{{n}} -  \E[\Omega^2]\Big| \geq\eps \right\}&\leq 2\exp\left(-c\,n\,\,\min(\eps^2/K_\omega^4,\eps/K_\omega^2)\right)\,.
%\end{align}
%\begin{align*}
%\Pro\left\{ \max\left\{ \left|  \frac{\|P^{\perp}_{S^t}\h \|_2}{\sqrt{n}} -  \frac{1}{\sqrt{\delta}} \right|\,,\, \left|\frac{\|\omegab\|_2}{\sqrt{n}}-\sqrt{\E[\Omega^2]}\right| \right\} \geq \eps \right\} \leq 4\exp\left(-c\eps^2n\right)
%\end{align*}
\begin{align*}
\Pro\left\{ \Big|A^2 -  \bar{A}^2\Big| \geq\eps \right\}&\leq 2\exp\left(-c\,n\,\,\min(\eps^2,\eps)\right) \\
\Pro\left\{ \Big|B^2-  \bar{B}^2\Big| \geq\eps \right\}&\leq 2\exp\left(-c\,n\,\,\min(\eps^2/K_\omega^4,\eps/K_\omega^2)\right)\,.
\end{align*}
Thus, (e.g. see \cite[Thm.~3.1.1]{Ver}), 
\begin{align}
\Pro\left\{ \big|{A} - \bar{A}\big| \geq \eps \right\} &\leq 2\exp\left(-c\,n\,\eps^2\right)\\
\Pro\left\{ \big|\frac{B}{\bar{B}} - 1\big| \geq \eps \right\} &\leq 2\exp\left(-c\,n\,\eps^2\bar{B}^4/K_\omega^4\right) \implies\Pro\left\{ \big|B- \bar{B}\big| \geq \eps\bar{B} \right\} \leq 2\exp\left(-c\,n\,\eps^2\bar{B}^4/K_\omega^4\right).
\end{align}

Now, conditioned on the event $\{|A-\bar A|\leq\eps,|B-\bar B|\}\leq \eps\bar B\}$ occurring with probability at least $1-4\exp\big(-c\,n\,\eps^2\min\{1,\bar{B}^4/K_\omega^4\}\big)$, it holds that
$$
|AB-\bar A\bar B|\leq C\bar{B}\max\{\eps^2,\eps\}.
$$
Above, we also used the facts that $\bar{A}\leq 1$ since $n>d$ and $\bar{B}\leq\sqrt{2}K_\omega$ by subgaussianity of the entries of $\omegab_t$ (e.g.  \cite[Prop.~2.5.2]{Ver}). 
Hence,
\begin{align}
\Pro\left\{|AB-\bar A\bar B|\geq \eps\right\}
&\leq C\exp\left(-c\,n\,\frac{\min\left(1,\bar{B}^4/K_\omega^4\right)}{\min(K_\omega,K_\omega^2)}\,\min\left(\eps,{\eps^2}\right)\right).\label{eq:AB}
\end{align}
For convenience, denote $C_\omega:=\frac{\min\left(1,\bar{B}^4/K_\omega^4\right)}{\min(K_\omega,K_\omega^2)}.$
%where the second inequality follows because: (i) $\bar A\leq 1$  since $n\geq d>d-2$; (ii) by sub-gaussianity of the entries of $\omegab_t$ it holds that $\bar B\leq \sqrt{2} K_\omega$ by \cite[Prop.~2.5.2]{Ver}.  

Finally, note that each entry of $\frac{1}{n}\inp{\g}{\omegab_t}$ is zero-mean subexponential with sub-exponential constant at most $CK_\omega/n$. Thus, by Bernestein's inequality
$$
\Pro(|\frac{1}{n}\inp{\g}{\omegab_t}|\geq \eps) \leq 2\exp\left(-c\,n\,\min\left(\eps^2/K_\omega^2,\eps/K_\omega\right)\right)
%\leq2\exp\left(-c\,n\,\frac{1}{1+K_\omega^2}\,\min\left(\eps^2,\eps\right)\right).
$$
Combining this with \eqref{eq:AB}, and further using the fact
\begin{align}
\bar{B}\big(\frac{1}{\sqrt{\delta}}-\frac{2\sqrt{\delta}}{n} \big) - \leq \bar{A}\bar{B} \leq \bar{B}\frac{1}{\sqrt{\delta}} \implies 
\bar{B}\frac{1}{\sqrt{\delta}}-\frac{C(\delta) K_\omega}{n} - \leq \bar{A}\bar{B} \leq \bar{B}\frac{1}{\sqrt{\delta}},
\end{align}
 we conclude with the desired:
%Now, note that
%$$
%2(AB-\bar A\bar B) = (A+B)^2 - (\bar A+\bar B)^2 - (A^2-\bar A ^2) - (B^2-\bar B ^2)
%$$
%Hence, $\beta_{\star,n}$ is subexponential with $\|\beta_{\star,n}\|_{\psi_1}\leq C/n$ and Bernstein's inequality gives \ct{Add some detail}
\begin{align}\label{eq:Bern_inp2}
\Pro\left\{ \abs{\beta_{\star,n}-\beta_{\star,t+1}} \geq \eps + \frac{\eta K_\omega \tilde C(\delta)} {n}\right\} \leq C\exp\left(-c\,C_\omega\,n\,\min\left(\eps,{\eps^2}\right)\right).
\end{align}

Now we will show that the unconstrained solution \eqref{eq:soln_n} of \eqref{eq:con_final_AO} is feasible (thus, optimal) when $\Dc:=\Bc_2(C_1)$. Here, recall that $C_1$ is a constant that can be made arbitrarily large without changing any of the results thus far. Specifically, it suffices from from \eqref{eq:Bern_inp1} and \eqref{eq:Bern_inp2} that
$$
C_1 > 2\sqrt{(\alpha_{\star,t+1}+\eps)^2+(\beta_{\star,t+1}+\eps)^2+(\xi_{\star,t+1}+\eps)^2}.
$$
(For example, $C_1^2=4(\alpha_{\star,t+1}^2+\beta_{\star,t+1}^2+\xi_{\star,t+1}^2)+12\eps^2+\frac{\eta^2K_\omega^2C^2}{n^2}$ suffices.) This guarantees that with the same probability as the RHS of \eqref{eq:Bern_inp2} 
%
% Hence, from \eqref{eq:Bern_inp1} and \eqref{eq:Bern_inp2}, letting $C_1 = 8 \max\{\alpha_{\star,t+1},\beta_{\star,t+1},\xi_{\star,t+1}\} > 2\sqrt{(\alpha_{\star,t+1}+\eps)^2+(\beta_{\star,t+1}+\eps)^2+(\xi_{\star,t+1}+\eps)^2}$ \ct{Need $\eps\leq \max\{\alpha_{\star,t+1},\beta_{\star,t+1},\xi_{\star,t+1}\}$} it holds with probability at least $1-C\exp\left(-c\,\min\left(n\eps^2,n\eps\right)\right)$ that 
 $\|\theta_n\|_2^2=\xi_{\star,n}^2+\alpha_{\star,n}^2+\beta_{\star,n}^2< C_1$, i.e. $(\xi_{\star,n},\alpha_{\star,n},\beta_{\star,n})$ is feasible in \eqref{eq:con_final_AO}. Hence, 
for large enough $C_1$, with the same probability:
\begin{align}
\wt\phi_{n,\Bc_2(C_1)} = -\frac{1}{2}\left(\alpha_{\star,n}^2+\beta_{\star,n}^2+\xi_{\star,n}^2\right).
\end{align}

When combined with \eqref{eq:Bern_inp1} and \eqref{eq:Bern_inp2}, these lead to the following for constants $C_4:=C_4(\delta,\eta,\alpha_{\star,t+1},\beta_{\star,t+1},\xi_{\star,t+1})$ and $C_5:=C_5(\delta,\eta,K_\omega,\beta_{\star,t+1})$:
\begin{align}\nn
\Pro\left\{\Big|\wt\phi_{n,\Bc_2(C_1)} - \bar\phi \Big| \geq {C_4} \max\{\eps,\eps^2\}+\frac{C_5}{n}\right\} \leq  C\exp\left(-c\,C_\omega\,n\,\min\left(\eps^2,\eps\right)\right),
%\max\left\{ \alpha_{\star,t+1}\, ,\,\beta_{\star,t+1}\, ,\,\xi_{\star,t+1}  \right\}\cdot 
\end{align}
with
\begin{align}\nn
\bar\phi:=-\frac{1}{2}\left(\alpha_{\star,t+1}^2+\beta_{\star,t+1}^2+\xi_{\star,t+1}^2\right)
\end{align}



==> sections/gordon/gordon.tex <==
%In this section, we formally derive and prove concentration of the one-step Gordon updates. A heuristic derivation was given earlier in Section \ref{sec:heuristic} for the special case of alternating projections for phase retrieval. Here, we present a rigorous unifying analysis of first- and second- order methods for both the (noisy) phase-retrieval and mixtures-of-gaussians models. 
%
%For the purpose of this section fix \emph{arbitrary} vector $\thetacur$ and consider the \emph{one-step} update:
%\begin{align}\label{eq:gordon_one_step}
%\thetaplus \in \arg\min_\theta \underbrace{\Lc(\theta;\thetacur,\X,\y)}_{\Lc_t(\theta)}.
%\end{align}
%While our analysis is rather general, of immediate interest to us are the two loss functions defined in Equations \eqref{eq:GD_gen} and \eqref{eq:sec_order_gen} for the first- and second- order methods,  respectively. While we keep the subscript $t$ in for $\thetacur$ and $\Lc_t$ in \eqref{eq:gordon_one_step}, we emphasize that the analysis in this section is specific to \emph{one-step} updates. The evolution of the updates is treated later in Sections \ref{sec:} \ct{ref:evolution}. To clarify this, we simply denote the minimizer in \eqref{eq:gordon_one_step} as $\thetaplus$ (instead of $\theta_{t+1}$).



The main result of this section (Theorem \ref{thm:gordon_main} below) shows $n^{-1/4}$-rate concentration  of the $(\xi,\sigma)$ updates around the one-step Gordon updates. 

%\subsection{Notation}
%Here, we introduce some necessary notation and assumption for our analysis. 
To state the theorem, recall some notation from Section \ref{sec:heuristic}. Let $S_t = {\sf span}(\thetastar, \thetacur)$ denote the two-dimensional subspace spanned by $\thetastar$ and $\thetacur$, and let $P_{S^t}$ and $P_{S^t}^{\perp}$ denote the projection matrices onto the subspace and onto its orthogonal complement, respectively. Accordingly let $P_{\theta^\star}^\perp$ denote the projection matrix onto the orthogonal complement of the subspace spanned by $\thetastar$. For any $\theta\in\R^d$ introduce the $\theta$-dependent variables
\begin{align}\label{eq:scal}
\begin{cases}
~\xitheta:={\inp{\theta}{\thetastar}}\\
~\alphatheta :=\frac{\inp{\theta}{P^{\perp}_{\thetastar} \thetacur}}{\|P^{\perp}_{\thetastar} \thetacur\|_2}
\\
~\betatheta := \|P^{\perp}_{S^t}\theta\|_2\,.
%~\sigma := \|P^\perp_{\thetastar} \theta\|_2.
\end{cases}
\end{align}
We remark in this notation
$
\sigmatheta^2 := \|P^\perp_{\thetastar} \theta\|_2^2 = \alphatheta^2+\betatheta^2.
$
Specifically, we define $\xinext,\alphanext$ and $\betanext$ for the minimizer $\thetaplus$ in \eqref{eq:gordon_one_step}. Finally, recall Assumption \ref{ass:omega} and Definition \ref{def:}


%






% $\bullet$~~Convex in $\theta$.
%
% $\bullet$~~Separable across samples: Suppose that we can write 
%  \begin{align}\label{eq:Lc}
%  \mathcal{L}_t(\theta) = h(\theta, \thetacur) + \frac{1}{n} \sum_{i = 1}^n g(\langle \bx_i, \theta \rangle, \langle \bx_i, \thetacur \rangle; y_i)
%  \end{align}
%   for some pair of functions $(h, g).$

%Define the following potential functions---corresponding to the projection of the iterate in the direction of the truth and orthogonal to the truth:
%\begin{align*}
%\xit  := \frac{\langle \thetacur, \thetastar \rangle}{ \| \thetastar \|_2^2} \quad \text{ and } \quad \sigmat  := \| P^{\perp}_{\thetastar} \thetacur \|_2.
%\end{align*}

%\subsection{Gordon updates and concentration (Theorem \ref{thm:gordon_main})}

%The theorem below shows concentration of the statistics $\xinext,\alphanext,\betanext$ of $\thetaplus$  for the two choices of loss functions in Equations \eqref{eq:GD_gen} and \eqref{eq:sec_order_gen}, respectively. Recall that these losses are parameterized by a weight function 
%$\omega:\R\times\R\rightarrow\R$. We require the following assumption on the concentration properties of this function.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{assumption}[Concentration of the weight function]\label{ass:omega}
%Let independent random vectors $\gammab_1,\gammab_2,\zb,\epsb\in\R^n$ each having iid entries from distributions $\Nn(0,1),$  $\Nn(0,1),$ $P_E$ and $P_Z$, respectively. 
%%Specifically, $\gammab_1,\gammab_2$ are standard normals, $\epsb\sim\Nn(0,s^2\mathbf{I}_n)$, and, $\zb$ is the randomness of the measurement link function.
%%\sim\Nn(0,\mathbf{I}_n) 
%%be independent standard Gaussian vectors. 
%Assume that the random vector 
%\begin{align}\label{eq:omegat_def}
%\omegab_t:= \omega\big(\xit \gammab_1+\sigmat \gammab_2\,,\,f(\gammab_1;\zb)+\epsb\big),
%\end{align}
%has independent entries sampled from a distribution $P_{\Omega_{t}}$ with the following properties. Let 
%$\Omega_t\sim P_{\omega_t}$, that is 
%\begin{align}\label{eq:omegat_def_scalar}
%\Omega_t:= \omega\big(\xit G_1+\sigmat G_2\,,\,f(G_1;Z)+E\big),\qquad G_1, G_2\sim\Nn(0,1),\,E\sim P_E,\,Z\sim P_Z.
%\end{align} 
%Then, 
%
%\begin{enumerate}[(i)]
%
%\item $\Omega_t$ is a $K_{\omega_t}$-subGaussian random variable for  universal constant  $K_{\omega_t}:=K_{\omega_t}(s)$ that may only depend on the noise level.
%
%\item For  absolute constants $C,c,c'>0$, it holds that $E[\Omega_t^2]-\left(E[G_1\Omega_t]\right)^2-\left(E[G_2\Omega_t]\right)^2>c$, $\E[G_2\Omega_t]\geq c'$ and $E[\Omega_t^2]<C$. 
%
%%\item $\E[G_2\Omega_t]\geq 0$.
%
%%\item For  absolute constants $c'>0$, it holds that $E[\Omega_t^2]-\left(E[G_1\Omega_t]\right)^2-\left(E[G_2\Omega_t]\right)^2>c'$%\ct{joint distribution of $G_1,G_2$ and $\Omega_t$}.
%\end{enumerate}
%\end{assumption}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\begin{remark}[Satisfying Assumption \ref{ass:omega}]\ct{More needed here. Move to corresponding Section.}\emph{
%For non-smooth GD in phase retrieval we have $\omega(x_1,x_2)=\sign(x_1)(|x_1|-x_2)$ and $f(x;z) = |x|$. It is not hard to see then that $\omega\big(\xi\gammab_1+\sigma\gammab_2\,,\,f(R\gammab_1;\zb)+\epsb\big)$ is a vector with independent subgaussian entries, hence Assumption \ref{ass:omega} holds by \cite[Thm.~3.1.1]{Vershynin}. 
%\\
%The same argument applies to Gradient EM for mixtures of two regressions for which $\omega(x_1,x_2) = x_1-x_2\tanh\big(\frac{x_2x_1}{s^2}\big)$ and $f(x;z)=zx$. }
%\end{remark}
%
%We also need to define the following \emph{one-step Gordon updates} for the two loss functions corresponding to first- and second- order methods. 
%\begin{definition}[One-step Gordon updates]
%\label{def:starnext}
% %Fix any $t\geq1$. 
%Let $G_1,G_2$ be independent standard normal random variables and $\Omega_t=\Omega_t(G_1,G_2)$ be as in Equation \eqref{eq:omegat_def_scalar} such that Assumption \ref{ass:omega} holds. 
%% Let Assumption \ref{ass:omega} hold   random variable $\Omega_t$ be as defined therein, and $G_1,G_2$  independent standard normal random variables. 
%%Finally, let $\Lc$ be the loss function in Theorem \ref{thm:gordon_main}.  
%If the loss function $\Lc$ is as in Equation \eqref{eq:sec_order_gen} then define
%\begin{align}
%\begin{cases}
%~\xinextstar=\E[G_1\Omega_t]\\
%~\alphanextstar=\E[G_2\Omega_t]\\
%~\betanextstar=\sqrt{\frac{\E[\Omega_t^2]-\left(\E[G_1\Omega_t]\right)^2-\left(\E[G_2\Omega_t]\right)^2}{\delta-1}}\,.
%\end{cases}
%\label{eq:theta_starnext_sec}
%\end{align}
%Else, if $\Lc$ is as in Equation \eqref{eq:GD_gen}, then define
%\begin{align}
%\begin{cases}
%~\xinextstar = \xit  + 2\eta\E\left[G_1 \Omega_t\right]\\
%~\alphanextstar = \sigmat  + 2\eta\E\left[G_2 \Omega_t\right]\\
%~\betanextstar = 2\eta\frac{1}{\sqrt{\delta}}\sqrt{\E\left[\Omega_t^2\right]}.\\
%\end{cases}
%\label{eq:theta_starnext_gd}
%\end{align}
%\end{definition}
%
%%Our main theorem below shows concentration, but towards different values depending on the loss function. 
%
%We are now ready to state the main result of this section.

\begin{theorem}[Concentration of one-step Gordon updates]
\label{thm:gordon_main}
 %Fix any $t\geq1$ and let
Consider the one-step update 
 $\thetaplus$ as defined in Equation \eqref{eq:gordon_one_step} for either of the two choices of loss functions $\Lc$ in  Equations \eqref{eq:GD_gen} and \eqref{eq:sec_order_gen}, respectively. Further let Assumption
 %ref{ass:loss}, 
 %\ref{ass:Lip}, \ref{ass:theta_bd}, and 
 \ref{ass:omega} hold. Consider the (loss-dependent) constants $\xinextstar, \alphanextstar, \betanextstar$ specified in Definition \ref{def:starnext_main} and let $\sigmanextstar:=\sqrt{\alphanextstar^2+\betanextstar^2}$. For $\eps>0$, define the following set 
\begin{align}\label{eq:Seps}
\Sc_\eps:=\left\{\theta\in\R^d\,\Big|\, \abs{\xitheta-\xinextstar}\vee \abs{\alphatheta-\alphanextstar}\vee\abs{\betatheta-\betanextstar}\leq \eps \right\}.
\end{align}
%where $\xitheta,\alphatheta,\betatheta$ are defined in Equation \eqref{eq:scal}.
  Then, there exist positive absolute constants $c,C,c_\delta,c'(\delta),C'$ such that for $\delta>c_\delta$ and any $c'(\delta)>\eps>C'n^{-\nicefrac{1}{4}}$ it holds that
  \begin{align}\label{eq:S_2show}
  \Pro\left(\thetaplus\in\Sc_\eps\right) \geq 1-Ce^{-cn\eps^4}.
  \end{align}
In particular, under the same conditions, there exists constant $C_1(\delta)>0$ such that
\begin{align}\label{eq:sigma_2show}
|\xiplus-\xinextstar|\leq\eps\qquad\text{and}\qquad|\sigmaplus-\sigmanextstar|\leq C_1 \eps,
\end{align}
with probability at least $1-Ce^{-cn\eps^4}.$
%  
%   it holds with probability at least $1-Ce^{-cn\eps^4}$ that
%\begin{align}
%\left|\xinext-\xinextstar\right|\vee\left|\alphanext-\alphanextstar\right|\vee
%\left|\betanext-\betanextstar\right| \leq \eps.
%\end{align}
%\ct{Moreover, $\sigmat $ concentrates as ...}
\end{theorem}

In the remaining of this section we formally derive the Gordon updates in Definition \ref{def:starnext_main} and prove Theorem \ref{thm:gordon_main}.


% ================================================= %
\subsection{Proof of Theorem \ref{thm:gordon_main}}
% ================================================= %
%For $\eps>0$, we will compute constants $\xi_{t+1},\alpha_{t+1},\beta_{t+1}$ and exponentially small probability $p=p(\eps,n)$ such that the solution $\thetanext$ of \eqref{eq:opt_gen_intro} satisfies with high probability $1-p$ \ct{to be specified}:




\subsubsection{Assumptions}\label{sec:gordon_assumptions}
To a great degree, we treat the two different loss functions corresponding to first- and second- order methods in a \emph{unifying} way. To do this, it is convenient to introduce the following set of assumptions. 
%\ct{We show in Section XXX that the two choices in \eqref{eq:GD_gen} and \eqref{eq:sec_order_gen} indeed satisfy these assumptions}. 
\ct{We will show in subsetion that these assumptions are satisfied by the two losses in Equations \eqref{eq:GD_gen} and \eqref{eq:sec_order_gen}}. 
We note however that these assumptions are rather weak and we expect the same analysis to apply to other instances of \eqref{eq:opt_gen_intro} not considered here.

First, we need the following decomposability and convexity assumptions about the loss.

\begin{assumption}[Deecomposability and convexity of Loss]\label{ass:loss}
The loss  $\Lc_t(\theta):={\mathcal{L}(\theta; \thetacur, \bd{X}, \bd{y})}$ has the following properties:

\begin{enumerate}[label=(\roman*)]
\item $\Lc_t(\theta)=\Fc_t(\X\theta,\theta)$ where the (random) function $\Fc_t:\R^n\times\R^d\rightarrow \R$ can be decomposed as 
\begin{align}\label{eq:Fc}
\Fc_t(\ub,\theta) := h(\theta, \thetacur) + g(\ub, \X\thetacur; \y ).
\end{align}
%  \begin{align}\label{eq:Lc}
%  \mathcal{L}_t(\theta) = h(\theta, \thetacur) + g(\X\theta,\X\thetacur;\y)
%  % \frac{1}{n} \sum_{i = 1}^n g(\langle \bx_i, \theta \rangle, \langle \bx_i, \thetacur \rangle; y_i)
%  \end{align}
   for some pair of functions $(h, g).$ 
   %\footnote{\ct{In fact, all we need here is that $ \mathcal{L}_t(\theta)=g(P_{S^t}\theta,\|P_{S^t}^\perp\theta\|_2,\X\theta,\X\thetacur;\y)$}}

\item The functions $(h,g)$ are convex on their first arguments.

\item $h(\theta,\thetacur)$ depends on $P_{S^t}^\perp\theta$ only through its norm $\beta=\norm{P_{S^t}^\perp\theta}_2$, that is, there exists function $\hscal:\R^3\times\R^d\rightarrow\R$ such that
 $$h(\theta,\thetacur)=\hscal(\xi,\alpha,\beta,\thetacur).$$
 

\item $\Lc_t(\theta)$ is coercive. 
\end{enumerate}
\end{assumption}
%For convenience, we introduce the following (random) function $\Fc_t:\R^n\times\R^d\rightarrow \R$:
%\begin{align}\label{eq:Fc}
%\Fc_t(\ub,\theta) := h(\theta, \thetacur) + g(\ub, \X\thetacur; \y ).
%\end{align}
%Note that  as per \eqref{eq:Lc}. 
\noindent 
%An important observation here, which we will use later in the proof, is 
Note here for later use that $\Fc_t(\ub,\theta)$ depends on the random matrix $\X$ only through the projections $\X\thetacur$ (appearing explicitly) and $\X\thetastar$ (appearing through the measurements $\y$). 

We further require the following Lipschitzness assumption.

\begin{assumption}[Lipschitzness of the Loss]\label{ass:Lip}
For any fixed $\theta$, the function $\Fc(\cdot,\theta)$ is $\frac{C_L(R)}{\sqrt{n}}$-Lipschitz in the domain  $\{\ub\,:\,\|\ub\|_2\leq C\sqrt{n}\}$ for constant $C>0$.
\end{assumption}

Finally, we need the following boundedness assumption on the minimizers $\thetaplus$.

\begin{assumption}[Boundedness of the iterates]\label{ass:theta_bd}
There exist constants $c,C,C_{\theta}>0$ such that
$\|\thetaplus\|_2\leq C_{\theta}$
with probability at least $1-e^{-cn}.$
\end{assumption}


\subsubsection{Proof strategy}
We prove Theorem \ref{thm:gordon_main} building on the CGMT framework \citep{thrampoulidis2015regularized,thrampoulidis2018precise}. As such, 
in order to prove Equation \eqref{eq:S_2show}, we will show equivalently and with the same probability  that there exists $\zeta(\eps)>0$ such that
\begin{align}\label{eq:2show}
\min_{\theta\in \Sc_\eps^c} \Lc(\theta) \geq \min_{\theta\in \R^d} \Lc(\theta) + \zeta(\eps).
\end{align}
Here, $\Sc_\eps^c$ denotes the complement of the set $\Sc_\eps$. 
Now, to prove Equation \eqref{eq:2show} we proceed in the following four steps paralleling the exposition in Section \ref{subsec:CGMT-heuristic}. 

\vp
\noindent\emph{Step 1: Write as bounded minimax optimization of a bi-linear form.}  This first step express the original optimization problem in \eqref{eq:opt_gen_intro} in an appropriate min-max form with \emph{bounded} constraints (as required by Theorem \ref{thm:gordon}).

\vp
\noindent\emph{Step 2: Invoke the CGMT.}  Here, we bring the bounded min-max optimization problem of the previous step in the appropriate form of a \eqref{eq:CGMT-PO}. Based on this, we formulate the corresponding, simpler to analyze, \eqref{eq:CGMT-AO}.

\vp
\noindent\emph{Step 3: Solving the AO.} Coming next, is the main step of the proof, which involves analyzing the \eqref{eq:CGMT-AO}. We organize the analysis in this part in two sub-steps as follows

\emph{Step 3a: Unifying analysis.} We reduce the \eqref{eq:CGMT-AO} to a simpler lower-dimensional optimization problem in which the variables $\xi(\theta),\alpha(\theta),\beta(\theta)$ appear explicitly as optimization variables. For this part, we operate under the general assumptions in Section \ref{sec:gordon_assumptions}.


\emph{Step 3b: Specializing to first- and second- order losses.} In this second part, we specialize the analysis to the two loss functions in Equations \eqref{eq:GD_gen} and \eqref{eq:sec_order_gen}. For these two losses, 
 we will show that the AO problem simplifies to an optimization problem over only a few scalar variables. This will allow us to  characterize key \emph{concentration} and \emph{deviation} properties of its optimal cost, which are required by the CGMT (see Theorem \ref{thm:CGMT} below).

\vp
\noindent\emph{Step 4: Completing the proof.} Once we have analyzed the \eqref{eq:CGMT-AO}, we complete the proof of Theorem \ref{thm:gordon_main} by invoking the CGMT.


%The core of the proof concerns the analysis of the AO. This is the subject of Sections XXX. Here, we show how to arrive at the AO.

%\paragraph{The Primary Optimization.} 
%We write the optimization problem in \eqref{eq:opt_gen_intro} in an equivalent min-max form. 
%We will need the following two assumptions.
%
%Here, we show how this is achieved and we proceed with explaining how the new min-max form allows the use of the framework.

\subsubsection{Step 1: Write as bounded minimax optimization  of a bi-linear form}
The following lemma, proved in Section \ref{sec:minmax_proof}, transforms the original problem \eqref{eq:opt_gen_intro} into a min-max problem with \emph{bounded} constraint sets.
%admissible by the CGMT \eqref{eq:CGMT-PO}.

\begin{lemma}[Bounded PO]\label{lem:minmax}
Let Assumptions \ref{ass:Lip} and \ref{ass:theta_bd}  hold. For $\eps>0$ consider the set $\Sc_\eps$ in Equation \eqref{eq:S_2show}. Let pair of sets $\bar\Dc, \Dc\subset\R^d$ be chosen as either one of the following two options: (i) $\bar\Dc=\R^d$, $\Dc = \Bc_2(C_1)$, or (ii) $\bar\Dc=\Sc_\eps^c$, $\Dc=\Bc_2(C_1)\cap\Sc_\eps^c$,
and define the primary optimization (PO), 
\begin{align}\label{eq:PO}
\Phi_{n,\Dc}:=\min_{ \substack{\theta\in\Dc\\ \|\ub\|_2\leq C_2\sqrt{n} } } \; \max_{\|\vb\|_2\leq C_3 } \; \;\frac{1}{\sqrt{n}}\langle \vb, \bX \theta - \ub \rangle + \Fc_t(\ub,\theta).
\end{align}
For sufficiently large positive constants $C_1,C_2=C_2(\delta),C_3=C_3(R)>0$, there exist positive $c,C>0$ such that
$
\Pro\big\{\min_{\theta \in \bar\Dc } \mathcal{L} (\theta ) =  \Phi_{n,\Dc} \big\} \geq 1-Ce^{-cn}.
$
%Moreover the $\theta$-minimization sets of the two problems above are identical.
\end{lemma}

For the optimization $\min_{\theta \in \bar\Dc } \mathcal{L} (\theta )$ in the statement of the lemma, note that the choices $\bar\Dc=\R^d$ and $\bar\Dc=\Sc_\eps^c$ correspond to the minimization problems in the RHS and LHS of the desired Equation \eqref{eq:2show}, respectively. 
%Note that both the minimization and maximization sets in \eqref{eq:PO} are bounded as required by Theorem \ref{thm:gordon}.  

\subsubsection{Step 2: Invoke the CGMT}
To continue, we use the decomposition property of $\Fc_t(\ub,\theta)$ in Assumption \ref{ass:loss}(i) and $\X=\X P_{S^t} +\X P^\perp_{S^t} $ to expand the objective function in \eqref{eq:PO} in the following form:
\begin{align}
h(\theta, \thetacur) + g(\ub, \X\thetacur; \y ) - \frac{1}{\sqrt{n}} \langle \vb, \ub \rangle + \frac{1}{\sqrt{n}}\langle \vb, \bX P_{S^t} \theta \rangle +\frac{1}{\sqrt{n}} \langle \vb, \bX P^{\perp}_{S^t} \theta \rangle\,,\notag
\end{align}
Here, observe that the matrix $\X P^{\perp}_{S^t}$ is Gaussian and uncorrelated, thus independent, of everything else random in the objective that otherwise only depends on $\X$ through $\X\thetacur$ and $\X\theta^\star$ (through $\y$). Thus, we can substitute $\X P^{\perp}_{S^t}$ with $\G P^{\perp}_{S^t}$ for an \emph{independent} copy $\G$ of $\X$. With these, we arrive at the specific form of the \eqref{eq:CGMT-PO} specialized to our problem of interest. With some abuse of terminology, we will refer to this optimization  as the \eqref{eq:PO2}. 
\begin{align}\label{eq:PO2}
\Phi_{n,\Dc}&:=\min_{ \substack{\theta\in\Dc \\ \|\ub\|_2\leq C_2\sqrt{n} } } \; \max_{\|\vb\|_2\leq C_3 } \; \;\frac{1}{\sqrt{n}} \langle \vb, \G P^{\perp}_{S^t} \theta \rangle \tag{\red{PO}} \\
&\qquad\qquad\qquad\qquad\qquad+ h(\theta, \thetacur) + g(\ub, \X\thetacur; \y ) - \frac{1}{\sqrt{n}} \langle \vb, \ub \rangle + \frac{1}{\sqrt{n}}\langle \vb, \bX P_{S^t} \theta \rangle\,. \nn
\end{align}
%%Thus, letting $\thetanext$ denote a solution to \eqref{eq:opt_gen_intro} and $\thetanexthat$ a solution to $\Phi_{n,\Bc_2(C_1)}$, Lemma \ref{lem:minimax} implies also that
%%\begin{align}\label{eq:pro_bd}
%%\Pro\left\{\thetanext\not\in\Sc_\eps \right\} \leq \Pro\left\{\thetanexthat\not\in\Sc_\eps \right\} + Ce^{-cn}.
%%\end{align}
%Now, we are ready to formulate the \eqref{eq:CGMT-AO} and establish its relation to the PO. To find the AO we rewrite \eqref{eq:PO} as follows:
%\begin{align}\label{eq:PO2}
%\Phi_{n,\Dc}:=\min_{ \substack{\theta\in\Dc \\ \|\ub\|_2\leq C_2\sqrt{n} } } \; \max_{\|\vb\|_2\leq C_3 } \; \;\Fc_t(\ub,\theta) - \frac{1}{\sqrt{n}} \langle \vb, \ub \rangle + \frac{1}{\sqrt{n}}\langle \vb, \bX P_{S^t} \theta \rangle +\frac{1}{\sqrt{n}} \langle \vb, \bX P^{\perp}_{S^t} \theta \rangle\,.\tag{\red{PO}}
%\end{align}
%This is the form of the \eqref{eq:CGMT-PO} specialized to our problem of interest. With some abuse of terminology, we will refer to this optimization  as the \eqref{eq:PO2}. 
%where we allow the minimization over $\theta$ to be over a compact set $\Dc$ that is chosen as either one of the following two:
%\begin{itemize}
%\item $\Dc:=\left\{\theta\,|\,\|\theta\|_2\leq C_1\right\}$ to retrieve \eqref{eq:PO}.
%\item $\Dc=\left\{\theta\,|\,\|\theta\|_2\leq C_1\right\}\cap \Sc_\eps^c$ corresponding to the `perturbed PO' in the LHS of \eqref{eq:2show}.
%\end{itemize}

To invoke the full power of the CGMT, note here that the objective function of the \eqref{eq:PO2} is convex-concave thanks to Assumption \eqref{ass:loss}(ii). Now, we can directly write the \eqref{eq:CGMT-AO} corresponding to \eqref{eq:PO2} as shown below  with $\h \sim {\sf N}(0, \bI_d)$ and $\g \sim {\sf N}(0, \bI_n)$ drawn independently of everything else:
\begin{align}
\phi_{n,\Dc}&:=\min_{ \substack{\theta\in\Dc \\ \|\ub\|_2\leq C_2\sqrt{n} } } \; \max_{\|\vb\|_2\leq C_3 } \; \; \frac{1}{\sqrt{n}} \| P^{\perp}_{S^t} \theta \|_2 \langle \vb, \g \rangle +\frac{1}{\sqrt{n}} \| \vb \|_2 \langle \h, P^{\perp}_{S^t} \theta \rangle \label{eq:AO}\tag{\red{AO}}
\\
&\qquad\qquad\qquad\qquad\qquad\qquad + h(\theta, \thetacur) + g(\ub, \X\thetacur; \y )  -\frac{1}{\sqrt{n}} \langle \vb, u \rangle +\frac{1}{\sqrt{n}} \langle \vb, \bX P_{S^t} \theta \rangle \nn.
\end{align}
%Here, 
%step $(i)$ holds with high probability (up to a fluctuation of size $1/ \sqrt{n}$ \apcomment{check}) by Gordon's comparison theorem, 


  The following lemma is a restatement of the CGMT \cite[Thm.~3]{thrampoulidis2015regularized} applied in our setting. It shows that it suffices analyzing the \eqref{eq:AO} to conclude about the minimizers of the bounded \eqref{eq:PO2}.
\begin{theorem}[CGMT]\label{thm:CGMT}
Consider the Auxiliary Optimization problem in \eqref{eq:AO} and the set $\Sc_\eps$ defined in Equation \eqref{eq:S_2show} for some $\eps>0$. Let Assumptions \ref{ass:loss}(i),(ii), \ref{ass:Lip} and \ref{ass:theta_bd} hold.  Suppose there exist constant $\bar\phi$ and $\zeta=\zeta(\eps)>0$ such that the following two conditions hold with probability $1-p_n(\eps)$ each:
\begin{subequations}\label{eq:cgmt_2prove}
\begin{align}
%(i)~~
~~\phi_{n,\Bc_2(C_1)} &\leq \bar\phi + \zeta,\\
%(ii)~~
~~\phi_{n,\Bc_2(C_1)\cap\Sc_\eps^c} &\geq \bar\phi + 2\zeta.
\end{align}
\end{subequations}
Then, it holds for the solution $\thetaplushat$ of the (bounded) \eqref{eq:PO2} with $\Dc=\Bc_2(C_1)$ that
$
\thetaplushat\in\Sc_\eps
$
with probability at least $1-4p_n(\eps).$
\end{theorem}



%\begin{theorem}[CGMT]\label{thm:CGMT}
% Let $\Dc$ a compact subset of $\Bc_2(C_1)$. The following statements are true:
%
%1. For all $t\in\R$, $\Pro\left\{ \Phi_{n,\Dc} \leq t \right\} \leq 2\Pro\left\{ \phi_{n,\Dc} \leq t \right\}$.
%
%2. If the set $\Dc$ is convex, then, it also holds for all $t$ that $\Pro\left\{ \Phi_{n,\Dc} \geq t \right\} \leq 2\Pro\left\{ \phi_{n,\Dc} \geq t \right\}$.
%
%3. For some $\eps>0$ consider the set $\Sc_\eps$ defined in \eqref{eq:S_2show}. Suppose there exist constant $\bar\phi$ and $\zeta=\zeta(\eps)$ such that the following two conditions hold with probability $1-p_n(\eps)$ each:
%\begin{align}\label{eq:cgmt_2prove}
%\begin{cases}
%(i)~~\phi_{n,\Bc_2(C_1)} \leq \bar\phi + \zeta,\\
%(ii)~~\phi_{n,\Bc_2(C_1)\cap\Sc_\eps^c} \geq \bar\phi + 2\zeta.
%\end{cases}
%\end{align}
%Then, it holds for the solution $\thetanexthat$ of the PO in \eqref{eq:PO2} with $\Dc=\Bc_2(C_1)$ that
%$
%\Pro\left\{\thetanexthat\in\Sc_\eps\right\} \geq 1-4p_n(\eps).
%$
%\end{theorem}
% together with Lipschitzness of the AO.

We can immediately translate these statements to the original optimization of interest in \eqref{eq:opt_gen_intro} using Lemma \ref{lem:minmax}. This leads to the following corollary.

\begin{corollary}\label{cor:unbounded_cgmt}
Assume the setting and conditions of Theorem \ref{thm:CGMT} hold. Then, for  $\thetaplus$ solving \eqref{eq:opt_gen_intro} it holds that 
$
\Pro\left\{\thetaplus\in\Sc_\eps\right\} \geq 1-4p_n(\eps)-Ce^{-cn}.
$
\end{corollary}
%\begin{proof}
%This is a direct corollary of Theorem \ref{thm:CGMT} combined with \eqref{eq:pro_bd} of Lemma \ref{lem:minmax}.
%\end{proof}

%\begin{proof}
%From the CGMT, the following two hold for all $c\in\R$
%
%1. $\Pro\left\{ \Phi_{n,\Dc} \leq c \right\} \leq 2\Pro\left\{ \phi_{n,\Dc} \leq c \right\}$.
%
%2. If the set $\Dc$ is convex, then  $\Pro\left\{ \Phi_{n,\Dc} \geq c \right\} \leq 2\Pro\left\{ \phi_{n,\Dc} \geq c \right\}$.
%
%
%\end{proof}

With these our goal becomes proving the two conditions in Equation \eqref{eq:cgmt_2prove} regarding the \eqref{eq:AO}.


%\subsection{Main result}

\subsubsection{Step 3: Solving the AO} 
As we discussed, much of our analysis is unified for the two losses of interest in Equations \eqref{eq:GD_gen} and \eqref{eq:sec_order_gen}. Here, we state our key final conclusion about the AO problems for the two specific cases of interest. 
%
Recall the definition of $\omegab_t$ in Assumption \ref{ass:omega}, and that $\gammab_1,\gammab_2,\g\in\R^n, \h\in\R^d$ denote independent standard normal vectors. Also, recall that for generic triplet $\xi,\alpha,\beta$ we denote
$
\thetathree=(\xi,\alpha,\beta)
$
for convenience. Similarly, we define the 3-dimensional projection of a set $\Dc\in\R^d$ on the $(\xi,\alpha,\beta)$-space, that is
\begin{align}\label{eq:Dcthree}
\Dcthree := 
\Big\{ \tb\in\R^3 \,\,:\,\,  \tb=\left(\xitheta,\alphatheta,\betatheta\right) \,\,\text{and}\,\, \theta\in\Dc\Big\}.
\end{align}

%\paragraph{Second-order methods.}

\paragraph{Step 3a: Unifying Analysis.}
The first lemma is a byproduct of our unifying analysis of the AO for general loss functions satisfying Assumption \ref{ass:loss} and reduces the \eqref{eq:AO} to a lower-dimensional min-max optimization that is explicitly parameterized in terms of the quantities of interest $\xi,\alpha,\beta$.


\begin{lemma}[Low-dimensional AO]\label{lem:lowAO}
Consider the \eqref{eq:AO} for a loss function satisfying Assumption \ref{ass:loss}. Let $\phi_{n,\Dc}$ denote its optimal cost. Then, there exist universal constants $C,c>0$ such that with probability at least $1-Ce^{-cn}$ it holds:
\begin{align}
{{\phi_{n,\Dc}=\min_{(\xi,\alpha,\beta)\in\Dcthree}\max_{\vb} \;\; \hscal(\xi,\alpha,\beta,\thetacur) - g^*(\vb,\X\thetacur;\y) -\beta \|P^{\perp}_{S^t}\h\|_2\|\vb\|_2+\inp{\beta\g+\xi\gammab_1+\alpha\gammab_2}{\vb}.}} \label{eq:lowAO}\tag{\red{low-dim. AO}}
\end{align}
Here, $g^*$ denotes the convex-conjugate function of the function $g$. The latter and $\hscal$ are as defined in Assumption \ref{ass:loss}(iii).
\end{lemma} 


\paragraph{Step 3b: Specializing to first- and second- order losses.}
The first lemma concerns the loss of second-order methods in Equation \eqref{eq:sec_order_gen}.

\begin{lemma}[AO analysis: second-order methods]\label{lem:AO_main_sec}
Consider the \eqref{eq:lowAO} for the loss function defined in \eqref{eq:sec_order_gen}. Let Assumption \ref{ass:omega} hold.
% and recall the definition 

\textbf{Part A---(Scalarization).}~For 
any  compact subset $\Dc\subset\Bc(C_1)$,   
sufficiently large constants $C_1,C_2>0$ and sufficiently large $C_3>0$,  there exist constants $c,C>0$ such that with probability at least $1-Ce^{-cn}$, the \eqref{eq:AO} reduces to 
\begin{align}
\phi_{n,\Dc}&=\left(\min_{ \substack{ (\xi,\alpha,\beta)\in\Dcthree  }} L_n(\thetathree)\right)_+\,\quad\text{where}~~ L_n(\thetathree) := \; \frac{\|\beta\g+\xi\gammab_1+\alpha\gammab_2-\omegab_t\|_2}{\sqrt{n}} -  \frac{\beta\| P^{\perp}_{S^t}\h \|_2}{\sqrt{n}}\label{eq:AO_final_main}\,.
\end{align}
Here, $(x)_+=x\vee 0.$

\textbf{Part B---(Concentration).}~For $n$ large enough, there exist absolute constants $C,c,C',c'>0$ and $c_\delta>1$ such that for all $\delta>c_\delta$ and  $c'>\eps>C'n^{-\nicefrac{1}{2}}$, with probability at least {$1-Ce^{-cn\eps^2}$}, the minimizer $\thetathree_n\in\arg\min_{\thetathree\in\Pc_3(\Bc_2(C_1))} L_n(\thetathree)$  is unique and satisfies
\begin{align}\label{eq:bar_L_sec}
\left| L_n(\thetathree_n)- \bar{L}\right|\leq \eps,\quad\text{where } \bar{L}:=\sqrt{\left(1-\frac{1}{\delta}\right)\left(\E[\Omega_t^2]-\left(\E[G_1\Omega_t]\right)^2-\left(\E[G_2\Omega_t]\right)^2\right)}.
\end{align}

\textbf{Part C---(Deviation).}~Under the same assumptions as in (Concentration) and with the same high probabability,
 the following strong convexity property holds for absolute constant $C_\tau>0$:
\begin{align}
\min_{\|\thetathree-\thetathree_n\|_2\geq \eps} L_n(\thetathree) \geq  L_n(\thetathree_n)+C_\tau\eps^2.
\end{align}
%
%\begin{enumerate}
%\item With probability at least {$1-Ce^{-cn\eps^2}$},
%\begin{subequations}
%\begin{align}\label{eq:tau_star_sec}
%&\left|\tau_n-\tau_\star\right|\leq \eps,\qquad\text{where}\quad\tau_\star = \sqrt{\left(\frac{\delta}{\delta-1}\right)\left(\E[\Omega_t^2]-\left(\E[G_1\Omega_t]\right)^2-\left(\E[G_2\Omega_t]\right)^2\right)}
%\\
%&\left|\xi_n-\xi_*\right| \vee \left|\alpha_n-\alpha_*\right| \vee \left|\beta_n-\beta_*\right| \leq \eps,\qquad\text{where}\quad\begin{cases}
%~\xi_*=\E[G_1\Omega_t]\\
%~\alpha_*=\E[G_2\Omega_t]\\
%~\beta_*={\tau_*}\big/{\sqrt{\delta}}.
%\end{cases}
%\label{eq:theta_star_sec}
%\end{align}
%\end{subequations}
%
%
%\item With probability at least {$1-Ce^{-cn\eps^2}$},
%\begin{align}\label{eq:bar_L_sec}
%\left| L_n(\thetathree_n)- \bar{L}\right|\leq \eps,\quad\text{where } \bar{L}:=\left(1-\frac{1}{\delta}\right)\tau_*.
%\end{align}
%
%
%\item With probability at least {$1-Ce^{-cn\eps^2}$}, there exists absolute constant $C_\tau>0$ following strong convexity property holds 
%\begin{align}
%%\min_{\|\thetathree-\thetathree_n\|_2\geq \eps} L_n(\thetathree) \geq  L_n(\thetathree_n)+\frac{1}{16\tau_*}\eps^2.
%\min_{\|\thetathree-\thetathree_n\|_2\geq \eps} L_n(\thetathree) \geq  L_n(\thetathree_n)+C_\tau\eps^2.
%\end{align}
%%for all $\eps>C'n^{-\nicefrac{1}{2}}.$
%
%\end{enumerate}


\end{lemma}

%\paragraph{First-order methods.}

Next, we present our result about the \eqref{eq:AO} for the loss of first-order methods in Equation \eqref{eq:GD_gen}.

\begin{lemma}[AO analysis: first-order methods]\label{lem:AO_main_gd}
Consider the \eqref{eq:AO} for the loss function defined in \eqref{eq:sec_order_gen}. Let Assumption \ref{ass:omega} hold.
% and recall the definition 

\textbf{Part A---(Scalarization).}~For 
any  compact subset $\Dc\subset\Bc(C_1)$,   
sufficiently large constants $C_1,C_2>0$ and sufficiently large $C_3>0$,  there exist constants $c,C>0$ such that with probability at least $1-Ce^{-cn}$, the \eqref{eq:AO} reduces to
\begin{align}
&\phi_{n,\Dc}=\min_{ { (\xi,\alpha,\beta)\in\Dcthree  }} L_n(\thetathree)
\label{eq:Ln_gd}
\\
&\text{where}\qquad L_{n}(\thetathree):=\frac{\xi^2+\alpha^2+\beta^2}{2} - \big(\xi\xit +\alpha\sigmat \big)  - \frac{2\eta}{n}\inp{\omegab_t}{\beta\g+\xi\gammab_1+\alpha\gammab_2} - \,\frac{2\eta \beta}{n} \| P^{\perp}_{S^t}\h \|_2 \|\omegab_t\|_2.\nn
\end{align}

\textbf{Part B---(Concentration).}~For $n$ large enough, there exist absolute constants $C,c,C',c'>0$ and $c_\delta>1$ such that for all $\delta>c_\delta$ and  $c'>\eps>C'n^{-\nicefrac{1}{2}}$, with probability at least {$1-Ce^{-cn\eps^2}$}, the minimizer $\thetathree_n\arg\min_{\thetathree\in\Pc_3(\Bc_2(C_1))} L_n(\thetathree)$ is unique and 
\begin{align}\label{eq:bar_L_sec}
\left| L_n(\thetathree_n)- \bar{L}\right|\leq \eps,\quad\text{where } \bar{L}:=-\frac{1}{2}\left(\xinextstar^2+\alphanextstar^2+\betanextstar^2\right),
\end{align}
and $\xinextstar,\alphanextstar,\betanextstar$ are as defined in Equation \eqref{eq:theta_starnext_gd_main}.

\textbf{Part C---(Deviation).}~It is always true (that is, for all realizations of $\g,\h,\gammab_1,\gammab_2,\omegab_t$) that
\begin{align}
\min_{\|\thetathree-\thetathree_n\|_2\geq \eps} L_n(\thetathree) \geq  L_n(\thetathree_n)+\frac{1}{2}\eps^2.
\end{align}
\end{lemma}

We prove Lemmas \ref{lem:AO_main_sec} and \ref{lem:AO_main_gd} in Sections \ref{sec:scal_proof_main} and \ref{sec:conc_proof_main}. Specifically, we split the analysis in two parts. In the first part (Section \ref{sec:scal_proof_main}), where we prove the \emph{(Scalarization)} results of the lemmas, we essentially unify the analysis over the two losses of interest. \emph{(Concentration)} and \emph{(Deviation)} require a case-by-case treatment for the two losses (Section \ref{sec:conc_proof_main}). 


%% ================================================== %%
\subsubsection{Step 4: Completing the proof}
%% ================================================== %%
We are now ready to complete the proof Theorem \ref{thm:gordon_main}. We do this for each one of the two loss functions using the corresponding Lemmas \ref{lem:AO_main_sec} and \ref{lem:AO_main_gd} to confirm the two conditions in Equation \eqref{eq:cgmt_2prove} required by the CGMT Theorem \ref{thm:CGMT}.

\paragraph{Proof for Second-order methods.}
 Consider the setting of Lemma \ref{lem:AO_main_sec}.
 % and constants $C',C_\tau$ as defined therein. 
Specifically, recall the definition of $\bar{L}$ and let $\thetathreestar$ denote the triplet $(\xinextstar,\alphanextstar,\betanextstar)$ as defined in \eqref{eq:theta_starnext_sec_main}. By Lemma \ref{lem:AO_main_sec}, there exist absolute constants $c',C',C_\tau,C,c>0$ such that for any $c'>\eps>C'n^{-\nicefrac{1}{2}}$ with probability at least $1-Ce^{-cn\eps^4}$,  the following hold:
\begin{subequations}\label{eq:event_thm_proof}
\begin{align}
\min_{\|\thetathree-\thetathree_n\|_2\geq \frac{\eps}{2}} L_n(\thetathree) &\geq  L_n(\thetathree_n)+\frac{C_\tau\eps^2}{4}\\
\|\thetathree_n-\thetathree_*\|_2&\leq \frac{\eps}{2}\\
\left|L_n(\thetathree_n)-\bar{L}\right|&\leq \frac{C_\tau\eps^2}{12}.\label{eq:Ln_conc}
\end{align}
\end{subequations}
Note here that we require in \eqref{eq:Ln_conc} concentration of order $\eps^2$ (instead of order $\eps$ as stated in Equation \eqref{eq:bar_L_sec}), thus making the probability of success $1-Ce^{-cn\eps^4}$ rather than $1-Ce^{-cn\eps^2}$ in Lemma \ref{lem:AO_main_sec}. 
Combined, these give the following, for $\zeta:=\frac{C_\tau\eps^2}{12}$,
\begin{subequations}\label{eq:done_sec}
\begin{align}
L_n(\thetathree_n) &\leq \bar{L} + \zeta
\\
\min_{\|\thetathree-\thetathree_*\|_2\geq \eps} L_n(\thetathree) &\geq \min_{\|\thetathree-\thetathree_n\|_2\geq \frac{\eps}{2}} L_n(\thetathree) \geq L_n(\thetathree) + 3\zeta \geq  \bar{L}+2\zeta\,.\label{eq:done_sec_b}
\end{align}
\end{subequations}
The first inequality in \eqref{eq:done_sec_b} follows from the chain of inequalities: $\eps\leq\|\thetathree-\thetathree_*\|_2 \leq \|\thetathree-\thetathree_n\|_2 + \|\thetathree_n-\thetathree_*\|_2 \leq \|\thetathree-\thetathree_n\|_2 + \eps/2\implies \|\thetathree-\thetathree_n\|_2 \geq \eps/2.$  Also, in the event of Equation \eqref{eq:Ln_conc} above, it holds $L_n(\thetathree_n)\geq \bar{L}-\zeta>0$ (for small enough $c'$). Thus, $\big(L_n(\thetathree_n)\big)_+ = L_n(\thetathree_n)$ and from Equation, \eqref{eq:AO_final_main}
$
\phi_{n,\Dc} = \min_{\thetathree\in\Dcthree}L_n(\theta).
$
Specifically, this implies the followings in the event of \eqref{eq:event_thm_proof}:
\begin{subequations}
\begin{align}
\phi_{n,\Bc_2(C_1)} &= \min_{\thetathree\in\Bc(C_1)}L_n(\theta)\\
\phi_{n,\Bc_2(C_1)\cap\Sc_\eps^c} &= \min_{\|\thetathree-\thetathreestar\|_{\infty}\geq\eps}L_n(\theta) \geq \min_{\|\thetathree-\thetathreestar\|_2\geq \eps}L_n(\theta).
\end{align}
\end{subequations}
In the last equation, we recalled the definition of the set $\Sc_\eps$ in the statement of Theorem \ref{thm:gordon_main} and used that $\theta\in\Sc_\eps^c\iff\|\thetathree-\thetathreestar\|_\infty\geq\eps\implies\|\thetathree-\thetathreestar\|_2\geq \eps$. Thus, the inequality follows by relaxing the minimization set.

Together, Equations \eqref{eq:done_sec} and \eqref{eq:event_thm_proof} confirm the validity of the two conditions in Equation \eqref{eq:cgmt_2prove} of Theorem \ref{thm:CGMT} (with $\bar\phi\leftarrow\bar{L}$).  Thus, from Corollary \ref{cor:unbounded_cgmt} with the desired probability $\thetaplus\in\Sc_\eps$ and the proof of Equation \eqref{eq:S_2show} is complete.
%\end{proof}

Now, we use \eqref{eq:S_2show} together with $\sigma(\thetaplus)=\sqrt{\alpha(\thetaplus)^2+\beta(\thetaplus)^2}$ to prove \eqref{eq:sigma_2show}. Onwards, we condition on the high-probability event in \eqref{eq:S_2show}.

 Using Assumption \ref{ass:omega}(ii), it is not hard to check in \eqref{eq:theta_starnext_sec_main} that $\alphanextstar\geq c>0$ and $\betanextstar\geq c(\delta)>0$. Thus, for $\eps$ smaller than appropriate constant, it holds that $0<\alphanextstar-\eps\leq|\alpha(\thetaplus)|\leq\alphanextstar+\eps$ and $0<\betanextstar-\eps\leq|\beta(\thetaplus)|\leq \betanextstar+\eps$.  Using these, we have the following with probability $1-Ce^{-cn\eps^2}$:
\begin{align*}
\sigma=\sqrt{\alpha(\thetaplus)^2+\beta(\thetaplus)^2} &\leq 
\sqrt{ \alphanextstar^2+\betanextstar^2+2\eps^2+2(\alphanextstar+\betanextstar)\eps } \\
&\leq 
\sqrt{ \alphanextstar^2+\betanextstar^2+C\eps } \\
&\leq 
\sqrt{ \alphanextstar^2+\betanextstar^2 } \sqrt{1+C(\delta)\eps } \leq \sqrt{\alphanextstar^2+\betanextstar^2} + C(\delta)\,\eps.
\end{align*}
In the second inequality, we used from Assumption \ref{ass:omega} that $\alphanextstar\vee\betanextstar\leq C$  and also $\eps<1$. In the second inequality, we used $\alphanextstar^2+\betanextstar^2\geq c(\delta)$ and the fact $\sqrt{1+x}\leq 1+x/2, \forall x$.
%Indeed, we can check that
%\begin{align*}
%&\sqrt{ \alphanextstar^2+\betanextstar^2+2\eps^2+2(\alphanextstar+\betanextstar)\eps } \leq \sqrt{\alphanextstar^2+\betanextstar^2} + C\eps\\
%&\qquad\Longleftarrow 2\eps^2+2(\alphanextstar+\betanextstar)\eps \leq  C^2\eps^2 + 2C\sqrt{\alphanextstar^2+\betanextstar^2} \,\eps\\
%& \qquad\Longleftarrow 2\eps^2+2\sqrt{2}\sqrt{\alphanextstar^2+\betanextstar^2}\eps \leq  C^2\eps^2 + 2C\sqrt{\alphanextstar^2+\betanextstar^2} \,\eps
% \Longleftarrow  C\geq \sqrt{2}.
%\end{align*} 

Similarly, 
\begin{align}
\sigma=\sqrt{\alpha(\thetaplus)^2+\beta(\thetaplus)^2} &\geq 
\sqrt{ \alphanextstar^2+\betanextstar^2+2\eps^2-2(\alphanextstar+\betanextstar)\eps } \nn
\\
&\geq 
\sqrt{ \alphanextstar^2+\betanextstar^2-C\eps } \nn
\\
&\geq 
\sqrt{ \alphanextstar^2+\betanextstar^2} \sqrt{1-C(\delta)\eps} 
\geq 
\left({1-C(\delta)\eps}\right) \sqrt{ \alphanextstar^2+\betanextstar^2} \nn\\
&\geq \sqrt{ \alphanextstar^2+\betanextstar^2} - C(\delta)\eps
\end{align}
In the second inequality, we used $\alphanextstar\vee\betanextstar\leq C$. The third inequality follows because $\alphanextstar^2+\betanextstar^2\geq c(\delta)$ and the fourth since $\sqrt{1-x}\geq 1-x, \forall x\in(0,1)$ and assuming $\eps$ small enough. The last inequality uses again  $\alphanextstar\vee\betanextstar\leq C$. 

Combining the above two displays shows \eqref{eq:sigma_2show} and completes the proof.
%for sufficiently small constant $c>0$. Here, we checked that for small enough $\eps$,
%\begin{align*}
%&\sqrt{ \alphanextstar^2+\betanextstar^2+2\eps^2-2(\alphanextstar+\betanextstar)\eps } \geq \sqrt{\alphanextstar^2+\betanextstar^2} - c\eps \\
%&\qquad\Longleftarrow 2\eps^2-2(\alphanextstar+\betanextstar)\eps \geq  c^2\eps^2 - 2c\sqrt{\alphanextstar^2+\betanextstar^2} \,\eps
% \Longleftarrow  c\leq \sqrt{2}.
%\end{align*}
%Combined, we have shown that there exists constant $c'>0$ such that with probability at least $1-Ce^{-cn\eps^2}$:
%$$
%\sigmanextstar - c'{\eps} \leq \sigma(\thetaplus) \leq \sigmanextstar + c'\eps.
%$$
%This completes the proof.


\paragraph{First-order methods.} The proof for first-order methods is identical to the proof above, only now we use Lemma \ref{lem:AO_main_sec} instead. Accordingly, the only change above is substituting $C_\tau\mapsto 1$ in Equations \eqref{eq:Ln_conc}. We omit repeating the details for brevity.



%% ================================================= %%
%\subsection{Analysis of the AO}

\subsection{Low-dimensional AO {(Proof of Lemma \ref{lem:lowAO})}}\label{sec:scal_proof_main}
In this section, we prove Lemma \ref{lem:lowAO}. In words --- under the general  Assumption \ref{ass:loss} on the loss, we reduce the original AO \eqref{eq:AO} to the low-dimensional \eqref{eq:lowAO}.
%\subsubsection{General loss}
%% ================================================= %%
We organize the analysis here in a series of steps, which we explain progressively. 

\paragraph{Scalarize maximization.}~First, we perform the maximization over the direction of $\vb$ to rewrite $\phi_{n,\Dc}$ as
\begin{align}
\phi_{n,\Dc}=&\min_{ \substack{\theta\in\Dc \\ \|\ub\|_2\leq C_2\sqrt{n} } } \; \max_{0\leq \rho_\vb\leq C_3 } \; \; \Fc_t(\ub,\theta) +\frac{\rho_\vb}{\sqrt{n}} \Big( \langle \h, P^{\perp}_{S^t} \theta \rangle + \Big\| \| P^{\perp}_{S^t} \theta \|_2 \g+ \X P_{S^t}\theta - \ub  \Big\|_2\Big).\label{eq:first_ao}
\end{align}
Now, we can optimize over the direction of $P_{S^t}^\perp\theta$ as follows. Recalling the notation in Equation \eqref{eq:scal} decompose
$
\theta =  P_{S^t}\theta +  P_{S^t}^\perp\theta =\xi\,{\thetastar} + \alpha \left( \nicefrac{P_{\thetastar}^\perp\thetacur}{\|P_{\thetastar}^\perp\thetacur\|_2} \right) + P_{S^t}^\perp\theta,
$ 
and note that for any function $f(\theta)$: 
$$\min_{\theta\in\Dc} f(\theta) = \min_{(\xi, \alpha, \beta) \in \Dcthree }\min_{\|P_{S^t}^\perp\theta\|_2=\beta}\, f\left( \xi\,{\thetastar} + \alpha \left( \nicefrac{P_{\thetastar}^\perp\thetacur}{\|P_{\thetastar}^\perp\thetacur\|_2} \right) + P_{S^t}^\perp\theta \right),$$
where recall the definition of $\Dcthree$ in \eqref{eq:Dcthree}. It is convenient to define
$$\gammab_1:=\X{\thetastar}\quad\text{and}\quad\gammab_2:=\X {P_{\thetastar}^\perp\thetacur}\big/{\|P_{\thetastar}^\perp\thetacur\|_2}\,.$$
Note that $\gammab_1\sim\Nn(0,\mathbf{I}_n),\gammab_2\sim\Nn(0,\mathbf{I}_n)$ and are independent of each other. Specifically, in this notation, we can write
$$
\y = f\big(\gammab_1;\zb\big)+\epsb\qquad\text{and}\qquad \X\thetacur=\xit \gammab_{1}+\sigmat \gammab_{2}.
$$

Recall now from Assumption \ref{ass:loss} that $h(\theta,\thetacur)$ depends on $P_{S^t}^\perp\theta$ only through its norm. Hence the direction of $P_{S^t}^\perp\theta$ enters the objective function in \eqref{eq:first_ao} only in the term $\inp{\h}{P_{S^t}^\perp\theta}$. In fact, for any value of $\rho_\vb\geq0$, the maximizer $P_{S^t}^\perp\theta$ takes the value $-\nicefrac{P_{S^t}^\perp\h}{\|P_{S^t}^\perp\h\|_2}$. Thus using \citep{KammounLemma}, the optimization \eqref{eq:first_ao}  simplifies to the following:
\begin{align}
\phi_{n,\Dc}=&\min_{ \substack{(\xi,\alpha,\beta)\in\Dcthree \\ \|\ub\|_2\leq C_2\sqrt{n} } } \; \max_{0\leq \rho_\vb\leq C_3 } \; \; \Fc_t(\ub,\theta) +\frac{\rho_\vb}{\sqrt{n}} \Big(\Big\| \beta \g+ \xi\gammab_1 + \alpha\gammab_2 - \ub  \Big\|_2 -  \beta\, \|P^{\perp}_{S^t}\h\|_2  \Big) 
%\nn\\
%=&\min_{ \substack{(\xi,\alpha,\beta)\in\Dcthree \\ \|\ub\|_2\leq C_2\sqrt{n} } } \; \max_{0\leq \rho_\vb\leq C_3 } \; \; \h(\theta,\thetacur)+\frac{1}{n}\sum_{i\in[n]}g(\ub_i,\inp{\x_i}{\thetacur};y_i) +\frac{\rho_\vb}{\sqrt{n}} \Big(\Big\| \beta \g+ \X P_{S^t}\theta - \ub  \Big\|_2 -  \beta\, \|P^{\perp}_{S^t}\h\|_2  \Big)
\label{eq:sec_ao},
\end{align}
where we used that $P_{S^t}\theta=\xi{\thetastar} + \alpha\left(\nicefrac{P_{\thetastar}^\perp\thetacur}{\|P_{\thetastar}^\perp\thetacur\|_2}\right) \implies \X P_{S^t}\theta=\xi\gammab_1 + \alpha\gammab_2.$




% and $\Fc_t(\ub,\theta)=f(\ub,\xi,\alpha,\beta)$ for appropriate function $f$ (as per Assumption \ref{ass:loss}).
%Define
%$$
%\Gc_{C_3}\big(\xi,\alpha,\beta,\ub\big) := \max_{0\leq \rho_\vb\leq C_3 } \; \; \Fc_t(\ub,\theta) +\frac{\rho_\vb}{\sqrt{n}} \Big(\Big\| \beta \g+ \X P_{S^t}\theta - \ub  \Big\|_2 -  \beta\, \|P^{\perp}_{S^t}\h\|_2  \Big).
%$$
%and note that the function is jointly convex in its arguments and also for every fixed $(\xi,\alpha,\beta,\ub)$:
%$$
%\lim_{C_3\rightarrow+\infty}\Gc_{C_3}\big(\xi,\alpha,\beta,\ub\big) = \sup_{\rho_\vb\geq 0 } \; \; \Fc_t(\ub,\theta) +\frac{\rho_\vb}{\sqrt{n}} \Big(\Big\| \beta \g+ \X P_{S^t}\theta - \ub  \Big\|_2 -  \beta\, \|P^{\perp}_{S^t}\h\|_2  \Big).
%$$
%But, point-wise convergence of convex functions implies uniform convergence over compact sets \cite[Thm. 10.8]{Roc}, i.e. $\Gc_{C_3}$

\paragraph{Reduce to constrained minimization.}~We now claim that we can always pick $C_3$ large enough (growing with $n$ if necessary) such that with probability at least $1-Ce^{cn}$:
%using $\frac{C_L(R)}{\sqrt{n}}$-Lipschitzness of $\Fc_t(\cdot,\theta)$ from Assumption \ref{ass:Lip} together with our choice of $C_3=2C_L(R)$ in Lemma \ref{lem:minmax}, we can show that the above simplifies to  \ct{to prove; same argument as Lemma \ref{lem:minmax}. Write a general lemma}
%\begin{align}\label{eq:conAO}
%\phi_{n,\Dc}=&\min_{ \substack{\theta\in\Dc \\ \|\ub\|_2\leq C_2\sqrt{n} } }  \; \Fc_t(\ub,\theta)\qquad \text{sub. to}~~~  \Big\| \| P^{\perp}_{S^t} \theta \|_2 \g+ \X P_{S^t}\theta - \ub  \Big\|_2\leq -\langle \h, P^{\perp}_{S^t} \theta \rangle.
%\end{align}
%Now, it is easy to optimize over the direction of $P^{\perp}_{S^t} \theta$: the optimal choice is to align with $-P^{\perp}_{S^t}\h$ such that the constraint set above is enlarged:
\begin{align}\label{eq:conAO2}
\phi_{n,\Dc}=&\min_{ \substack{ (\xi,\alpha,\beta)\in\Dcthree \\ \|\ub\|_2\leq C_2\sqrt{n} } }  \; \Fc_t(\ub,\theta)\qquad \text{sub. to}~~~  \Big\| \beta \g+ \xi\gammab_1 + \alpha\gammab_2 - \ub  \Big\|_2\leq \beta \|P^{\perp}_{S^t}\h\|_2 .
\end{align}
Note that the above reduction would be straightforward if  the maximization over $\rho_\vb$ was unbounded. We prove that large enough $C_3$ suffices in Section \ref{sec:proof_unbd_v}. 


\paragraph{Optimize over $\ub$.} Now, we will optimize over $\ub$. We do this in two steps. 

\noindent\underline{Step 1: Linearize.}~By Assumption \ref{ass:loss}, the objective function in \eqref{eq:conAO2} can be decomposed as $$
\Fc_t(\ub,\theta)=h(\theta,\thetacur)+g(\ub,\X\thetacur;y) = \hscal(\xi,\alpha,\beta,\thetacur)+g(\ub,\X\thetacur;y)
$$
 Moreover, $g(\cdot,\X\thetacur;y)$ is convex. Thus, letting $g^*(\cdot,\X\thetacur;y)$ denote its convex conjugate, we can linearize the minimization in \eqref{eq:conAO2}. Concretely, the optimization in \eqref{eq:conAO2} is equivalent to the following
\begin{align}
\phi_{n,\Dc}=&\min_{(\xi,\alpha,\beta)\in\Dcthree}\max_{\vb} \;\; \hscal(\xi,\alpha,\beta,\thetacur)- g^*(\vb,\X\thetacur;\y) + \min_{\|\ub\|_2\leq C_2\sqrt{n}} \inp{\ub}{\vb}\nn \\
&\qquad\text{sub. to}~~~~~~  \Big\| \beta \g+ \xi\gammab_1 + \alpha\gammab_2 - \ub  \Big\|_2\leq \beta \|P^{\perp}_{S^t}\h\|_2.\label{eq:conAO2_lin}
\end{align}
To arrive at this, we have further flipped the order of min-max between $\ub$ and $\vb$ which is allowed since the optimization set for $\ub$ is compact and the objective is convex on $\ub$ and concave on $\vb$. \footnote{\ct{Technically this is constrained min-max so seems a bit tricky. But you can arrive at the same by introducing $\vb$ earlier in \eqref{eq:sec_ao}.}}  This comes at the cost of introducing an additional maximization, but we will see that this will be easy to simplify.

\noindent\underline{Step 2: Minimize over $\ub$.}~We can now explicitly optimize over $\ub$ provided that the constant $C_2$ is large enough. This is shown in the next lemma.

\begin{lemma}\label{lem:phi_tilde_aux}
Let $A,B>0$ and vectors $\ab,\tb\in\R^n$. Assume that
%\begin{align}\label{eq:u_opt_lem_cond}
$
\|A\left(\nicefrac{\ab}{\|\ab\|_2}\right)+\tb\|_2\leq B.
$
%\end{align}
 Then, the optimal cost of the quadratic program
%\begin{align}\label{eq:u_opt_lem}
$\Big\{\min_{\|\ub\|_2\leq B} \inp{\ab}{\ub}\quad\text{sub. to}~~\|\tb-\ub\|_2\leq A \Big\}$ is equal to  $-A\,\|\ab\|_2+\inp{\ab}{\tb}.$
%\end{align}
\end{lemma}

Specifically,  note that the quadratic program in the lemma corresponds to the inner minimization with respect to $\ub$ in \eqref{eq:conAO2_lin} with the following substitutions
$$
\ab\leftarrow \vb,\quad \tb\leftarrow\beta\g+\xi\gammab_1+\alpha\gammab_2,\quad A\leftarrow \beta\| P^{\perp}_{S^t}\h \|_2, \quad B\leftarrow C_2\sqrt{n}.
$$
Moreover, we can always guarantee the condition in the statement of the lemma holds by making $C_2$ large enough. This is because of Gaussianity of $\g,\gammab_1,\gammab_2,\h$. The details together with the proof of Lemma \ref{lem:phi_tilde_aux} are deferred to Section \ref{sec:}. To summarize, the optimzation in \eqref{eq:conAO2_lin} is equivalent to \eqref{eq:lowAO}. That is, {with probability at least $1-Ce^{-cn}$}:
\begin{align}\label{eq:conAO2_no_u}
{{\phi_{n,\Dc}=\min_{(\xi,\alpha,\beta)\in\Dcthree}\max_{\vb} \;\; \hscal(\xi,\alpha,\beta,\thetacur) - g^*(\vb,\X\thetacur;\y) -\beta \|P^{\perp}_{S^t}\h\|_2\|\vb\|_2+\inp{\beta\g+\xi\gammab_1+\alpha\gammab_2}{\vb}.}}
\end{align}
%Here, recall that $h$ is a function of $(\alpha,\beta,\xi)$ as per Assumption \ref{ass:loss}.

%Our last step is to write the minimization over  $\ub$ in a more convenient form. For this, we go back to the Lagrangian formulation of \eqref{eq:conAO2} but only after squaring the two sides of the inequality constraint.  Additionally, we use the  {convexity assumption of $g(\cdot,\X\thetacur;\y)$} to apply Sion's min-max theorem \cite{} and bring the minimization over $\ub$ inside, as follows:
%\begin{align}\label{eq:AO_gen_fin}
%&\min_{ (\xi,\alpha,\beta)\in\Dcthree } \bigg\{ h(\theta,\theta_t) +  \; \max_{\lambda \geq 0 } \; \; \big\{- \frac{\lambda}{2n} \beta^2 \| P^{\perp}_{S^t}\h \|_2^2  \nn
%\\
%&\qquad\qquad\qquad\qquad\qquad+\min_{\|\ub\|_2\leq C_2\sqrt{n}}\big\{ \frac{\la}{2n}\Big\|\X P_{S^t}\theta + \beta \g - \ub\Big\|_2^2+ g(\ub,\X\thetacur;\y)\big\} \Big\} \bigg\}.
%\end{align}
%Now recall that
%$
%\thetacur = \xit \cdot\frac{\thetastar}{\|\thetastar\|_2} + P_{\thetastar}^\perp\thetacur,\qquad\text{with}~~\|P_{\thetastar}^\perp\thetacur\|_2=\sigmat .
%$
%and further denote 
%$$\gammab_1:=\X{\thetastar}\quad\text{and}\quad\gammab_2:=\X \frac{P_{\thetastar}^\perp\thetacur}{\|P_{\thetastar}^\perp\thetacur\|_2}$$
%where $\gammab_1\sim\Nn(0,\mathbf{I}_n),\gammab_2\sim\Nn(0,\mathbf{I}_n)$ and are independent of each other. In this notation, 
%$$
%\y = f\big(\gammab_1;\zb\big)+\epsb\qquad\text{and}\qquad \X\thetacur=\xit \gammab_{1}+\sigmat \gammab_{2}.
%$$
%
%Hence, the optimization in  \eqref{eq:AO_gen_fin} becomes
%\begin{align}
%&\min_{ (\xi,\alpha,\beta)\in\Dcthree} \; \max_{\lambda \geq 0 } \; \; h(\theta, \thetacur) - \frac{\lambda}{2n} \| P^{\perp}_{S^t}\h \|_2^2 \beta^2\nn \\
%&\qquad\qquad\qquad\qquad+\min_{\|\ub\|_2\leq C_2\sqrt{n}}\Big\{ \frac{\la}{2n}\Big\| \xi\gammab_1 + \alpha\gammab_2 + \beta \g - \ub\Big\|_2^2+ g(\ub,\xit \gammab_1+\sigmat \gammab_2;\y)\Big\},   \label{eq:AO_gen_fin2}
%\end{align}
%where recall that $h$ is a function of $(\alpha,\beta,\xi)$ (cf. Assumption \ref{ass:loss}).

%To proceed, we specialize our analysis to the specific choices of $h$ and $g$ corresponding to the two losses in Equations \eqref{eq:GD_gen} and \eqref{eq:sec_order_gen}, respectively.



%\subsection{First- and second- order losses}










\input{sections/Gordon/gordon_second_order}




%Our goal is to minimize over $\ub$ in \eqref{eq:AO_gen_fin2}. To do this we use variational form of the the $\ell_2$-norm to linearize $\|\omegab_t-\ub\|_2$ and appropriately flip the order of min-max thanks to convex-concavity. With these, we end up with  
%\begin{align}\label{eq:2min_over_u_sec}
%\min_{ { (\xi,\alpha,\beta)\in\Dcthree } }\;\max_{\|\vb\|_2\leq \sqrt{n}} \left\{  \frac{1}{n}\vb^T\omegab_t + \max_{\la>0} \left\{ -\frac{\la\beta^2}{2n} \|P^{\perp}_{S^t}\h\|_2^2 + \frac{1}{n}\min_{\|\ub\|_2\leq C_2\sqrt{n}} \left\{ \frac{\la}{2}\Big\| \beta \g+ \X P_{S^t}\theta - \ub  \Big\|_2^2-\vb^T\ub\right\}\right\}\right\}.
%\end{align} 
%Here, we recognize that the inner max-min over $\la$ and $\ub$ is of identical form to that in \eqref{eq:2min_u} for the first-order method. Thus, using the exact same argument to explicitly perform the joint optimization, we end up with the exact analogue of Lemma \ref{lem:phi_tilde}.

%\begin{lemma}\label{lem:phi_tilde_sec}
%Let $\phi_{n,\Dc}$ be the optimal cost in \eqref{eq:2min_over_u_sec}. Then, for large enough constant $C_2$, there exist constants $C,c$ such that:
%$$
%\Pro\left\{\phi_{n,\Dc}=\wt\phi_{n,\Dc}\right\} \geq 1-Ce^{-cn}
%$$
%where $\wt\phi_{n,\Dc}$ is as follows:
%\begin{align}
%\wt\phi_{n,\Dc}&:=\min_{ { (\xi,\alpha,\beta)\in\Dcthree  }}\;\max_{\|\vb\|_2\leq \sqrt{n}} \; \frac{1}{n}\inp{\omegab_t}{\vb} -\frac{1}{n}\inp{\beta\g+\xi\gamma_1+\alpha\gamma_2}{\vb}-\frac{\beta}{n} \| P^{\perp}_{S^t}\h \|_2 \|\vb\|_2 \label{eq:con_final_AO_sec_pre}\\
%&=\left(\min_{ \substack{ (\xi,\alpha,\beta)\in\Dcthree  }} \; \frac{1}{\sqrt{n}}\|\beta\g+\xi\gammab_1+\alpha\gammab_2-\omegab_t\|_2 - \beta \frac{\| P^{\perp}_{S^t}\h \|_2}{\sqrt{n}}\right)_+\label{eq:con_final_AO_sec}\,.
%\end{align}
%\end{lemma}
%The proof of the lemma is omitted as is identical to that of Lemma \ref{lem:phi_tilde}. The only difference here is the reduction of \eqref{eq:con_final_AO_sec_pre} to \eqref{eq:con_final_AO_sec}. This follows easily by explicitly maximizing over $\vb$. Here, recall that $(x)_+$ denotes $\max\{x,0\}.$

%\noindent\textbf{Pointwise concentration:} For convenience, let $L_n(\xi,\alpha,\beta)$ denote the objective of \eqref{eq:con_final_AO_sec}. We show that for every fixed $(\xi,\alpha,\beta)$, $L_n(\xi,\alpha,\beta)$ concentrates to 
%$$
%L(\xi,\alpha,\beta) = \sqrt{} - \beta/\sqrt{\delta}
%$$

 
%
%Recall from \eqref{eq:sec_order_gen} that
%\begin{align}
%\thetanext = \argmin_{\theta \in \mathbb{R}^d} \frac{1}{2n}\sum_{i=1}^{n}\left( \wfun(\langle \bd{x}_i, \thetacur\rangle, y_i) - \langle \bd{x}_i, \theta \rangle\right)^2.
%\end{align}
%This corresponds to setting 
%$$
%h(\theta,\thetacur) = 0 \qquad \text{and}\quad g(u_i,\inp{\x_i}{\thetacur};y_i) =\left( \wfun(\langle \bd{x}_i, \thetacur\rangle, y_i) - u_i\right)^2
%$$
%in \eqref{eq:AO_gen_fin2}, which leads to the following scalarized (with respect to the $\theta$-minimization) version of the AO:
%%Hence, the optimization in  \eqref{eq:AO_gen_fin} becomes
%\begin{align}
%&\min_{ (\xi,\alpha,\beta)\in\Dcthree } \; \max_{\lambda \geq 0 } \; \;  - \beta^2\frac{\lambda}{2n} \| P^{\perp}_{S^t}\h \|_2^2   + \frac{1}{n}\min_{\|\ub\|_2\leq C_2\sqrt{n}}\Big\{
%\frac{\la}{2}\Big\|\beta\g+\xi\gammab_1+\alpha\gammab_2-\ub\Big\|_2^2+\Big\|\omegab_t-\ub\Big\|_2^2
%\Big\},\label{eq:2min_u_sec}
%%\sum_{i = 1}^n \min_{\ub_i \in \mathbb{R}} \left\{ \frac{\lambda}{2} \big( \ub_i - \xi \gammab_{1,i} - \alpha \gammab_{2,i} - \beta \g_i \big)^2 + \ub_i\, \omega_i)  \right\},
%\end{align}
%where as in \eqref{eq:omegat_def} we have set
%$
%\omegab_t:=\omegab(\xit ,\sigmat ):=\omega\big(\xit \gammab_{1}+\sigmat \gammab_{2}\,,\, f\big(R\gammab_{1};\zb\big)+\epsb\big).
%$
%%and it is understood that the functions $\omega$ and $f$ apply element-wise to the entries of their vector arguments.

%We can now explicitly minimize over $\ub$ as the corresponding optimization in \eqref{eq:2min_u_sec} is separable over the entries of $\ub$ modulo the norm constraint $\|\ub\|_2\leq C_2\sqrt{n}$. The unconstrained minimizer is easily computed:
%$$
%\ub_\star(\la) = \frac{\la}{2+\la}(\beta\g+\xi\gammab_1+\alpha\gammab_2)+\frac{2}{\la+2}\omegab_t.
%$$
%Substituting this in the objective in \eqref{eq:2min_u_sec} gives
%\begin{align}
%-\frac{\la\beta^2}{2}\frac{\|P_{S^t}^\perp\h\|_2^2}{n} + \frac{\la}{2+\la}\frac{\|\beta\g+\xi\gammab_1+\alpha\gammab_2-\omegab_t\|_2^2}{n}
%\end{align}


\subsubsection{First-order methods}\label{sec:gd_ao}

Consider now the loss in Equation \eqref{eq:GD_gen} of gradient descend, that is 
  $\Lc(\theta;\thetacur;\X\y)= \frac{1}{2} \| \theta \|_2^2 - \langle \theta, \thetacur \rangle - \frac{2\eta}{n} \sum_{i = 1}^n { \omega\big(\langle \x_i,\thetacur\rangle,y_i\big) \cdot \langle \bx_i, \theta \rangle}.$ 
This corresponds to setting 
\begin{align*}
h(\theta,\thetacur) &= \frac{1}{2}\|\theta\|_2^2 - \inp{\theta}{\thetacur} = \frac{1}{2}(\xi^2+\alpha^2+\beta^2) - \big(\xi\xit +\alpha\sigmat \big) 
\\
g(\ub,\X\thetacur;\y) &=- \frac{2\eta}{n}\inp{\ub}{\omegab_t} \implies g^*(\vb,\X\thetacur;\y)=\begin{cases} 0 &\text{if } \vb=\frac{2\eta}{n}\omegab_t, \\ +\infty &\text{otherwise}. \end{cases}%u_i\cdot\omega(\inp{\x_i}{\thetacur},y_i)
\end{align*}
%Above, for simplicity we used the shorthand
%\begin{align}\label{eq:omegat_def}
%\omegab_t:=\omegab(\xit ,\sigmat ):=\omega\big(\xit \gammab_{1}+\sigmat \gammab_{2}\,,\, f\big(R\gammab_{1};\zb\big)+\epsb\big),
%\end{align}
%and it is understood that the functions $\omega$ and $f$ apply element-wise to the entries of their vector arguments. 
Using this in \eqref{eq:conAO2_no_u} directly implies \eqref{eq:Ln_gd}, as desired.


We have the following lemma characterizing the properties of \eqref{eq:con_final_AO}.


\begin{lemma}\label{lem:deviation_lem_gd}
Consider the minimization in \eqref{eq:} over $\Dc=\Bc_2(C_1)$. For $n$ large enough, there exist absolute constants $C,c,C',c'>0$ and $c_\delta>1$ such that the following statements hold for all $\delta>c_\delta$ and  $c'>\eps>C'n^{-\nicefrac{1}{2}}$.

% Let $n$ be large enough, $\delta>c_\delta$ for appropriate constant $c_\delta>1$, and  any $\eta>0$ smaller than some absolute constant.
\begin{enumerate}
\item With probability $1-Ce^{-cn}$ the minimizer $\thetathree_n:=[\xi_n,\alpha_n,\beta_n]$ is unique and takes the form
\begin{subequations}\label{eq:soln_n}
\begin{align}
~\xi_{n} &= \xit  + \frac{2\eta}{n}\inp{\gammab_1}{\omegab_t}\\
~\alpha_{n} &= \sigmat  + \frac{2\eta}{n}\inp{\gammab_2}{\omegab_t}\\
~\beta_{n} &= \frac{2\eta}{n}\inp{\g}{\omegab_t} + \frac{2\eta}{n}\| P^{\perp}_{S^t}\h \|_2 \|\omegab_t\|_2.
\end{align}
\end{subequations}

\item With probability at least {$1-Ce^{-cn\eps^2}$},
\begin{align}
\left|\xi_n-\xi_*\right| \vee \left|\alpha_n-\alpha_*\right| \vee \left|\beta_n-\beta_*\right| \leq \eps,%\qquad\text{where}\quad
%\begin{cases}
%~\xi_* = \xit  + 2\eta\E\left[G1\cdot\Omega_t\right]\\
%~\alpha_* = \sigmat  + 2\eta\E\left[G_2\cdot\Omega_t\right]\\
%~\beta_* = 2\eta\frac{1}{\sqrt{\delta}}\sqrt{\E\left[\Omega_t^2\right]}.\\
%\end{cases}
%\label{eq:theta_star_gd}
\end{align}
where $\xinextstar,\alphanextstar,\betanextstar$ are as defined in Equation \eqref{eq:theta_starnext_gd}.
%\quad\begin{cases}
%~\xinextstar=\E[G_1\Omega_t]\\
%~\alphanextstar=\E[G_2\Omega_t]\\
%~\betanextstar={\tau_*}\big/{\sqrt{\delta}}.
%\end{cases}
%\end{subequations}


\item Part B of Lemma \ref{lem:AO_main_gd} holds.
%With probability at least {$1-Ce^{-cn\eps^2}$},
%\begin{align}\label{eq:bar_L_sec}
%\left| L_n(\thetathree_n)- \bar{L}\right|\leq \eps,\quad\text{where } \bar{L}:=\left(1-\frac{1}{\delta}\right)\tau_*.
%\end{align}

\item Part C of Lemma \ref{lem:AO_main_gd} holds.
\end{enumerate}
%
%
%\item With probability at least {$1-Ce^{-cn\eps^2}$},
%\begin{align}\label{eq:bar_L_gd}
%\left| L_n(\thetathree_n)- \bar{L}\right|\leq \eps,\quad\text{where } \bar{L}:=-\frac{1}{2}\left(\alpha_*^2+\beta_*^2+\xi_*^2\right).
%\end{align}
%
%
%\item The following strong convexity property holds:
%\begin{align}
%%\min_{\|\thetathree-\thetathree_n\|_2\geq \eps} L_n(\thetathree) \geq  L_n(\thetathree_n)+\frac{1}{16\tau_*}\eps^2.
%\min_{\|\thetathree-\thetathree_n\|_2\geq \eps} L_n(\thetathree) \geq  L_n(\thetathree_n)+\frac{1}{2}\eps^2.
%\end{align}
%%for all $\eps>C'n^{-\nicefrac{1}{2}}.$
%
%\end{enumerate}

\end{lemma}

%With this result, we are now ready to apply the CGMT Theorem \ref{thm:CGMT} and prove our main result below. 

%\begin{theorem}\label{eq:gordon_thm_gd}
% Fix any $t\geq1$. Let $\theta_{t+1}$ be as in \eqref{eq:first_order_min} and $\xi_{t+1}, \alpha_{t+1}, \beta_{t+1}$ defined accordingly. Recall the definition of $\xi_*,\alpha_*,\beta_*$ in \eqref{eq:theta_star_gd}. Let Assumptions \ref{ass:Lip}, \ref{ass:}, \ref{ass:} and \ref{ass:omega} hold. Then, there exist absolute constants $c,C,c_\delta,c',C'$ such that for any $c'>\eps>C'n^{-\nicefrac{1}{4}}$ it holds with probability at least $1-Ce^{-cn\eps^4}$ that
%\begin{align}
%\left|\xi_{t+1}-\xi_*\right|\vee\left|\alpha_{t+1}-\alpha_*\right|\vee
%\left|\beta_{t+1}-\beta_*\right| \leq \eps.
%\end{align}
%\end{theorem}

%The proof of the theorem is almost identical to that of Theorem \eqref{eq:gordon_thm_sec} only now we rely on Lemma \ref{lem:deviation_lem_gd}. We omit the details for brevity.


%The optimization above is a strongly convex quadratic in $\xi,\alpha,\beta$ with \emph{unconstrained} minimizers:
%%\begin{subequations}\label{eq:soln_n}
%\begin{align}\label{eq:soln_n}
%\begin{cases}
%~\xi_{\star,n} = \xit  + \frac{2\eta}{n}\inp{\gammab_1}{\omegab_t}\\
%~\beta_{\star,n} = \frac{2\eta}{n}\inp{\g}{\omegab_t} + \frac{2\eta}{n}\| P^{\perp}_{S^t}\h \|_2 \|\omegab_t\|_2\\
%~\alpha_{\star,n} = \sigmat  + \frac{2\eta}{n}\inp{\gammab_2}{\omegab_t}.
%\end{cases}
%\end{align}
%\end{subequations}

%Let $\xi_*,\alpha_*$ and $\beta_*$ defined as follows for $G_1,G_2\sim\Nn(0,1)$, $E\sim\Nn(0,s^2)$, $Z\sim P_{z_1}$ and 
%$
%\Omega_t:=\omega\big(\xit G_1+\sigmat G_2\,,\,f(RG_1;Z)+E\big):
%$
%%\begin{subequations}
%\begin{align}
%\begin{cases}
%~\xi_* = \xit  + 2\eta\E\left[G1\cdot\Omega_t\right]\\
%~\beta_* := 2\eta\frac{1}{\sqrt{\delta}}\sqrt{\E\left[\Omega_t^2\right]}\\
%~\alpha_* = \sigmat  + 2\eta\E\left[G_2\cdot\Omega_t\right],
%\end{cases}
%\end{align}

%Note that, by definition, $\xi_*=\E[\xi_{\star,n}]$, $\alpha_* = \E[\alpha_{\star,n}].$ Assuming $\omegab_t$ is subgaussian, $\beta_*$ is also close to $\E[\beta_{\star,n}].$
%We will need  the following assumption on the concentration of the weight function $\omega$. 

\noindent\textbf{Proof of Lemma \ref{lem:deviation_lem_gd}.}~~ Throughout the proof, we will condition on the intersection
$\Ec=\Ec_1\cap\Ec_2$ of the following events for $\eps>Cn^{-\nicefrac{1}{2}}$:
\begin{subequations}\label{eq:good_events_gd}
\begin{align}
\Ec_1&:=\left\{ \frac{1}{\sqrt{\delta}} - C'\left(n^{-1}\vee\eta\right)\leq\frac{\|P_{S^t}^\perp\h\|_2}{\sqrt{n}}\leq \frac{1}{\sqrt{\delta}} + \eps
\right\}\\
\Ec_2&:=\left\{ \left| \frac{\|\omegab_t\|_2}{\sqrt{n}} - \sqrt{\E\Omega_t^2} \right|\leq \eps
\right\}
\\
\Ec_3&:=\left\{ \left| \frac{1}{n}\gammab_1^T\omegab_t - \E[G_1\Omega_t] \right| \vee 
\left| \frac{1}{n}\gammab_2^T\omegab_t - \E[G_2\Omega_t] \right| \vee
\left| \frac{1}{n}\g_1^T\omegab_t  \right|
\leq \eps\right\}
\end{align}
\end{subequations}
We show in lemma XXX that $\Pro(\Ec)\geq 1- Ce^{-cn\eta^2}$ for constatns $C,c>0$. 

\noindent\textbf{Proof of Statement 1.}~The objective $L_n(\thetathree)$ is a strongly convex quadratic function. It is easy to verify by first-order optimality conditions that $\thetathree_n$ as given in Equation \eqref{eq:} is indeed the unique minimizer of the \emph{unconstrained} minimization of $L_n(\thetathree)$ over $\R^3$. To prove that nothing changes when restricting the minimization over $\Bc_2(C_1)$ we condition on the event $\Ec$ (for some fixed small $\eps$). 

Using Assumption \ref{ass:omega}  the unconstrained minimizers \eqref{eq:soln_n} have the following concentration properties.
\begin{lemma}\label{lem:conc_lemma}
Fix $\eps>0$. Consider the scalarized AO problem in \eqref{eq:Ln_gd} with $\Dc=\Bc(C_1)$ for large enough positive constant $C_1$. 
%:=C_1(\eps,\eta,K_\omega,\alpha_*,\beta_*,\xi_*)$. 
Then, the following statements are true.

\noindent 1. The minimizers $(\xi_{\star,n},\alpha_{\star,n},\beta_{\star,n})$ in \eqref{eq:soln_n} concentrate as follows:
\begin{align}\label{eq:Bern_inp1_lemma}
&\Pro\left\{ \max\left\{ \left| \xi_{\star,n} - \xi_* \right|\,,\,\left| \alpha_{\star,n} - \alpha_* \right| \right\} \geq \eps \right\} \leq C\exp\left(-c\,n\,\min\left(\eps^2/K_\omega^2,\eps/K_\omega\right)\right)\,
\\
&\Pro\left\{ \abs{\beta_{\star,n}-\beta_*} \geq \eps + \frac{\eta K_\omega \tilde C(\delta)}{n} \right\} \leq C\exp\left(-c\,{\min\left(1,\bar{B}^4/K_\omega^4\right)}\,n\,\min\left(\eps/K_\omega,{\eps^2}/K_\omega^2\right)\right).
\end{align}

\noindent 2.  The optimal cost concentrates as follows:
\begin{align}\label{eq:cost_conv}
\Pro\left\{\Big|\wt\phi_{n,\Bc_2(C_1)} - \bar\phi \Big| \geq \max\{\eps,\eps^2\}+\frac{C_5}{n}\right\} \leq  C\exp\left(-c_2\,C_\omega\,n\,\min\left(\eps^2,\eps\right)\right),
%\max\left\{ \alpha_*\, ,\,\beta_*\, ,\,\xi_*  \right\}\cdot 
\end{align}
with
\begin{align}\label{eq:phi_bar}
\bar\phi:=-\frac{1}{2}\left(\alpha_*^2+\beta_*^2+\xi_*^2\right)
\end{align}
Above, the constants $C_1,c_2,C_5$ may depend only on $\eps,\eta,K_\omega,\alpha_*,\beta_*,\xi_*$.
\end{lemma}

% such that
%\begin{align}\label{eq:AO_conc}
%\Pro\left\{\abs{\phi_{n,\Bc_2(C_1)}-\bar\phi} > 3C_1\,\eps\right\}\leq C\exp\left(-c\,n\,\min\left(\eps^2,\eps,1\right)\right).
%\end{align}
%From the lemma, the minimizers $(\alpha_{\star,n},\beta_{\star,n},\xi_{\star,n})$ satisfy

It will be convenient to use the shorthand $\thetathree:=(\alpha,\beta,\xi)$. Define accordingly, $\thetathree_{\star,n}$ and $\thetathree_*$.
Combining the two inequalities in Equation \eqref{eq:Bern_inp1_lemma}, it holds that
\begin{align}\label{eq:minimizers_conv}
\Pro\left\{ \big\|\thetathree_{\star,n}-\thetathree_*\big\|_2^2>\eps^2 + \eps \frac{C_5}{\sqrt{n}} + \frac{C_5}{n}\right\} \leq C\exp\left(-c\,C_\omega\,n\,\min\left(\eps^2,\eps\right)\right).
\end{align}

Consider now the perturbed AO over $\Dc=\Bc_2(C_1)\cap \Sc_\eps^c.$ The objective function in \eqref{eq:con_final_AO} is clearly $\tau$-strongly convex in $(\alpha,\beta,\xi)$ with $\tau\geq 1$. Thus, for any $\tilde\eps>0$ (and any realization of $\g,\h,\gammab_1,\gammab_2$):
\begin{align}
&\wt\phi_{n,\Bc_2(C_1)\cap \Sc_{\tilde\eps}^c} \geq  \wt\phi_{n,\Bc_2(C_1)} + \frac{1}{2} \min_{\thetathree\in\Sc_{\tilde\eps}^c} \big\| \thetathree - \thetathree_{\star,n} \big\|_2^2 \nn
%\\
%&\geq  \phi_{n,\Bc_2(C_1)} + \frac{1}{2} \min_{\thetathree\in\Sc_{\tilde\eps}^c} \big\| \thetathree - \thetathree_*\Big\|_2 - \Big\|\thetathree_* - \thetathree_{\star,n} \big\|_2^2
\end{align} 
Now, condition on the event in Equation \eqref{eq:minimizers_conv}. For any $\thetathree\in\Sc_{2\eps}^c$: 
\begin{align}
\big\| \thetathree - \thetathree_{\star,n} \big\|_2 &\geq 
\big\| \thetathree - \thetathree_*\big\|_2 - \big\|\thetathree_* - \thetathree_{\star,n} \big\|_2 \nn \geq 2\eps - \eps - C_5/n = \eps-C_5/n.\nn
\end{align}
Hence, 
$$
\Pro\left\{ \wt\phi_{n,\Bc_2(C_1)\cap \Sc_{2\eps}^c} \geq  \wt\phi_{n,\Bc_2(C_1)} +\frac{\eps^2}{2} + \frac{C_5}{n^2} \right\} \geq 1- C\exp\left(-c\,C_\omega\,n\,\min\left(\eps^2,\eps\right)\right).
$$
To finish, combine this with Equation \eqref{eq:cost_conv} to find that
\begin{align}
&\Pro\left\{\wt\phi_{n,\Bc_2(C_1)\cap \Sc_{2\eps}^c} < \bar\phi + \frac{\eps^2}{4}\right\} \nn
\\
&\qquad\qquad\leq\Pro\left\{\wt\phi_{n,\Bc_2(C_1)\cap \Sc_{2\eps}^c} < \bar\phi + \frac{\eps^2}{4}\,\big|\,\wt\phi_{n,\Bc_2(C_1)}\geq \bar\phi-\frac{\eps^2}{4}\right\} + \Pro\left\{\wt\phi_{n,\Bc_2(C_1)} < \bar\phi-\frac{\eps^2}{4}\right\}\nn
\\
&\qquad\qquad\leq\Pro\left\{\phi_{n,\Bc_2(C_1)\cap \Sc_{2\eps}^c}< \phi_{n,\Bc_2(C_1)} + \frac{\eps^2}{2}\right\} + C\exp\left(-c\,\min\left(n\eps^4,n\eps^2\right)\right)\nn
\\
&\qquad\qquad\leq C\exp\left(-c\,\min\left(n\eps^2,n\eps\right)\right)+C\exp\left(-c\,\min\left(n\eps^4,n\eps^2\right)\right).
\label{eq:AO_conc2}
\end{align}

\begin{lemma}\label{lem:GD_lem_AO}
 Let $\bar\phi$ be defined as in \eqref{eq:phi_bar}. For any $0<\eps<\max\left\{\alpha_*,\beta_*,\xi_*\right\}$ the following statements are true about the optimal cost of the auxiliary optimization:
\begin{align}
\Pro\left\{\abs{\phi_{n,\Bc_2(C_1)}-\bar\phi} > \eps\right\}&\leq C\exp\left(-c\,n\,\min\left(\eps^2,\eps,1\right)\right)
\\
\Pro\left\{\phi_{n,\Bc_2(C_1)\cap \Sc_{\eps}^c} < \bar\phi + \frac{\eps^2}{16}\right\} &\leq C\exp\left(-c\,n\,\min\left(\eps^4,\eps^2,\eps,1\right)\right).
\end{align}
\end{lemma}


\textbf{Completing the proof.}~We are now ready to apply Theorem \ref{thm:CGMT}. Specifically, we apply its third statement with $\bar\phi$ as in \eqref{eq:phi_bar} and $\zeta=\zeta(\eps)=\eps^2/16$ as we know from Lemma \ref{lem:GD_lem_AO} that  $\phi_{n,\Bc_2(C_1)}<\bar\phi+\zeta$ and $\phi_{n,\Bc_2(C_1)\cap\Sc_\eps^c}>\bar\phi-\zeta$ with probability at least $1-C\exp\left(-c\,\min\left(n\eps^4,n\eps^2\right)\right)$ each. Thus, we conclude that
$$\Pro\left\{\thetanexthat\in\Sc_\epsilon\right\} \geq 1-C\exp\left(-c n\,\min\left(\eps^4,\eps^2,\eps,1\right)\right).$$







==> sections/gordon/gordon_second_order-copy-copy.tex <==
\subsection{Second order methods}\label{sec:sec_ord_ao}
Recall from \eqref{eq:sec_order_gen} that
$$
\thetanext = \argmin_{\theta \in \mathbb{R}^d} \frac{1}{2n}\sum_{i=1}^{n}\left( \wfun(\langle \bd{x}_i, \thetacur\rangle, y_i) - \langle \bd{x}_i, \theta \rangle\right)^2 = \argmin_{\theta \in \mathbb{R}^d} \frac{1}{\sqrt{n}}\|\omega(\X\thetacur,\y)-\X\thetacur\|_2.
$$
This corresponds to setting $\Fc_t(\ub,\theta)=\|\omegab_t-\ub\|_2$; equivalently, 
$$
h(\theta,\thetacur)=0\qquad\text{and}\qquad g(\ub,\X\thetacur;\y)=\frac{1}{\sqrt{n}}\|\omegab_t-\ub\|_2,
$$
 where  as in \eqref{eq:omegat_def} we have set
$
\omegab_t:=\omegab(\xi_t,\sigma_t):=\omega\big(\xi_t\gammab_{1}+\sigma_t\gammab_{2}\,,\, f\big(R\gammab_{1};\zb\big)+\epsb\big).
$
We see for the convex conjugate function that $$g^*(\vb,\X\thetacur;\y)=\begin{cases}
\inp{\vb}{\omegab_t}&\text{if } \|\vb\|_2\leq \frac{1}{\sqrt{n}},\\
+\infty &\text{otherwise}.
\end{cases}
$$
Therefore, the AO in \eqref{eq:conAO2_no_u} simplifies as follows:
\begin{align}
\phi_{n,\Dc}&=\min_{ { (\xi,\alpha,\beta)\in\Dc_3  }}\;\max_{\|\vb\|_2\leq \frac{1}{\sqrt{n}}} \; \inp{\omegab_t}{\vb} -\inp{\beta\g+\xi\gammab_1+\alpha\gammab_2}{\vb}-{\beta} \| P^{\perp}_{S^t}\h \|_2 \|\vb\|_2 \label{eq:con_final_AO_sec_pre}\\
&=\left(\min_{ \substack{ (\xi,\alpha,\beta)\in\Dc_3  }} \; \frac{1}{\sqrt{n}}\|\beta\g+\xi\gammab_1+\alpha\gammab_2-\omegab_t\|_2 - \beta \frac{\| P^{\perp}_{S^t}\h \|_2}{\sqrt{n}}\right)_+\label{eq:con_final_AO_sec}\,.
\end{align}
The second equality follows easily by explicitly maximizing over $\vb$. Here, recall that $(x)_+$ denotes $\max\{x,0\}.$

Now, we focus on the inner minimization above. To lighten notation, denote
\begin{align*}
\sqrt{\kappa_n}:=\frac{\| P^{\perp}_{S^t}\h \|_2}{\sqrt{n}}\quad \A:=\big[\gammab_1,\gammab_2,\g\big]\in\R^{n\times 3}\quad \vb_n=[0,0,\sqrt{\kappa_n}]^T\in\R^3,
\end{align*}
and recall that $\thetathree=[\xi,\alpha,\beta].$ With this notation, the minimization in \eqref{eq:con_final_AO_sec} writes
\begin{align}
\min_{ \substack{ \thetathree\in\Dc_3  }} \;L_n(\thetathree):= \frac{1}{\sqrt{n}}\|\A\thetathree-\omegab_t\|_2 - \vb_n^T\thetathree.\label{eq:scal_min_sec}
\end{align}

%We can compute
%$$
%\nabla^2L_n(\thetathree) = \frac{1}{\|\A\thetathree-\omegab_t\|_2^3}\A^T\left(\|\A\thetathree-\omegab_t\|_2^2\cdot\mathbf{I}_3-\left(\A\thetathree-\omegab_t\right)\left(\A\thetathree-\omegab_t\right)^T\right)\A
%$$

\begin{lemma}
The following  statements are true about the minimization in \eqref{eq:scal_min_sec}. Let $n$ be large enough, $\delta>c_\delta$ for appropriate constant $c_\delta>1$, and  any $\eta>0$ smaller than some absolute constant.
\begin{enumerate}
\item With probability at least {$1-Ce^{-cn}$}, the minimizer $\thetathree_n=[\xi_n,\alpha_n,\beta_n]$ takes the form:
\begin{align}
&\thetathree_n:=\thetathree_n(\tau_n):=(\A^T\A)^{-1}\A^T\omegab_t + \tau_n\cdot n\cdot(\A^T\A)^{-1}\vb_n,\quad\nn\\
&\qquad\qquad\text{where},\quad\tau_n=\frac{\frac{1}{\sqrt{n}}\|\left(\mathbf{I}_n-\A(\A^T\A)^{-1}\A^T\right)\omegab_t\|_2}{\sqrt{1-n\cdot\vb_n^T(\A^T\A)^{-1}\vb_n}}.\label{eq:tau_n}
\end{align}

\item With probability at least {$1-Ce^{-cn\eta^2}$} the following statements hold:
\begin{subequations}
\begin{align}\label{eq:tau_star_sec}
&\left|\tau_n-\tau_\star\right|\leq \big(\eta\vee n^{-\nicefrac{1}{2}}\big),\quad\text{where}\quad\tau_\star = \sqrt{\left(\frac{\delta}{\delta-1}\right)\left(\E[\Omega_t^2]-\left(\E[G_1\Omega_t]\right)^2-\left(\E[G_2\Omega_t]\right)^2\right)}
\\
&\left|\xi_n-\E[G_1\Omega_t]\right| \vee \left|\alpha_n-\E[G_2\Omega_t]\right| \vee \left|\beta_n-\frac{\tau_*}{\sqrt{\delta}}\right| \leq \big(\eta\vee n^{-\nicefrac{1}{2}}\big)
\label{eq:theta_star_sec}
\end{align}
\end{subequations}


\item With probability at least {$1-Ce^{-cn\eta^2}$}
\begin{align}
\left| L_n(\thetathree_n)- \bar{L}\right|\leq \big(\eps\vee n^{-\nicefrac{1}{2}}\big),\quad\text{where } \bar{L}:=\left(1-\frac{1}{\delta}\right)\tau_*.
\end{align}


\item There exist constants $C,c,C'>0$ such that the following strong convexity property holds with probability at least {$1-Ce^{-cn\eps^2}$}
\begin{align}
\min_{\|\thetathree-\thetathree_n\|_2\geq \eps} L_n(\thetathree) > L_n(\thetathree_n)+\frac{\widetilde{\tau}_{\max}}{2}\eps^2,
\end{align}
for all $\eps>C'n^{-\nicefrac{1}{2}}.$

\end{enumerate}
\end{lemma}


\begin{proof} 
The first step in the proof is to rewrite the minimization in 
 \eqref{eq:scal_min_sec} equivalently as \ct{Can we switch order of mins here? Might need to adjust this or justify}

\begin{align}
\min_{\thetathree\in\Dc_3}L_n(\thetathree) &=
\min_{ \substack{ \thetathree\in\Dc_3  }} \;\inf_{\tau>0}\; \tilde{L}_n(\thetathree,\tau):= \frac{\tau}{2}+\frac{1}{2\tau n}\|\A\thetathree-\omegab_t\|_2^2 - \vb_n^T\thetathree\nn \\
&=
 \inf_{\tau>0}\;\min_{ \substack{ \thetathree\in\Dc_3  }} \;\tilde{L}_n(\thetathree,\tau).\label{eq:scal_min_sec_tau}
\end{align}
%The first equality holds by noting that $x=\inf_{\tau>0}\frac{\tau}{2}+\frac{x^2}{2\tau}$ for all $x\geq0$. The flip of min-inf in the second equality is possible as follows. For  


Throughout the proof, we will condition on the intersection
$\Ec=\Ec_1\cap\Ec_2\cap\Ec_3\cap\Ec_4\cap\Ec_5$ of the following events for $\eta\in(0,1)$:
\begin{subequations}\label{eq:good_events_quad}
\begin{align}
\Ec_1&:=\left\{ \left(1-C'\left(n^{-\nicefrac{1}{2}}\vee\eta\right)\right)\,\mathbf{I}_3 \preceq n(\A^T\A)^{-1} \preceq 
\left(1+C'\left(n^{-\nicefrac{1}{2}}\vee\eta\right)\right)\,\mathbf{I}_3
\right\}
\\
\Ec_2&:=\left\{ \frac{1}{\delta} - C'\left(n^{-1}\vee\eta\right)\leq\|\vb_n\|_2^2\leq \frac{1}{\delta} + \eta
\right\}\\
\Ec_3&:=\left\{ \left| \frac{\|\omegab_t\|_2^2}{n} - \E\Omega_t^2 \right|\leq \eta
\right\}
\\
\Ec_4&:=\left\{ \left| \frac{1}{n}\gammab_1^T\omegab_t - \E[G_1\Omega_t] \right| \vee 
\left| \frac{1}{n}\gammab_2^T\omegab_t - \E[G_2\Omega_t] \right| \vee
\left| \frac{1}{n}\g_1^T\omegab_t  \right|
\leq \eta\right\}
\\
\Ec_5&:=\left\{ \left| \frac{\|\A^T\omegab_t\|^2}{n^2} - \left(\E[G_1\Omega_t]\right)^2 - \left(\E[G_2\Omega_t]\right)^2 \right|\leq \eta\right\}.
\end{align}
\end{subequations}
We show in lemma XXX that $\Pro(\Ec)\geq 1- Ce^{-cn\eta^2}$ for constatns $C,c>0$. 

\noindent\textbf{Proof of Statement 1.}~Let $\thetathree_n(\tau)$ denote the solution of the inner quadratic minimization above. Specifically,
$$
\thetathree_n(\tau) = (\A^T\A)^{-1}\A^T\omegab_t + \tau\cdot n\cdot(\A^T\A)^{-1}\vb_n.
$$
Then, we can minimize over $\tau$ by solving
\begin{align}\label{eq:tilde_L_tau}
\min_{\tau>0}\;\tilde{L}_n\big((\thetathree_n(\tau),\tau)\big)=\frac{1}{2\tau n}\|\left(\mathbf{I}_n-\A(\A^T\A)^{-1}\A^T\right)\omegab_t\|_2^2 + \frac{\tau}{2}\left(1-n\cdot\vb_n^T(\A^T\A)^{-1}\vb_n\right)-\vb_n^T(\A^T\A)^{-1}\A\omegab_t,
\end{align}
which yields 
\begin{align}
\tau_n=\frac{\frac{1}{\sqrt{n}}\|\left(\mathbf{I}_n-\A(\A^T\A)^{-1}\A^T\right)\omegab_t\|_2}{\sqrt{1-n\cdot\vb_n^T(\A^T\A)^{-1}\vb_n}},\label{eq:tau_n}
\end{align}
provided that 
\begin{align}\label{eq:check_for_tau_n}
n\cdot\vb_n^T\left({\A^T\A}\right)^{-1}\vb_n<1.
\end{align}
%But, from Lemma \ref{lem:wishartineq} on quadratic forms of Wishart matrices, it holds with probability at least $1-e^{-cn}$ that 
%$\vb_n^T\left({\A^T\A}\right)^{-1}\vb_n\leq \kappa_n\frac{2}{n-2}.$ Moreover, from \eqref{eq:???}: for all $\eps\in(0,1)$:  $\kappa_n\leq 1/\delta + \eps$ with probability at least $1-e^{-c\eps^2n}$. Thus, there exist constants $c_\delta>1$ and $c>0$ such that 
%\begin{align}\label{eq:tau_denom}
%\Pro\left(\vb_n^T(\A^T\A)^{-1}\vb_n<\frac{1}{2n}\right)\geq 1-e^{-cn},
%\end{align}
%provided that $\delta>c_\delta.$ This proves the first statement of the lemma.




Denote ${\rm{num}}({\tau_n}),\rm{den}({\tau_n})$ the numerator and denominator in \eqref{eq:tau_n}. In the event $\Ec$ the following are true. First, with probability at least $1-Ce^{-cn\eta^2}$,
\begin{align}\nn
\sqrt{1-\frac{1}{\delta}\left(1+\frac{6n^{-1/2}+4\eta}{1+6n^{-1/2}+3\eta}\right)}&\leq {\rm{den}}({\tau_n})\leq\sqrt{1-\frac{1}{\delta}\left(1-\frac{6n^{-1/2}+4\eta}{1-6n^{-1/2}-3\eta}\right)}\\
\sqrt{1-\frac{1}{\delta}-\frac{6n^{-1/2}+4\eta}{1+6n^{-1/2}+3\eta}}&\leq {\rm{den}}({\tau_n})\leq\sqrt{1-\frac{1}{\delta}+\frac{6n^{-1/2}+4\eta}{1-6n^{-1/2}-3\eta}}\nn
\\
\sqrt{1-\frac{1}{\delta}-C\left(n^{-1/2}\vee\eta\right)}&\leq{\rm{den}}({\tau_n})\leq\sqrt{1-\frac{1}{\delta}+C\left(n^{-1/2}\vee\eta\right)}.\label{eq:den}
\end{align}
In the second line we used that $\delta>c_\delta\gg1$ and in the third line we used $\eta$ small enough and $n$ larger than a constant. Note that this
%Assuming here large enough constant $\delta>C\gg 1,$ 
guarantees the non-negativity of the denominator, that is \eqref{eq:check_for_tau_n} is satisfied, which completes the proof of the first statement of the lemma. 

\noindent\textbf{Proof of Statement 2.}~Second, it holds that 
$$
{{\rm{num}}}({\tau_n}) = \sqrt{\frac{1}{n}\|\omegab_t\|_2^2-\frac{1}{n^2}\omegab_t^T\A^T\left(n\left(\A^T\A\right)^{-1}\right)\A\omegab_t}\,.
$$
Hence,
\ct{Simplify}
{\tiny
\begin{align*}
-\frac{(\E[G_1\Omega_t])^2+(\E[G_2\Omega_t])^2}{1-6n^{-1/2}-3\eta}-\frac{\left(3 + 4\sqrt{\E[\Omega_t^2]}\right)\eta}{1-6n^{-1/2}-3\eta}&\leq-\frac{\omegab_t^T\A^T\left(\A^T\A\right)^{-1}\A\omegab_t}{n}\leq-\frac{(\E[G_1\Omega_t])^2+(\E[G_2\Omega_t])^2}{1+6n^{-1/2}+3\eta}+\frac{\left(3 + 4\sqrt{\E[\Omega_t^2]}\right)\eta}{1+6n^{-1/2}+3\eta}
\\
-{(\E[G_1\Omega_t])^2-\E[G_2\Omega_t])^2}-
C\left(n^{-1/2}\vee\eta\right)
&\leq-\frac{\omegab_t^T\A^T\left(\A^T\A\right)^{-1}\A\omegab_t}{n}\leq-{(\E[G_1\Omega_t])^2-(\E[G_2\Omega_t])^2}+C\left(n^{-1/2}\vee\eta\right),
\end{align*}
}
where we used again Cauchy-Schwartz and $\E[\Omega_t^2]<C$.
This leads to 
\begin{align}
\left| \left({{\rm{num}}}({\tau_n})\right)^2-\left(\E[\Omega_t^2]-{(\E[G_1\Omega_t])^2-(\E[G_2\Omega_t])^2} \right)\right| \leq C\left(n^{-1/2}\vee\eta\right).\label{eq:num}
\end{align}

Putting together \eqref{eq:num} and \eqref{eq:den} we conclude that
\begin{align}
\sqrt{\frac{a-C\left(n^{-1/2}\vee \eta\right)}{b+C\left(n^{-1/2}\vee \eta\right)}}\leq \tau_n\leq \sqrt{\frac{a+C\left(n^{-1/2}\vee \eta\right)}{b-C\left(n^{-1/2}\vee \eta\right)}}
\end{align}
where we set $a:=\E[\Omega_t^2]-(\E[G_1\Omega_t])^2-(\E[G_2\Omega_t])^2$ and $b:=1-1/\delta$, for simplicity. Assuming constants such that $\delta>c>1$ (thus, $b>c'$) and $a>c$, this leads to 
\begin{align}
\left|\tau_n-\sqrt{\frac{a}{b}}\right|\leq C\left(n^{-1/2}\vee \eta\right).\end{align}
Here, we used that
\begin{align*}
\sqrt{\frac{a+\eps}{b-\eps}}-\sqrt{\frac{a}{b}}= \sqrt{\frac{a}{b}}\left(\sqrt{1+\frac{\frac{\eps}{b}+\frac{\eps}{a}}{1-\frac{\eps}{b}}}-1\right)  \leq
\sqrt{\frac{a}{b}} \left(\frac{\frac{\eps}{b}+\frac{\eps}{a}}{2(1-\frac{\eps}{b})}\right) \leq C\eps.
\end{align*}
The first inequality follows by $\sqrt{1+x}\leq1+x/2$ and the second inequality uses constant lower and upper bounds on $a,b$.
Noting that $\tau_*=\sqrt{a/b}$ completes the proof of Equation \eqref{eq:tau_star_sec}.

Now, we prove \eqref{eq:theta_star_sec}. We show here the upper bounds, as the lower bounds follow in the same way.  For $i=1,2$ and $\eb_i$ the corresponding basis vectors in $\R^3$, we have the desired thanks to events $\Ec_1$ and $\Ec_4$:
$$
\eb_i^T\thetathree_n \leq\left(1+C(n^{-1/2}\vee \eta)\right)\frac{1}{n}\eb_i^T\A\omegab_t \leq \left(1+C(n^{-1/2}\vee \eta)\right)\left(\E[G_i\Omega_t]+\eta\right) \leq \E[G_i\Omega_t] + C(n^{-1/2}\vee \eta).
$$
The bounds on $\beta_n=\eb_3^T\thetathree_n$ follow similarly thanks to events $\Ec_1, \Ec_4$, $\Ec_2$. We omit the details for brevity.


%To continue, we first argue that we can restrict the range of $\tau$ minimization in \eqref{eq:scal_min_sec_tau} in the interval $(0,T]$ for sufficiently large constant $T>0$. It suffices to show that $\tau_n<T$ with high probability. Focus on the numerator in Equation \eqref{eq:tau_n}. Let $\ab_1^T,\ldots\ab_n^T\in\R^3$, denote the rows of $\A$ and $\B_{-1}=\sum_{i=2}^{n}\ab_i\ab_i^T$. Note that $\A^T\A=\ab_1\ab_1^T+\B$ and $\B$ is a $3\times3$ Wishart matrix with $n-1$ degrees of freedom independent of $\ab_1$. Using a standard leave-one-out argument together with the matrix inversion lemma and some algebra, we can show that 
%\begin{align}\label{eq:tau_num}
%\|\left(\mathbf{I}_n-\A(\A^T\A)^{-1}\A^T\right)\omegab_t\|_2 = \|\omegab_t\|_2\sqrt\frac{1}{1+\ab_1^T\B^{-1}\ab_1}.
%\end{align}
%Specifically, this means that $\|\left(\mathbf{I}_n-\A(\A^T\A)^{-1}\A^T\right)\omegab_t\|_2 \leq \|\omegab_t\|_2$. In turn, from Assumption \ref{ass:omega} and \eqref{eq:}, this is further upper bounded by $2\sqrt{n}\sqrt{\E[\Omega^2]}$ with probability at least $1-2e^{-cn(\E[\Omega^2])^2/K_\omega^4}.$ These, combined with \eqref{eq:tau_denom}, show that for $\delta>c_\delta$ there exists (sufficiently large) $T>0$ and $c,C>0$ such that $\tau_n\leq T$ with probability at least $1-Ce^{-cn(\E[\Omega^2])^2/K_\omega^4}$.

\vp
\noindent\textbf{Proof of Statement 3.}~
Recall that $L_n(\theta_n)=\tilde L_n(\theta_n(\tau_n),\tau_n)$. Thus, from \eqref{eq:tilde_L_tau}:
\begin{align}\label{eq:Ln_conc_proof_sec}
L_n(\theta_n) = \left({\rm{den}{(\tau_n)}}\right)^2\tau_n-\vb_n^T(\A^T\A)^{-1}\A\omegab_t.
\end{align}
Note that $\vb_n^T\A\omegab_t=\sqrt{\kappa_n}\g^T\omegab_t$. From this and thanks to $\Ec_1, \Ec_4$, we have that $|\vb_n^T(\A^T\A)^{-1}\A\omegab_t|\leq C\left(n^{-1/2}\vee\eta\right).$ For the first therm in \eqref{eq:Ln_conc_proof_sec} recall Equations \eqref{eq:den} and \eqref{eq:tau_n}. The desired follows from these and simple calculations

\vp
\noindent\textbf{Proof of Statement 4.}~
 Condition on the event $|\tau_*-\tau_n|\leq (\eta\vee n^{-1/2})=:\zeta$ for some $\eta>0$ that we pick later in the proof. From concentration of $\tau_n$, we can restrict the range of $\tau$-minimization in \eqref{eq:scal_min_sec_tau}, and in this event the minimization in \eqref{eq:scal_min_sec} is equivalent to 
\begin{align}
\min_{\tau\in[\tau_*-\zeta,\tau_*+\zeta]}\min_{ \substack{ \thetathree\in\Dc_3  }} \;\tilde{L}_n(\thetathree,\tau)\label{eq:scal_min_sec_tau_small}.
\end{align}

First, note that the objective function $\tilde{L}(\thetathree,\tau)$ is $1/\tau$ strongly convex in $\thetathree$ for fixed $\tau$.  Thus, for every fixed $\tau\in[\tau_*-\zeta,\tau_*+\zeta]$ and any $\thetathree\in\Dc_3$, it holds that
\begin{align}
\tilde{L}_n(\thetathree,\tau)\geq \tilde{L}_n(\thetathree_n(\tau),\tau) + \frac{1}{2\tau}\|\thetathree-\thetathree_n(\tau)\|_2^2 \geq \tilde{L}_n(\thetathree_n(\tau),\tau) + \frac{1}{4\tau_*}\|\thetathree-\thetathree_n(\tau)\|_2^2,\label{eq:strong_tau}
\end{align}
where we also assume small enough $\eta>0$, such that $\tau_*+\eta\leq 2\tau_*$. 
%Onwards, we always assume $\tau\in[\tau_*-\zeta,\tau_*+\zeta]$ and $\thetathree\in\Sc_\eps^c:=\left\{\thetathree\;|\;\|\thetathree-\thetathree_n(\tau_n)\|\geq \eps\right\}$, unless otherwise stated. 

Second, in the event $\Ec$, there exists constant $C>$ such that
\begin{align*}
\forall\tau\in[\tau_*-\zeta,\tau_*+\zeta] :\; \|\thetathree_n(\tau)-\thetathree_n(\tau_n)\|_2&=\|n(\A^T\A)^{-1}\vb_n\|_2\cdot|\tau-\tau_n|\leq C\zeta,
\leq
\left(\frac{2}{\delta}\right)\left(\frac{1+\eta}{1-6n^{-1/2}-3\eta}\right)\zeta\\
&\leq
C\left(\frac{1+\eta}{1-6n^{-1/2}-3\eta}\right)\zeta=:\eps^\prime.
\end{align*}
where we also used that $\delta>c_\delta$.
Thus, for all 
$$
%\|\thetathree-\thetathree_n(\tau_n)\|\geq \eps 
\forall\tau\in[\tau_*-\zeta,\tau_*+\zeta] :\; \thetathree\in\Sc_\eps^c:=\left\{\thetathree\;|\;\|\thetathree-\thetathree_n(\tau_n)\|\geq \eps\right\}
\implies
\|\thetathree-\thetathree_n(\tau)\|\geq \eps-C\zeta.
$$
Now, provided $\eps>2C/\sqrt{n}$, we choose $\eta$ (hence, $\zeta$), such that $C\zeta=\eps/2\implies \eta=\nicefrac{\eps}{2C}$. With this choice, and combining the above display with \eqref{eq:strong_tau}, we find that 
\begin{align}
\forall\tau\in[\tau_*-\zeta,\tau_*+\zeta]\,,\,\thetathree\in\Sc_\eps^c :\; \tilde{L}_n(\thetathree,\tau)\geq \tilde{L}_n(\thetathree_n(\tau),\tau)+\frac{1}{16\tau_*}\eps^2.\label{eq:str_cvx_res}
\end{align}
We are now ready to prove the desired as shown in the display below:
\begin{align*}
\min_{\|\thetathree-\thetathree_n\|_2\geq \eps} L_n(\thetathree) &=
\min_{\tau\in[\tau_*-\zeta,\tau_*+\zeta]}\min_{\|\thetathree-\thetathree_n\|_2\geq \eps} \tilde{L}_n(\thetathree,\tau)
\\
&\stackrel{\eqref{eq:str_cvx_res}}{\geq} \min_{\tau\in[\tau_*-\zeta,\tau_*+\zeta]}\min_{\|\thetathree-\thetathree_n\|_2\geq \eps} \tilde{L}_n(\thetathree_n(\tau),\tau)+\frac{1}{16\tau_*}\eps^2.
\\
&=\min_{\tau\in[\tau_*-\zeta,\tau_*+\zeta]}\tilde{L}_n(\thetathree_n(\tau),\tau)+\frac{1}{16\tau_*}\eps^2.
\\
&=\tilde{L}_n(\thetathree_n(\tau_n),\tau_n)+\frac{1}{16\tau_*}\eps^2.
\\
&={L}_n(\thetathree_n)+\frac{1}{16\tau_*}\eps^2.
\end{align*}
This completes the proof of the lemma. 
\end{proof} 

%In our proof, we need the following standard lemma to bound quadratic forms of Wishart matrix (see for example \cite[Lemma 2]{muthukumar2020classification}).
%\begin{lemma}\label{lem:wishartineq}
%Define $p^\prime(n) := (n-p+1)$. Let matrix $\A\in\R^{n\times p}$ with entries IID standard normal. For any unit Euclidean-norm vector $\vb$ and any $t >0$, we have
%\begin{align*}
%    \Pro\Big({\vb^T(\A^T\A)^{-1}\vb} < \big(p^\prime(n) + \sqrt{2tp^\prime(n)}+2t\big)^{-1}\Big) &\le e^{-t}\\
%    \Pro\Big({\vb^T(\A^T\A)^{-1}\vb} > \big(p^\prime(n) - \sqrt{2tp^\prime(n)}\big)^{-1}\Big) &\le e^{-t},
%\end{align*}
%provided that $p^\prime(n) > 2\max\{t, 1\}$.
%\end{lemma}


\subsubsection{Proofs for Section \ref{sec:sec_ord_ao}}

\begin{lemma} Recall the definitions of $\A\in\R^{n\times 3}, \omegab_t\in\R^n, \vb_n\in\R^3$ in Section XXX. Further let Assumption \ref{ass:omega} hold. For large enough $n$, $\delta>c_\delta$ and any $\eta>0$ smaller than some constant, there exist constants $C,c,C'>0$ such that each one of the events $\Ec_i, i\in[4]$ in \eqref{eq:good_events_quad} holds with probability at least $1-Ce^{-cn\eta^2}$.
\end{lemma}
\begin{proof}
We will prove the following refined version of \eqref{eq:good_events_quad}.
\begin{subequations}
\begin{align}
\Ec_1&:=\left\{ \frac{1}{1+6n^{-1/2}+3\eta}\,\mathbf{I}_3 \preceq n(\A^T\A)^{-1} \preceq 
\frac{1}{1-6n^{-1/2}-3\eta}\,\mathbf{I}_3
\right\}
\\
\Ec_2&:=\left\{ \frac{1}{\delta}(1-\eta)-\frac{2}{n}\leq\|\vb_n\|_2^2\leq \frac{1}{\delta}(1+\eta)
\right\}\\
\Ec_3&:=\left\{ \left| \frac{\|\omegab_t\|_2^2}{n} - \E\Omega_t^2 \right|\leq \eta
\right\}
\\
\Ec_4&:=\left\{ \left| \frac{1}{n}\gammab_1^T\omegab_t - \E[G_1\Omega_t] \right| \vee 
\left| \frac{1}{n}\gammab_2^T\omegab_t - \E[G_2\Omega_t] \right| \vee
\left| \frac{1}{n}\g_1^T\omegab_t  \right|
\leq C'\eta\right\}
\\
\Ec_5&:=\left\{ \left| \frac{\|\A^T\omegab_t\|^2}{n^2} - \left(\E[G_1\Omega_t]\right)^2 - \left(\E[G_2\Omega_t]\right)^2 \right|\leq 3\eta^2 + 2\eta\left(\E[G_1\Omega_t]+\E[G_2\Omega_t]\right)\right\}
\end{align}
\end{subequations}
All these events hold with high-probability. Specifically,
\begin{subequations}
\begin{align}
\Pro(\Ec_1)\wedge\Pro(\Ec_2)&\geq 1 - Ce^{-c n \eta^2}
\\
\Pro(\Ec_3)&\geq 1 - 2e^{-cn\left(\frac{\eta^2}{K_\omega^4}\wedge\frac{\eta}{K_\omega^2}\right)}
\\
\Pro(\Ec_4)\wedge\Pro(\Ec_5)&\geq 1 - 2e^{-cn\frac{\eta^2}{K_\omega^2}}
\end{align}
\end{subequations}
\ct{From Assumption \ref{ass:omega}, $K_\omega<C$ and $\E[\Omega^2]<C$.}

Using $\E[G_1\Omega_t]\vee\E[G_2\Omega_t]\leq\sqrt{\E[\Omega_t^2]}$ and $\eta\in(0,1)$ on the event $\Ec$, we have that
\begin{align*}
\left| \frac{\|\A^T\omegab_t\|^2}{n^2} - \left(\E[G_1\Omega_t]\right)^2 - \left(\E[G_2\Omega_t]\right)^2 \right|&\leq \left(3 + 4\sqrt{\E[\Omega_t^2]}\right)\eta
%\\&\leq \left(3 + 4\sqrt{K_\omega}\right)\eta\leq C\left(1\vee \sqrt{K_\omega}\right)\eta\leq 
\leq C\eta,
\end{align*}
where we used Cauchy-Schwartz in the first inequality and $\E[\Omega_t^2]<C$ in the second inequality, respectively.


\end{proof}



==> sections/gordon/gordon_second_order.tex <==

\subsection{Scalarization, Concentration and deviation of the AO (Proof of Lemmas \ref{lem:AO_main_sec} and \ref{lem:AO_main_gd} )}
\label{sec:conc_proof_main}

Here we show how to obtain the concentration and deviation results of Lemmas \ref{lem:AO_main_sec} and \ref{lem:AO_main_gd}. 

\subsubsection{Second-order methods}\label{sec:sec_ord_ao}

\ct{I will edit this first part}Recall from Equation \eqref{eq:sec_order_gen} that
$\Lc(\theta,\theta^t;\X,\y):=\frac{1}{\sqrt{n}}\|\omega(\X\thetacur,\y)-\X\thetacur\|_2.$
This corresponds to setting $\Fc_t(\ub,\theta)=\|\omegab_t-\ub\|_2$; equivalently, 
$
h(\theta,\thetacur)=0
$
and 
$
 g(\ub,\X\thetacur;\y)=\frac{1}{\sqrt{n}}\|\omegab_t-\ub\|_2.
$
% where we defined
%\begin{align}\label{eq:omegat_def}
%\omegab_t:=\omegab(\xit ,\sigmat ):=\omega\big(\xit \gammab_{1}+\sigmat \gammab_{2}\,,\, f\big(R\gammab_{1};\zb\big)+\epsb\big).
%\end{align}
We see for the convex conjugate function that $$g^*(\vb,\X\thetacur;\y)=\begin{cases}
\inp{\vb}{\omegab_t}&\text{if } \|\vb\|_2\leq \frac{1}{\sqrt{n}},\\
+\infty &\text{otherwise}.
\end{cases}
$$
Therefore, the AO in \eqref{eq:conAO2_no_u} simplifies as follows:
\begin{align}
\phi_{n,\Dc}&=\min_{ { (\xi,\alpha,\beta)\in\Dcthree  }}\;\max_{\|\vb\|_2\leq \frac{1}{\sqrt{n}}} \; \inp{\omegab_t}{\vb} -\inp{\beta\g+\xi\gammab_1+\alpha\gammab_2}{\vb}-{\beta} \| P^{\perp}_{S^t}\h \|_2 \|\vb\|_2 \label{eq:con_final_AO_sec_pre}\\
&=\left(\min_{ \substack{ (\xi,\alpha,\beta)\in\Dcthree  }} \; \frac{1}{\sqrt{n}}\|\beta\g+\xi\gammab_1+\alpha\gammab_2-\omegab_t\|_2 - \beta \frac{\| P^{\perp}_{S^t}\h \|_2}{\sqrt{n}}\right)_+\label{eq:con_final_AO_sec_2}\,.
\end{align}
The second equality follows easily by explicitly maximizing over $\vb$. 



We start with the AO formulation in \eqref{eq:con_final_AO_sec_2} and  focus on the inner minimization. To lighten notation, denote
\begin{align}\label{eq:AO_notation_conc}
\sqrt{\kappa_n}:=\frac{\| P^{\perp}_{S^t}\h \|_2}{\sqrt{n}},\qquad \A:=\big[\gammab_1,\gammab_2,\g\big]\in\R^{n\times 3},\qquad \vb_n=[0,0,\sqrt{\kappa_n}]^T\in\R^3,
\end{align}
and recall that $\thetathree=[\xi,\alpha,\beta].$ With this notation, the \emph{unconstrained} (that is, with $\Dc=\Bc_2(C_1)$)  inner minimization in \eqref{eq:con_final_AO_sec_2} becomes:  
\ct{Argue that unconstrained vs contrained is no difference}
\begin{align}
\min_{ \substack{ \thetathree\in\Dcthreeu  }} \;L_n(\thetathree):= \frac{1}{\sqrt{n}}\|\A\thetathree-\omegab_t\|_2 - \vb_n^T\thetathree.\label{eq:scal_min_sec}
\end{align}

The following result is essentially a restatement of Parts B (concentration of the optimal cost) and C (strong convexity)  of Lemma \ref{lem:AO_main_sec} together with together with a statement that shows concentration of the minimizers of the AO. The purpose of this section is to prove Lemma \ref{lem:deviation_sec}.

\begin{lemma}\label{lem:deviation_sec}
Consider the minimization in \eqref{eq:scal_min_sec}. For $n$ large enough, there exist absolute constants $C,c,C',c'>0$ and $c_\delta>1$ such that the following statements hold for all $\delta>c_\delta$ and  $c'>\eps>C'n^{-\nicefrac{1}{2}}$.

% Let $n$ be large enough, $\delta>c_\delta$ for appropriate constant $c_\delta>1$, and  any $\eta>0$ smaller than some absolute constant.
\begin{enumerate}
\item With probability at least {$1-Ce^{-cn}$}, the minimizer $\thetathree_n:=[\xi_n,\alpha_n,\beta_n]=
\arg\min_{\thetathree\in\Dcthreeu } L_n(\thetathree),
$ is unique and takes the form:
\begin{subequations}
\begin{align}
&\thetathree_n:=\thetathree_n(\tau_n):=(\A^T\A)^{-1}\A^T\omegab_t + \tau_n\cdot n\cdot(\A^T\A)^{-1}\vb_n,\quad\label{eq:thetathree_n}\\
&\qquad\qquad\text{where},\quad\tau_n=\frac{\frac{1}{\sqrt{n}}\|\left(\mathbf{I}_n-\A(\A^T\A)^{-1}\A^T\right)\omegab_t\|_2}{\sqrt{1-n\cdot\vb_n^T(\A^T\A)^{-1}\vb_n}}.\label{eq:tau_n}
\end{align}
\end{subequations}

\item With probability at least {$1-Ce^{-cn\eps^2}$},
\begin{subequations}
\begin{align}\label{eq:tau_star_sec}
&\left|\tau_n-\tau_\star\right|\leq \eps,\qquad\text{where}\quad\tau_\star = \sqrt{\left(\frac{\delta}{\delta-1}\right)\left(\E[\Omega_t^2]-\left(\E[G_1\Omega_t]\right)^2-\left(\E[G_2\Omega_t]\right)^2\right)}
\\
&\left|\xi_n-\xinextstar\right| \vee \left|\alpha_n-\alphanextstar\right| \vee \left|\beta_n-\betanextstar\right| \leq \eps,
\label{eq:theta_star_sec}
\end{align}
where $\xinextstar,\alphanextstar,\betanextstar$ are as defined in Equation \eqref{eq:theta_starnext_sec}.
%\quad\begin{cases}
%~\xinextstar=\E[G_1\Omega_t]\\
%~\alphanextstar=\E[G_2\Omega_t]\\
%~\betanextstar={\tau_*}\big/{\sqrt{\delta}}.
%\end{cases}
\end{subequations}


\item Part B of Lemma \ref{lem:AO_main_sec} holds.
%With probability at least {$1-Ce^{-cn\eps^2}$},
%\begin{align}\label{eq:bar_L_sec}
%\left| L_n(\thetathree_n)- \bar{L}\right|\leq \eps,\quad\text{where } \bar{L}:=\left(1-\frac{1}{\delta}\right)\tau_*.
%\end{align}

\item Part C of Lemma \ref{lem:AO_main_sec} holds.

%\item With probability at least {$1-Ce^{-cn\eps^2}$}, there exists absolute constant $C_\tau>0$ following strong convexity property holds 
%\begin{align}
%%\min_{\|\thetathree-\thetathree_n\|_2\geq \eps} L_n(\thetathree) \geq  L_n(\thetathree_n)+\frac{1}{16\tau_*}\eps^2.
%\min_{\|\thetathree-\thetathree_n\|_2\geq \eps} L_n(\thetathree) \geq  L_n(\thetathree_n)+C_\tau\eps^2.
%\end{align}
%for all $\eps>C'n^{-\nicefrac{1}{2}}.$

\end{enumerate}
\end{lemma}

%We are now ready to state and prove our main result for second order methods.


%In our proof, we need the following standard lemma to bound quadratic forms of Wishart matrix (see for example \cite[Lemma 2]{muthukumar2020classification}).
%\begin{lemma}\label{lem:wishartineq}
%Define $p^\prime(n) := (n-p+1)$. Let matrix $\A\in\R^{n\times p}$ with entries IID standard normal. For any unit Euclidean-norm vector $\vb$ and any $t >0$, we have
%\begin{align*}
%    \Pro\Big({\vb^T(\A^T\A)^{-1}\vb} < \big(p^\prime(n) + \sqrt{2tp^\prime(n)}+2t\big)^{-1}\Big) &\le e^{-t}\\
%    \Pro\Big({\vb^T(\A^T\A)^{-1}\vb} > \big(p^\prime(n) - \sqrt{2tp^\prime(n)}\big)^{-1}\Big) &\le e^{-t},
%\end{align*}
%provided that $p^\prime(n) > 2\max\{t, 1\}$.
%\end{lemma}



%\subsubsection{Proofs for Section \ref{sec:sec_ord_ao}}
%\ct{Eventually move to appendix.}

\begin{proof}[\textbf{Proof of Lemma \ref{lem:deviation_sec}}]
Throughout the proof, we will condition on the intersection
$\Ec=\Ec_1\cap\Ec_2\cap\Ec_3\cap\Ec_4\cap\Ec_5$ of the following events for $\eta>Cn^{-\nicefrac{1}{2}}$:
\begin{subequations}\label{eq:good_events_quad}
\begin{align}
\Ec_1&:=\left\{ \left(1-C'\left(n^{-\nicefrac{1}{2}}\vee\eta\right)\right)\,\mathbf{I}_3 \preceq n(\A^T\A)^{-1} \preceq 
\left(1+C'\left(n^{-\nicefrac{1}{2}}\vee\eta\right)\right)\,\mathbf{I}_3
\right\}
\\
\Ec_2&:=\left\{ \frac{1}{\delta} - C'\left(n^{-1}\vee\eta\right)\leq\|\vb_n\|_2^2\leq \frac{1}{\delta} + \eta
\right\}\\
\Ec_3&:=\left\{ \left| \frac{\|\omegab_t\|_2^2}{n} - \E\Omega_t^2 \right|\leq \eta
\right\}
\\
\Ec_4&:=\left\{ \left| \frac{1}{n}\gammab_1^T\omegab_t - \E[G_1\Omega_t] \right| \vee 
\left| \frac{1}{n}\gammab_2^T\omegab_t - \E[G_2\Omega_t] \right| \vee
\left| \frac{1}{n}\g_1^T\omegab_t  \right|
\leq \eta\right\}
\\
\Ec_5&:=\left\{ \left| \frac{\|\A^T\omegab_t\|^2}{n^2} - \left(\E[G_1\Omega_t]\right)^2 - \left(\E[G_2\Omega_t]\right)^2 \right|\leq \eta\right\}.
\end{align}
\end{subequations}
We show in lemma XXX that $\Pro(\Ec)\geq 1- Ce^{-cn\eta^2}$ for constatns $C,c>0$. 


The first step in the proof is to rewrite the minimization in 
 \eqref{eq:scal_min_sec} equivalently as \ct{Can we switch order of mins here? Might need to adjust this or justify}
\begin{align}
\min_{\thetathree\in\Dcthreeu}L_n(\thetathree) &=
\min_{ \substack{ \thetathree\in\Dcthreeu  }} \;\inf_{\tau>0}\; \tilde{L}_n(\thetathree,\tau):= \frac{\tau}{2}+\frac{1}{2\tau n}\|\A\thetathree-\omegab_t\|_2^2 - \vb_n^T\thetathree\nn \end{align}
We will argue that, 
\begin{align}\label{eq:no_range_space}
\text{in the event $\Ec$,}~~\forall \thetathree\in\R^3\;:\; \|\A\thetathree-\omegab_t\|_2>0.
\end{align}
 Thus, the minimum over $\tau$ in the optimization above is always attained in this event, so we can equivalently write 
 \begin{align}
% \min_{\thetathree\in\Dcthreeu}L_n(\thetathree) =
L_n(\thetathree_n) = \inf_{\tau>0}\;\min_{ \substack{ \thetathree\in\Dcthreeu  }} \;\frac{\tau}{2}+\frac{1}{2\tau n}\|\A\thetathree-\omegab_t\|_2^2 - \vb_n^T\thetathree.\label{eq:scal_min_sec_tau}
 \end{align}
To prove \eqref{eq:no_range_space}, it suffices to show that $\omegab_t$ is not in the range space of $\A$.
% that is $\|(\mathbf{I}_n-\A(\A^T\A)^{-1}\A^T)\omegab_t\|_2>0$. 
 We will soon prove this in \eqref{eq:num} by showing in the event $\Ec$ such that $\|(\mathbf{I}_n-\A(\A^T\A)^{-1}\A^T)\omegab_t\|_2 \geq \left(\E[\Omega_t^2]-(\E[G_1\Omega_t])^2-(\E[G_2\Omega_t])^2 \right) - C\left(n^{-1/2}\vee\eta\right)>c-C\left(n^{-1/2}\vee\eta\right)$. The last inequality here follows by Assumption \ref{ass:omega}. Thus, for sufficiently large $n$ and $\eta$ smaller than some constant, the previous expression is strictly positive. This proves \eqref{eq:no_range_space}. 

%The first equality holds by noting that $x=\inf_{\tau>0}\frac{\tau}{2}+\frac{x^2}{2\tau}$ for all $x\geq0$. The flip of min-inf in the second equality is possible as follows. For  

\noindent\textbf{Proof of Statement 1.}~Let $\thetathree_n(\tau)$ denote the solution of the inner quadratic minimization in \eqref{eq:scal_min_sec_tau}. Specifically,
$$
\thetathree_n(\tau) = (\A^T\A)^{-1}\A^T\omegab_t + \tau\cdot n\cdot(\A^T\A)^{-1}\vb_n.
$$
Then, we can minimize over $\tau$ by solving
\begin{align}\label{eq:tilde_L_tau}
\min_{\tau>0}\;\tilde{L}_n\big((\thetathree_n(\tau),\tau)\big)=\frac{1}{2\tau n}\|\left(\mathbf{I}_n-\A(\A^T\A)^{-1}\A^T\right)\omegab_t\|_2^2 + \frac{\tau}{2}\left(1-n\cdot\vb_n^T(\A^T\A)^{-1}\vb_n\right)-\vb_n^T(\A^T\A)^{-1}\A\omegab_t,
\end{align}
which yields 
\begin{align}
\tau_n=\frac{\frac{1}{\sqrt{n}}\|\left(\mathbf{I}_n-\A(\A^T\A)^{-1}\A^T\right)\omegab_t\|_2}{\sqrt{1-n\cdot\vb_n^T(\A^T\A)^{-1}\vb_n}},\label{eq:tau_n}
\end{align}
provided that 
\begin{align}\label{eq:check_for_tau_n}
n\cdot\vb_n^T\left({\A^T\A}\right)^{-1}\vb_n<1.
\end{align}
%But, from Lemma \ref{lem:wishartineq} on quadratic forms of Wishart matrices, it holds with probability at least $1-e^{-cn}$ that 
%$\vb_n^T\left({\A^T\A}\right)^{-1}\vb_n\leq \kappa_n\frac{2}{n-2}.$ Moreover, from \eqref{eq:???}: for all $\eps\in(0,1)$:  $\kappa_n\leq 1/\delta + \eps$ with probability at least $1-e^{-c\eps^2n}$. Thus, there exist constants $c_\delta>1$ and $c>0$ such that 
%\begin{align}\label{eq:tau_denom}
%\Pro\left(\vb_n^T(\A^T\A)^{-1}\vb_n<\frac{1}{2n}\right)\geq 1-e^{-cn},
%\end{align}
%provided that $\delta>c_\delta.$ This proves the first statement of the lemma.




Denote ${\rm{num}}({\tau_n}),\rm{den}({\tau_n})$ the numerator and denominator in \eqref{eq:tau_n}. In the event $\Ec$ the following are true. 
First, \ct{from XXX} with probability at least $1-Ce^{-cn\eta^2}$, \ct{I will clean}
\begin{align}
\sqrt{1-\frac{1}{\delta}-C\left(n^{-1/2}\vee\eta\right)}&\leq{\rm{den}}({\tau_n})\leq\sqrt{1-\frac{1}{\delta}+C\left(n^{-1/2}\vee\eta\right)}.\label{eq:den}
\end{align} 
Note that this
%Assuming here large enough constant $\delta>C\gg 1,$ 
guarantees the non-negativity of the denominator, that is \eqref{eq:check_for_tau_n} is satisfied, which completes the proof of the first statement of the lemma. 

\noindent\textbf{Proof of \emph{2}.}~\ct{Second, ....}
This leads to 
\begin{align}
\left| \left({{\rm{num}}}({\tau_n})\right)^2-\left(\E[\Omega_t^2]-{(\E[G_1\Omega_t])^2-(\E[G_2\Omega_t])^2} \right)\right| \leq C\left(n^{-1/2}\vee\eta\right).\label{eq:num}
\end{align}

Putting together \eqref{eq:num} and \eqref{eq:den} we conclude that
\begin{align}
\sqrt{\frac{a-C\left(n^{-1/2}\vee \eta\right)}{b+C\left(n^{-1/2}\vee \eta\right)}}\leq \tau_n\leq \sqrt{\frac{a+C\left(n^{-1/2}\vee \eta\right)}{b-C\left(n^{-1/2}\vee \eta\right)}}
\end{align}
where we set $a:=\E[\Omega_t^2]-(\E[G_1\Omega_t])^2-(\E[G_2\Omega_t])^2$ and $b:=1-1/\delta$, for simplicity. Assuming constants such that $\delta>c>1$ (thus, $b>c'$) and $a>c$, this leads to 
\begin{align}
\left|\tau_n-\sqrt{\frac{a}{b}}\right|\leq C\left(n^{-1/2}\vee \eta\right).\end{align}
Here, we used that
\begin{align*}
\sqrt{\frac{a+\eps}{b-\eps}}-\sqrt{\frac{a}{b}}= \sqrt{\frac{a}{b}}\left(\sqrt{1+\frac{\frac{\eps}{b}+\frac{\eps}{a}}{1-\frac{\eps}{b}}}-1\right)  \leq
\sqrt{\frac{a}{b}} \left(\frac{\frac{\eps}{b}+\frac{\eps}{a}}{2(1-\frac{\eps}{b})}\right) \leq C\eps.
\end{align*}
The first inequality follows by $\sqrt{1+x}\leq1+x/2$ and the second inequality uses constant lower and upper bounds on $a,b$.
Noting that $\tau_*=\sqrt{a/b}$ completes the proof of Equation \eqref{eq:tau_star_sec}.

Now, we prove \eqref{eq:theta_star_sec}. We show only the concentration upper bounds, since the lower bounds follow in the same way.  For $i=1,2$ and $\eb_i$ the corresponding basis vectors in $\R^3$, we have the desired thanks to events $\Ec_1$ and $\Ec_4$:
$$
\eb_i^T\thetathree_n \leq\left(1+C(n^{-1/2}\vee \eta)\right)\frac{1}{n}\eb_i^T\A\omegab_t \leq \left(1+C(n^{-1/2}\vee \eta)\right)\left(\E[G_i\Omega_t]+\eta\right) \leq \E[G_i\Omega_t] + C(n^{-1/2}\vee \eta).
$$
The bounds on $\beta_n=\eb_3^T\thetathree_n$ follow similarly thanks to events $\Ec_1, \Ec_4$, $\Ec_2$. We omit the details for brevity.


%To continue, we first argue that we can restrict the range of $\tau$ minimization in \eqref{eq:scal_min_sec_tau} in the interval $(0,T]$ for sufficiently large constant $T>0$. It suffices to show that $\tau_n<T$ with high probability. Focus on the numerator in Equation \eqref{eq:tau_n}. Let $\ab_1^T,\ldots\ab_n^T\in\R^3$, denote the rows of $\A$ and $\B_{-1}=\sum_{i=2}^{n}\ab_i\ab_i^T$. Note that $\A^T\A=\ab_1\ab_1^T+\B$ and $\B$ is a $3\times3$ Wishart matrix with $n-1$ degrees of freedom independent of $\ab_1$. Using a standard leave-one-out argument together with the matrix inversion lemma and some algebra, we can show that 
%\begin{align}\label{eq:tau_num}
%\|\left(\mathbf{I}_n-\A(\A^T\A)^{-1}\A^T\right)\omegab_t\|_2 = \|\omegab_t\|_2\sqrt\frac{1}{1+\ab_1^T\B^{-1}\ab_1}.
%\end{align}
%Specifically, this means that $\|\left(\mathbf{I}_n-\A(\A^T\A)^{-1}\A^T\right)\omegab_t\|_2 \leq \|\omegab_t\|_2$. In turn, from Assumption \ref{ass:omega} and \eqref{eq:}, this is further upper bounded by $2\sqrt{n}\sqrt{\E[\Omega^2]}$ with probability at least $1-2e^{-cn(\E[\Omega^2])^2/K_\omega^4}.$ These, combined with \eqref{eq:tau_denom}, show that for $\delta>c_\delta$ there exists (sufficiently large) $T>0$ and $c,C>0$ such that $\tau_n\leq T$ with probability at least $1-Ce^{-cn(\E[\Omega^2])^2/K_\omega^4}$.

\vp
\noindent\textbf{Proof of Statement 3.}~
Recall that $L_n(\theta_n)=\tilde L_n(\theta_n(\tau_n),\tau_n)$. Thus, from \eqref{eq:tilde_L_tau}:
\begin{align}\label{eq:Ln_conc_proof_sec}
L_n(\theta_n) = \left({\rm{den}{(\tau_n)}}\right)^2\tau_n-\vb_n^T(\A^T\A)^{-1}\A\omegab_t.
\end{align}
Note that $\vb_n^T\A\omegab_t=\sqrt{\kappa_n}\g^T\omegab_t$. From this and thanks to $\Ec_1, \Ec_4$, we have that $|\vb_n^T(\A^T\A)^{-1}\A\omegab_t|\leq C\left(n^{-1/2}\vee\eta\right).$ For the first therm in \eqref{eq:Ln_conc_proof_sec} recall Equations \eqref{eq:den} and \eqref{eq:tau_n}. The desired follows from these and simple calculations

\vp
\noindent\textbf{Proof of Statement 4.}~
 Condition on the event $|\tau_*-\tau_n|\leq (\eta\vee n^{-1/2})=:\zeta$ for some $\eta>0$ that we pick later in the proof. From concentration of $\tau_n$, we can restrict the range of $\tau$-minimization in \eqref{eq:scal_min_sec_tau}, and in this event the minimization in \eqref{eq:scal_min_sec} is equivalent to 
\begin{align}
\min_{\tau\in[\tau_*-\zeta,\tau_*+\zeta]}\min_{ \substack{ \thetathree\in\Dcthree  }} \;\tilde{L}_n(\thetathree,\tau)\label{eq:scal_min_sec_tau_small}.
\end{align}

First, note that the objective function $\tilde{L}(\thetathree,\tau)$ is $1/\tau$ strongly convex in $\thetathree$ for fixed $\tau$.  Thus, for every fixed $\tau\in[\tau_*-\zeta,\tau_*+\zeta]$ and any $\thetathree\in\Dcthree$, it holds that
\begin{align}
\tilde{L}_n(\thetathree,\tau)\geq \tilde{L}_n(\thetathree_n(\tau),\tau) + \frac{1}{2\tau}\|\thetathree-\thetathree_n(\tau)\|_2^2 \geq \tilde{L}_n(\thetathree_n(\tau),\tau) + \frac{1}{4\tau_*}\|\thetathree-\thetathree_n(\tau)\|_2^2,\label{eq:strong_tau}
\end{align}
where we also assume small enough $\eta>0$, such that $\tau_*+\eta\leq 2\tau_*$. 
%Onwards, we always assume $\tau\in[\tau_*-\zeta,\tau_*+\zeta]$ and $\thetathree\in\Sc_\eps^c:=\left\{\thetathree\;|\;\|\thetathree-\thetathree_n(\tau_n)\|\geq \eps\right\}$, unless otherwise stated. 

Second, in the event $\Ec$, there exists constant $C>$ such that
\begin{align*}
\forall\tau\in[\tau_*-\zeta,\tau_*+\zeta] :\; \|\thetathree_n(\tau)-\thetathree_n(\tau_n)\|_2&=\|n(\A^T\A)^{-1}\vb_n\|_2\cdot|\tau-\tau_n|
\\&\leq \left(\frac{2}{\delta}\right)\left(\frac{1+\eta}{1-6n^{-1/2}-3\eta}\right)\zeta \leq C\zeta,
%\leq
%\left(\frac{2}{\delta}\right)\left(\frac{1+\eta}{1-6n^{-1/2}-3\eta}\right)\zeta\\
%&\leq
%C\left(\frac{1+\eta}{1-6n^{-1/2}-3\eta}\right)\zeta=:\eps^\prime.
\end{align*}
where we also used that $\delta>c_\delta$.
Thus, for all 
$$
%\|\thetathree-\thetathree_n(\tau_n)\|\geq \eps 
\forall\tau\in[\tau_*-\zeta,\tau_*+\zeta] :\; \thetathree\in\Sc_\eps^c:=\left\{\thetathree\;|\;\|\thetathree-\thetathree_n(\tau_n)\|\geq \eps\right\}
\implies
\|\thetathree-\thetathree_n(\tau)\|\geq \eps-C\zeta.
$$
Now, provided $\eps>2C/\sqrt{n}$, we choose $\eta$ (hence, $\zeta$), such that $C\zeta=\eps/2\implies \eta=\nicefrac{\eps}{2C}$. With this choice, and combining the above display with \eqref{eq:strong_tau}, we find that 
\begin{align}
\forall\tau\in[\tau_*-\zeta,\tau_*+\zeta]\,,\,\thetathree\in\Sc_\eps^c :\; \tilde{L}_n(\thetathree,\tau)\geq \tilde{L}_n(\thetathree_n(\tau),\tau)+\frac{1}{16\tau_*}\eps^2.\label{eq:str_cvx_res}
\end{align}
We are now ready to prove the desired as shown in the display below:
\begin{align*}
\min_{\|\thetathree-\thetathree_n\|_2\geq \eps} L_n(\thetathree) &=
\min_{\tau\in[\tau_*-\zeta,\tau_*+\zeta]}\min_{\|\thetathree-\thetathree_n\|_2\geq \eps} \tilde{L}_n(\thetathree,\tau)
\\
&\stackrel{\eqref{eq:str_cvx_res}}{\geq} \min_{\tau\in[\tau_*-\zeta,\tau_*+\zeta]}\min_{\|\thetathree-\thetathree_n\|_2\geq \eps} \tilde{L}_n(\thetathree_n(\tau),\tau)+\frac{1}{16\tau_*}\eps^2.
\\
&=\min_{\tau\in[\tau_*-\zeta,\tau_*+\zeta]}\tilde{L}_n(\thetathree_n(\tau),\tau)+\frac{1}{16\tau_*}\eps^2.
\\
&=\tilde{L}_n(\thetathree_n(\tau_n),\tau_n)+\frac{1}{16\tau_*}\eps^2.
\\
&={L}_n(\thetathree_n)+\frac{1}{16\tau_*}\eps^2.
\end{align*}
To finish the proof, note that $\tau_*\leq \sqrt{1+\frac{1}{c_\delta-1}}$. Thus, we can pick appropriate constant $C_\tau>0$ as in the statement of the lemma. This completes the proof. 
\end{proof} 


\begin{lemma}[Concentration results] Let Assumption \ref{ass:omega} hold and define $\A$ and $\vb_n$ as in Equation \eqref{eq:AO_notation_conc} .
\item
\begin{enumerate}
\item
\begin{align}
\big|{n\cdot\vb_n^T(\A^T\A)^{-1}\vb_n - \frac{1}{\delta}}\big|\leq \left(n^{-1/2}\vee\eta\right),
\end{align}

\item
\begin{align}
\left|\frac{\omegab_t^T\A^T\left(\A^T\A\right)^{-1}\A\omegab_t}{n} - \left((\E[G_1\Omega_t])^2+(\E[G_2\Omega_t])^2\right)\right|\leq \left(n^{-1/2}\vee\eta\right),
\end{align}

\end{enumerate}

\end{lemma}
\begin{proof}
First, with probability at least $1-Ce^{-cn\eta^2}$, \ct{I will clean}
\begin{align}\nn
\sqrt{1-\frac{1}{\delta}\left(1+\frac{6n^{-1/2}+4\eta}{1+6n^{-1/2}+3\eta}\right)}&\leq {\rm{den}}({\tau_n})\leq\sqrt{1-\frac{1}{\delta}\left(1-\frac{6n^{-1/2}+4\eta}{1-6n^{-1/2}-3\eta}\right)}\\
\sqrt{1-\frac{1}{\delta}-\frac{6n^{-1/2}+4\eta}{1+6n^{-1/2}+3\eta}}&\leq {\rm{den}}({\tau_n})\leq\sqrt{1-\frac{1}{\delta}+\frac{6n^{-1/2}+4\eta}{1-6n^{-1/2}-3\eta}}\nn
\\
\sqrt{1-\frac{1}{\delta}-C\left(n^{-1/2}\vee\eta\right)}&\leq{\rm{den}}({\tau_n})\leq\sqrt{1-\frac{1}{\delta}+C\left(n^{-1/2}\vee\eta\right)}.\label{eq:den}
\end{align}
In the second line we used that $\delta>c_\delta\gg1$ and in the third line we used $\eta$ small enough and $n$ larger than a constant.


it holds that 
$$
{{\rm{num}}}({\tau_n}) = \sqrt{\frac{1}{n}\|\omegab_t\|_2^2-\frac{1}{n^2}\omegab_t^T\A^T\left(n\left(\A^T\A\right)^{-1}\right)\A\omegab_t}\,.
$$
Hence,
\ct{Simplify}
{\tiny
\begin{align*}
-\frac{(\E[G_1\Omega_t])^2+(\E[G_2\Omega_t])^2}{1-6n^{-1/2}-3\eta}-\frac{\left(3 + 4\sqrt{\E[\Omega_t^2]}\right)\eta}{1-6n^{-1/2}-3\eta}&\leq-\frac{\omegab_t^T\A^T\left(\A^T\A\right)^{-1}\A\omegab_t}{n}\leq-\frac{(\E[G_1\Omega_t])^2+(\E[G_2\Omega_t])^2}{1+6n^{-1/2}+3\eta}+\frac{\left(3 + 4\sqrt{\E[\Omega_t^2]}\right)\eta}{1+6n^{-1/2}+3\eta}
\\
-{(\E[G_1\Omega_t])^2-\E[G_2\Omega_t])^2}-
C\left(n^{-1/2}\vee\eta\right)
&\leq-\frac{\omegab_t^T\A^T\left(\A^T\A\right)^{-1}\A\omegab_t}{n}\leq-{(\E[G_1\Omega_t])^2-(\E[G_2\Omega_t])^2}+C\left(n^{-1/2}\vee\eta\right),
\end{align*}
}
where we used again Cauchy-Schwartz and $\E[\Omega_t^2]<C$.
\end{proof}


==> sections/heuristic-derivation/heuristic-derivation.tex <==
%!TEX root = ../../convergence-gordon.tex

Before stating the main results and their proofs, we pause to provide a non-rigorous derivation of the Gordon updates.  Whereas the population state evolution is typically straightforward to derive, deriving the Gordon state evolution requires several steps even at the heuristic level.  For simplicity, we derive the updates for alternating minimization for noiseless phase retrieval.  

%\subsection{Main ingredient: the CGMT}
%\label{subsec:heuristic-CGMT}
Before diving into the derivations of the updates, we pause to discuss the CGMT (Convex Gaussian Min-max Theorem), which forms the bedrock of each derivation.  
\begin{theorem}
	\label{thm:gordon}
	Let $G = (G_{i,j})_{1 \leq i \leq n, 1 \leq j \leq d} \sim N(0,1)$, $g \sim N(0, I_{n})$, and $h \sim N(0,
	I_n)$.  Let also $D_u \subseteq \mathbb{R}^{d}$, $D_v \subseteq
	\mathbb{R}^n$ be compact sets and $Q: D_u \times D_v \rightarrow \mathbb{R}$
	continuous.
	Define the functions:
	\begin{align}
		P(G) &:= \min_{u \in D_u} \max_{v \in D_v} \langle v, G u \rangle + Q(u, v) \tag{Primary Optimization}\label{eq:CGMT-PO}\\
		A(g, h) &:= \min_{u \in D_u} \max_{v \in D_v} \| v \|_2 \langle g, u \rangle + \| u \|_2 \langle h, v \rangle + Q(u, v) \tag{Auxiliary Optimization}\label{eq:CGMT-AO}.
	\end{align}
	Then we have:
	\begin{enumerate}[label=(\alph*)]
		\item For all $t \in \mathbb{R}$:
		\[\Pr\left\{P(G) \leq t\right\} \leq 2\Pr\left\{A (g, h) \leq
		t\right\}.\]
		\item If $D_u, D_v$ convex and $Q$ convex-concave, then for all $t \in
		\mathbb{R}$:
		\[\Pr\left\{P (G) \geq t\right\} \leq 2\Pr\left\{A(g, h) \geq
		t\right\}.\]
	\end{enumerate}
\end{theorem} 
The proof of this theorem is, by now, standard and can be found in~\cite[Appendix C]{thrampoulidis2015regularized}.  Its utility will be made clear through the derivations in the subsequent subsection.  For now, we give a rough outline of the steps involved in deriving the Gordon updates, using the CGMT.  Consider a function $\mathcal{L}(\theta;G)$ which depends implicitly on a Gaussian matrix $G$ and suppose you are interested in finding its minimizers (over $\theta \in \mathbb{R}^d$).\\

\emph{Step 1: Write as minimax optimization of a bi-linear form in $G$.}  That is, this first step involves showing that there exists some function $P$ of the form~\eqref{eq:CGMT-PO} such that
\[
\min_{\theta \in \mathbb{R}^d} \mathcal{L}(\theta; G) = P(G).
\]
We will often refer to the function $P$ as the Primary optimization, or PO.\\

\emph{Step 2: Invoke the CGMT.}  The optimization~\eqref{eq:CGMT-PO} can often be complicated.  However, under Parts 1 and 2 of Theorem~\ref{thm:gordon}, there is a sharp characterization of $P(G)$ in terms of the function $A(g, h)$~\eqref{eq:CGMT-AO}.  We will often refer to the function $A$ as the Auxiliary Optimization, or AO.\\

\emph{Step 3: Solving the AO.} In many cases of interest, the AO can be solved in a straightforward manner.  In the examples we pursue, the function $Q$ will be separable over its coordinates, which enables the \emph{scalarization} of the problem.\\

The following subsection clarifies these abstract steps through a concrete example.  We emphasize again that the derivations in the next subsection is heuristic and aims to provide, through a simple example, a recipe for deriving Gordon updates in other problems of interest.  We defer precise statements and their proofs to Section~\ref{sec:main-results}.

\subsection{Example: alternating minimization for noiseless phase retrieval}
\label{subsec:heuristic-second-order}
Our first example is alternating projections for noiseless phase retrieval.  Recall that given an iterate $\thetacur$, the update can be written as
\begin{align*}
\thetanext &= \argmin_{\theta \in \mathbb{R}^{d}} \frac{1}{n} \sum_{i=1}^{n} (\mathsf{sgn}(\langle x_i, \thetacur \rangle)y_i - \langle x_i, \theta \rangle)^2\\
&\overset{\1}{=} \argmin_{\theta \in \mathbb{R}^d} \frac{1}{n} \| X\theta - \mathsf{sgn}(X \theta_t) \odot y\|_2^2\\
&= \argmin_{\theta \in \mathbb{R}^d} \frac{1}{\sqrt{n}} \| X\theta - \mathsf{sgn}(X \theta_t) \odot y\|_2,
\end{align*}
where in step $\1$ we have written the update using matrix-vector notation, specifically letting $\odot$ denote the Hadamard product between two vectors.  Next, define the loss
\[
\mathcal{L}(\theta; X) =  \frac{1}{\sqrt{n}} \| X\theta - \mathsf{sgn}(X \theta_t) \odot y\|_2.
\]
With this notation in hand, we pursue the steps outlined in Subsection~\ref{subsec:heuristic-CGMT}.  At the end of each step, we highlight the points at which rigor was abandoned.  These issues are carefully handled in the proofs of our main theorems, but at this heuristic level distract from the derivation.  

\paragraph{Step 1: Write as the minimax optimization of a bi-linear form in $X$.}
First, observe that 
\[
 \frac{1}{\sqrt{n}} \| X\theta - \mathsf{sgn}(X \theta_t) \odot y\|_2 = \max_{\| v \|_2 \leq 1} \frac{1}{\sqrt{n}}\langle v, X\theta \rangle - \frac{1}{\sqrt{n}}\langle v, \mathsf{sgn}(X \theta_t) \odot y \rangle.
\]
Thus, we can define the function
\[
P(X) = \min_{\theta \in \mathbb{R}^d} \max_{\| v \|_2 \leq 1} \frac{1}{\sqrt{n}}\langle v, X\theta \rangle - \frac{1}{\sqrt{n}}\langle v, \mathsf{sgn}(X \theta_t) \odot y \rangle, 
\]
where we recognize that $P(X)$ is of the required form.  Evidently, we have found that
\[
\min_{\theta \in \mathbb{R}^d} \mathcal{L}(\theta; X) = P(X).
\]
Note that our original motivation was to study the iterate $\thetanext$, which is the \emph{minimizer} of $\mathcal{L}(\theta; X)$, whereas here we are simply studying the minima.  Although a priori this has nothing to say about the minimizers, we proceed to the next step.  


\paragraph{Step 2: Invoke the CGMT.}  In order to use the CGMT, we require for bi-linear form to be independent of the function $Q$.  Unfortunately, for the natural candidate 
\[
Q_{\mathsf{attempt}}(\theta, v) = \frac{1}{\sqrt{n}} \langle v, \mathsf{sgn}(X \theta_t) \odot y \rangle,
\]
this is not the case as the random matrix $X$ appears in both terms.  To remedy this issue, consider the subspace $S_t = \mathsf{span}(\thetastar, \thetacur)$ and write
\[
P(X) = \min_{\theta \in \mathbb{R}^d} \max_{\| v \|_2 \leq 1} \frac{1}{\sqrt{n}}\langle v, X \proj_{S_t}^{\perp}\theta \rangle + \frac{1}{\sqrt{n}}\langle v, X \proj_{S_t}\theta \rangle- \frac{1}{\sqrt{n}}\langle v, \mathsf{sgn}(X \theta_t) \odot y \rangle.
\]
The first term is now independent of the rest, so we may introduce the function
\[
A(g, h) = \min_{\theta \in \mathbb{R}^d} \max_{\| v \|_2 \leq 1} \frac{1}{\sqrt{n}} \| v \|_2 \langle g, \proj_{S_t}^{\perp} \theta \rangle + \frac{1}{\sqrt{n}}\| \proj_{S_t}^{\perp} \theta \|_2 \langle h, v \rangle + \underbrace{\frac{1}{\sqrt{n}}\langle v, X \proj_{S_t}\theta \rangle- \frac{1}{\sqrt{n}}\langle v, \mathsf{sgn}(X \theta_t) \odot y \rangle}_{Q(\theta, v)}.
\]
We may now invoke the CGMT to see that
\[
P(X) \approx A(g, h).
\]
A few comments emphasizing the heuristic nature of this step are in order.  First, we did not restrict the minimization over $\theta$ to lie in a compact set, technically barring the application of the CGMT.  Second, the CGMT shows that $P(X)$ and $A(g, h)$ are equivalent with high probability, not in the deterministic sense of the above display.  

\paragraph{Step 3: Solving the AO.} 
We begin by applying the Cauchy-Schwarz inequality to maximize over $v$, obtaining
\[
A(g, h) = \min_{\theta \in \mathbb{R}^d} \max_{\| v \|_2 \leq 1} \frac{\| v \|_2}{\sqrt{n}}\bigl(\langle g, \proj_{S_t}^{\perp} \theta \rangle + \bigl\|\mathsf{sgn}(X \theta_t) \odot y - \|\proj_{S_t}^{\perp}\theta \|_2 h - X \proj_{S_t} \theta\bigr\|_2 \bigr).
\]
Note that the objective is linear in $\| v \|_2$ as well as in the direction $\proj_{S_t}^{\perp} \theta/ \| \proj_{S_t}^{\perp} \theta\|_2$, so we may minimize over both to obtain
\begin{align*}
A(g, h) &= \min_{\theta \in \mathbb{R}^d} \max_{\| v \|_2 \leq 1} \frac{\| v \|_2}{\sqrt{n}}\bigl(-\| \proj_{S_t}^{\perp} \theta \|_2 \| \proj_{S_t}^{\perp} g\|_2 + \bigl\|\mathsf{sgn}(X \theta_t) \odot y - \|\proj_{S_t}^{\perp}\theta \|_2 h - X \proj_{S_t} \theta\bigr\|_2 \bigr)\\
&= \min_{\theta \in \mathbb{R}^d} \bigl(-\| \proj_{S_t}^{\perp} \theta \|_2 \frac{\| \proj_{S_t}^{\perp} g\|_2}{\sqrt{n}} + \frac{1}{\sqrt{n}}\bigl\|\mathsf{sgn}(X \theta_t) \odot y - \|\proj_{S_t}^{\perp}\theta \|_2 h - X \proj_{S_t} \theta\bigr\|_2 \bigr)_{+},
\end{align*}
where the final equality follows by maximizing over the magnitude $\| v \|_2$.  We now scalarize the problem by introducing the change of variables
\begin{align}
	\label{eq:heuristic-gordon-change-of-var}
\xi = \langle \theta, \thetastar \rangle, \qquad \alpha = \frac{\langle \theta, \proj_{\thetastar}^{\perp}\thetacur\rangle}{\| \proj_{\thetastar}^{\perp}\theta_t \|_2}, \qquad \text{ and } \beta = \| \proj_{S_t}^{\perp} \theta \|_2, 
\end{align}
where we interpret $\xi$ as the projection of the decision variable $\theta$ onto the ground-truth $\thetastar$ (since by assumption $\| \thetastar \|_2 = 1$), $\alpha$ as  projection of $\theta$ onto the component of the current iterate $\thetacur$ orthogonal to the ground-truth (that is onto the unit vector $\proj_{\thetastar}^{\perp}\theta/\|\proj_{\thetastar}^{\perp}\theta\|_2$), and $\beta$ as the magnitude of the portion of $\theta$ orthogonal to the subspace spanned by the ground-truth and the current iterate.  Additionally, define the previous iterates as 
\[
\xicur = \langle \thetacur, \thetastar \rangle, \qquad \text{ and } \sigmacur = \| \proj_{\thetastar}^{\perp} \thetacur \|_2,
\]
and define the random vectors \ct{$z_1,z_2$ notation here can be tricky in view of $z_i$ in data model Eqn. (1).}
\[
z_1 = X \thetastar, \qquad \text{ and } z_2 = \frac{X \proj_{\thetastar}^{\perp} \thetacur}{\| \proj_{\thetastar}^{\perp} \thetacur \|_2},
\]
noting that $z_1 \sim \mathsf{N}(0, I_n)$, $z_2 \sim \mathsf{N}(0, I_n)$ and are independent.  Then, recalling that in noiseless phase retrieval $y = \lvert X \thetastar \rvert$ we obtain
\[
X\theta_t = \xi_t z_1 + \sigma_t z_2, \qquad y = \lvert z_1 \rvert, \qquad \text{ and } \qquad X\proj_{S_t}^{\perp} \theta = \xi z_1 + \alpha z_2.
\]
Thus, 
\begingroup
\allowdisplaybreaks
\begin{align}
A(g, h) &= \min_{\xi \in \mathbb{R}, \alpha \in \mathbb{R}, \beta \geq 0} \Bigl( - \beta \frac{\| \proj_{S_t}^{\perp} g\|_2}{\sqrt{n}} + \frac{1}{\sqrt{n}}\bigl\| \underbrace{\mathsf{sgn}(\xi_t z_1 + \sigma_t z_2) \odot \lvert z_1 \rvert}_{\omega_t(z_1, z_2)}  - \beta h - \xi z_1 - \alpha z_2 \bigr\|_2 \Bigr)_{+}\nonumber\\
&= \Bigl(\min_{\xi \in \mathbb{R}, \alpha \in \mathbb{R}, \beta \geq 0} - \beta \frac{\| \proj_{S_t}^{\perp} g\|_2}{\sqrt{n}} + \frac{1}{\sqrt{n}}\bigl\| \omega_t(z_1, z_2)  - \beta h - \xi z_1 - \alpha z_2 \bigr\|_2 \Bigr)_{+}\nonumber\\
&\overset{\1}{\approx} \Bigl(\min_{\xi \in \mathbb{R}, \alpha \in \mathbb{R}, \beta \geq 0} - \frac{\beta}{\sqrt{\delta}} + \frac{1}{\sqrt{n}}\bigl\| \omega_t(z_1, z_2)  - \beta h - \xi z_1 - \alpha z_2 \bigr\|_2 \Bigr)_{+}\nonumber\\
&\overset{\2}{=} \Bigl(\min_{\xi \in \mathbb{R}, \alpha \in \mathbb{R}, \beta \geq 0} \inf_{\tau > 0} - \frac{\beta}{\sqrt{\delta}}  + \frac{\tau}{2} + \frac{1}{2\tau n}\bigl\| \omega_t(z_1, z_2)  - \beta h - \xi z_1 - \alpha z_2 \bigr\|_2^2 \Bigr)_{+}\nonumber\\
&\overset{\3}{\approx} \Bigl(\min_{\xi \in \mathbb{R}, \alpha \in \mathbb{R}, \beta \geq 0} \inf_{\tau > 0} - \frac{\beta}{\sqrt{\delta}}  + \frac{\tau}{2} + \frac{1}{2\tau} \EE \bigl\{\bigl(\Omega_t(Z_1, Z_2)  - \beta H - \xi Z_1 - \alpha Z_2\bigr)^2\bigr\}\Bigr)_{+}\nonumber\\
&\overset{\4}{=} \Bigl(\inf_{\tau > 0} \min_{\xi \in \mathbb{R}, \alpha \in \mathbb{R}, \beta \geq 0} - \frac{\beta}{\sqrt{\delta}}  + \frac{\tau}{2} + \frac{1}{2\tau} \EE \bigl\{\bigl(\Omega_t(Z_1, Z_2)   - \beta H - \xi Z_1 - \alpha Z_2\bigr)^2\bigr\}\Bigr)_{+} \nonumber
\end{align}
\endgroup
where the approximation $\1$ follows since $g \sim \mathsf{N}(0, I_d)$ is independent of all other randomness, so that $\| \proj_{S_t}^{\perp} g \|_2/\sqrt{n} \approx 1/\sqrt{\delta}$; step $\2$ follows from the identity $\| x \|_2 = \inf_{\tau > 0} \tau/2 + 1/(2\tau) \| x\|_2^2$; the approximation $\3$ follows by applying the law of large numbers and introducing the independent random variables $Z_1, Z_2, H \sim \mathsf{N}(0, 1)$ as well as $\Omega_t(Z_1, Z_2) = \mathsf{sgn}(\xi_t Z_1 + \sigma_t Z_2) \lvert Z_1 \rvert$; and step $\4$ is justified whenever the expectation exists.  Motivated by this calculation, we define the deterministic quanitity
\[
A_{\star} = \Bigl(\inf_{\tau > 0} \min_{\xi \in \mathbb{R}, \alpha \in \mathbb{R}, \beta \geq 0} - \frac{\beta}{\sqrt{\delta}}  + \frac{\tau}{2} + \frac{1}{2\tau} \EE \bigl\{\bigl(\Omega_t(Z_1, Z_2)   - \beta H - \xi Z_1 - \alpha Z_2\bigr)^2\bigr\}\Bigr)_{+},
\]
so that 
\[
A(g, h) \approx A_{\star}
\]
Zooming in (and dropping the arguments of $\Omega_t$), we note that $H$ is independent of $Z_1$ and $Z_2$, so that 
\begin{align*}
- \frac{\beta}{\sqrt{\delta}}  + \frac{\tau}{2} + \frac{1}{2\tau} \EE \bigl\{\bigl(\Omega_t   - \beta H - \xi Z_1 - \alpha Z_2\bigr)^2\bigr\} = - \frac{\beta}{\sqrt{\delta}} + \frac{\beta^2}{2\tau}  + \frac{\tau}{2} + \frac{1}{2\tau} \EE \bigl\{\bigl(\Omega_t - \xi Z_1 - \alpha Z_2\bigr)^2\bigr\}.
\end{align*}
it is straightforward to see that the minimizers $\xi_{\star}$ and $\alpha_{\star}$ of the RHS on the display above are given by
\begin{align*}
\xi_{\star} = \EE\{ Z_1 \Omega_t\}, \qquad \text{ and } \alpha_{\star} = \EE\{ Z_2 \Omega_t\}.
\end{align*}
Plugging this back into $A_{\star}$, we have
\begin{align*}
	A_{\star} &= \Bigl(\inf_{\tau > 0} \min_{\beta \geq 0} - \frac{\beta}{\sqrt{\delta}} + \frac{\beta^2}{2\tau} + \frac{\tau}{2} + \frac{1}{2\tau} \bigl(\EE\{\Omega_t^2\} - (\EE\{Z_1 \Omega_t\})^2 - (\EE\{Z_2 \Omega_t\})^2 \bigr)\Bigr)_{+}\\
	&=\Bigl( \min_{\beta \geq 0}\inf_{\tau > 0} - \frac{\beta}{\sqrt{\delta}} + \frac{\beta^2}{2\tau} + \frac{\tau}{2} + \frac{1}{2\tau} \bigl(\EE\{\Omega_t^2\} - (\EE\{Z_1 \Omega_t\})^2 - (\EE\{Z_2 \Omega_t\})^2 \bigr)\Bigr)_{+}\\
	&= \Bigl( \min_{\beta \geq 0} -\frac{\beta}{\sqrt{\delta}} + \sqrt{\beta^2 + \bigl(\EE\{\Omega_t^2\} - (\EE\{Z_1 \Omega_t\})^2 - (\EE\{Z_2 \Omega_t\})^2 \bigr)}\Bigr)_{+}.
\end{align*}
Minimizing the above in $\beta$, we obtain
\[
\beta_{\star} = \sqrt{\frac{\EE\{\Omega_t^2\} - (\EE\{Z_1 \Omega_t\})^2 - (\EE\{Z_2 \Omega_t\})^2}{\delta - 1}}.
\]

Before giving the Gordon state evolution, we pause once more to remark on the heuristic nature of this derivation.  First, several deterministic approximations were made to random quantities.  Second, there is a priori no reason to believe the minimizers $(\xi_{\star}, \alpha_{\star}, \beta_{\star})$ have anything to do with $\thetanext$ as the only connection was made through the loss function.  Both of these concerns are carefully addressed in the proofs of our main results.

\paragraph{Obtaining the Gordon state evolution.}
Recall the change of variables~\eqref{eq:heuristic-gordon-change-of-var} and note that
\[
\| \proj_{\thetastar}^{\perp} \theta \|_2 = \sqrt{\beta^2 + \alpha^2}.
\]
Thus, 
\[
\sigma_{t+1} = \| \proj_{\thetastar}^{\perp} \thetanext \|_2 = \sqrt{\beta_{\star}^2 + \alpha_{\star}^2} = \sqrt{(\EE\{Z_2 \Omega_t\})^2 + \frac{\EE\{\Omega_t^2\} - (\EE\{Z_1 \Omega_t\})^2 - (\EE\{Z_2 \Omega_t\})^2}{\delta - 1}}.
\]
Letting $\alpha_t = \tan^{-1}(\sigma_t/\xi_t)$, a straightforward calculation shows that
\begin{align*}
	\EE\{Z_1 \Omega_t\} = 1 - \frac{1}{\pi}(2 \alpha_t - \sin(2\alpha_t)), \qquad \EE\{Z_2 \Omega_t\} = \frac{2}{\pi} \sin^2(\alpha_t), \qquad \text{ and } \qquad \EE\{\Omega_t^2\} = 1.
\end{align*}
Thus, recalling that $\xi_{\star} = \EE\{Z_1 \Omega_t\}$, we obtain the Gordon state evolution:
\begin{align*}
	\langle \thetanext, \thetastar \rangle = \xi_{t+1} &= 1 - \frac{1}{\pi}(2 \alpha_t - \sin(2\alpha_t)),\\
	\| \proj_{\thetastar}^{\perp} \thetanext \|_2 = \sigma_{t+1} &= \sqrt{\frac{4}{\pi^2} \sin^4(\alpha_t) + \frac{1 - (1 - \frac{1}{\pi}(2 \alpha_t - \sin(2\alpha_t)))^2 - \frac{4}{\pi^2} \sin^4(\alpha_t)}{\delta - 1}}.
\end{align*}


\subsection{General result: Concentration of $(\xi,\sigma)$ updates (Theorem \ref{thm:one_step_main})}
Following the heuristic derivation or the special case of alternating projections for phase retrieval,
we now formally derive and prove concentration of the one-step Gordon updates for first- and second- order methods for both the (noisy) phase-retrieval and mixtures-of-gaussians models. 

For the purpose of this section fix \emph{arbitrary} vector $\thetacur$ and consider the \emph{one-step} update \footnote{While we keep the subscript $t$ in for $\thetacur$ and $\Lc_t$ in \eqref{eq:gordon_one_step}, we emphasize that the analysis in this section is specific to \emph{one-step} updates. The evolution of the updates is treated later in Sections \ref{sec:} \ct{ref:evolution}. To clarify this, we simply denote the minimizer in \eqref{eq:gordon_one_step} as $\thetaplus$ (instead of $\theta_{t+1}$).}:
\begin{align}\label{eq:gordon_one_step}
\thetaplus \in \arg\min_\theta \underbrace{\Lc(\theta;\thetacur,\X,\y)}_{\Lc_t(\theta)},
\end{align}
where the loss function takes either of the forms in Equations \eqref{eq:GD_gen} and \eqref{eq:sec_order_gen}. Let $\xicur:=\inp{\thetacur}{\theta^*}$ and $\sigmacur:=\|P^\perp_{\thetastar} \thetacur\|_2$. Also, define $\xiplus$ and $\sigmaplus$ corresponding to $\thetaplus$, accordingly.
%
%%Here, we introduce some necessary notation and assumption for our analysis. 
%Recall the following notation from Subsection \ref{subsec:heuristic-second-order}: $S_t = {\sf span}(\thetastar, \thetacur)$ denotes the two-dimensional subspace spanned by $\thetastar$ and $\thetacur$; $P_{S^t}$ and $P_{S^t}^{\perp}$ denote the projection matrices onto this subspace and onto its orthogonal complement, respectively. Accordingly, $P_{\theta^\star}^\perp$ denotes the projection matrix onto the orthogonal complement of the subspace spanned by $\thetastar$. For any $\theta\in\R^d$ we introduced the $\theta$-dependent variables
%\begin{align}\label{eq:scal}
%\begin{cases}
%~\xitheta:={\inp{\theta}{\thetastar}}\\
%~\alphatheta :=\frac{\inp{\theta}{P^{\perp}_{\thetastar} \thetacur}}{\|P^{\perp}_{\thetastar} \thetacur\|_2}
%\\
%~\betatheta := \|P^{\perp}_{S^t}\theta\|_2\,.
%%~\sigma := \|P^\perp_{\thetastar} \theta\|_2.
%\end{cases}
%\end{align}
%In this notation
%$
%\sigmatheta^2 := \|P^\perp_{\thetastar} \theta\|_2^2 = \alphatheta^2+\betatheta^2.
%$
%Specifically, for the iterates $\thetacur$ we denote the corresponding quantities as $\xicur,\alphacur$ and $\betacur$. Accordingly, we define $\xinext,\alphanext$ and $\betanext$ for the minimizer $\thetaplus$ in \eqref{eq:gordon_one_step}. 




%






% $\bullet$~~Convex in $\theta$.
%
% $\bullet$~~Separable across samples: Suppose that we can write 
%  \begin{align}\label{eq:Lc}
%  \mathcal{L}_t(\theta) = h(\theta, \thetacur) + \frac{1}{n} \sum_{i = 1}^n g(\langle \bx_i, \theta \rangle, \langle \bx_i, \thetacur \rangle; y_i)
%  \end{align}
%   for some pair of functions $(h, g).$

%Define the following potential functions---corresponding to the projection of the iterate in the direction of the truth and orthogonal to the truth:
%\begin{align*}
%\xit  := \frac{\langle \thetacur, \thetastar \rangle}{ \| \thetastar \|_2^2} \quad \text{ and } \quad \sigmat  := \| P^{\perp}_{\thetastar} \thetacur \|_2.
%\end{align*}

%\subsection{Gordon updates and concentration (Theorem \ref{thm:gordon_main})}

The main result of this section shows concentration of the statistics $\xiplus,\sigmaplus$ of $\thetaplus$. Recall that the losses in Equations \eqref{eq:GD_gen} and \eqref{eq:sec_order_gen} are parameterized by a weight function 
$\omega:\R\times\R\rightarrow\R$. We require the following assumption.
% on the concentration properties of this function.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{assumption}[Concentration of the weight function]\label{ass:omega}
Let independent random vectors $\gammab_1,\gammab_2,\zb,\epsb\in\R^n$ each having iid entries from distributions $\Nn(0,1),$  $\Nn(0,1),$ $P_E$ and $P_Z$, respectively. 
%Specifically, $\gammab_1,\gammab_2$ are standard normals, $\epsb\sim\Nn(0,s^2\mathbf{I}_n)$, and, $\zb$ is the randomness of the measurement link function.
%\sim\Nn(0,\mathbf{I}_n) 
%be independent standard Gaussian vectors. 
Assume that the random vector 
\begin{align}\label{eq:omegat_def_main}
\omegab_t:= \omega\big(\xit \gammab_1+\sigmat \gammab_2\,,\,f(\gammab_1;\zb)+\epsb\big),
\end{align}
has independent entries sampled from a distribution $P_{\Omega_{t}}$ with the following properties. Let 
$\Omega_t\sim P_{\omega_t}$, that is 
\begin{align}\label{eq:omegat_def_scalar_main}
\Omega_t:= \omega\big(\xit G_1+\sigmat G_2\,,\,f(G_1;Z)+E\big),\qquad G_1, G_2\sim\Nn(0,1),\,E\sim P_E,\,Z\sim P_Z.
\end{align} 
Then, 

\begin{enumerate}[label=(\roman*)]

\item $\Omega_t$ is a $K_{\omega_t}$-subGaussian random variable for  universal constant  $K_{\omega_t}:=K_{\omega_t}(s)$ that may only depend on the noise level.

\item For  absolute constants $C,c,c'>0$, it holds that $E[\Omega_t^2]-\left(E[G_1\Omega_t]\right)^2-\left(E[G_2\Omega_t]\right)^2>c$, $\E[G_2\Omega_t]\geq c'$ and $E[\Omega_t^2]<C$. 

%\item $\E[G_2\Omega_t]\geq 0$.

%\item For  absolute constants $c'>0$, it holds that $E[\Omega_t^2]-\left(E[G_1\Omega_t]\right)^2-\left(E[G_2\Omega_t]\right)^2>c'$%\ct{joint distribution of $G_1,G_2$ and $\Omega_t$}.
\end{enumerate}
\end{assumption}
%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{remark}[Satisfying Assumption \ref{ass:omega}]\ct{More needed here. Move to corresponding Section.}\emph{
For non-smooth GD in phase retrieval we have $\omega(x_1,x_2)=\sign(x_1)(|x_1|-x_2)$ and $f(x;z) = |x|$. It is not hard to see then that $\omega\big(\xi\gammab_1+\sigma\gammab_2\,,\,f(R\gammab_1;\zb)+\epsb\big)$ is a vector with independent subgaussian entries, hence Assumption \ref{ass:omega} holds by \cite[Thm.~3.1.1]{Vershynin}. 
\\
The same argument applies to Gradient EM for mixtures of two regressions for which $\omega(x_1,x_2) = x_1-x_2\tanh\big(\frac{x_2x_1}{s^2}\big)$ and $f(x;z)=zx$. }
\end{remark}

We are now ready to define the following \emph{one-step $(\xi,\sigma)$ Gordon updates} for the two loss functions corresponding to first- and second- order methods. 
\begin{definition}[One-step Gordon updates]
\label{def:starnext_main}
 %Fix any $t\geq1$. 
Let $G_1,G_2$ be independent standard normal random variables and $\Omega_t=\Omega_t(G_1,G_2)$ be as in Equation \eqref{eq:omegat_def_scalar_main} such that Assumption \ref{ass:omega} holds. 
% Let Assumption \ref{ass:omega} hold   random variable $\Omega_t$ be as defined therein, and $G_1,G_2$  independent standard normal random variables. 
%Finally, let $\Lc$ be the loss function in Theorem \ref{thm:gordon_main}.  
If the loss function $\Lc$ is as in Equation \eqref{eq:sec_order_gen} then define
\begin{align}
\begin{cases}
~\xinextstar&=\E[G_1\Omega_t]\,, \\
~\alphanextstar&=\E[G_2\Omega_t]\,, \qquad
~\betanextstar=\sqrt{\left({\E[\Omega_t^2]-\left(\E[G_1\Omega_t]\right)^2-\left(\E[G_2\Omega_t]\right)^2}\right)\big/{\left(\delta-1\right)}}\,,\\
~ \sigmanextstar&=\sqrt{\alphanextstar^2+\betanextstar^2}\,.
%~\alphanextstar=\E[G_2\Omega_t]\\
%~\betanextstar=\sqrt{\frac{\E[\Omega_t^2]-\left(\E[G_1\Omega_t]\right)^2-\left(\E[G_2\Omega_t]\right)^2}{\delta-1}}\,.
\end{cases}
\label{eq:theta_starnext_sec_main}
\end{align}
Else, if $\Lc$ is as in Equation \eqref{eq:GD_gen}, then define
\begin{align}
\begin{cases}
~\xinextstar = \xit  + 2\eta\E\left[G_1 \Omega_t\right]\,,\\
~\alphanextstar = \sigmat  + 2\eta\E\left[G_2 \Omega_t\right]\,,\qquad \betanextstar = 2\eta\sqrt{\E\left[\Omega_t^2\right]\big/\delta}\,,\\
~\sigmanextstar = \sqrt{\alphanextstar^2+\betanextstar^2} \,.
%\\~\betanextstar = 2\eta\frac{1}{\sqrt{\delta}}\sqrt{\E\left[\Omega_t^2\right]}.\\
\end{cases}
\label{eq:theta_starnext_gd_main}
\end{align}
\end{definition}

%Our main theorem below shows concentration, but towards different values depending on the loss function. 

With these, our main result characterizing the concentration of the statistics $\xiplus$ and $\sigmaplus$ is as follows.

\begin{theorem}[Concentration of the $(\xi,\sigma)$ updates]
\label{thm:one_step_main}
 %Fix any $t\geq1$ and let
 Let 
 $\thetaplus \in \argmin_{\theta \in \mathbb{R}^d} {\mathcal{L}(\theta; \thetacur, \bd{X}, \bd{y})}$ for either of the two choices of loss functions $\Lc$ in  Equations \eqref{eq:GD_gen} and \eqref{eq:sec_order_gen}, respectively. Further let Assumption
 %ref{ass:loss}, 
 %\ref{ass:Lip}, \ref{ass:theta_bd}, and 
 \ref{ass:omega} hold. Consider the loss-dependent constants $\xinextstar$ and $\sigmanextstar$ specified in Definition \ref{def:starnext}. There exist universal constants $c,C,c_\delta,c'(\delta),C',C_1(\delta)>0$ such that for $\delta>c_\delta$ the following statements hold. 
 
 \begin{subequations} \label{eq:main-conc}
 \begin{enumerate}[label=(\roman*)]
 \item \textbf{($\xi$-update)} For all $1 \geq \epsilon > C'n^{-\nicefrac{1}{2}}$, 
 \begin{align}\label{eq:xi_conc_main}
 \Pro\left( \bigl \lvert \xiplus-\xinextstar \bigr\rvert  \leq C\bigl( \epsilon + \exp\{-c(\epsilon \sqrt{n})^{1/3}\}\bigr) \right) \geq 1-Ce^{-c(\epsilon \sqrt{n})^{2/5}}.
 \end{align}
 \item \textbf{($\sigma$-update)} For all $c'(\delta)>\eps>C'n^{-\nicefrac{1}{4}}$,
 \begin{align}\label{eq:sigma_conc_main}
 \Pro\left( |\sigmaplus-\sigmanextstar|\leq C(\delta)\eps \right) \geq 1-Ce^{-cn\eps^4}.
 \end{align}
 \end{enumerate}
 \end{subequations}
\end{theorem}

We will formally derive the one-step Gordon updates $\xinextstar,\sigmanextstar$ of Definition \ref{def:starnext_main} in Section \ref{sec:gordon}. In the same section, we will prove an $n^{-1/4}$ concentration of the statistics $\xiplus,\sigmaplus$. Later, in Section \ref{sec:random-init-signal}, we refine the concentration rate for $\xiplus$ and prove Equation \eqref{eq:xi_conc_main}.




==> sections/main-results/main-results.tex <==
%!TEX root = ../../convergence-gordon.tex

In this section, we state our main results for two specific models and algorithms, although it is important to note that the Gordon recipe itself---presented in detail in Section XXX---is much more broadly applicable. 
As mentioned before, for each iterate $\theta$, we will track a two-dimensional state evolution $\xi(\theta), \sigma(\theta)$, with
$\xi(\theta) = \inprod{\theta}{\thetastar}$ and $\sigma = \| P_{\thetastar}^{\perp} \theta \|$. By definition, we have $\| \theta - \theta^* \|^2 = (1 - \xi(\theta))^2 + (\sigma(\theta))^2$.

%\apcomment{Write the following in terms of two-dimensional recursions.}
We begin with two formal definitions of convergence rates, measuring linear (geometric) and faster-than-linear convergence. For a given element of the state evolution $\nu = (\xi, \sigma)$, define two metrics
\begin{align} \label{eq:metrics}
\DeltaSELtwo(\nu) := \sqrt{ (1 - \xi)^2 + \sigma^2} \qquad \text{ and } \qquad \DeltaSEangle(\nu) = \tan^{-1} (\sigma/\xi),
\end{align}
which denote the $\ell_2$ distance from the corresponding parameter to the ground truth $\thetastar$, and the angle between the parameter and $\thetastar$, respectively.
% \begin{definition}[Linear convergence]
% For two constants $0 < c \leq C < 1$, an operator $\mathcal{T}: \Theta \to \Theta$ is said to exhibit $(c, C)$-linear convergence in the set $\mathbb{G}$ to an $\varepsilon$-neighborhood of a point $\thetastar$ if for all $\theta \in \mathbb{G}$, we have $T(\theta) \in \mathbb{G}$ and 
% \begin{align*}
% c \left( \| \theta - \thetastar \| + \varepsilon \right) \leq \| \mathcal{T}(\theta) - \thetastar \| \leq C \left( \| \theta - \thetastar \| + \varepsilon \right).
% \end{align*}
% \end{definition}

% \begin{definition}[Super-linear convergence]
% For $\lambda > 1$, an operator $\mathcal{T}: \Theta \to \Theta$ is said to exhibit $(c, C, \lambda)$-superlinear convergence in the set $\mathbb{G} \subseteq \mathbb{B}(\thetastar; C^{1- \lambda})$ to an $\varepsilon$-neighborhood of a point $\thetastar$ if for all $\theta \in \mathbb{G}$, we have $T(\theta) \in \mathbb{G}$ and 
% \begin{align*}
% c \left( \| \theta - \thetastar \|^{\lambda} + \varepsilon \right) \leq \| \mathcal{T}(\theta) - \thetastar \| \leq C \left( \| \theta - \thetastar \|^{\lambda} + \varepsilon \right).
% \end{align*}
% \end{definition}
\begin{definition}[Linear convergence of state evolution] \label{def:linear}
A state evolution operator $\mathcal{S}: \mathbb{S} \to \mathbb{S}$ is said to exhibit $(c, C)$-linear convergence in the metric $\DeltaSE$ within the set $\mathbb{G}$ to level $\varepsilon$ if for all $\nu \in \mathbb{G}$, we have $\mathcal{S}(\nu) \in \mathbb{G}$ and 
\begin{align*}
c \cdot [\DeltaSE(\nu)]^2 + \varepsilon \leq [\DeltaSE(\mathcal{S}(\nu))]^2 \leq C \cdot [\DeltaSE(\nu)]^2 + \varepsilon.
\end{align*}
Here $0 < c \leq C < 1$ are constants.
\end{definition}

\begin{definition}[Super-linear convergence] \label{def:superlinear}
For $\lambda > 1$, a state evolution operator $\mathcal{S}: \mathbb{S} \to \mathbb{S}$ is said to exhibit $(c, C, \lambda, t_0)$-superlinear convergence in the metrix $\DeltaSE$ within the set $\mathbb{G}$ to level $\varepsilon$ if for all $\nu \in \mathbb{G}$, we have $\mathcal{S}(\nu) \in \mathbb{G}$ and 
\begin{align*}
[\DeltaSE(\mathcal{S}(\nu))]^2 &\leq C \cdot [\DeltaSE(\nu)]^{2\lambda} + \varepsilon \text{ and } \\
[\DeltaSE(\mathcal{S}^{t+1}(\nu))]^2 &\geq c \cdot [\DeltaSE(\mathcal{S}^{t}(\nu))]^{2\lambda} + \varepsilon  \text{ for all } t \geq t_0. 
\end{align*}
\end{definition}
\apcomment{Modify.} We have defined both notions of convergence in terms of the squared $\ell_2$ distance $[\DeltaSE(\nu)]^2$ for convenience. Note that one can use the elementary inequalities $\frac{\sqrt{a} + \sqrt{b}}{\sqrt{2}} \leq \sqrt{a + b} \leq \sqrt{a} + \sqrt{b}$ to translate these into statements purely about the $\ell_2$ distance. Also note that the definitions require both upper and lower bounds on the per-step behavior of the algorithm, where the lower bound applies after a ``burn-in'' period of $t_0$ iterations. This is a key feature of our framework, in that we are able to exactly characterize the convergence behavior as opposed to solely providing upper bounds.

%As a final remark, we note once again that our results are obtained as a consequence of tracking a two-dimensional state evolution measuring two notions of distance to the ground truth parameter $\thetastar$. In particular, for each $\theta \in \real^d$, we have $\xi(\theta) = \inprod{\theta}{\thetastar}$ and $\sigma = \| P_{\thetastar}^{\perp} \theta \|$.

\subsection{Phase retrieval}

As is common is such nonconvex optimization problems, our convergence guarantee will be established in two stages. In the first stage, the algorithm converges (typically slowly) to a ``good region'' around the optimal solution. Once in the good region, the algorithm converges much faster. For phase retrieval, the following definition of the good region suffices.

\begin{definition}[Good region for phase retrieval]
Define the region
\[
\GPR = \{ (\xi, \sigma) \mid \xi \lor \sigma \leq 1.05, \; \xi^2 + \sigma^2 \geq 0.9, \text{ and } \xi/\sigma \geq 5 \}.
\]
With slight abuse of terminology, we say that $\theta \in \GPR$ if $(\xi(\theta), \sigma(\theta)) \in \GPR$.
\end{definition}
It is important to note that the constants have not been optimized to be sharp, and that this is simply a sufficient condition for fast convergence.

\subsubsection{Alternating minimization}

The empirical update at iteration $t$ is given by
\begin{align} \label{eq:empirics-AM-PR}
\mathcal{T}_n(\theta) = \left( \frac{1}{n} \sum_{i = 1}^n x_i x_i^\top \right)^{-1} \; \left( \frac{1}{n} \sum_{i = 1}^n \sign(\inprod{x_i}{\theta}) \cdot y_i \cdot x_i \right).
\end{align}

The Gordon state evolution is derived in the following lemma, proved in Appendix XXX. 
\begin{lemma} \label{lem:Gordon-SE-AM-PR}
Let $\xi = \xi(\theta)$ and $\sigma = \sigma(\theta)$ with $\nu = (\xi, \sigma)$ and $\alpha = \tan^{-1}\left(\frac{\sigma}{\xi}\right)$. Let $(\xigordon, \sigmagordon) = \mathcal{S}_{gor}(\nu)$ denote the Gordon state evolution for alternating minimization in phase retrieval. We have
\begin{subequations} \label{eq:Gordon-AM-PR}
\begin{align}
\xigordon &= 1 - \frac{1}{\pi}(2\alpha - \sin(2\alpha))  \quad \text{ and } \label{eq:Gordon-AM-PR-xi} \\
\sigmagordon &= \sqrt{\frac{4}{\pi^2}\sin^4(\alpha) + \frac{1}{\delta - 1}\left(1 - (1 - \frac{1}{\pi}(2\alpha - \sin(2\alpha)))^2 - \frac{4}{\pi^2}\sin^4(\alpha) + s^2 \right)} \label{eq:Gordon-AM-PR-sigma}
\end{align}
\end{subequations}
\end{lemma}

From~\eqref{eq:Gordon-AM-PR}, it is possible to recover the following population state evolution by letting $\delta \to \infty$, which is given by
\begin{align}\label{eq:Pop-AM-PR}
\xipop = 1 - \frac{1}{\pi}(2\alpha - \sin(2\alpha))  \quad \text{ and }  \quad \sigmapop = \frac{2}{\pi}\sin^2(\alpha).
\end{align}
It is easy to show that the population state evolution predicts superlinear convergence with exponent~$2$ (i.e., quadratic convergence) in the good region.
\begin{fact} \label{prop:Pop-PR}
The population state evolution $\mathcal{S}_{pop}$ is $(\frac{1}{20}, 1, \lambda, t_0)$-superlinearly convergent in the $\ell_2$ metric\footnote{In fact, the population state evolution~\eqref{eq:Pop-AM-PR} enjoys \emph{global} quadratic convergence in the angular metric $\DeltaSEangle$; see Remark XXX in the appendix.} $\DeltaSELtwo$ within the region $\GPR$ to level $\varepsilon = 0$, where $\lambda = 2$ and $t_0 = 1$.
\end{fact}

However, the following theorem shows that the empirics are instead tracked faithfully by the Gordon state evolution, which converges more slowly than the population state evolution.
\begin{theorem} \label{thm:AM-PR}
Consider the alternating minimization algorithm~\eqref{eq:empirics-AM-PR} and the associated Gordon state evolution update~\eqref{eq:Gordon-AM-PR}. There is a universal positive constant $C$ such that the following is true. If $\delta \geq C (1 + s^2)$, then:

\noindent (a) The Gordon state evolution update 
\begin{center}
$\mathcal{S}_{gor}$ is $(c_{\delta}, C_\delta, \lambda, t_0)$-superlinearly convergent in the $\ell_2$ metric $\DeltaSELtwo$ within $\GPR$ to level $\varepsilon_{n, d} = \frac{s^2}{\delta - 1}$,
\end{center} 
where $0 \leq c_\delta \leq C_{\delta} \leq 1$ are constants depending solely on $\delta$, and we have
\begin{align*}
\lambda = 3/2 \qquad \text{ and } \qquad t_0 = 1.
\end{align*}

\noindent (b) For any $\theta$ such that $\nu = (\xi(\theta), \sigma(\theta)) \in \GPR$, we have
\begin{align*}
\max_{1 \leq t \leq T} \; | \DeltaSE(\mathcal{S}^t_{gor}(\nu)) - \| \mathcal{T}^t_n(\theta) - \thetastar \| | \leq C \left( \frac{\log n}{n} \right)^{1/4}
\end{align*}
with probability exceeding $1 - 2T n^{-10}$.

\noindent (c) Suppose $\theta_0$ denotes a point such that $\frac{\xi_0}{\sigma_0} \geq \frac{1}{100 \sqrt{d}}$ and further suppose that $\delta \geq C \cdot \log^3 \left( \frac{1 + \log d}{\epsilon} \right)$. 
%Let $\nu_0 = (\xi_0, \sigma_0)$ for $\xi_0 = \xi(\theta_0)$ and $\sigma_0 = \sigma(\theta_0)$. 
Then for some $t_0 \leq C\log d$, we have
\begin{align*}
\mathcal{T}_{n}^{t_0}(\theta_0) \in \GPR
\end{align*} 
with probability exceeding $1 - \epsilon$.
\end{theorem}

Note that if $\theta_0$ is chosen at random from the unit ball $\mathbb{B}(1)$, then we have $\frac{\xi_0}{\sigma_0} \geq \frac{1}{100 \sqrt{d}}$ with probability at least $0.99$. Theorem~\ref{thm:AM-PR} then shows that after $\tau = \mathcal{O}( \log d + \log \log (\delta/s^2))$ iterations, the empirics satisfy
\begin{align}
\| \mathcal{T}_{n}^{\tau}(\theta_0) - \thetastar \| \lesssim \frac{s}{\sqrt{\delta - 1}} + n^{-1/4}
\end{align}
with high probability, where $\lesssim$ here hides a logarithmic factor.


Remarks:
\begin{itemize}
\item We have superlinear convergence with non-standard exponent $3/2$ whenever $\delta$ is bounded above. In other words the population update is overly optimistic, and this corroborates what we saw in Fig XXX. Non-standard superlinear convergence was recently observed in the noiseless case of this problem~\cite{}, but a larger exponent was conjectured. Theorem~\ref{thm:AM-PR} shows that the exponent $3/2$ is indeed sharp, since we obtain both upper and lower bounds on the error of the algorithm. Concretely, this implies that the AM update converges \emph{very} fast to the optimal parameter in terms of iteration complexity, even though each iteration involves solving a linear system.
\item The convergence rate is superlinear with exponent $3/2$ for every value of the noise level. As we will see shortly, this is not the case for the closely related model of mixtures of regressions, in which the convergence rate of this algorithm is linear as soon as $s > 0$.
\item Our assumption that $s^2 / \delta$ be bounded above by a universal constant should not be viewed as restrictive, since otherwise, running just one step of the update from a random initialization satisfies $\| \theta_1 - \theta^* \|^2 = O(s^2 / \delta)$ and attains the optimal rate. \apcomment{Expand on this perhaps?}
\item The empirics are shown to be within a radius $n^{-1/4}$ of the Gordon updates, which is strictly dominated by the $s/\sqrt{\delta}$ term in modern high dimensional problems. We do not believe that this radius is optimal, and conjecture that it can be improved to $n^{-1/2}$. Indeed, we do so for first-order methods in Section XXX (see Theorem~\ref{thm:GD-PR} below).
\item Our convergence result is \emph{global}, and holds from a random initialization. In particular, part (c) of the theorem guarantees that within $O(\log d)$ iterations, the iterations enter the good region $\GPR$, at which point parts (a) and (b) of the theorem become active. Convergence from a random initialization is also established by showing that the empirical state evolution tracks its Gordon counterpart closely. But rather than showing two deterministic envelopes around the empirical trajectory, we leverage closeness of the updates iterate-by-iterate. It is worth noting that this is the only step that requires the condition $n \asymp d \log^3 (\log d)$; all other steps only require sample complexity that is linear in dimension.
\item Showing that the empirics are close to Gordon at near-random initialization requires significant subtlety since the update involves a matrix inversion. We employ a leave-one-out trick (aka the cavity method) to show a sharpened version of a result by Zhang~\cite{}, and believe that this technique will prove more broadly useful in analyzing higher-order updates such as EM and (Gauss-)Newton methods from a random intialization.
\end{itemize}

\subsubsection{Subgradient descent}

To contrast with the superlinear convergence shown in the previous section, we now consider subgradient descent with step-size $1/2$. As will be shown shortly, this update shares the same population update as AM, but convergence is only linear, as expected from a first-order method. The Gordon update is able to capture this.
The general subgradient method for PR is given by the update
\begin{align} \label{eq:GD-PR}
\mathcal{T}_n(\theta) = \theta - \frac{2\eta}{n} \cdot \sum_{i = 1}^n (|\inprod{x_i}{\theta}| - y_i) \cdot \sign(\inprod{x_i}{\theta}) \cdot x_i,
\end{align}
where $\eta > 0$ denotes the step-size. The Gordon update is given by the following lemma.
\begin{lemma} \label{lem:Gordon-SE-GD-PR}
Let $\xi = \xi(\theta)$ and $\sigma = \sigma(\theta)$ with $\alpha = \tan^{-1}\left(\frac{\sigma}{\xi}\right)$. Let $(\xigordon, \sigmagordon) = \Sopgordon(\xi, \sigma)$ denote the Gordon state evolution update for subgradient descent in phase retrieval. We have
\begin{subequations} \label{eq:Gordon-GD-PR}
\begin{align}
\xigordon &= (1 - 2\eta) \xi + 2\eta \left(1 - \frac{1}{\pi} (2 \alpha - \sin(2 \alpha)) \right), \text{ and } \label{eq:Gordon-GD-PR-xi}\\
\sigmagordon &= \Big( (1 - 2\eta) \sigma^2 + 2 \eta \cdot \frac{4}{\pi^2} \sin^4 \alpha \notag \\
&\qquad \qquad \qquad + \frac{4 \eta^2}{\delta - 1} \Big\{ \xi^2 + \sigma^2 - 2\xi \left(1 - \frac{1}{\pi} (2 \alpha - \sin(2 \alpha)) \right) - 2\sigma \cdot \frac{2}{\pi} \sin^2 \alpha + 1 + s^2 \Big\} \Big)^{1/2}. \label{eq:Gordon-GD-PR-sigma}
\end{align}
\end{subequations}
\end{lemma}

Sending $\delta \to \infty$ in equation~\eqref{eq:Gordon-GD-PR} recovers the infinite-sample population state evolution
\begin{subequations} \label{eq:Pop-GD-PR}
\begin{align}
\xipop &= (1 - 2\eta) \xi + 2\eta \left(1 - \frac{1}{\pi} (2 \alpha - \sin(2 \alpha)) \right), \text{ and } \label{eq:Pop-GD-PR-xi}\\
\sigmapop &= \Big( (1 - 2\eta) \sigma^2 + 2 \eta \cdot \frac{4}{\pi^2} \sin^4 \alpha \Big)^{1/2}.  \label{eq:Pop-GD-PR-sigma}
\end{align}
\end{subequations}

As previously noted, our interest\footnote{Our techniques are also applicable to analyzing the algorithm with general stepsize $\eta$, but we do not do so in this paper since a variety of other analysis methods tailored to first order updates (e.g.~\cite{}) also work in this case.} will be in analyzing the special case $\eta = 1/2$ so as to compare and contrast with the AM update. In this case, the population updates~\eqref{eq:Pop-AM-PR} and~\eqref{eq:Pop-GD-PR} coincide, and so Proposition~\ref{prop:Pop-PR} suggests that subgradient descent ought to converge quadratically fast. This would be quite surprising for a first-order method, and already suggests that the population update may even more optimistic than before. However, the Gordon updates~\eqref{eq:Gordon-AM-PR} and~\eqref{eq:Gordon-GD-PR} are distinct, and as we saw before, these provide much more faithful predictions of convergence behavior. 

\begin{theorem} \label{thm:GD-PR}
Consider the sub-gradient descent algorithm~\eqref{eq:GD-PR} and the associated Gordon state evolution update~\eqref{eq:Gordon-GD-PR}, with stepsize $\eta = 1/2$. There is a universal positive constant $C$ such that the following is true. If $\delta \geq C (1 + s^2)$, then:

\noindent (a) The Gordon state evolution update
\begin{center}
$\mathcal{S}_{gor}$  is $(c_{\delta}, C_\delta)$-linearly convergent in the $\ell_2$ metric $\DeltaSELtwo$ on $\GPR$ to level $\varepsilon_{n, d} = \frac{s^2}{\delta - 1}$.
\end{center}
Here $0 \leq c_\delta \leq C_{\delta} \leq 1$ are constants depending solely on $\delta$.

\noindent (b) For any $\theta$ such that $\nu = (\xi(\theta), \sigma(\theta)) \in \GPR$, we have
\begin{align*}
\max_{1 \leq t \leq T} \; | \DeltaSE(\mathcal{S}^t_{gor}(\nu)) - \| \mathcal{T}_n^t(\theta) - \thetastar \| | \leq C \left( \frac{\log n}{n} \right)^{1/2}
\end{align*}
with probability exceeding $1 - 2T n^{-10}$.

\noindent (c) Suppose $\theta_0$ denotes a point such that $\frac{\xi_0}{\sigma_0} \geq \frac{1}{100 \sqrt{d}}$ and further suppose that $\delta \geq C \cdot \log^3 \left( \frac{1 + \log d}{\epsilon} \right)$. 
%Let $\nu_0 = (\xi_0, \sigma_0)$ for $\xi_0 = \xi(\theta_0)$ and $\sigma_0 = \sigma(\theta_0)$. 
Then for some $t_0 \leq C\log d$, we have
\begin{align*}
\mathcal{T}_{n}^{t_0}(\theta_0) \in \GPR
\end{align*} 
with probability exceeding $1 - \epsilon$.
\end{theorem}

To be concrete once again, we have shown that if $\theta_0$ is chosen at random from the unit ball, then for some $\tau = \mathcal{O}( \log d + \log(\delta/s^2))$, the empirics satisfy
\begin{align}
\| \mathcal{T}_{n}^{\tau}(\theta_0) - \thetastar \| \lesssim \frac{s}{\sqrt{\delta - 1}} + n^{-1/2}
\end{align}
with high probability. Once again, the notation $\lesssim$ here hides a logarithmic factor.

Remarks:
\begin{itemize}
\item As expected, subgradient descent only converges linearly in the good region, which corroborates what we saw in Fig XXX. The population update is thus significantly optimistic in this case.
\item Unlike before, the empirics here are shown to be within a radius $O(n^{-1/2})$ of the Gordon updates, which we believe to be optimal.
\item Once again, our convergence result is \emph{global}, and holds from a random initialization. Once again, we establish it by showing that the empirical update tracks the Gordon update closely, iterate-by-iterate. Our proof technique for this portion of the convergence result resembles some prior work~\cite{chen,wu} for first-order updates.
\end{itemize}

\subsection{Mixtures of regressions}

It suffices to work with the following definition of a good region for mixtures of regressions.

\begin{definition}[Good region for mixtures of regressions]
Define the region
\[
\GMR = \{ (\xi, \sigma) \mid \sigma \leq 1.05, \;\; \xi \geq 0.55, \;\; \text{ and } \xi / \sigma \geq 5 \}.
\]
With slight abuse of terminology, we say that $\theta \in \GMR$ if $(\xi(\theta), \sigma(\theta)) \in \GMR$.
\end{definition}
Once again, the constants have not been optimized to be sharp.

\subsubsection{Alternating minimization}

The update applied at $\theta$ is given by
\begin{align}
	\label{eq:empirics-AM-MLR}
\mathcal{T}_n(\theta) = \left( \frac{1}{n} \sum_{i = 1}^n x_i x_i^\top \right)^{-1} \; \left( \frac{1}{n} \sum_{i = 1}^n \sign(y_i \cdot \inprod{x_i}{\theta}) \cdot y_i \cdot x_i \right).
\end{align}
The Gordon updates here are given by the following lemma.
\begin{lemma} \label{lem:Gordon-SE-AM-MLR}
Let $\xi = \xi(\theta)$ and $\sigma = \sigma(\theta)$ with $\nu = (\xi, \sigma)$ and $\rho = \frac{\sigma}{\xi}$. Let $(\xigordon, \sigmagordon) = \mathcal{S}_{gor}(\nu)$ denote the Gordon state evolution for alternating minimization in mixtures of regressions. Letting
\begin{align*}
A(\rho) := \frac{2}{\pi}\tan^{-1}\left(\sqrt{\rho^2 + \noisestd^2 + \noisestd^2 \rho^2}\right) \quad \text{ and } \quad
B(\rho) := \frac{2}{\pi} \frac{\sqrt{\rho^2 + \noisestd^2 + \noisestd^2\rho^2}}{1 + \rho^2},
\end{align*}
we have
\begin{subequations} \label{eq:Gordon-AM-MLR}
\begin{align}
\xigordon &= 1 - A(\rho) + B(\rho), \text{ and } \\
\sigmagordon &= \sqrt{\rho^2 B(\rho)^2 + \frac{1}{\delta - 1}\left(1 + \noisestd^2 - (1 - A(\rho) + B(\rho))^2 - \rho^2 B(\rho)^2\right)}.
\end{align}
\end{subequations}
\end{lemma}
By taking $\delta \to \infty$, we recover the population update for this case, given by
\begin{align}\label{eq:Pop-AM-MLR}
\xipop = 1 - A(\rho) + B(\rho)  \quad \text{ and }  \quad \sigmapop = \rho B(\rho).
\end{align}
This update has no dependence on the aspect ratio $\delta$ and thus cannot recover the noise floor of the problem. As before, the following theorem shows that the empirics are tracked faithfully by the Gordon update.
\begin{theorem} \label{thm:AM-MLR}
Consider the alternating minimization algorithm~\eqref{eq:empirics-AM-MLR} and the associated Gordon state evolution update~\eqref{eq:Gordon-AM-MLR}. There are universal positive constants $(c, C)$ such that the following is true. If $\delta \geq C$ and $s \leq c$, then:

\noindent (a) The Gordon state evolution update 
\begin{center}
$\mathcal{S}_{gor}$ is $(c_{\delta, s}, C_{\delta, s})$-linearly convergent in the angular metric $\DeltaSEangle$ on $\GMR$ to level $\varepsilon_{n, d} = \frac{s^2}{\delta - 1}$,
\end{center} 
where $0 \leq c_{\delta, s} \leq C_{\delta, s} \leq 1$ are constants depending solely on the pair $(\delta, s)$.

\noindent (b) For any $\theta$ such that $\nu = (\xi(\theta), \sigma(\theta)) \in \GMR$, we have
\begin{align*}
\max_{1 \leq t \leq T} \; | \DeltaSEangle(\mathcal{S}^t_{gor}(\nu)) - \angle(\theta, \thetastar) | \leq C \left( \frac{\log n}{n} \right)^{1/4}
\end{align*}
with probability exceeding $1 - 2T n^{-10}$.

\noindent (c) Suppose $\theta_0$ denotes a point such that $\frac{\xi_0}{\sigma_0} \geq \frac{1}{100 \sqrt{d}}$ and further suppose that $\delta \geq C \cdot \log^3 \left( \frac{1 + \log d}{\epsilon} \right)$. 
%Let $\nu_0 = (\xi_0, \sigma_0)$ for $\xi_0 = \xi(\theta_0)$ and $\sigma_0 = \sigma(\theta_0)$. 
Then for some $t_0 \leq C\log d$, we have
\begin{align*}
\mathcal{T}_{n}^{t_0}(\theta_0) \in \GPR
\end{align*} 
with probability exceeding $1 - \epsilon$.
\end{theorem}
Theorem~\ref{thm:AM-MLR} shows that with a random initialization $\theta_0$ and after $\tau = \mathcal{O}( \log d + \log \log (\delta/s^2))$ iterations, the empirics satisfy
\begin{align}
\angle \left( \mathcal{T}_{n}^{\tau}(\theta_0), \thetastar \right) \lesssim \frac{s}{\sqrt{\delta - 1}} + n^{-1/4}
\end{align}
with high probability, where $\lesssim$ here hides a logarithmic factor.


Remarks:
\begin{itemize}
\item Convergence here is in angular metric and not in $\ell_2$. \apcomment{Unpack.}
\item Note that when $s = 0$, mixtures of regressions and phase retrieval coincide. In particular, Theorem XXX already shows that in the noiseless case, AM for both of these models has superlinear convergence with exponent $3/2$. However, the convergence behavior changes dramatically for mixtures when there is noise, unlike in phase retrieval. While Theorem~\ref{} shows that superlinear convergence is preserved even for noisy phase retrieval, Theorem~\ref{} demonstrates that for any $s > 0$, the convergence of AM for mixtures is linear and not superlinear.
\item Our assumption on the noise level in this case is that $s^2$ be bounded above by a universal constant. While this is more stringent than in phase retrieval, we see that in the absence of such a condition, the algorithm does not converge to the optimal neighborhood, as shown in Figure XXX. Interestingly, the Gordon update still tracks the behavior of the algorithm in this case, showing the lack of convergence and demonstrating the broader use of our deterministic recursion in predicting not just the rate of convergence but also the presence or absence of convergence.
\item Finally, our convergence result is once again global and holds from a random initialization. As before, this is the only step that requires the condition $n \asymp d \log d$; all other steps only require sample complexity that is linear in dimension. As before, we employ a leave-one-out trick (aka the cavity method) to show that the empirics as sharply tracked by the Gordon update from a random intialization.
\end{itemize}

\subsubsection{Subgradient descent}

For completeness, we also present a subgradient version of the AM update for mixtures of linear regressions. To the best of our knowledge, this update has not been considered in the literature, but it is natural for us to consider it since when the stepsize $\eta = 1/2$, it shares the same population update as AM. Given that AM converges linearly for mixtures of regressions, it is natural to ask if the first-order method---which has a much lower per-iteration cost---enjoys a similar convergence rate.

The update---with stepsize $\eta$---is given by
\begin{align} \label{eq:empirics-GD-MLR}
\mathcal{T}_n(\theta) = \theta - \frac{2\eta}{n} \cdot \sum_{i = 1}^n (|\inprod{x_i}{\theta}| - y_i) \cdot \sign(\inprod{x_i}{\theta}) \cdot x_i.
\end{align}

The Gordon update here is given by the following lemma.
\begin{lemma} \label{lem:Gordon-SE-GD-MLR}
Let $\xi = \xi(\theta)$ and $\sigma = \sigma(\theta)$ with $\nu = (\xi, \sigma)$ and $\rho = \frac{\sigma}{\xi}$. Let $(\xigordon, \sigmagordon) = \mathcal{S}_{gor}(\nu)$ denote the Gordon state evolution corresponding to the update~\eqref{eq:empirics-GD-MLR}. Letting
\begin{align*}
A(\rho) := \frac{2}{\pi}\tan^{-1}\left(\sqrt{\rho^2 + \noisestd^2 + \noisestd^2 \rho^2}\right) \quad \text{ and } \quad
B(\rho) := \frac{2}{\pi} \frac{\sqrt{\rho^2 + \noisestd^2 + \noisestd^2\rho^2}}{1 + \rho^2},
\end{align*}
we have
\begin{subequations} \label{eq:Gordon-GD-MLR}
\begin{align}
\xigordon &= (1 - 2\eta) \xi + 2 \eta \cdot \left( 1 - A(\rho) + B(\rho) \right), \text{ and } \\
\sigmagordon &= \Big( (1 - 2 \eta) \sigma^2 + 2\eta \cdot \rho^2 B(\rho)^2 \notag \\
&\qquad \qquad + \frac{4 \eta^2}{\delta - 1}\left\{ \xi^2 + \sigma^2 - 2\xi(1 - A(\rho) + B(\rho)) - 2 \sigma \rho B(\rho) + 1 + \noisestd^2 \right\} \Big)^{1/2}.
\end{align}
\end{subequations}
\end{lemma}
Once again, our interest will be in analyzing the special case $\eta = 1/2$, in which case the population updates of both the first-order and higher-order algorithm coincide. The following theorem then establishes a sharp characterization of the subgradient method.
\begin{theorem} \label{thm:GD-MLR}
Consider the subgradient method~\eqref{eq:empirics-AM-MLR} and the associated Gordon state evolution update~\eqref{eq:Gordon-GD-MLR}. There are universal positive constants $(c, C)$ such that the following is true. If $\delta \geq C$ and $s \leq c$, then:

\noindent (a) The Gordon state evolution update 
\begin{center}
$\mathcal{S}_{gor}$ is $(c_{\delta, s}, C_{\delta, s})$-linearly convergent in the angular metric $\DeltaSEangle$ on $\GMR$ to level $\varepsilon_{n, d} = \frac{s^2}{\delta - 1}$,
\end{center} 
where $0 \leq c_{\delta, s} \leq C_{\delta, s} \leq 1$ are constants depending solely on the pair $(\delta, s)$.

\noindent (b) For any $\theta$ such that $\nu = (\xi(\theta), \sigma(\theta)) \in \GMR$, we have
\begin{align*}
\max_{1 \leq t \leq T} \; | \DeltaSEangle(\mathcal{S}^t_{gor}(\nu)) - \angle(\theta, \thetastar) | \leq C \left( \frac{\log n}{n} \right)^{1/4}
\end{align*}
with probability exceeding $1 - 2T n^{-10}$.

\noindent (c) Suppose $\theta_0$ denotes a point such that $\frac{\xi_0}{\sigma_0} \geq \frac{1}{100 \sqrt{d}}$ and further suppose that $\delta \geq C \cdot \log^3 \left( \frac{1 + \log d}{\epsilon} \right)$. 
%Let $\nu_0 = (\xi_0, \sigma_0)$ for $\xi_0 = \xi(\theta_0)$ and $\sigma_0 = \sigma(\theta_0)$. 
Then for some $t_0 \leq C\log d$, we have
\begin{align*}
\mathcal{T}_{n}^{t_0}(\theta_0) \in \GPR
\end{align*} 
with probability exceeding $1 - \epsilon$.
\end{theorem}
As in the case of the AM algorithm, Theorem~\ref{thm:GD-MLR} shows that with a random initialization $\theta_0$ and after $\tau = \mathcal{O}( \log d + \log \log (\delta/s^2))$ iterations, the empirics satisfy
\begin{align}
\angle \left( \mathcal{T}_{n}^{\tau}(\theta_0), \thetastar \right) \lesssim \frac{s}{\sqrt{\delta - 1}} + n^{-1/4}
\end{align}
with high probability, where $\lesssim$ here hides a logarithmic factor.

Remarks:
\begin{itemize}
\item As expected, subgradient descent converges linearly in the good region, with slope of the order $\delta^{-1} \lor s$. On the other hand, we saw that the slope of the AM recursion was of the order $s$, and so strictly better than the first-order method. Having said that, the first order method may not be a bad choice for problems in which $s \approx \delta^{-1}$, since it enjoys a much smaller per-iteration cost for comparable convergence behavior.
\item Given that the method is a first order method, the empirics can be shown to be within $n^{-1}$ of the Gordon updates. As in the phase retrieval case, the random init is handled by a similar argument to prior work~\cite{}.
\end{itemize}
